TIDEE: Tidying Up Novel Rooms using Visuo-Semantic Commonsense Priors

We introduce TIDEE, an embodied agent that tidies up a disordered scene based on learned commonsense object placement and room arrangement priors. TIDEE explores a home environment, detects objects that are out of their natural place, infers plausible object contexts for them, localizes such contexts in the current scene, and repositions the objects. Commonsense priors are encoded in three modules: i) visuo-semantic detectors that detect out-of-place objects, ii) an associative neural graph memory of objects and spatial relations that proposes plausible semantic receptacles and surfaces for object repositions, and iii) a visual search network that guides the agent's exploration for efficiently localizing the receptacle-of-interest in the current scene to reposition the object. We test TIDEE on tidying up disorganized scenes in the AI2THOR simulation environment. TIDEE carries out the task directly from pixel and raw depth input without ever having observed the same room beforehand, relying only on priors learned from a separate set of training houses. Human evaluations on the resulting room reorganizations show TIDEE outperforms ablative versions of the model that do not use one or more of the commonsense priors. On a related room rearrangement benchmark that allows the agent to view the goal state prior to rearrangement, a simplified version of our model significantly outperforms a top-performing method by a large margin. Code and data are available at the project website: https://tidee-agent.github.io/.

==> 7_ref.tex <==
@inproceedings{DBLP:conf/humanoids/YamaguchiA16,
  author    = {Akihiko Yamaguchi and
               Christopher G. Atkeson},
  title     = {Differential dynamic programming for graph-structured dynamical systems:
               Generalization of pouring behavior with different skills},
  booktitle = {16th {IEEE-RAS} International Conference on Humanoid Robots, Humanoids
               2016, Cancun, Mexico, November 15-17, 2016},
  pages     = {1029--1036},
  year      = {2016},
  crossref  = {DBLP:conf/humanoids/2016},
  url       = {https://doi.org/10.1109/HUMANOIDS.2016.7803398},
  doi       = {10.1109/HUMANOIDS.2016.7803398},
  timestamp = {Wed, 17 May 2017 10:54:30 +0200},
  biburl    = {http://dblp.org/rec/bib/conf/humanoids/YamaguchiA16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/abs-1912-08195,
  author    = {Luca Weihs and
               Aniruddha Kembhavi and
               Winson Han and
               Alvaro Herrasti and
               Eric Kolve and
               Dustin Schwenk and
               Roozbeh Mottaghi and
               Ali Farhadi},
  title     = {Artificial Agents Learn Flexible Visual Representations by Playing
               a Hiding Game},
  journal   = {CoRR},
  volume    = {abs/1912.08195},
  year      = {2019},
  url       = {http://arxiv.org/abs/1912.08195},
  eprinttype = {arXiv},
  eprint    = {1912.08195},
  timestamp = {Fri, 03 Jan 2020 16:10:45 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1912-08195.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@inproceedings{DBLP:conf/humanoids/YamaguchiANO14,
  author    = {Akihiko Yamaguchi and
               Christopher G. Atkeson and
               Scott Niekum and
               Tsukasa Ogasawara},
  title     = {Learning pouring skills from demonstration and practice},
  booktitle = {14th {IEEE-RAS} International Conference on Humanoid Robots, Humanoids
               2014, Madrid, Spain, November 18-20, 2014},
  pages     = {908--915},
  year      = {2014},
  crossref  = {DBLP:conf/humanoids/2014},
  url       = {https://doi.org/10.1109/HUMANOIDS.2014.7041472},
  doi       = {10.1109/HUMANOIDS.2014.7041472},
  timestamp = {Wed, 17 May 2017 10:54:28 +0200},
  biburl    = {http://dblp.org/rec/bib/conf/humanoids/YamaguchiANO14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}




@article{17RAS-BiswasVeloso,
  title = "Episodic non-Markov Localization",
  author = "Joydeep Biswas and Manuela Veloso", 
  journal = "Robotics and Autonomous Systems",
  volume = "87",
  pages = "162--176",
  year = "2017"}

@inproceedings{17roman-logs,
        author = "Vittorio Perera and Manuela Veloso",
        title = "{ Learning to Understand Questions on the Task History of a Service Robot}",
        booktitle = {Proceedings of RO-MAN'17, the IEEE International
                  Symposium on Robot and Human Interactive
                  Communication}, 
        year = {2017}, Month="August", Address="Lisbon, Portugal"}

@article{16ieeesystems-1000,
  title = {The 1,000-km Challenge: Insights and Quantitative and Qualitative Results},
  author = {Joydeep Biswas and Manuela Veloso},
  doi = {10.1109/MIS.2016.53},
  publisher = {IEEE},
  year = {2016},
  pages = {86--96},
  number = {3},
  volume = {31},
  journal = {IEEE Intelligent Systems},
}

@InProceedings(15robot-BarPaiVel,
    Author="Kim Baraka and Ana Paiva and Manuela Veloso",
    Title="{Expressive Lights for Revealing Mobile Service Robot State}",
    BookTitle="Proceedings of Robot'2015, the Second Iberian Robotics Conference",
    Year="2015", Month="November", Address="Lisbon, Portugal")

@inproceedings{15ijcai-PerVel,
        author = "Vittorio Perera and Manuela Veloso",
        title ="{Handling Complex Commands for Service Robot Task Requests}",
        booktitle ={Proceedings of IJCAI'15, the International Joint Conference
                  on Artificial Intelligence},
        year = {2015}, Month="July", Address="Buenos Aires, Argentina"}

@inproceedings{15ijcai-CoBots,
        author = "Manuela Veloso and Joydeep Biswas and Brian Coltin
                  and Stephanie Rosenthal",
        title="{CoBots: Robust Symbiotic Autonomous Mobile Service Robots}",
        booktitle ={Proceedings of IJCAI'15, the International Joint Conference
                  on Artificial Intelligence},
        year = {2015}, Month="July", Address="Buenos Aires, Argentina"}

@Article(13ijrr-BiswasVeloso,
   Author="Joydeep Biswas and Manuela Veloso",
   title = "{Localization and Navigation of the CoBots over Long-term Deployments}",
  Journal="International Journal of Robotics Research", 
  Year="2013", Volume=32, Number=14, Pages = "1679--1694", Month="December")

@article{15robotics-PerEtAl,
  author    = {Vittorio Perera and
               Robin Soetens and
               Thomas Kollar and
               Mehdi Samadi and
               Yichao Sun and
               Daniele Nardi and
               Ren{\'{e}} van de Molengraft and
               Manuela Veloso},
  title     = {Learning Task Knowledge from Dialog and Web Access},
  journal   = {Robotics},
  volume    = {4},
  number    = {2},
  pages     = {223--252},
  year      = {2015}}

@PhDThesis(Biswas:thesis,
	Author="Joydeep Biswas",	
	Title=" Vector Map-Based, Non-Markov Localization for
                  Long-Term Deployment of Autonomous Mobile Robot",
	School="The Robotics Institute, Carnegie Mellon
	University, Pittsburgh, PA", Year="2014", Month="December",
	note="Available as technical report CMU-RI-14-25")

@InProceedings(biswas2011cgr,
       Title="{Corrective Gradient Refinement for Mobile Robot Localization}",
       Author="Joydeep Biswas and Brian Coltin and Manuela Veloso",
       Booktitle="Proceedings of IROS'11, the IEEE/RSJ International Conference on
       Intelligent Robots and Systems",
       Year="2011", Month="September", Address="San Francisco, CA")

@inproceedings{biswas2010wifi,
  title={Wifi localization and navigation for autonomous indoor mobile robots},
  author={Biswas, J. and Veloso, M.},
  booktitle={Proc. of the IEEE Int. Conf. on Robotics and Automation (ICRA)},
  pages={4379--4384},
  year={2010},
  organization={IEEE}
}

@Inproceedings(biswasdepth,
       Author="Joydeep Biswas and Manuela Veloso",
       title = "{Depth Camera Based Indoor Mobile Robot Localization and Navigation}",
       BookTitle="Proceedings of ICRA'12, the IEEE International Conference on Robotics and Automation",
       Year="2012", Month="May", Address="St. Paul, MN")

@Inproceedings(rosenthal2010effective,
       Author="Stephanie Rosenthal and Joydeep Biswas and Manuela Veloso",
       Title="{An Effective Personal Mobile Robot Agent Through Symbiotic Human-Robot Interaction}",
       BookTitle="Proceedings of AAMAS'10, the
       Ninth International Joint Conference on Autonomous Agents and Multi-Agent Systems", 
       Year="2010", Month="May", Address="Toronto, Canada")

@Inproceedings(12aaai-SamadiKollarVeloso,
       Author = "Mehdi Samadi and Thomas Kollar and Manuela Veloso",
       Title = "{Using the Web to Interactively Learn to Find Objects}",
      booktitle = {Proceedings of AAAI'12, the Twenty-Sixth AAAI Conference on Artificial Intelligence},
       Year="2012", Month="July", Address="Toronto, Canada")

@PhDThesis(Rosenthal:thesis,
	Author="Stephanie Rosenthal",	
	Title="Human-Centered Planning for Effective Task Autonomy",
	School="Computer Science Department, Carnegie Mellon
	University, Pittsburgh, PA", Year="2012", Month="May",
	note="Available as technical report CMU-CS-12-110")

@PhDThesis(Coltin:thesis,
	Author="Brian Coltin",	
	Title="Multi-agent Pickup and Delivery Planning with Transfers ",
	School="The Robotics Institute, Carnegie Mellon
	University, Pittsburgh, PA", Year="2014", Month="May",
	note="Available as technical report CMU-RI-14-05")

@PhDThesis(Wang:thesis,
	Author="Richard Wang",	
	Title="Collecting, Analyzing, and Using Fine-Grain Sensor Data with Mobile Platforms",
	School="Computer Science Department, Carnegie Mellon
	University, Pittsburgh, PA", Year="2016", Month="May",
	note="Available as technical report CMU-CS-16-110")

@article{coltineffective,
  title={Effective Semi-autonomous Telepresence},
  author={Coltin, B. and Biswas, J. and Pomerleau, D. and Veloso, M.},
  journal={Proceedings of the RoboCup Symposium},
  year={2011},
  month={July},
  pages={289--300},
}


@Inproceedings(13icra-KollarEtAl,
       Author="Thomas Kollar and Vittorio Perera and Daniele Nardi and Manuela Veloso",
       title = "{Learning Environmental Knowledge from Task-Based Human-Robot Dialog}",
       BookTitle="Proceedings of ICRA'13, the IEEE International Conference on Robotics and Automation",
       Year="2013", Month="June", Address="Karlsruhe, Germany")

@Inproceedings(14icra-ColtinVeloso,
       Author = "Brian Coltin and Manuela Veloso",
       Title = "{Online Pickup and Delivery Planning with Transfers for Mobile Robots}",
       BookTitle="Proceedings of ICRA'14, 
                  the IEEE International Conference on Robotics and Automation",
       Year="2014", Month="June", Address="Hong Kong, China")




@article{reward,
author = { Fish Tung  and  Katerina Fragkiadaki},
title = {Reward Learning using Natural Language},
journal = {CVPR},
year = {2018}
}

@article{aaai-azaria-2016,
author = { Amos Azaria and Jayant Krishnamurthy and Tom M. Mitchell},
title = {Instructable Intelligent Personal Agent},
journal = {Proceedings of the AAAI Conference},
year = {2016},
url = {http://ai2-website.s3.amazonaws.com/publications/LearnByInst.pdf}
}


@article{shashank-2017,
author = {Shashank Srivastava and Igor Labutov and Tom M. Mitchell},
title = {Joint Concept Learning and Semantic Parsing from Natural Language Explanations},
journal = {Proceedings of Conference on Empirical Methods in Natural Language Processing (EMNLP)},
year = {2017},
url = {http://aclweb.org/anthology/D17-1161}
}



@article{shashank-2018,
author = {Shashank Srivastava and Igor Labutov and Tom M. Mitchell},
title = {Zeroshot Learning from Natural Language Quantification (submitted)},
year = {2018},
}

@article{toby-CHI2018,
author = {Toby Jia-Jun Li and Igor Labutov and Brad A. Myers and Tom M. Mitchell},
title = {Supporting Co-Adaptive Human-Agent Relationship through Programming by Demonstration using Existing GUIs (submitted)},
journal = {Proceedings of the 2018 CHI Workshop on Rethinking Interaction},
year = {2018},
url = {https://ex-situ.lri.fr/workshops/rethinkinginteraction-18}
}


@incollection{toby-showtell,
author = {Toby Jia-Jun Li and Igor Labutov and Brad A. Myers and Amos Azaria and Alexander I. Rudnicky and Tom M. Mitchell},
title = {An End User Development Approach for Failure Handling in Goal-oriented Conversational Agents},
publisher = {Springer (in press)},
booktitle = {Studies in Conversational UX Design},
editor = {Robert J. Moore and Margaret H. Szymanski and Raphael Arar and Guang-Jie Ren},
year = {2018}
}


@article{doi:10.1162/1064546053278973,
author = { Linda Smith  and  Michael Gasser },
title = {The Development of Embodied Cognition: Six Lessons from Babies},
journal = {Artificial Life},
volume = {11},
number = {1-2},
pages = {13-29},
year = {2005},
doi = {10.1162/1064546053278973},

URL = { 
        https://doi.org/10.1162/1064546053278973
    
},
eprint = { 
        https://doi.org/10.1162/1064546053278973
    
}
,
    abstract = { The embodiment hypothesis is the idea that intelligence emerges in the interaction of an agent with an environment and as a result of sensorimotor activity. We offer six lessons for developing embodied intelligent agents suggested by research in developmental psychology. We argue that starting as a baby grounded in a physical, social, and linguistic world is crucial to the development of the flexible and inventive intelligence that characterizes humankind. }
}




@article{DBLP:journals/corr/LillicrapHPHETS15,
  author    = {Timothy P. Lillicrap and
               Jonathan J. Hunt and
               Alexander Pritzel and
               Nicolas Heess and
               Tom Erez and
               Yuval Tassa and
               David Silver and
               Daan Wierstra},
  title     = {Continuous control with deep reinforcement learning},
  journal   = {CoRR},
  volume    = {abs/1509.02971},
  year      = {2015},
  url       = {http://arxiv.org/abs/1509.02971},
  archivePrefix = {arXiv},
  eprint    = {1509.02971},
  timestamp = {Wed, 07 Jun 2017 14:40:26 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LillicrapHPHETS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/KanskySMELLDSPG17,
  author    = {Ken Kansky and
               Tom Silver and
               David A. M{\'{e}}ly and
               Mohamed Eldawy and
               Miguel L{\'{a}}zaro{-}Gredilla and
               Xinghua Lou and
               Nimrod Dorfman and
               Szymon Sidor and
               D. Scott Phoenix and
               Dileep George},
  title     = {Schema Networks: Zero-shot Transfer with a Generative Causal Model
               of Intuitive Physics},
  journal   = {CoRR},
  volume    = {abs/1706.04317},
  year      = {2017},
  url       = {http://arxiv.org/abs/1706.04317},
  archivePrefix = {arXiv},
  eprint    = {1706.04317},
  timestamp = {Tue, 04 Jul 2017 09:48:42 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/KanskySMELLDSPG17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/HausmanCSSL17,
  author    = {Karol Hausman and
               Yevgen Chebotar and
               Stefan Schaal and
               Gaurav S. Sukhatme and
               Joseph J. Lim},
  title     = {Multi-Modal Imitation Learning from Unstructured Demonstrations using
               Generative Adversarial Nets},
  journal   = {CoRR},
  volume    = {abs/1705.10479},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.10479},
  archivePrefix = {arXiv},
  eprint    = {1705.10479},
  timestamp = {Sun, 26 Nov 2017 16:54:43 +0100},
  biburl    = {http://dblp.org/rec/bib/journals/corr/HausmanCSSL17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/FinnL16,
  author    = {Chelsea Finn and
               Sergey Levine},
  title     = {Deep Visual Foresight for Planning Robot Motion},
  journal   = {CoRR},
  volume    = {abs/1610.00696},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.00696},
  archivePrefix = {arXiv},
  eprint    = {1610.00696},
  timestamp = {Wed, 07 Jun 2017 14:42:20 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/FinnL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/NairCAIAML17,
  author    = {Ashvin Nair and
               Dian Chen and
               Pulkit Agrawal and
               Phillip Isola and
               Pieter Abbeel and
               Jitendra Malik and
               Sergey Levine},
  title     = {Combining Self-Supervised Learning and Imitation for Vision-Based
               Rope Manipulation},
  journal   = {CoRR},
  volume    = {abs/1703.02018},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.02018},
  archivePrefix = {arXiv},
  eprint    = {1703.02018},
  timestamp = {Wed, 07 Jun 2017 14:41:24 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/NairCAIAML17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/abs-1709-10087,
  author    = {Aravind Rajeswaran and
               Vikash Kumar and
               Abhishek Gupta and
               John Schulman and
               Emanuel Todorov and
               Sergey Levine},
  title     = {Learning Complex Dexterous Manipulation with Deep Reinforcement Learning
               and Demonstrations},
  journal   = {CoRR},
  volume    = {abs/1709.10087},
  year      = {2017},
  url       = {http://arxiv.org/abs/1709.10087},
  archivePrefix = {arXiv},
  eprint    = {1709.10087},
  timestamp = {Thu, 05 Oct 2017 09:43:05 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/abs-1709-10087},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{JMLR:v16:vapnik15b,
  author  = {Vladimir Vapnik and Rauf Izmailov},
  title   = {Learning Using Privileged Information: Similarity Control and Knowledge Transfer},
  journal = {Journal of Machine Learning Research},
  year    = {2015},
  volume  = {16},
  pages   = {2023-2049},
  url     = {http://jmlr.org/papers/v16/vapnik15b.html}
}

@article{DBLP:journals/corr/FinnLA16,
  author    = {Chelsea Finn and
               Sergey Levine and
               Pieter Abbeel},
  title     = {Guided Cost Learning: Deep Inverse Optimal Control via Policy Optimization},
  journal   = {CoRR},
  volume    = {abs/1603.00448},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.00448},
  archivePrefix = {arXiv},
  eprint    = {1603.00448},
  timestamp = {Wed, 07 Jun 2017 14:41:08 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/FinnLA16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Ng:2000:AIR:645529.657801,
 author = {Ng, Andrew Y. and Russell, Stuart J.},
 title = {Algorithms for Inverse Reinforcement Learning},
 booktitle = {Proceedings of the Seventeenth International Conference on Machine Learning},
 series = {ICML '00},
 year = {2000},
 isbn = {1-55860-707-2},
 pages = {663--670},
 numpages = {8},
 url = {http://dl.acm.org/citation.cfm?id=645529.657801},
 acmid = {657801},
 publisher = {Morgan Kaufmann Publishers Inc.},
 address = {San Francisco, CA, USA},
} 




@article{DBLP:journals/corr/ChenFLVGDZ15,
  author    = {Xinlei Chen and
               Hao Fang and
               Tsung{-}Yi Lin and
               Ramakrishna Vedantam and
               Saurabh Gupta and
               Piotr Doll{\'{a}}r and
               C. Lawrence Zitnick},
  title     = {Microsoft {COCO} Captions: Data Collection and Evaluation Server},
  journal   = {CoRR},
  volume    = {abs/1504.00325},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.00325},
  archivePrefix = {arXiv},
  eprint    = {1504.00325},
  timestamp = {Wed, 07 Jun 2017 14:41:06 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/ChenFLVGDZ15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/GuHLL16,
  author    = {Shixiang Gu and
               Ethan Holly and
               Timothy P. Lillicrap and
               Sergey Levine},
  title     = {Deep Reinforcement Learning for Robotic Manipulation},
  journal   = {CoRR},
  volume    = {abs/1610.00633},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.00633},
  archivePrefix = {arXiv},
  eprint    = {1610.00633},
  timestamp = {Wed, 07 Jun 2017 14:40:31 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/GuHLL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/KroemerS16,
  author    = {Oliver Kroemer and
               Gaurav S. Sukhatme},
  title     = {Learning Relevant Features for Manipulation Skills using Meta-Level
               Priors},
  journal   = {CoRR},
  volume    = {abs/1605.04439},
  year      = {2016},
  url       = {http://arxiv.org/abs/1605.04439},
  archivePrefix = {arXiv},
  eprint    = {1605.04439},
  timestamp = {Wed, 07 Jun 2017 14:42:29 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/KroemerS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Akgun:2012:TKK:2157689.2157815,
 author = {Akgun, Baris and Cakmak, Maya and Yoo, Jae Wook and Thomaz, Andrea Lockerd},
 title = {Trajectories and Keyframes for Kinesthetic Teaching: A Human-robot Interaction Perspective},
 booktitle = {Proceedings of the Seventh Annual ACM/IEEE International Conference on Human-Robot Interaction},
 series = {HRI '12},
 year = {2012},
 isbn = {978-1-4503-1063-5},
 location = {Boston, Massachusetts, USA},
 pages = {391--398},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/2157689.2157815},
 doi = {10.1145/2157689.2157815},
 acmid = {2157815},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {learning from demonstration},
} 



@article{DBLP:journals/corr/SungJS15,
  author    = {Jaeyong Sung and
               Seok Hyun Jin and
               Ashutosh Saxena},
  title     = {Robobarista: Object Part based Transfer of Manipulation Trajectories
               from Crowd-sourcing in 3D Pointclouds},
  journal   = {CoRR},
  volume    = {abs/1504.03071},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.03071},
  archivePrefix = {arXiv},
  eprint    = {1504.03071},
  timestamp = {Wed, 07 Jun 2017 14:42:19 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/SungJS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/RahmatizadehABL17,
  author    = {Rouhollah Rahmatizadeh and
               Pooya Abolghasemi and
               Ladislau B{\"{o}}l{\"{o}}ni and
               Sergey Levine},
  title     = {Vision-Based Multi-Task Manipulation for Inexpensive Robots Using
               End-To-End Learning from Demonstration},
  journal   = {CoRR},
  volume    = {abs/1707.02920},
  year      = {2017},
  url       = {http://arxiv.org/abs/1707.02920},
  archivePrefix = {arXiv},
  eprint    = {1707.02920},
  timestamp = {Sat, 05 Aug 2017 14:56:06 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/RahmatizadehABL17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{DBLP:journals/corr/LiuGAL17,
  author    = {Yuxuan Liu and
               Abhishek Gupta and
               Pieter Abbeel and
               Sergey Levine},
  title     = {Imitation from Observation: Learning to Imitate Behaviors from Raw
               Video via Context Translation},
  journal   = {CoRR},
  volume    = {abs/1707.03374},
  year      = {2017},
  url       = {http://arxiv.org/abs/1707.03374},
  archivePrefix = {arXiv},
  eprint    = {1707.03374},
  timestamp = {Sat, 05 Aug 2017 14:56:08 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LiuGAL17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{PatrauceanHC16,
  author    = {Viorica P{\u a}tr{\u a}ucean and
               Ankur Handa and
               Roberto Cipolla},
  title     = {Spatio-temporal video autoencoder with differentiable memory},
  booktitle = {International Conference on Learning Representations (ICLR) Workshop},
  year      = {2016}
}


@article{DBLP:journals/corr/SadeghianAS17,
  author    = {Amir Sadeghian and
               Alexandre Alahi and
               Silvio Savarese},
  title     = {Tracking The Untrackable: Learning To Track Multiple Cues with Long-Term
               Dependencies},
  journal   = {CoRR},
  volume    = {abs/1701.01909},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.01909},
  timestamp = {Wed, 07 Jun 2017 14:40:23 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/SadeghianAS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/McCormacHDL16,
  author    = {John McCormac and
               Ankur Handa and
               Andrew J. Davison and
               Stefan Leutenegger},
  title     = {SemanticFusion: Dense 3D Semantic Mapping with Convolutional Neural
               Networks},
  journal   = {CoRR},
  volume    = {abs/1609.05130},
  year      = {2016},
  url       = {http://arxiv.org/abs/1609.05130},
  timestamp = {Wed, 07 Jun 2017 14:42:17 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/McCormacHDL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/MalmaudHRJRM15,
  author    = {Jonathan Malmaud and
               Jonathan Huang and
               Vivek Rathod and
               Nick Johnston and
               Andrew Rabinovich and
               Kevin Murphy},
  title     = {What's Cookin'? Interpreting Cooking Videos using Text, Speech and
               Vision},
  journal   = {CoRR},
  volume    = {abs/1503.01558},
  year      = {2015},
  url       = {http://arxiv.org/abs/1503.01558},
  timestamp = {Wed, 07 Jun 2017 14:42:04 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MalmaudHRJRM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/RedmonF16,
  author    = {Joseph Redmon and
               Ali Farhadi},
  title     = {{YOLO9000:} Better, Faster, Stronger},
  journal   = {CoRR},
  volume    = {abs/1612.08242},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.08242},
  timestamp = {Wed, 07 Jun 2017 14:40:20 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RedmonF16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/LongSD14,
  author    = {Jonathan Long and
               Evan Shelhamer and
               Trevor Darrell},
  title     = {Fully Convolutional Networks for Semantic Segmentation},
  journal   = {CoRR},
  volume    = {abs/1411.4038},
  year      = {2014},
  url       = {http://arxiv.org/abs/1411.4038},
  timestamp = {Wed, 07 Jun 2017 14:42:28 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LongSD14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@ARTICLE{SilverHuangEtAl16nature,
  author = {Silver, David and Huang, Aja and Maddison, Chris J. and Guez, Arthur and Sifre, Laurent and van den Driessche, George and Schrittwieser, Julian and Antonoglou, Ioannis and Panneershelvam, Veda and Lanctot, Marc and Dieleman, Sander and Grewe, Dominik and Nham, John and Kalchbrenner, Nal and Sutskever, Ilya and Lillicrap, Timothy and Leach, Madeleine and Kavukcuoglu, Koray and Graepel, Thore and Hassabis, Demis},
  journal = {Nature},
  title = {Mastering the Game of Go with Deep Neural Networks and Tree Search},
  volume = {529},
  year = {2016}
}

@inproceedings{Hasselt:2016:DRL:3016100.3016191,
 author = {Hasselt, Hado van and Guez, Arthur and Silver, David},
 title = {Deep Reinforcement Learning with Double Q-Learning},
 booktitle = {Proceedings of the Thirtieth AAAI Conference on Artificial Intelligence},
 series = {AAAI'16},
 year = {2016},
 location = {Phoenix, Arizona},
 pages = {2094--2100},
 numpages = {7},
 url = {http://dl.acm.org/citation.cfm?id=3016100.3016191},
 acmid = {3016191},
 publisher = {AAAI Press},
} 


@inproceedings{cao2017realtime,
  author = {Zhe Cao and Tomas Simon and Shih-En Wei and Yaser Sheikh},
  booktitle = {CVPR},
  title = {Realtime Multi-Person 2D Pose Estimation using Part Affinity Fields},
  year = {2017}
}

@inproceedings{simon2017hand,
  author = {Tomas Simon and Hanbyul Joo and Iain Matthews and Yaser Sheikh},
  booktitle = {CVPR},
  title = {Hand Keypoint Detection in Single Images using Multiview Bootstrapping},
  year = {2017}
}

@inproceedings{wei2016cpm,
  author = {Shih-En Wei and Varun Ramakrishna and Takeo Kanade and Yaser Sheikh},
  booktitle = {CVPR},
  title = {Convolutional pose machines},
  year = {2016}
}

@article{DBLP:journals/corr/PathakAED17,
  author    = {Deepak Pathak and
               Pulkit Agrawal and
               Alexei A. Efros and
               Trevor Darrell},
  title     = {Curiosity-driven Exploration by Self-supervised Prediction},
  journal   = {CoRR},
  volume    = {abs/1705.05363},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.05363},
  archivePrefix = {arXiv},
  eprint    = {1705.05363},
  timestamp = {Wed, 07 Jun 2017 14:41:47 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/PathakAED17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@ARTICLE{Browne2012,
  ABSTRACT = {Monte Carlo Tree Search (MCTS) is a recently proposed search method that combines the precision of tree search with the generality of random sampling. It has received considerable interest due to its spectacular success in the difficult problem of computer Go, but has also proved beneficial in a range of other domains. This paper is a survey of the literature to date, intended to provide a snapshot of the state of the art after the first five years of MCTS research. We outline the core algorithm’s derivation, impart some structure on the many variations and enhancements that have been proposed, and summarise the results from the key game and non-game domains to which MCTS methods have been applied. A number of open research questions indicate that the field is ripe for future work.},
  AUTHOR   = {Browne, Cb and Powley, Edward},
  DOI      = {10.1109/TCIAIG.2012.2186810},
  FILE     = {http://bib.unthinkingdepths.fr/seb/pdf/Browne, Powley_2012_A survey of monte carlo tree search methods.pdf},
  ISSN     = {1943-068X},
  JOURNAL  = {Intelligence and AI},
  NUMBER   = {1},
  PAGES    = {1--49},
  TITLE    = {{A survey of monte carlo tree search methods}},
  URL      = {http://ieeexplore.ieee.org/xpls/abs_all.jsp?arnumber=6145622},
  VOLUME   = {4},
  YEAR     = {2012},
}

@inproceedings{deitke2020robothor,
  title={Robothor: An open simulation-to-real embodied AI platform. In 2020 IEEE},
  author={Deitke, Matt and Han, Winson and Herrasti, Alvaro and Kembhavi, Aniruddha and Kolve, Eric and Mottaghi, Roozbeh and Salvador, Jordi and Schwenk, Dustin and VanderBilt, Eli and Wallingford, Matthew and others},
  booktitle={CVF Conference on Computer Vision and Pattern Recognition, CVPR},
  pages={13--19},
  year={2020}
}

@article{murali2019pyrobot,
  title={Pyrobot: An open-source robotics framework for research and benchmarking},
  author={Murali, Adithyavairavan and Chen, Tao and Alwala, Kalyan Vasudev and Gandhi, Dhiraj and Pinto, Lerrel and Gupta, Saurabh and Gupta, Abhinav},
  journal={arXiv preprint arXiv:1906.08236},
  year={2019}
}


@article{DBLP:journals/corr/KhorevaBIBS17,
  author    = {Anna Khoreva and
               Rodrigo Benenson and
               Eddy Ilg and
               Thomas Brox and
               Bernt Schiele},
  title     = {Lucid Data Dreaming for Object Tracking},
  journal   = {CoRR},
  volume    = {abs/1703.09554},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.09554},
  timestamp = {Wed, 07 Jun 2017 14:43:15 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KhorevaBIBS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@INPROCEEDINGS{Whelan-RSS-15, 
    AUTHOR    = {Thomas Whelan AND Stefan Leutenegger AND Renato Salas Moreno AND Ben Glocker AND Andrew Davison}, 
    TITLE     = {ElasticFusion: Dense SLAM Without A Pose Graph}, 
    BOOKTITLE = {Proceedings of Robotics: Science and Systems}, 
    YEAR      = {2015}, 
    ADDRESS   = {Rome, Italy}, 
    MONTH     = {July},
    DOI       = {10.15607/RSS.2015.XI.001} 
} 
  
  
@article{DBLP:journals/corr/RitchieHG16,
  author    = {Daniel Ritchie and
               Paul Horsfall and
               Noah D. Goodman},
  title     = {Deep Amortized Inference for Probabilistic Programs},
  journal   = {CoRR},
  volume    = {abs/1610.05735},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.05735},
  timestamp = {Wed, 07 Jun 2017 14:42:26 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RitchieHG16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@misc{ceres-solver,
  author = "Sameer Agarwal and Keir Mierle and Others",
  title = "Ceres Solver",
  howpublished = "\url{http://ceres-solver.org}",
}

@article{DBLP:journals/corr/CarreiraAFM15,
  author    = {Jo{\~{a}}o Carreira and
               Pulkit Agrawal and
               Katerina Fragkiadaki and
               Jitendra Malik},
  title     = {Human Pose Estimation with Iterative Error Feedback},
  journal   = {CoRR},
  volume    = {abs/1507.06550},
  year      = {2015},
}

@article{DBLP:journals/corr/FischerDIHHGSCB15,
  author    = {Philipp Fischer and
               Alexey Dosovitskiy and
               Eddy Ilg and
               Philip H{\"{a}}usser and
               Caner Hazirbas and
               Vladimir Golkov and
               Patrick van der Smagt and
               Daniel Cremers and
               Thomas Brox},
  title     = {FlowNet: Learning Optical Flow with Convolutional Networks},
  journal   = {CoRR},
  volume    = {abs/1504.06852},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.06852},
  timestamp = {Wed, 07 Jun 2017 14:41:04 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/FischerDIHHGSCB15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@incollection{NIPS2014_5421,
title = {Deep Learning for Real-Time Atari Game Play Using Offline Monte-Carlo Tree Search Planning},
author = {Guo, Xiaoxiao and Singh, Satinder and Lee, Honglak and Lewis, Richard L and Wang, Xiaoshi},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {3338--3346},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5421-deep-learning-for-real-time-atari-game-play-using-offline-monte-carlo-tree-search-planning.pdf}
}

@inproceedings{Silberer2013ModelsOS,
  title={Models of Semantic Representation with Visual Attributes},
  author={Carina Silberer and Vittorio Ferrari and Mirella Lapata},
  booktitle={ACL},
  year={2013}
}

@article{carreira2017quo,
  title={Quo Vadis, Action Recognition? A New Model and the Kinetics Dataset},
  author={Carreira, Joao and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1705.07750},
  year={2017}
}

@article{DBLP:journals/corr/WestonCB14,
  author    = {Jason Weston and
               Sumit Chopra and
               Antoine Bordes},
  title     = {Memory Networks},
  journal   = {CoRR},
  volume    = {abs/1410.3916},
  year      = {2014},
  url       = {http://arxiv.org/abs/1410.3916},
  timestamp = {Wed, 07 Jun 2017 14:41:04 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/WestonCB14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@incollection{NIPS2015_5945,
title = {Teaching Machines to Read and Comprehend},
author = {Hermann, Karl Moritz and Kocisky, Tomas and Grefenstette, Edward and Espeholt, Lasse and Kay, Will and Suleyman, Mustafa and Blunsom, Phil},
booktitle = {Advances in Neural Information Processing Systems 28},
editor = {C. Cortes and N. D. Lawrence and D. D. Lee and M. Sugiyama and R. Garnett},
pages = {1693--1701},
year = {2015},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5945-teaching-machines-to-read-and-comprehend.pdf}
}

@article{DBLP:journals/corr/KadlecSBK16,
  author    = {Rudolf Kadlec and
               Martin Schmid and
               Ondrej Bajgar and
               Jan Kleindienst},
  title     = {Text Understanding with the Attention Sum Reader Network},
  journal   = {CoRR},
  volume    = {abs/1603.01547},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.01547},
  timestamp = {Wed, 07 Jun 2017 14:41:38 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KadlecSBK16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Article:00:Glenberg:hallsa,
    author = {Glenberg, A. and Robertson, D.},
    citeulike-article-id = {850491},
    citeulike-linkout-0 = {http://psych.wisc.edu/glenberg/},
    journal = {Journal of {M}emory and {L}anguage},
    keywords = {bibtex-import},
    posted-at = {2006-09-20 03:18:45},
    priority = {0},
    title = {Symbol grounding and meaning: {A} comparison of high-dimensional and embodied theories of meaning.},
    url = {http://psych.wisc.edu/glenberg/},
    year = {2000}
}



@article{DBLP:journals/corr/DhingraLCS16,
  author    = {Bhuwan Dhingra and
               Hanxiao Liu and
               William W. Cohen and
               Ruslan Salakhutdinov},
  title     = {Gated-Attention Readers for Text Comprehension},
  journal   = {CoRR},
  volume    = {abs/1606.01549},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.01549},
  timestamp = {Wed, 07 Jun 2017 14:42:11 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/DhingraLCS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/SeoKFH16,
  author    = {Min Joon Seo and
               Aniruddha Kembhavi and
               Ali Farhadi and
               Hannaneh Hajishirzi},
  title     = {Bidirectional Attention Flow for Machine Comprehension},
  journal   = {CoRR},
  volume    = {abs/1611.01603},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.01603},
  timestamp = {Wed, 07 Jun 2017 14:41:03 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/SeoKFH16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}







@inproceedings{donahue2015long,
  title={Long-term Recurrent Convolutional Networks for Visual Recognition and Description},
  author={Donahue, Jeff and Hendricks, Lisa Anne and Guadarrama, Sergio and Rohrbach, Marcus and Venugopalan, Subhashini and Saenko, Kate and Darrell, Trevor},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2015}
}



@inproceedings{kazemi2014one,
  title={One Millisecond Face Alignment with an Ensemble of Regression Trees},
  author={Kazemi, Vahid and Sullivan, Josephine},
  booktitle={CVPR},
  year={2014}
}

@article{DBLP:journals/corr/KimLL15a,
  author    = {Jiwon Kim and
               Jung Kwon Lee and
               Kyoung Mu Lee},
  title     = {Deeply-Recursive Convolutional Network for Image Super-Resolution},
  journal   = {CoRR},
  volume    = {abs/1511.04491},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.04491},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KimLL15a},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{pennington2014glove,
  author = {Jeffrey Pennington and Richard Socher and Christopher D. Manning},
  booktitle = {Empirical Methods in Natural Language Processing (EMNLP)},
  title = {GloVe: Global Vectors for Word Representation},
  year = {2014},
  pages = {1532--1543},
  url = {http://www.aclweb.org/anthology/D14-1162},
}

@article{Gupta:2015:ISU:2750551.2750559,
 author = {Gupta, Saurabh and Arbel\'{a}ez, Pablo and Girshick, Ross and Malik, Jitendra},
 title = {Indoor Scene Understanding with RGB-D Images: Bottom-up Segmentation, Object Detection and Semantic Segmentation},
 journal = {Int. J. Comput. Vision},
 issue_date = {April     2015},
 volume = {112},
 number = {2},
 month = apr,
 year = {2015},
 issn = {0920-5691},
 pages = {133--149},
 numpages = {17},
 url = {http://dx.doi.org/10.1007/s11263-014-0777-6},
 doi = {10.1007/s11263-014-0777-6},
 acmid = {2750559},
 publisher = {Kluwer Academic Publishers},
 address = {Hingham, MA, USA},
 keywords = {RGB-D contour detection, RGB-D image segmentation, RGB-D object detection, RGB-D scene classification, RGB-D semantic segmentation},
} 

@article{DBLP:journals/corr/TungHSF17,
  author    = {Hsiao{-}Yu Fish Tung and
               Adam Harley and
               William Seto and
               Katerina Fragkiadaki},
  title     = {Adversarial Inversion: Inverse Graphics with Adversarial Priors},
  journal   = {CoRR},
  volume    = {abs/1705.11166},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.11166},
  timestamp = {Wed, 07 Jun 2017 14:41:13 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/TungHSF17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{turbosquid,
  author       = {https://www.turbosquid.com/6},
}

@article{cgtrader,
  author    = {https://www.cgtrader.com/},
 % url       = {https://www.cgtrader.com/},
}


@article{mocap,
  author    = {Hsiao{-}Yu Fish Tung and
               Wei Tung and
               Ersin Yumer and
               Katerina Fragkiadaki},
  title     = {Self-supervised learning of Motion Capture},
  journal   = {under submission},
  year      = {2017}
}

@inproceedings{andriluka14cvpr,
               author = {Mykhaylo Andriluka and Leonid Pishchulin and Peter Gehler and Schiele, Bernt},
               title = {2D Human Pose Estimation: New Benchmark and State of the Art Analysis},
               booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
               year = {2014},
               month = {June}
}
@article{inversionearlier,
  author    = {Fish Tung and Katerina Fragkiadaki},
  title     = {Inverse Problems in Computer Vision with Adversarial Imagination Priors},
  journal   = {openreview},
  year      = {2016}
}




@article{deeppaint,
  author    = {Kushagr Gupta and
               Suleman Kazi and
               Terry Kong},
  title     = {DeepPaint: A Tool for Image Inpainting},
  journal   = {tech. report},
  year      = {2016}
}

@article{DBLP:journals/corr/DongNWG17,
  author    = {Hao Dong and
               Paarth Neekhara and
               Chao Wu and
               Yike Guo},
  title     = {Unsupervised Image-to-Image Translation with Generative Adversarial
               Networks},
  journal   = {CoRR},
  volume    = {abs/1701.02676},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.02676},
  timestamp = {Wed, 01 Feb 2017 17:47:56 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/DongNWG17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/YanYSL15,
  author    = {Xinchen Yan and
               Jimei Yang and
               Kihyuk Sohn and
               Honglak Lee},
  title     = {Attribute2Image: Conditional Image Generation from Visual Attributes},
  journal   = {CoRR},
  volume    = {abs/1512.00570},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.00570},
  timestamp = {Sat, 02 Jan 2016 11:38:49 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/YanYSL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{DBLP:journals/corr/LedigTHCATTWS16,
  author    = {Christian Ledig and
               Lucas Theis and
               Ferenc Huszar and
               Jose Caballero and
               Andrew P. Aitken and
               Alykhan Tejani and
               Johannes Totz and
               Zehan Wang and
               Wenzhe Shi},
  title     = {Photo-Realistic Single Image Super-Resolution Using a Generative Adversarial
               Network},
  journal   = {CoRR},
  volume    = {abs/1609.04802},
  year      = {2016},
  url       = {http://arxiv.org/abs/1609.04802},
  timestamp = {Tue, 04 Oct 2016 08:10:36 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LedigTHCATTWS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/cvpr/MaoHTCY016,
  author    = {Junhua Mao and
               Jonathan Huang and
               Alexander Toshev and
               Oana Camburu and
               Alan L. Yuille and
               Kevin Murphy},
  title     = {Generation and Comprehension of Unambiguous Object Descriptions},
  booktitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016},
  pages     = {11--20},
  year      = {2016},
  crossref  = {DBLP:conf/cvpr/2016},
  url       = {https://doi.org/10.1109/CVPR.2016.9},
  doi       = {10.1109/CVPR.2016.9},
  timestamp = {Thu, 25 May 2017 00:41:21 +0200},
  biburl    = {http://dblp.org/rec/bib/conf/cvpr/MaoHTCY016},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/BrunaSL15,
  author    = {Joan Bruna and
               Pablo Sprechmann and
               Yann LeCun},
  title     = {Super-Resolution with Deep Convolutional Sufficient Statistics},
  journal   = {CoRR},
  volume    = {abs/1511.05666},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.05666},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/BrunaSL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}












@article{ramakrishna2012reconstructing,
  title={{Reconstructing 3d Human Pose from 2d Image Landmarks}},
  author={Ramakrishna, V. and Kanade, T. and Sheikh, Y.},
  journal={Computer Vision--ECCV 2012},
  pages={573--586},
  year={2012},
  publisher={Springer}
}

@article{DBLP:journals/corr/ChenR16a,
  author    = {Ching{-}Hang Chen and
               Deva Ramanan},
  title     = {3D Human Pose Estimation = 2D Pose Estimation + Matching},
  journal   = {CoRR},
  volume    = {abs/1612.06524},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.06524},
  timestamp = {Mon, 02 Jan 2017 11:09:15 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/ChenR16a},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/icra/JaeglePD16,
  author    = {Andrew Jaegle and
               Stephen Phillips and
               Kostas Daniilidis},
  title     = {Fast, robust, continuous monocular egomotion computation},
  booktitle = {2016 {IEEE} International Conference on Robotics and Automation, {ICRA}
               2016, Stockholm, Sweden, May 16-21, 2016},
  pages     = {773--780},
  year      = {2016},
  crossref  = {DBLP:conf/icra/2016},
  url       = {http://dx.doi.org/10.1109/ICRA.2016.7487206},
  doi       = {10.1109/ICRA.2016.7487206},
  timestamp = {Tue, 14 Jun 2016 19:35:07 +0200},
  biburl    = {http://dblp2.uni-trier.de/rec/bib/conf/icra/JaeglePD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/RogezS16,
  author    = {Gr{\'{e}}gory Rogez and
               Cordelia Schmid},
  title     = {MoCap-guided Data Augmentation for 3D Pose Estimation in the Wild},
  journal   = {CoRR},
  volume    = {abs/1607.02046},
  year      = {2016},
  url       = {http://arxiv.org/abs/1607.02046},
  timestamp = {Tue, 02 Aug 2016 12:59:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RogezS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}
@article{DBLP:journals/corr/ZhouZPLDD17,
  author    = {Xiaowei Zhou and
               Menglong Zhu and
               Georgios Pavlakos and
               Spyridon Leonardos and
               Konstantinos G. Derpanis and
               Kostas Daniilidis},
  title     = {MonoCap: Monocular Human Motion Capture using a {CNN} Coupled with
               a Geometric Prior},
  journal   = {CoRR},
  volume    = {abs/1701.02354},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.02354},
  timestamp = {Wed, 01 Feb 2017 17:47:56 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/ZhouZPLDD17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/PavlakosZDD16,
  author    = {Georgios Pavlakos and
               Xiaowei Zhou and
               Konstantinos G. Derpanis and
               Kostas Daniilidis},
  title     = {Coarse-to-Fine Volumetric Prediction for Single-Image 3D Human Pose},
  journal   = {CoRR},
  volume    = {abs/1611.07828},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.07828},
  timestamp = {Thu, 01 Dec 2016 19:32:08 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/PavlakosZDD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/TomeRA17,
  author    = {Denis Tom{\`{e}} and
               Chris Russell and
               Lourdes Agapito},
  title     = {Lifting from the Deep: Convolutional 3D Pose Estimation from a Single
               Image},
  journal   = {CoRR},
  volume    = {abs/1701.00295},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.00295},
  timestamp = {Wed, 01 Feb 2017 17:47:56 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/TomeRA17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{liu2015faceattributes,
 author = {Ziwei Liu and Ping Luo and Xiaogang Wang and Xiaoou Tang},
 title = {Deep Learning Face Attributes in the Wild},
 booktitle = {Proceedings of International Conference on Computer Vision (ICCV)},
 month = December,
 year = {2015} 
}


@book{lumpkin2012high,
  title={A High Level Language for Human Robot Interaction},
  author={Lumpkin, B.T.},
  url={https://books.google.com/books?id=PO5FnQAACAAJ},
  year={2012}
}


@article{DBLP:journals/corr/DePalmaB16a,
  author    = {Nick DePalma and
               Cynthia Breazeal},
  title     = {Towards learning through robotic interaction alone: the joint guided
               search task},
  journal   = {CoRR},
  volume    = {abs/1606.02632},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.02632},
  archivePrefix = {arXiv},
  eprint    = {1606.02632},
  timestamp = {Wed, 07 Jun 2017 14:41:12 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/DePalmaB16a},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Mohseni-Kabir:2016:IRP:2906831.2906936,
 author = {Mohseni-Kabir, Anahita and Chernova, Sonia and Rich, Charles},
 title = {Identifying Reusable Primitives in Narrated Demonstrations},
 booktitle = {The Eleventh ACM/IEEE International Conference on Human Robot Interaction},
 series = {HRI '16},
 year = {2016},
 isbn = {978-1-4673-8370-7},
 location = {Christchurch, New Zealand},
 pages = {479--480},
 numpages = {2},
 url = {http://dl.acm.org/citation.cfm?id=2906831.2906936},
 acmid = {2906936},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
 keywords = {human action segmentation, human behavior understanding, human-robot interaction, learning action primitives, motif discovery, robot learning from demonstration},
} 


@incollection{Bengio+chapter2007,
author = {Bengio, Yoshua and LeCun, Yann},
booktitle = {Large Scale Kernel Machines},
publisher = {MIT Press},
title = {Scaling Learning Algorithms Towards {AI}},
year = {2007}
}

@article{Hinton06,
author = {Hinton, Geoffrey E. and Osindero, Simon and Teh, Yee Whye},
journal = {Neural Computation},
pages = {1527--1554},
title = {A Fast Learning Algorithm for Deep Belief Nets},
volume = {18},
year = {2006}
}

@article{DBLP:journals/corr/UmmenhoferZUMID16,
  author    = {Benjamin Ummenhofer and
               Huizhong Zhou and
               Jonas Uhrig and
               Nikolaus Mayer and
               Eddy Ilg and
               Alexey Dosovitskiy and
               Thomas Brox},
  title     = {DeMoN: Depth and Motion Network for Learning Monocular Stereo},
  journal   = {CoRR},
  volume    = {abs/1612.02401},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.02401},
  timestamp = {Wed, 07 Jun 2017 14:41:36 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/UmmenhoferZUMID16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@misc{45166,
title = {TensorFlow: Large-Scale Machine Learning on Heterogeneous Distributed Systems},
author  = {Martín Abadi and Ashish Agarwal and Paul Barham and Eugene Brevdo and Zhifeng Chen and Craig Citro and Greg Corrado and Andy Davis and Jeffrey Dean and Matthieu Devin and Sanjay Ghemawat and Ian Goodfellow and Andrew Harp and Geoffrey Irving and Michael Isard and Yangqing Jia and Rafal Jozefowicz and Lukasz Kaiser and Manjunath Kudlur and Josh Levenberg and Dan Mané and Rajat Monga and Sherry Moore and Derek Murray and Chris Olah and Mike Schuster and Jonathon Shlens and Benoit Steiner and Ilya Sutskever and Kunal Talwar and Paul Tucker and Vincent Vanhoucke and Vijay Vasudevan and Fernanda Viégas and Oriol Vinyals and Pete Warden and Martin Wattenberg and Martin Wicke and Yuan Yu and Xiaoqiang Zheng},
year  = 2015,
URL = {http://download.tensorflow.org/paper/whitepaper2015.pdf}
}



@incollection{NIPS2012_4824,
title = {ImageNet Classification with Deep Convolutional Neural Networks},
author = {Alex Krizhevsky and Sutskever, Ilya and Geoffrey E. Hinton},
booktitle = {Advances in Neural Information Processing Systems 25},
editor = {F. Pereira and C. J. C. Burges and L. Bottou and K. Q. Weinberger},
pages = {1097--1105},
year = {2012},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/4824-imagenet-classification-with-deep-convolutional-neural-networks.pdf}
}

@inproceedings{imagenet_cvpr09,
        AUTHOR = {Deng, J. and Dong, W. and Socher, R. and Li, L.-J. and Li, K. and Fei-Fei, L.},
        TITLE = {{ImageNet: A Large-Scale Hierarchical Image Database}},
        BOOKTITLE = {CVPR09},
        YEAR = {2009},
        BIBSOURCE = "http://www.image-net.org/papers/imagenet_cvpr09.bib"}
        
        
@article{mnist,
  added-at = {2010-06-28T21:16:30.000+0200},
  author = {LeCun, Yann and Cortes, Corinna},
  biburl = {http://www.bibsonomy.org/bibtex/2935bad99fa1f65e03c25b315aa3c1032/mhwombat},
  groups = {public},
  howpublished = {http://yann.lecun.com/exdb/mnist/},
  interhash = {21b9d0558bd66279df9452562df6e6f3},
  intrahash = {935bad99fa1f65e03c25b315aa3c1032},
  keywords = {MSc _checked character_recognition mnist network neural},
  lastchecked = {2016-01-14 14:24:11},
  timestamp = {2016-07-12T19:25:30.000+0200},
  title = {{MNIST} handwritten digit database},
  url = {http://yann.lecun.com/exdb/mnist/},
  username = {mhwombat},
  year = 2010
}

@INPROCEEDINGS{grosse09intrinsic,
   AUTHOR = "Roger Grosse and Micah K. Johnson and Edward H. Adelson and William T. Freeman",
    TITLE = "Ground-truth dataset and baseline evaluations for intrinsic image algorithms",
    PAGES = "2335--2342",
     YEAR = "2009",
BOOKTITLE = "International Conference on Computer Vision",
      DOI = "http://dx.doi.org/10.1109/ICCV.2009.5459428"
}

@article{DBLP:journals/corr/TomeRA17,
  author    = {Denis Tom{\`{e}} and
               Chris Russell and
               Lourdes Agapito},
  title     = {Lifting from the Deep: Convolutional 3D Pose Estimation from a Single
               Image},
  journal   = {CoRR},
  volume    = {abs/1701.00295},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.00295},
  timestamp = {Wed, 01 Feb 2017 17:47:56 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/TomeRA17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/WangWLYG14,
  author    = {Chunyu Wang and
               Yizhou Wang and
               Zhouchen Lin and
               Alan L. Yuille and
               Wen Gao},
  title     = {Robust Estimation of 3D Human Poses from a Single Image},
  journal   = {CoRR},
  volume    = {abs/1406.2282},
  year      = {2014},
  url       = {http://arxiv.org/abs/1406.2282},
  timestamp = {Tue, 31 May 2016 18:15:20 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/WangWLYG14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Aubry14,
  title={Seeing 3D chairs: exemplar part-based 2D-3D alignment using a large dataset of CAD models},
  author={Aubry, Mathieu and Maturana, Daniel and Efros, Alexei, and Russell, Bryan and Sivic, Josef},
  booktitle={CVPR},
  year={2014},
}

@inproceedings{SUN,
  added-at = {2014-07-31T00:00:00.000+0200},
  author = {Xiao, Jianxiong and Hays, James and Ehinger, Krista A. and Oliva, Aude and Torralba, Antonio},
  biburl = {http://www.bibsonomy.org/bibtex/232294b312a372e89fbb447d12d904dc7/dblp},
  booktitle = {CVPR},
  crossref = {conf/cvpr/2010},
  ee = {http://doi.ieeecomputersociety.org/10.1109/CVPR.2010.5539970},
  interhash = {496f3934a4f2a511117f43d385da847c},
  intrahash = {32294b312a372e89fbb447d12d904dc7},
  isbn = {978-1-4244-6984-0},
  keywords = {dblp},
  pages = {3485-3492},
  publisher = {IEEE Computer Society},
  timestamp = {2015-06-19T16:09:09.000+0200},
  title = {SUN database: Large-scale scene recognition from abbey to zoo.},
  url = {http://dblp.uni-trier.de/db/conf/cvpr/cvpr2010.html#XiaoHEOT10},
  year = 2010
}


@inproceedings{LSUN,
	author     = {Fisher Yu and Yinda Zhang and Shuran Song and Ari Seff and Jianxiong Xiao},
	title      = {{LSUN}: Construction of a Large-scale Image Dataset using Deep Learning with Humans in the Loop},
	booktitle  = arXiv,
	year       = {2015},
}

@inproceedings{PICTURE,
  added-at = {2015-10-16T00:00:00.000+0200},
  author = {Kulkarni, Tejas D. and Kohli, Pushmeet and Tenenbaum, Joshua B. and Mansinghka, Vikash K.},
  biburl = {http://www.bibsonomy.org/bibtex/28cb5b89a60ae4e2624c880bfb7c50638/dblp},
  booktitle = {CVPR},
  crossref = {conf/cvpr/2015},
  ee = {http://dx.doi.org/10.1109/CVPR.2015.7299068},
  interhash = {a234af7842af65c7bfe363459cfd6e3d},
  intrahash = {8cb5b89a60ae4e2624c880bfb7c50638},
  isbn = {978-1-4673-6964-0},
  keywords = {dblp},
  pages = {4390-4399},
  publisher = {IEEE Computer Society},
  timestamp = {2016-04-29T11:54:14.000+0200},
  title = {Picture: A probabilistic programming language for scene perception.},
  url = {http://dblp.uni-trier.de/db/conf/cvpr/cvpr2015.html#KulkarniKTM15},
  year = 2015
}

@TECHREPORT{Yu03computationalmodels,
    author = {Stella Yu},
    title = {Computational Models of Perceptual Organization},
    institution = {Robotics Institute, Carnegie Mellon University},
    year = {2003}
}
@book{Knill:1996:PBI:239481,
 editor = {Knill, David C. and Richards, Whitman},
 title = {Perception As Bayesian Inference},
 year = {1996},
 isbn = {0-521-46109-X},
 publisher = {Cambridge University Press},
 address = {New York, NY, USA},
} 
@inproceedings{bruno,
  author = {Olshausen, Bruno},
  booktitle = {The Cognitive Neurosciences},
  publisher = {MIT Press},
  timestamp = {2016-04-29T11:54:14.000+0200},
  title = {Perception as an Inference Problem},
  year = 2013
}


@incollection{NIPS2014_5423,
title = {Generative Adversarial Nets},
author = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {2672--2680},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5423-generative-adversarial-nets.pdf}
}

@inproceedings{Sheikh_2008_6196,
   author = "Ijaz Akhter and Yaser Ajmal Sheikh and Sohaib Khan and Takeo Kanade",
   title = "Nonrigid Structure from Motion in Trajectory Space",
   booktitle = "Neural Information Processing Systems",
   month = "December",
   year = "2008",
}


@inproceedings{DBLP:conf/cvpr/NarihiraMY15,
  author    = {Takuya Narihira and
               Michael Maire and
               Stella X. Yu},
  title     = {Learning lightness from human judgement on relative reflectance},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2015, Boston, MA, USA, June 7-12, 2015},
  pages     = {2965--2973},
  year      = {2015},
  crossref  = {DBLP:conf/cvpr/2015},
  url       = {http://dx.doi.org/10.1109/CVPR.2015.7298915},
  doi       = {10.1109/CVPR.2015.7298915},
  timestamp = {Thu, 28 Apr 2016 10:52:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/cvpr/NarihiraMY15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{h36m_pami,
author = {Ionescu, Catalin and Papava, Dragos and Olaru, Vlad and Sminchisescu,  Cristian},
title = {Human3.6M: Large Scale Datasets and Predictive Methods for 3D Human Sensing in Natural Environments},
journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
publisher = {IEEE Computer Society},
volume = {36},
number = {7},
pages = {1325-1339},
month = {jul},
year = {2014}
}

@article{DBLP:journals/corr/KulkarniWKT15,
  author    = {Tejas D. Kulkarni and
               Will Whitney and
               Pushmeet Kohli and
               Joshua B. Tenenbaum},
  title     = {Deep Convolutional Inverse Graphics Network},
  journal   = {CoRR},
  volume    = {abs/1503.03167},
  year      = {2015},
  url       = {http://arxiv.org/abs/1503.03167},
  timestamp = {Thu, 09 Apr 2015 11:33:20 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KulkarniWKT15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/DongLHT15,
  author    = {Chao Dong and
               Chen Change Loy and
               Kaiming He and
               Xiaoou Tang},
  title     = {Image Super-Resolution Using Deep Convolutional Networks},
  journal   = {CoRR},
  volume    = {abs/1501.00092},
  year      = {2015},
  url       = {http://arxiv.org/abs/1501.00092},
  timestamp = {Mon, 02 Feb 2015 14:12:25 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/DongLHT15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{larochelle2011,
  title={The Neural Autoregressive Distribution Estimator},
  author={Hugo Larochelle and Iain Murray},
  journal={JMLR: W\&CP},
  volume={15},
  pages={29--37},
  year={2011}
}

@article{DBLP:journals/corr/NarihiraMY15,
  author    = {Takuya Narihira and
               Michael Maire and
               Stella X. Yu},
  title     = {Direct Intrinsics: Learning Albedo-Shading Decomposition by Convolutional
               Regression},
  journal   = {CoRR},
  volume    = {abs/1512.02311},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.02311},
  timestamp = {Sat, 02 Jan 2016 11:38:49 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/NarihiraMY15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/BrunaSL15,
  author    = {Joan Bruna and
               Pablo Sprechmann and
               Yann LeCun},
  title     = {Super-Resolution with Deep Convolutional Sufficient Statistics},
  journal   = {CoRR},
  volume    = {abs/1511.05666},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.05666},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/BrunaSL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

    @inproceedings{Misra2015EnvironmentDrivenLI,
  title={Environment-Driven Lexicon Induction for High-Level Instructions},
  author={Dipendra Kumar Misra and Kejia Tao and Percy Liang and Ashutosh Saxena},
  booktitle={ACL},
  year={2015}
}


  @INPROCEEDINGS{Misra-RSS-14, 
    AUTHOR    = {Dipendra Kumar Misra AND Jaeyong Sung AND Kevin Lee AND Ashutosh Saxena}, 
    TITLE     = {Tell Me Dave: Context-Sensitive Grounding of Natural Language to Manipulation Instructions}, 
    BOOKTITLE = {Proceedings of Robotics: Science and Systems}, 
    YEAR      = {2014}, 
    ADDRESS   = {Berkeley, USA}, 
    MONTH     = {July},
    DOI       = {10.15607/RSS.2014.X.005} 
} 


@article{DBLP:journals/tacl/ArtziZ13,
  author    = {Yoav Artzi and
               Luke Zettlemoyer},
  title     = {Weakly Supervised Learning of Semantic Parsers for Mapping Instructions
               to Actions},
  journal   = {{TACL}},
  volume    = {1},
  pages     = {49--62},
  year      = {2013},
  url       = {https://tacl2013.cs.columbia.edu/ojs/index.php/tacl/article/view/27},
  timestamp = {Thu, 28 May 2015 17:23:25 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/tacl/ArtziZ13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@INPROCEEDINGS{FirmanCVPR2016,
 author    = {Firman, Michael and Mac Aodha, Oisin and Julier, Simon and Brostow, Gabriel J.},
 title     = {{Structured Prediction of Unobserved Voxels From a Single Depth Image}},
 booktitle = {CVPR},
 year      = {2016},
}

@inproceedings{Efros:1999:TSN:850924.851569,
 author = {Efros, Alexei A. and Leung, Thomas K.},
 title = {Texture Synthesis by Non-Parametric Sampling},
 booktitle = {Proceedings of the International Conference on Computer Vision-Volume 2 - Volume 2},
 series = {ICCV '99},
 year = {1999},
 isbn = {0-7695-0164-8},
 pages = {1033--},
 url = {http://dl.acm.org/citation.cfm?id=850924.851569},
 acmid = {851569},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
} 

@article{DBLP:journals/corr/MakhzaniSJG15,
  author    = {Alireza Makhzani and
               Jonathon Shlens and
               Navdeep Jaitly and
               Ian J. Goodfellow},
  title     = {Adversarial Autoencoders},
  journal   = {CoRR},
  volume    = {abs/1511.05644},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.05644},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MakhzaniSJG15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/YehCLHD16,
  author    = {Raymond Yeh and
               Chen Chen and
               Teck{-}Yian Lim and
               Mark Hasegawa{-}Johnson and
               Minh N. Do},
  title     = {Semantic Image Inpainting with Perceptual and Contextual Losses},
  journal   = {CoRR},
  volume    = {abs/1607.07539},
  year      = {2016},
  url       = {http://arxiv.org/abs/1607.07539},
  timestamp = {Wed, 05 Oct 2016 14:51:31 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/YehCLHD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{Raiko:2014:INA:2968826.2968863,
 author = {Raiko, Tapani and Yao, Li and Cho, KyungHyun and Bengio, Yoshua},
 title = {Iterative Neural Autoregressive Distribution Estimator (NADE-k)},
 booktitle = {Proceedings of the 27th International Conference on Neural Information Processing Systems},
 series = {NIPS'14},
 year = {2014},
 location = {Montreal, Canada},
 pages = {325--333},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=2968826.2968863},
 acmid = {2968863},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 

@article{sonderby2014apparent,
  title={Amortised MAP Inference for Image Super-resolution},
  author={S{\o}nderby, Casper Kaae and Caballero, Jose and Theis ,Lucas and Shi, Wenzhe and Husz\'{a}r, Ferenc},
  journal={arXiv preprint arXiv:1610.04490},
  year={2016}
}

@incollection{hurley2005perspectives,
  title={Perspectives on Imitation: {F}rom Neuroscience to Social Science. {I}mitation, human development and culture. 2},
  author={Hurley, S. and Chater, N.},
  isbn={9780262582520},
  url={https://books.google.com/books?id=NZA\_ngEACAAJ},
  year={2005},
  publisher={MIT Press}
}

@inproceedings{3dgan,
    author = {Jiajun Wu, Chengkai Zhang, Tianfan Xue, William T. Freeman, and Joshua B. Tenenbaum},
    Title = {Learning a Probabilistic Latent Space of Object Shapes via 3D Generative-Adversarial Modeling},
    Booktitle = NIPS,
    Year = {2016}
}

@article{DBLP:journals/corr/YehCLHD16,
  author    = {Raymond Yeh and
               Chen Chen and
               Teck{-}Yian Lim and
               Mark Hasegawa{-}Johnson and
               Minh N. Do},
  title     = {Semantic Image Inpainting with Perceptual and Contextual Losses},
  journal   = {CoRR},
  volume    = {abs/1607.07539},
  year      = {2016},
  url       = {http://arxiv.org/abs/1607.07539},
  timestamp = {Wed, 05 Oct 2016 14:51:31 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/YehCLHD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{pathakCVPR16context,
    Author = {Pathak, Deepak and
    Kr\"ahenb\"uhl, Philipp and
    Donahue, Jeff and
    Darrell, Trevor and
    Efros, Alexei},
    Title = {Context Encoders:
    Feature Learning by Inpainting},
    Booktitle = CVPR,
    Year = {2016}
}


@article{DBLP:journals/corr/EigenPF14,
  author    = {David Eigen and
               Christian Puhrsch and
               Rob Fergus},
  title     = {Depth Map Prediction from a Single Image using a Multi-Scale Deep
               Network},
  journal   = {CoRR},
  volume    = {abs/1406.2283},
  year      = {2014},
  url       = {http://arxiv.org/abs/1406.2283},
  timestamp = {Tue, 01 Jul 2014 11:58:08 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/EigenPF14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/iccv/EfrosL99,
  author    = {Alexei A. Efros and
               Thomas K. Leung},
  title     = {Texture Synthesis by Non-parametric Sampling},
  booktitle = {{ICCV}},
  pages     = {1033--1038},
  year      = {1999},
  url       = {http://dx.doi.org/10.1109/ICCV.1999.790383},
  doi       = {10.1109/ICCV.1999.790383},
  timestamp = {Thu, 12 May 2016 10:37:23 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/iccv/EfrosL99},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Yang:2010:ISV:1892456.1892463,
 author = {Yang, Jianchao and Wright, John and Huang, Thomas S. and Ma, Yi},
 title = {Image Super-resolution via Sparse Representation},
 journal = {Trans. Img. Proc.},
 issue_date = {November 2010},
 volume = {19},
 number = {11},
 month = nov,
 year = {2010},
 issn = {1057-7149},
 pages = {2861--2873},
 numpages = {13},
 url = {http://dx.doi.org/10.1109/TIP.2010.2050625},
 doi = {10.1109/TIP.2010.2050625},
 acmid = {1892463},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
 keywords = {Face hallucination, face hallucination, image super-resolution (SR), nonnegative matrix factorization, sparse coding, sparse representation},
} 


@inproceedings{f-gan-training-generative-neural-samplers-using-variational-divergence-minimization,
author = {Sebastian Nowozin, Botond Cseke, Ryota Tomioka},
title = {f-GAN: Training Generative Neural Samplers using Variational Divergence Minimization},
booktitle = {Neural Information Processing Systems 2016},
year = {2016},
month = {October},
abstract = {Generative neural samplers are probabilistic models that implement sampling using feedforward neural networks: they take a random input vector and produce a sample from a probability distribution defined by the network weights. These models are expressive and allow efficient computation of samples and derivatives, but cannot be used for computing likelihoods or for marginalization. The generative-adversarial training method allows to train such models through the use of an auxiliary discriminative neural network. We show that the generative-adversarial approach is a special case of an existing more general variational divergence estimation approach. We show that any f-divergence can be used for training generative neural samplers. We discuss the benefits of various choices of divergence functions on training complexity and the quality of the obtained generative models.},
publisher = {Neural Information Processing Systems},
address = {},
pages = {},
journal = {},
volume = {},
chapter = {},
isbn = {},
}


@article{DBLP:journals/corr/RadfordMC15,
  author    = {Alec Radford and
               Luke Metz and
               Soumith Chintala},
  title     = {Unsupervised Representation Learning with Deep Convolutional Generative
               Adversarial Networks},
  journal   = {CoRR},
  volume    = {abs/1511.06434},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.06434},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RadfordMC15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}




@article{Gilbert2007677,
title = "Brain States: Top-Down Influences in Sensory Processing ",
journal = "Neuron ",
volume = "54",
number = "5",
pages = "677 - 696",
year = "2007",
note = "",
issn = "0896-6273",
doi = "http://dx.doi.org/10.1016/j.neuron.2007.05.019",
url = "http://www.sciencedirect.com/science/article/pii/S0896627307003765",
author = "Charles D. Gilbert and Mariano Sigman"
}

@ARTICLE{10.3389/fpsyg.2012.00620,
  
AUTHOR={Panichello, Matthew and Cheung, Olivia and Bar, Moshe},   
	 
TITLE={Predictive Feedback and Conscious Visual Experience},      
	
JOURNAL={Frontiers in Psychology},      
	
VOLUME={3},      

PAGES={620},     
	
YEAR={2013},      
	  
URL={http://journal.frontiersin.org/article/10.3389/fpsyg.2012.00620},       
	
DOI={10.3389/fpsyg.2012.00620},      
	
ISSN={1664-1078},   
   
ABSTRACT={The human brain continuously generates predictions about the environment based on learned regularities in the world. These predictions actively and efficiently facilitate the interpretation of incoming sensory information. We review evidence that, as a result of this facilitation, predictions directly influence conscious experience. Specifically, we propose that predictions enable rapid generation of conscious percepts and bias the contents of awareness in situations of uncertainty. The possible neural mechanisms underlying this facilitation are discussed. }
}

@inproceedings{Torralba:2011:ULD:2191740.2191773,
 author = {Torralba, A. and Efros, A. A.},
 title = {Unbiased Look at Dataset Bias},
 booktitle = {Proceedings of the 2011 IEEE Conference on Computer Vision and Pattern Recognition},
 series = {CVPR '11},
 year = {2011},
 isbn = {978-1-4577-0394-2},
 pages = {1521--1528},
 numpages = {8},
 url = {http://dx.doi.org/10.1109/CVPR.2011.5995347},
 doi = {10.1109/CVPR.2011.5995347},
 acmid = {2191773},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
 keywords = {algorithm evaluation protocols, contemporary object recognition, data capture, recognition datasets, relative data bias, cross dataset generalization, closed world assumption effects, sample value},
} 




@inproceedings{Gal:2016:DBA:3045390.3045502,
 author = {Gal, Yarin and Ghahramani, Zoubin},
 title = {Dropout As a Bayesian Approximation: Representing Model Uncertainty in Deep Learning},
 booktitle = {Proceedings of the 33rd International Conference on International Conference on Machine Learning - Volume 48},
 series = {ICML'16},
 year = {2016},
 location = {New York, NY, USA},
 pages = {1050--1059},
 numpages = {10},
 url = {http://dl.acm.org/citation.cfm?id=3045390.3045502},
 acmid = {3045502},
 publisher = {JMLR.org},
} 



@inproceedings{andriluka14cvpr,
    author = {Mykhaylo Andriluka and Leonid Pishchulin and Peter Gehler and Schiele, Bernt},
    title = {2D Human Pose Estimation: {N}ew Benchmark and State of the Art Analysis},
    booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
    year = {2014},
    month = {June}
}


@Inbook{Wu2016,
author="Wu, Jiajun
and Xue, Tianfan
and Lim, Joseph J.
and Tian, Yuandong
and Tenenbaum, Joshua B.
and Torralba, Antonio
and Freeman, William T.",
editor="Leibe, Bastian
and Matas, Jiri
and Sebe, Nicu
and Welling, Max",
title="Single Image 3D Interpreter Network",
bookTitle="Computer Vision -- ECCV 2016: 14th European Conference, Amsterdam, The Netherlands, October 11-14, 2016, Proceedings, Part VI",
year="2016",
publisher="Springer International Publishing",
address="Cham",
pages="365--382",
isbn="978-3-319-46466-4",
doi="10.1007/978-3-319-46466-4_22",
url="http://dx.doi.org/10.1007/978-3-319-46466-4_22"
}

@techreport{amos2016openface,
  title={OpenFace: A general-purpose face recognition
    library with mobile applications},
  author={Amos, Brandon and Bartosz Ludwiczuk and Satyanarayanan, Mahadev},
  year={2016},
  institution={CMU-CS-16-118, CMU School of Computer Science},
}

@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}

@inproceedings{Theis2016a,
  author = "L. Theis and A. van den Oord and M. Bethge",
  title = "A note on the evaluation of generative models",
  year = 2016,
  booktitle = "International Conference on Learning Representations",
  month = "Apr",
  keywords = "generative modeling",
  url = "http://arxiv.org/abs/1511.01844"
}

@article{DBLP:journals/corr/MathieuCL15,
  author    = {Micha{\"{e}}l Mathieu and
               Camille Couprie and
               Yann LeCun},
  title     = {Deep multi-scale video prediction beyond mean square error},
  journal   = {CoRR},
  volume    = {abs/1511.05440},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.05440},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MathieuCL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{wei2016cpm,
    author = {Shih-En Wei and Varun Ramakrishna and Takeo Kanade and Yaser Sheikh},
    booktitle = {CVPR},
    title = {Convolutional pose machines},
    year = {2016}
}


@article{rezende2014stochastic,
  title={Stochastic backpropagation and approximate inference in deep generative models},
  author={Rezende, Danilo Jimenez and Mohamed, Shakir and Wierstra, Daan},
  journal={arXiv preprint arXiv:1401.4082},
  year={2014}
}

@inproceedings{handa2016gvnn,
  title={gvnn: Neural network library for geometric computer vision},
  author={Handa, Ankur and Bloesch, Michael and P{\u{a}}tr{\u{a}}ucean, Viorica and Stent, Simon and McCormac, John and Davison, Andrew},
  booktitle={Computer Vision--ECCV 2016 Workshops},
  pages={67--82},
  year={2016},
  organization={Springer International Publishing}
}

@article{flownet2,
  author    = {Eddy Ilg and
               Nikolaus Mayer and
               Tonmoy Saikia and
               Margret Keuper and
               Alexey Dosovitskiy and
               Thomas Brox},
  title     = {FlowNet 2.0: Evolution of Optical Flow Estimation with Deep Networks},
  journal   = {CoRR},
  volume    = {abs/1612.01925},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.01925},
  timestamp = {Mon, 02 Jan 2017 11:09:15 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/IlgMSKDB16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@misc{blender,
  author = {{Blender Online Coummunity}},
  organization = {Blender Foundation},
  title = {Blender},
  url = {https://www.blender.org/},
}



@article{DBLP:journals/corr/ChenWLSTLCC16,
  author    = {Wenzheng Chen and
               Huan Wang and
               Yangyan Li and
               Hao Su and
               Changhe Tu and
               Dani Lischinski and
               Daniel Cohen{-}Or and
               Baoquan Chen},
  title     = {Synthesizing Training Images for Boosting Human 3D Pose Estimation},
  journal   = {CoRR},
  volume    = {abs/1604.02703},
  year      = {2016},
  url       = {http://arxiv.org/abs/1604.02703},
  timestamp = {Mon, 02 May 2016 18:22:52 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/ChenWLSTLCC16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@misc{caesar,
  author = {Robinette, K., Daanen, H. and Paquet, E.},
  organization = {3DIM’99},
  title = {The CAESAR project: A 3-D surface anthropometry survey.},
}

@inproceedings{Wulff:ECCVws:2012,
 title = {Lessons and insights from creating a synthetic optical flow benchmark},
 author = {Wulff, J. and Butler, D. J. and Stanley, G. B. and Black, M. J.},
 booktitle = {ECCV Workshop on Unsolved Problems in Optical Flow and Stereo Estimation},
 editor = {{A. Fusiello et al. (Eds.)}},
 publisher = {Springer-Verlag},
 series = {Part II, LNCS 7584},
 month = oct,
 pages = {168--177},
 year = {2012}
}

@article{sun,
	author     = {Jianxiong Xiao and Krista A. Ehinger and James Hays and Antonio Torralba and Aude Oliva},
	title      = {{SUN} Database: Exploring a Large Collection of Scene Categories},
	journal    = {IJCV},
	year       = {2014},
}





@techreport{shapenet2015,
  title       = {{ShapeNet: An Information-Rich 3D Model Repository}},
  author      = {Chang, Angel X. and Funkhouser, Thomas and Guibas, Leonidas and Hanrahan, Pat and Huang, Qixing and Li, Zimo and Savarese, Silvio and Savva, Manolis and Song, Shuran and Su, Hao and Xiao, Jianxiong and Yi, Li and Yu, Fisher},
  number      = {arXiv:1512.03012 [cs.GR]},
  institution = {Stanford University --- Princeton University --- Toyota Technological Institute at Chicago},
  year        = {2015}
}

@inproceedings{epicflow,
TITLE = {{EpicFlow}: Edge-Preserving Interpolation of Correspondences for Optical Flow},
  AUTHOR = {Revaud, Jerome and Weinzaepfel, Philippe and Harchaoui, Zaid and Schmid, Cordelia},
  BOOKTITLE = {CVPR}, 
  YEAR = {2015},
}

@article{deepflow,
  TITLE = {{DeepMatching}: Hierarchical Deformable Dense Matching},
  AUTHOR = {Revaud, Jerome and Weinzaepfel, Philippe and Harchaoui, Zaid and Schmid, Cordelia},
  JOURNAL = {IJCV},
  YEAR = {2016},
}

@article{DBLP:journals/corr/MirzaO14,
  author    = {Mehdi Mirza and
               Simon Osindero},
  title     = {Conditional Generative Adversarial Nets},
  journal   = {CoRR},
  volume    = {abs/1411.1784},
  year      = {2014},
  url       = {http://arxiv.org/abs/1411.1784},
  timestamp = {Mon, 01 Dec 2014 14:32:13 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MirzaO14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{CycleGAN2017,
  title={Unpaired Image-to-Image Translation using Cycle-Consistent Adversarial Networks},
  author={Zhu, Jun-Yan and Park, Taesung and Isola, Phillip and Efros, Alexei A},
  journal={arXiv preprint arXiv:1703.10593},
  year={2017}
}

@article{DBLP:journals/corr/AlldieckKM17,
  author    = {Thiemo Alldieck and
               Marc Kassubeck and
               Marcus A. Magnor},
  title     = {Optical Flow-based 3D Human Motion Estimation from Monocular Video},
  journal   = {CoRR},
  volume    = {abs/1703.00177},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.00177},
  timestamp = {Mon, 03 Apr 2017 12:41:34 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/AlldieckKM17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{unpublished,
  title={Unpaired Image-to-Image Translation using Cycle-Consistent Adversarial Networks},
  author={Zhu, Jun-Yan and Park, Taesung and Isola, Phillip and Efros, Alexei A},
  journal={arXiv preprint arXiv:1703.10593},
  year={2017}
}

 @InProceedings{sfmnet,
  author = 	 {Vijayanarasimhan S. and  Ricco S. and  Schmid C. and  Sukthankar R. and Fragkiadaki K.},
  title = 	 {SfM-Net: Learning of Structure and Motion from Video},
  booktitle = {arxiv},
  year = 	 2017}
  
   @InProceedings{tinghuisfm,
  author = 	 {Tinghui Zhou and Matthew Brown and Noah Snavely and David G. Lowe},
  title = 	 {Unsupervised Learning of Depth and Ego-Motion from Video},
  booktitle = {arxiv},
  year = 	 2017}





@inproceedings{Thewlis2016,
title = {Fully-Trainable Deep Matching},
author = {James Thewlis and Shuai Zheng and Philip H.S. Torr and Andrea Vedaldi},
booktitle={BMVC},
year = {2016}
}

@inproceedings{Kong:ICCV:2015,
  title = {Intrinsic Depth: Improving Depth Transfer with Intrinsic Images},
  author = {Kong, Naejin and Black, Michael J.},
  booktitle = {IEEE International Conference on Computer Vision (ICCV)},
  pages = {3514--3522},
  month = dec,
  year = {2015}
}

@ARTICLE{Geiger2013IJRR,
  author = {Andreas Geiger and Philip Lenz and Christoph Stiller and Raquel Urtasun},
  title = {Vision meets Robotics: The KITTI Dataset},
  journal = {International Journal of Robotics Research (IJRR)},
  year = {2013}
} 

@InProceedings{sturm12iros,
	author = {J. Sturm and N. Engelhard and F. Endres and W. Burgard and D. Cremers},
	title = "A Benchmark for the Evaluation of {RGB-D SLAM} Systems",
	booktitle = "IROS",
	year = "2012",
}

@Inbook{Russell2014,
author="Russell, Chris
and Yu, Rui
and Agapito, Lourdes",
editor="Fleet, David
and Pajdla, Tomas
and Schiele, Bernt
and Tuytelaars, Tinne",
title="Video Pop-up: Monocular 3D Reconstruction of Dynamic Scenes",
bookTitle="Computer Vision -- ECCV 2014: 13th European Conference, Zurich, Switzerland, September 6-12, 2014, Proceedings, Part VII",
year="2014",
publisher="Springer International Publishing",
address="Cham",
pages="583--598",
isbn="978-3-319-10584-0",
doi="10.1007/978-3-319-10584-0_38",
url="http://dx.doi.org/10.1007/978-3-319-10584-0_38"
}

@InProceedings{sturm12iros,
	author = {J. Sturm and N. Engelhard and F. Endres and W. Burgard and D. Cremers},
	title = "A Benchmark for the Evaluation of {RGBD} {SLAM} Systems",
	booktitle = "IROS",
	year = "2012",
}

@inproceedings{conf/cvpr/PrestLCSF12,
  added-at = {2014-07-31T00:00:00.000+0200},
  author = {Prest, Alessandro and Leistner, Christian and Civera, Javier and Schmid, Cordelia and Ferrari, Vittorio},
  biburl = {http://www.bibsonomy.org/bibtex/2826cada174d8324d3429d3f27682708f/dblp},
  booktitle = {CVPR},
  crossref = {conf/cvpr/2012},
  ee = {http://doi.ieeecomputersociety.org/10.1109/CVPR.2012.6248065},
  interhash = {c77cf607bee39b622c42e08da6d1da68},
  intrahash = {826cada174d8324d3429d3f27682708f},
  isbn = {978-1-4673-1226-4},
  keywords = {dblp},
  timestamp = {2015-06-19T15:56:14.000+0200},
  title = {Learning object class detectors from weakly annotated video.},
  url = {http://dblp.uni-trier.de/db/conf/cvpr/cvpr2012.html#PrestLCSF12},
  year = 2012
}

@inproceedings{DBLP:journals/corr/WalkerDGH16,
  author    = {Jacob Walker and
               Carl Doersch and
               Abhinav Gupta and
               Martial Hebert},
  title     = {An Uncertain Future: Forecasting from Static Images using Variational
               Autoencoders},
  booktitle = {ECCV},
  year      = {2016},
}

@article{Horn:1981,
 author = {Horn, Berthold K.P. and Schunck, Brian G.},
 title = {Determining Optical Flow},
 year = {1981},
 journal = {Artificial Intelligence},
 volume = 17,
} 


@inproceedings{Silberman:ECCV12,
  author    = {Nathan Silberman and Derek Hoiem and Pushmeet Kohli and Rob Fergus},
  title     = {Indoor Segmentation and Support Inference from {RGBD} Images},
  booktitle = {ECCV},
  year      = {2012}
}


@INPROCEEDINGS{Geiger2012CVPR,
  author = {Andreas Geiger and Philip Lenz and Raquel Urtasun},
  title = {Are we ready for Autonomous Driving? {T}he {KITTI} Vision Benchmark Suite},
  booktitle = {CVPR},
  year = {2012}
} 

@inproceedings{Butler:ECCV:2012,
title = {A naturalistic open source movie for optical flow evaluation},
author = {Butler, D. J. and Wulff, J. and Stanley, G. B. and Black, M. J.},
booktitle = {ECCV},
year = 2012,
}


@InProceedings{Hornacek_2014_CVPR,
author = {Hornacek, Michael and Fitzgibbon, Andrew and Rother, Carsten},
title = {{SphereFlow}: 6 {DoF} Scene Flow from {RGB-D} Pairs},
booktitle = {CVPR},
year = {2014}
}




@article{Nir_IJCV2008,
    abstract = {{A novel optical flow estimation process based on a spatio-temporal model with varying coefficients multiplying a set of basis functions at each pixel is introduced. Previous optical flow estimation methodologies did not use such an over parameterized representation of the flow field as the problem is ill-posed even without introducing any additional parameters: Neighborhood based methods of the Lucas---Kanade type determine the flow at each pixel by constraining the flow to be described by a few parameters in small neighborhoods. Modern variational methods represent the optic flow directly via the flow field components at each pixel. The benefit of over-parametrization becomes evident in the smoothness term, which instead of directly penalizing for changes in the optic flow, accumulates a cost of deviating from the assumed optic flow model. Our proposed method is very general and the classical variational optical flow techniques are special cases of it, when used in conjunction with constant basis functions. Experimental results with the novel flow estimation process yield significant improvements with respect to the best results published so far.}},
    address = {Hingham, MA, USA},
    author = {Nir, Tal and Bruckstein, AlfredM and Kimmel, Ron},
    journal = {IJCV},
    citeulike-article-id = {6766220},
    citeulike-linkout-0 = {http://portal.acm.org/citation.cfm?id=1331491},
    citeulike-linkout-1 = {http://dx.doi.org/10.1007/s11263-007-0051-2},
    citeulike-linkout-2 = {http://link.springer.com/article/10.1007/s11263-007-0051-2},
    doi = {10.1007/s11263-007-0051-2},
    issn = {0920-5691},
    keywords = {computer\_vision, optic\_flow, variational\_method},
    number = {2},
    pages = {205--216},
    posted-at = {2016-05-24 16:29:23},
    priority = {2},
    publisher = {Springer US},
    title = {{Over-Parameterized Variational Optical Flow}},
    url = {http://dx.doi.org/10.1007/s11263-007-0051-2},
    volume = {76},
    year = {2008}
}

@article{KILNER2013R1057,
title = "What We Know Currently about Mirror Neurons",
journal = "Current Biology",
volume = "23",
number = "23",
pages = "R1057 - R1062",
year = "2013",
note = "",
issn = "0960-9822",
doi = "http://dx.doi.org/10.1016/j.cub.2013.10.051",
url = "http://www.sciencedirect.com/science/article/pii/S0960982213013262",
author = "J.M. Kilner and R.N. Lemon",

}


@article{Ramachandran00,
  abstract = {The discovery of mirror neurons in the frontal lobes of monkeys, and their potential relevance to human brain evolution — which I speculate on in this essay — is the single most important "unreported" (or at least, unpublicized) story of the decade. I predict that mirror neurons will do for psychology what DNA did for biology: they will provide a unifying framework and help explain a host of mental abilities that have hitherto remained mysterious and inaccessible to experiments.
},
  added-at = {2007-01-23T18:03:44.000+0100},
  author = {Ramachandran, V.S.},
  biburl = {https://www.bibsonomy.org/bibtex/21f56be84a986504a25a4b620e8c8b3d7/yish},
  date = {00]},
  description = {EDGE: MIRROR NEURONS},
  interhash = {a0170113f3387eb21d84c02f7e7f6f47},
  intrahash = {1f56be84a986504a25a4b620e8c8b3d7},
  journal = {Edge},
  keywords = {imported},
  timestamp = {2007-01-23T18:03:44.000+0100},
  title = {MIRROR NEURONS and imitation learning as the driving force behind "the great leap forward" in human evolution},
  url = {http://www.edge.org/3rd_culture/ramachandran/ramachandran_index.html},
  volume = 69,
  year = 2000
}





@InProceedings{Fragkiadaki_2015_CVPR,
author = {Fragkiadaki, Katerina and Arbelaez, Pablo and Felsen, Panna and Malik, Jitendra},
title = {Learning to Segment Moving Objects in Videos},
booktitle = {CVPR},
month = {June},
year = {2015}
}

@InProceedings{kerl13iros,
  author =    {C. Kerl and J. Sturm and D. Cremers},
  title =     {Dense Visual {SLAM} for {RGB-D} Cameras},
  booktitle = {IROS},
  year =      2013,
  keywords={dense visual odometry,dense visual slam,rgb-d,rgb-d benchmark}
}

@article{DBLP:journals/corr/GodardAB16,
  author    = {Cl{\'{e}}ment Godard and
               Oisin {Mac Aodha} and
               Gabriel J. Brostow},
  title     = {Unsupervised Monocular Depth Estimation with Left-Right Consistency},
  journal   = {CoRR},
  volume    = {abs/1609.03677},
  year      = {2016},
  url       = {http://arxiv.org/abs/1609.03677},
  timestamp = {Mon, 03 Oct 2016 17:51:10 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/GodardAB16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@INPROCEEDINGS{Geiger2012CVPR,
  author = {Andreas Geiger and Philip Lenz and Raquel Urtasun},
  title = {Are we ready for Autonomous Driving? The KITTI Vision Benchmark Suite},
  booktitle = {Conference on Computer Vision and Pattern	Recognition (CVPR)},
  year = {2012}
}
@INPROCEEDINGS{Menze2015CVPR,
  author = {Moritz Menze and Andreas Geiger},
  title = {Object Scene Flow for Autonomous Vehicles},
  booktitle = {Conference on Computer Vision and Pattern	Recognition (CVPR)},
  year = {2015}
} 
@inproceedings{mocapcmu,
author={http://mocap.cs.cmu.edu/},
title={CMU mocap database},
}


@inproceedings{schoeps14ismar,
author={T. Sch\"ops and J. Engel and D. Cremers},
title={Semi-Dense Visual Odometry for {AR} on a Smartphone},
year= {2014},
booktitle = "ISMAR",
}

@inproceedings{engel14eccv,
author={J. Engel and T. Sch\"ops and D. Cremers},
title={{LSD-SLAM}: Large-Scale Direct Monocular {SLAM}},
year= {2014},
booktitle = "ECCV",
keywords={rgb-d, monocular, slam, semidense, lsdslam},
award = {Oral Presentation}
}



@inproceedings{warehouse,
 url = {https://3dwarehouse.sketchup.com/index.html},
}

@inproceedings{Izadi:2011:KRR:2047196.2047270,
 author = {Izadi, Shahram and Kim, David and Hilliges, Otmar and Molyneaux, David and Newcombe, Richard and Kohli, Pushmeet and Shotton, Jamie and Hodges, Steve and Freeman, Dustin and Davison, Andrew and Fitzgibbon, Andrew},
 title = {KinectFusion: Real-time 3D Reconstruction and Interaction Using a Moving Depth Camera},
 booktitle = {Proceedings of the 24th Annual ACM Symposium on User Interface Software and Technology},
 series = {UIST '11},
 year = {2011},
 isbn = {978-1-4503-0716-1},
 location = {Santa Barbara, California, USA},
 pages = {559--568},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/2047196.2047270},
 doi = {10.1145/2047196.2047270},
 acmid = {2047270},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {3D, AR, GPU, depth cameras, geometry-aware interactions, physics, surface reconstruction, tracking},
} 


@inproceedings{garg2016unsupervised,
  title={Unsupervised CNN for single view depth estimation: Geometry to the rescue},
  author={Garg, Ravi and Kumar, BG Vijay and Carneiro, Gustavo and Reid, Ian},
  booktitle={European Conference on Computer Vision},
  pages={740--756},
  year={2016},
  organization={Springer}
}

@article{DBLP:journals/corr/GargBR16,
  author    = {Ravi Garg and
               Vijay Kumar BG and
               Ian D. Reid},
  title     = {Unsupervised {CNN} for Single View Depth Estimation: Geometry to the
               Rescue},
  journal   = {CoRR},
  volume    = {abs/1603.04992},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.04992},
  timestamp = {Fri, 08 Apr 2016 07:34:30 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/GargBR16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Bergen:1992:HMM:645305.648720,
 author = {Bergen, James R. and Anandan, P. and Hanna, Keith J. and Hingorani, Rajesh},
 title = {Hierarchical Model-Based Motion Estimation},
 booktitle = {ECCV},
 year = {1992},
} 


@article{DBLP:journals/corr/FragkiadakiAFM14,
  author    = {Katerina Fragkiadaki and
               Pablo Andr{\'{e}}s Arbel{\'{a}}ez and
               Panna Felsen and
               Jitendra Malik},
  title     = {Spatio-Temporal Moving Object Proposals},
  journal   = {CoRR},
  volume    = {abs/1412.6504},
  year      = {2014},
  url       = {http://arxiv.org/abs/1412.6504},
  timestamp = {Thu, 01 Jan 2015 19:51:08 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/FragkiadakiAFM14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{citeulike:2638091,
    abstract = {{Traditional plane alignment techniques are typically performed between pairs of frames. In this paper, we present a method for extending existing two-frame planar motion estimation techniques into a simultaneous multi-frame estimation, by exploiting multiframe subspace constraints of planar surfaces. The paper has three main contributions: 1 ) we show that when the camera calibration does not change, the collection of all parametric image motions of a planar surface in the scene across...}},
    author = {Manor, L. Z. and Irani, M.},
    citeulike-article-id = {2638091},
    citeulike-linkout-0 = {http://citeseerx.ist.psu.edu/viewdoc/summary?doi=10.1.1.12.8166},
    journal = {PAMI},
    keywords = {optical-flow-multi-frame},
    number = {10},
    pages = {1105--1116},
    posted-at = {2008-04-07 16:42:55},
    priority = {2},
    title = {{Multi-Frame Estimation of Planar Motion}},
    url = {http://citeseerx.ist.psu.edu/viewdoc/summary?doi=10.1.1.12.8166},
    volume = {22},
    year = {2000}
}



@article{monodepthlr2016,
  author       = {Godard, Clément and Mac Aodha, Oisin and Brostow, Gabriel J.},
  title        = {Unsupervised Monocular Depth Estimation with Left-Right Consistency},
  journal      = "CoRR",
  volume       = {abs/1609.03677},
  year         = {2016},
}

@inproceedings{stn,
  author    = {Max Jaderberg and
               Karen Simonyan and
               Andrew Zisserman and
               Koray Kavukcuoglu},
  title     = {Spatial Transformer Networks},
  booktitle = {NIPS}, 
  year      = {2015}
}

Don't use this one -- use the ECCV one below
@article{DBLP:journals/corr/YuHD16,
  author    = {Jason J. Yu and
               Adam W. Harley and
               Konstantinos G. Derpanis},
  title     = {Back to Basics: Unsupervised Learning of Optical Flow via Brightness
               Constancy and Motion Smoothness},
  journal   = {CoRR},
  volume    = {abs/1608.05842},
  year      = {2016},
  url       = {http://arxiv.org/abs/1608.05842},
  timestamp = {Fri, 02 Sep 2016 17:46:24 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/YuHD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{back_to_basics:2016,
  author    = {Jason J. Yu and
               Adam W. Harley and
               Konstantinos G. Derpanis},
  title     = {Back to Basics: Unsupervised Learning of Optical Flow via Brightness
               Constancy and Motion Smoothness},
  booktitle = "ECCV",
  year = 2016,
}


@InProceedings{flownet,
  author       = "A. Dosovitskiy and P. Fischer and E. Ilg and P. H{\"a}usser and C. Hazirbas and V. Golkov and P. Smagt and D. Cremers and T. Brox",
  title        = "{FlowNet}: Learning Optical Flow with Convolutional Networks",
  booktitle    = "ICCV",
  year         = "2015",
}

@inproceedings{interpreter,
author="Wu, Jiajun
and Xue, Tianfan
and Lim, Joseph J.
and Tian, Yuandong
and Tenenbaum, Joshua B.
and Torralba, Antonio
and Freeman, William T.",
title="Single Image {3D} Interpreter Network",
bookTitle="ECCV",
year="2016",
}


@article{SE3-Nets,
 author = {A. Byravan and D. Fox},
 title = {{SE3-Nets}: Learning Rigid Body Motion using Deep Neural Networks},
 journal = "CoRR",
 volume = "abs/1606.02378",
 year = 2016,
}

@InProceedings{flyingthings16,
	author = {N. Mayer and E. Ilg and P. H\"ausser and P. Fischer and D. Cremers and A. Dosovitskiy and T. Brox},
title = {A large dataset to train convolutional networks for disparity, optical flow, and scene flow estimation},
booktitle = {CVPR},
year = {2016}
}



@INPROCEEDINGS{5459407, 
author={Brubaker, Marcus A. and Sigal, L. and Fleet, D.J.}, 
booktitle={Computer Vision, 2009 IEEE 12th International Conference on}, 
title={Estimating contact dynamics}, 
year={2009}, 
pages={2389-2396}, 
keywords={Biological system modeling;Geometry;Gravity;Humans;Inference algorithms;Joints;Motion estimation;Solid modeling;Testing;Tracking}, 
doi={10.1109/ICCV.2009.5459407}, 
ISSN={1550-5499}, 
month={Sept}
}

@inproceedings{conf/eccv/BhatSP02,
  added-at = {2011-06-30T00:00:00.000+0200},
  author = {Bhat, Kiran S. and Seitz, Steven M. and Popovic, Jovan},
  biburl = {http://www.bibsonomy.org/bibtex/20fafe53b2d695d4262da2e3aa2219521/dblp},
  booktitle = {ECCV},
  crossref = {conf/eccv/2002-1},
  editor = {Heyden, Anders and Sparr, Gunnar and Nielsen, Mads and Johansen, Peter},
  ee = {http://dx.doi.org/10.1007/3-540-47969-4_37},
  interhash = {3cc5e0f9b763368da2cb82bfddb514b9},
  intrahash = {0fafe53b2d695d4262da2e3aa2219521},
  isbn = {3-540-43745-2},
  keywords = {dblp},
  pages = {551-565},
  publisher = {Springer},
  series = {Lecture Notes in Computer Science},
  timestamp = {2011-07-01T11:39:44.000+0200},
  title = {Computing the Physical Parameters of Rigid-Body Motion from Video.},
  url = {http://dblp.uni-trier.de/db/conf/eccv/eccv2002-1.html#BhatSP02},
  volume = 2350,
  year = 2002
}


@incollection{NIPS2015_5780,
title = {Galileo: Perceiving Physical Object Properties by Integrating a Physics Engine with Deep Learning},
author = {Wu, Jiajun and Yildirim, Ilker and Lim, Joseph J and Freeman, Bill and Tenenbaum, Josh},
booktitle = {Advances in Neural Information Processing Systems 28},
editor = {C. Cortes and N.D. Lawrence and D.D. Lee and M. Sugiyama and R. Garnett and R. Garnett},
pages = {127--135},
year = {2015},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5780-galileo-perceiving-physical-object-properties-by-integrating-a-physics-engine-with-deep-learning.pdf}
}

@misc {Kristan2016a,
	title = {The Visual Object Tracking VOT2016 challenge results},
	url = {http://www.springer.com/gp/book/9783319488806},
	author = {Matej Kristan and Ale\v{s} Leonardis and Jiri Matas and Michael Felsberg and Roman Pflugfelder and Luka \v{C}ehovin and Tomas Vojir and Gustav H\"{a}ger and Alan Luke\v{z}i\v{c} and Gustavo Fernandez},
	month = {Oct},
	year = {2016},
	howpublished = {Springer}
}


@article{DBLP:journals/corr/Leal-TaixeMRRS15,
  author    = {Laura Leal{-}Taix{\'{e}} and
               Anton Milan and
               Ian D. Reid and
               Stefan Roth and
               Konrad Schindler},
  title     = {MOTChallenge 2015: Towards a Benchmark for Multi-Target Tracking},
  journal   = {CoRR},
  volume    = {abs/1504.01942},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.01942},
  archivePrefix = {arXiv},
  eprint    = {1504.01942},
  timestamp = {Wed, 07 Jun 2017 14:40:39 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/Leal-TaixeMRRS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/MottaghiBRF15,
  author    = {Roozbeh Mottaghi and
               Hessam Bagherinezhad and
               Mohammad Rastegari and
               Ali Farhadi},
  title     = {Newtonian Image Understanding: Unfolding the Dynamics of Objects in
               Static Images},
  journal   = {CoRR},
  volume    = {abs/1511.04048},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.04048},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MottaghiBRF15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{conf/iccv/SalzmannU11,
  added-at = {2012-01-19T00:00:00.000+0100},
  author = {Salzmann, Mathieu and Urtasun, Raquel},
  biburl = {http://www.bibsonomy.org/bibtex/24d6e35c0f411d7427b602d8e24304f0f/dblp},
  booktitle = {ICCV},
  crossref = {conf/iccv/2011},
  editor = {Metaxas, Dimitris N. and Quan, Long and Sanfeliu, Alberto and Gool, Luc J. Van},
  ee = {http://dx.doi.org/10.1109/ICCV.2011.6126480},
  interhash = {56d5fa22b622d3e98adf7879ee4573f7},
  intrahash = {4d6e35c0f411d7427b602d8e24304f0f},
  isbn = {978-1-4577-1101-5},
  keywords = {dblp},
  pages = {2064-2071},
  publisher = {IEEE},
  timestamp = {2012-01-20T11:33:25.000+0100},
  title = {Physically-based motion models for 3D tracking: A convex formulation.},
  url = {http://dblp.uni-trier.de/db/conf/iccv/iccv2011.html#SalzmannU11},
  year = 2011
}



@article{DBLP:journals/corr/AgrawalNAML16,
  author    = {Pulkit Agrawal and
               Ashvin Nair and
               Pieter Abbeel and
               Jitendra Malik and
               Sergey Levine},
  title     = {Learning to Poke by Poking: Experiential Learning of Intuitive Physics},
  journal   = {CoRR},
  volume    = {abs/1606.07419},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.07419},
  archivePrefix = {arXiv},
  eprint    = {1606.07419},
  timestamp = {Wed, 07 Jun 2017 14:42:59 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/AgrawalNAML16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/FragkiadakiALM15,
  author    = {Katerina Fragkiadaki and
               Pulkit Agrawal and
               Sergey Levine and
               Jitendra Malik},
  title     = {Learning Visual Predictive Models of Physics for Playing Billiards},
  journal   = {CoRR},
  volume    = {abs/1511.07404},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.07404},
  timestamp = {Wed, 07 Jun 2017 14:43:08 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/FragkiadakiALM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{DBLP:conf/bmvc/KyriazisOA11,
  author    = {Nikolaos Kyriazis and
               Iason Oikonomidis and
               Antonis A. Argyros},
  title     = {Binding Computer Vision to Physics Based Simulation: The Case Study
               of a Bouncing Ball},
  booktitle = {British Machine Vision Conference, {BMVC} 2011, Dundee, UK, August
               29 - September 2, 2011. Proceedings},
  pages     = {1--11},
  year      = {2011},
  crossref  = {DBLP:conf/bmvc/2011},
  url       = {http://dx.doi.org/10.5244/C.25.43},
  doi       = {10.5244/C.25.43},
  timestamp = {Wed, 24 Apr 2013 17:19:07 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/bmvc/KyriazisOA11},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{conf/eccv/BhatSP02,
  added-at = {2011-06-30T00:00:00.000+0200},
  author = {Bhat, Kiran S. and Seitz, Steven M. and Popovic, Jovan},
  biburl = {http://www.bibsonomy.org/bibtex/20fafe53b2d695d4262da2e3aa2219521/dblp},
  booktitle = {ECCV (1)},
  crossref = {conf/eccv/2002-1},
  editor = {Heyden, Anders and Sparr, Gunnar and Nielsen, Mads and Johansen, Peter},
  ee = {http://dx.doi.org/10.1007/3-540-47969-4_37},
  interhash = {3cc5e0f9b763368da2cb82bfddb514b9},
  intrahash = {0fafe53b2d695d4262da2e3aa2219521},
  isbn = {3-540-43745-2},
  keywords = {dblp},
  pages = {551-565},
  publisher = {Springer},
  series = {Lecture Notes in Computer Science},
  timestamp = {2011-07-01T11:39:44.000+0200},
  title = {Computing the Physical Parameters of Rigid-Body Motion from Video.},
  url = {http://dblp.uni-trier.de/db/conf/eccv/eccv2002-1.html#BhatSP02},
  volume = 2350,
  year = 2002
}

@inproceedings{42854,
title = {Large-Scale Object Classification Using Label Relation Graphs},
author  = {Jia Deng and Nan Ding and Yangqing Jia and Andrea Frome and Kevin Murphy and Samy Bengio and Yuan Li and Hartmut Neven and Hartwig Adam},
year  = 2014,
booktitle = {European Conference on Computer Vision}
}



@article{smith2005development,
  title={The development of embodied cognition: Six lessons from babies},
  author={Smith, Linda and Gasser, Michael},
  journal={Artificial life},
  volume={11},
  number={1-2},
  pages={13--29},
  year={2005}
}

@article{hansen2001completely,
  title={Completely derandomized self-adaptation in evolution strategies},
  author={Hansen, Nikolaus and Ostermeier, Andreas},
  journal={Evolutionary computation},
  volume={9},
  number={2},
  pages={159--195},
  year={2001},
  publisher={MIT Press}
}

@article{actionconditioned,
  title={Action-Conditional Video Prediction using Deep Networks in Atari Games},
  author={Oh, Junhyuk and Guo, Xiaoxiao and Lee, Honglak and Lewis, Richard and Singh, Satinder},
  journal={arXiv preprint arXiv:1507.08750},
  year={2015}
}

@inproceedings{hamrick2011internal,
  title={Internal physics models guide probabilistic judgments about object dynamics},
  author={Hamrick, Jessica and Battaglia, Peter and Tenenbaum, Joshua B},
  booktitle={Proceedings of the 33rd annual conference of the cognitive science society},
  pages={1545--1550},
  year={2011},
  organization={Cognitive Science Society Austin, TX}
}

@article{jordan1992forward,
  title={Forward models: Supervised learning with a distal teacher},
  author={Jordan, Michael I and Rumelhart, David E},
  journal={Cognitive science},
  volume={16},
  number={3},
  pages={307--354},
  year={1992},
  publisher={Wiley Online Library}
}

@article{wolpert1995internal,
  title={An internal model for sensorimotor integration},
  author={Wolpert, Daniel M and Ghahramani, Zoubin and Jordan, Michael I},
  journal={Science-AAAS-Weekly Paper Edition},
  volume={269},
  number={5232},
  pages={1880--1882},
  year={1995},
  publisher={New York, NY:[sn] 1880-}
}



@article{thesisblocks,
  title={Machine perception of three-dimensional solids},
  author={Roberts, Lawrence},
  year={1963},
  publisher={MIT}
}

@article{haruno2001mosaic,
  title={Mosaic model for sensorimotor learning and control},
  author={Haruno, Masahiko and Wolpert, David H and Kawato, Mitsuo},
  journal={Neural computation},
  volume={13},
  number={10},
  pages={2201--2220},
  year={2001},
  publisher={MIT Press}
}

@inproceedings{todorov2003unsupervised,
  title={Unsupervised learning of sensory-motor primitives},
  author={Todorov, Emanuel and Ghahramani, Zoubin},
  booktitle={Engineering in Medicine and Biology Society, 2003. Proceedings of the 25th Annual International Conference of the IEEE},
  volume={2},
  pages={1750--1753},
  year={2003},
  organization={IEEE}
}

@article{DBLP:journals/corr/WahlstromSD15,
  author    = {Niklas Wahlstr{\"{o}}m and
               Thomas B. Sch{\"{o}}n and
               Marc Peter Deisenroth},
  title     = {From Pixels to Torques: Policy Learning with Deep Dynamical Models},
  journal   = {CoRR},
  volume    = {abs/1502.02251},
  year      = {2015},
  url       = {http://arxiv.org/abs/1502.02251},
  timestamp = {Mon, 02 Mar 2015 00:00:00 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/WahlstromSD15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/DonahueHGRVSD14,
  author    = {Jeff Donahue and
               Lisa Anne Hendricks and
               Sergio Guadarrama and
               Marcus Rohrbach and
               Subhashini Venugopalan and
               Kate Saenko and
               Trevor Darrell},
  title     = {Long-term Recurrent Convolutional Networks for Visual Recognition
               and Description},
  journal   = {CoRR},
  year      = {2014},
}

@article{DeepMindContinuous,
  author    = {Timothy P. Lillicrap and Jonathan J. Hunt and Alexander Pritzel and Nicolas Heess and Tom Erez and Yuval Tassa and David Silver and Daan Wierstra},
  title     = {Continuous control with deep reinforcement learning},
  journal   = {CoRR},
  volume    = {abs/1509.02971},
  year      = {2015}
}

@article{DBLP:journals/corr/WatterSBR15,
  author    = {Manuel Watter and
               Jost Tobias Springenberg and
               Joschka Boedecker and
               Martin A. Riedmiller},
  title     = {Embed to Control: {A} Locally Linear Latent Dynamics Model for Control
               from Raw Images},
  journal   = {CoRR},
  volume    = {abs/1506.07365},
  year      = {2015},
  url       = {http://arxiv.org/abs/1506.07365},
  timestamp = {Wed, 01 Jul 2015 15:10:24 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/WatterSBR15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/ijcnn/LangeRV12,
  author    = {Sascha Lange and
               Martin A. Riedmiller and
               Arne Voigtl{\"{a}}nder},
  title     = {Autonomous reinforcement learning on raw visual input data in a real
               world application},
  booktitle = {The 2012 International Joint Conference on Neural Networks (IJCNN),
               Brisbane, Australia, June 10-15, 2012},
  pages     = {1--8},
  year      = {2012},
  crossref  = {DBLP:conf/ijcnn/2012},
  url       = {http://dx.doi.org/10.1109/IJCNN.2012.6252823},
  doi       = {10.1109/IJCNN.2012.6252823},
  timestamp = {Wed, 01 Apr 2015 20:06:23 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/ijcnn/LangeRV12},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/icra/BootsBF14,
  author    = {Byron Boots and
               Arunkumar Byravan and
               Dieter Fox},
  title     = {Learning predictive models of a depth camera {\&} manipulator
               from raw execution traces},
  booktitle = {2014 {IEEE} International Conference on Robotics and Automation, {ICRA}
               2014, Hong Kong, China, May 31 - June 7, 2014},
  pages     = {4021--4028},
  year      = {2014},
  crossref  = {DBLP:conf/icra/2014},
  url       = {http://dx.doi.org/10.1109/ICRA.2014.6907443},
  doi       = {10.1109/ICRA.2014.6907443},
  timestamp = {Tue, 07 Oct 2014 13:28:58 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icra/BootsBF14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/LevineFDA15,
  author    = {Sergey Levine and
               Chelsea Finn and
               Trevor Darrell and
               Pieter Abbeel},
  title     = {End-to-End Training of Deep Visuomotor Policies},
  journal   = {CoRR},
  volume    = {abs/1504.00702},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.00702},
  timestamp = {Sat, 02 May 2015 17:50:32 +0200},
  biburl    = {http://dblp2.uni-trier.de/rec/bib/journals/corr/LevineFDA15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{GuptaEfrosHebert_ECCV10,
   author="Abhinav Gupta and Alexei A. Efros and Martial Hebert", 
   title="Blocks World Revisited: Image Understanding Using Qualitative Geometry and Mechanics", 
   booktitle="European Conference on Computer Vision(ECCV)", 
   year="2010", 
}


@inproceedings{Urtasun:2006:PTG:1153170.1153448,
 author = {Urtasun, Raquel and Fleet, David J. and Fua, Pascal},
 title = {3D People Tracking with Gaussian Process Dynamical Models},
 booktitle = {CVPR},
 year = {2006}
} 


@article{Weng:2006:VOT:1223195.1223208,
 author = {Weng, Shiuh-Ku and Kuo, Chung-Ming and Tu, Shu-Kang},
 title = {Video Object Tracking Using Adaptive Kalman Filter},
 journal = {J. Vis. Comun. Image Represent.},
 issue_date = {December, 2006},
 volume = {17},
 number = {6},
 year = {2006},
 issn = {1047-3203},
 pages = {1190--1208},
 numpages = {19},
 url = {http://dx.doi.org/10.1016/j.jvcir.2006.03.004},
 doi = {10.1016/j.jvcir.2006.03.004},
 acmid = {1223208},
 publisher = {Academic Press, Inc.},
 address = {Orlando, FL, USA},
 keywords = {Adaptive Kalman filter, HSI color space, Occlusion ratio},
} 

  @inproceedings{Brand:1997:CHM:794189.794420,
  author = {Brand, M. and Oliver, N. and Pentland, A.},
  title = {Coupled hidden Markov models for complex action recognition},
  booktitle = {CVPR},
  year = {1997}
  }

  @article{Ghahramani:1997:FHM:274158.274165,
  author = {Ghahramani, Zoubin and Jordan, Michael I.},
  title = {Factorial Hidden Markov Models},
  journal = {Mach. Learn.},
  volume = {29},
  year = {1997}
  }

@inproceedings{lenz_deepMPC_2015,
  title={DeepMPC: Learning Deep Latent Features for Model Predictive Control},
  author={Ian Lenz and Ross Knepper and Ashutosh Saxena},
  year={2015},
  booktitle={RSS}
}


@article{citeulike:13838961,
    author = {Abadi, Mart\'{\i}n and Agarwal, Ashish and Barham, Paul and Brevdo, Eugene and Chen, Zhifeng and Citro, Craig and Corrado, Greg S. and Davis, Andy and Dean, Jeffrey and Devin, Matthieu and Ghemawat, Sanjay and Goodfellow, Ian and Harp, Andrew and Irving, Geoffrey and Isard, Michael and Jia, Yangqing and Jozefowicz, Rafal and Kaiser, Lukasz and Kudlur, Manjunath and Levenberg, Josh and Man\'{e}, Dan and Monga, Rajat and Moore, Sherry and Murray, Derek and Olah, Chris and Schuster, Mike and Shlens, Jonathon and Steiner, Benoit and Sutskever, Ilya and Talwar, Kunal and Tucker, Paul and Vanhoucke, Vincent and Vasudevan, Vijay and Vi\'{e}gas, Fernanda and Vinyals, Oriol and Warden, Pete and Wattenberg, Martin and Wicke, Martin and Yu, Yuan and Zheng, Xiaoqiang},
    title = {{TensorFlow}: Large-Scale Machine Learning on Heterogeneous Distributed Systems},
    journal = {arXiv:1603.04467},
    year = 2016,
}


@INPROCEEDINGS{Viola01rapidobject,
    author = {Paul Viola and Michael Jones},
    title = {Rapid object detection using a boosted cascade of simple features},
    booktitle = {},
    year = {2001},
    pages = {511--518}
}

@article{Chetverikov2005299,
title = "Robust Euclidean alignment of 3D point sets: the trimmed iterative closest point algorithm ",
journal = "Image and Vision Computing ",
volume = "23",
number = "3",
pages = "299 - 309",
year = "2005",
note = "",
author = "Dmitry Chetverikov and Dmitry Stepanov and Pavel Krsek"
}



@INPROCEEDINGS{jooiccv2015,
author = {Hanbyul Joo, Hao Liu, Lei Tan, Lin Gui, Bart Nabbe, Iain Matthews, Takeo Kanade, Shohei Nobuhara, and Yaser Sheikh},
title = {Panoptic Studio: A Massively Multiview System for Social Motion Capture},
booktitle = {ICCV},
year = {2015}
}



@INPROCEEDINGS{4409106, 
author={Saragih, J. and Goecke, R.}, 
booktitle={Computer Vision, 2007. ICCV 2007. IEEE 11th International Conference on}, 
title={A Nonlinear Discriminative Approach to AAM Fitting}, 
year={2007}, 
month={Oct}, 
pages={1-8}, 
keywords={computer vision;convergence of numerical methods;image registration;iterative methods;learning (artificial intelligence);AAM fitting formulation;active appearance model;boosting procedure;convergence rates;deformable visual object modeling;deformable visual object registration;iterative framework;linear parameter update model;nonlinear discriminative approach;Active appearance model;Cost function;Deformable models;Error correction;Fitting;Parametric statistics;Power engineering and energy;Power generation;Principal component analysis;Shape}, 
doi={10.1109/ICCV.2007.4409106}, 
ISSN={1550-5499},}

@incollection{NIPS2014_5573,
title = {Joint Training of a Convolutional Network and a Graphical Model for Human Pose Estimation},
author = {Tompson, Jonathan J and Jain, Arjun and LeCun, Yann and Bregler, Christoph},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N.D. Lawrence and K.Q. Weinberger},
pages = {1799--1807},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5573-joint-training-of-a-convolutional-network-and-a-graphical-model-for-human-pose-estimation.pdf}
}


@article{Mellinger:2012:TGC:2190635.2190636,
 author = {Mellinger, Daniel and Michael, Nathan and Kumar, Vijay},
 title = {Trajectory Generation and Control for Precise Aggressive Maneuvers with Quadrotors},
 journal = {Int. J. Rob. Res.},
 issue_date = {April     2012},
 volume = {31},
 number = {5},
 month = apr,
 year = {2012},
 issn = {0278-3649},
 pages = {664--674},
 numpages = {11},
 url = {http://dx.doi.org/10.1177/0278364911434236},
 doi = {10.1177/0278364911434236},
 acmid = {2190636},
 publisher = {Sage Publications, Inc.},
 address = {Thousand Oaks, CA, USA},
 keywords = {Trajectory generation, control, quadrotors},
} 

@inproceedings{YangR_CVPR_2011,
    author = "Yang, Yi and Ramanan, Deva",
    booktitle = "CVPR",
    year = "2011",
    title = "Articulated pose estimation with flexible mixtures-of-parts"
}


@INPROCEEDINGS{1315258, 
author={Agarwal, A. and Triggs, B.}, 
booktitle={Computer Vision and Pattern Recognition, 2004. CVPR 2004. Proceedings of the 2004 IEEE Computer Society Conference on}, 
title={3D human pose from silhouettes by relevance vector regression}, 
year={2004}, 
month={June}, 
volume={2}, 
pages={II-882-II-888 Vol.2}, 
keywords={errors;image segmentation;image sequences;learning (artificial intelligence);least squares approximations;motion estimation;multidimensional signal processing;regression analysis;3D human pose;direct nonlinear regression;histogram-of-shape-contexts descriptors;human motion capture data;image silhouettes;learning based method;mean angular errors;monocular image sequences;regularized least squares;relevance vector machine;relevance vector regression;shape descriptor vectors;silhouette segmentation errors;Biological system modeling;Humans;Image sequences;Kernel;Labeling;Learning systems;Robustness;Shape;Testing;Vectors}, 
doi={10.1109/CVPR.2004.1315258}, 
ISSN={1063-6919},}


@Inproceedings {export:145347,
author       = {Jamie Shotton and Andrew Fitzgibbon and Mat Cook and Toby Sharp and Mark
                Finocchio and Richard Moore and Alex Kipman and Andrew Blake},
booktitle    = {CVPR},
month        = {June},
publisher    = {IEEE},
title        = {Real-Time Human Pose Recognition in Parts from a Single Depth Image},
url          = {http://research.microsoft.com/apps/pubs/default.aspx?id=145347},
year         = {2011},
}

@inproceedings{DollarCVPR10pose,
  author = "P. Doll\'ar and P. Welinder and P. Perona",
  title = "Cascaded Pose Regression",
  booktitle = "CVPR",
  year = "2010",
}

@inproceedings{ionescu2014iterated,
  title={Iterated second-order label sensitive pooling for 3d human pose estimation},
  author={Ionescu, Catalin and Carreira, Joao and Sminchisescu, Cristian},
  booktitle={Computer Vision and Pattern Recognition (CVPR), 2014 IEEE Conference on},
  pages={1661--1668},
  year={2014},
  organization={IEEE}
}

@inproceedings{li2013fixed,
  title={Fixed-point model for structured labeling},
  author={Li, Quannan and Wang, Jingdong and Tu, Zhuowen and Wipf, David P},
  booktitle={Proceedings of the 30th International Conference on Machine Learning (ICML-13)},
  pages={214--221},
  year={2013}
}

@inproceedings{tu2008auto,
  title={Auto-context and its application to high-level vision tasks},
  author={Tu, Zhuowen},
  booktitle={Computer Vision and Pattern Recognition, 2008. CVPR 2008. IEEE Conference on},
  pages={1--8},
  year={2008},
  organization={IEEE}
}

@article{lafferty2001conditional,
  title={Conditional random fields: Probabilistic models for segmenting and labeling sequence data},
  author={Lafferty, John and McCallum, Andrew and Pereira, Fernando CN},
  year={2001}
}

@article{krahenbuhl2012efficient,
  title={Efficient inference in fully connected crfs with gaussian edge potentials},
  author={Kr{\"a}henb{\"u}hl, Philipp and Koltun, Vladlen},
  journal={arXiv preprint arXiv:1210.5644},
  year={2012}
}





@article{zhu2015segdeepm,
  title={segDeepM: Exploiting segmentation and context in deep neural networks for object detection},
  author={Zhu, Yukun and Urtasun, Raquel and Salakhutdinov, Ruslan and Fidler, Sanja},
  journal={arXiv preprint arXiv:1502.04275},
  year={2015}
}

@article{gidaris2015object,
  title={Object detection via a multi-region \& semantic segmentation-aware CNN model},
  author={Gidaris, Spyros and Komodakis, Nikos},
  journal={arXiv preprint arXiv:1505.01749},
  year={2015}
}

@incollection{ramakrishna2014pose,
  title={Pose Machines: Articulated Pose Estimation via Inference Machines},
  author={Ramakrishna, Varun and Munoz, Daniel and Hebert, Martial and Bagnell, James Andrew and Sheikh, Yaser},
  booktitle={Computer Vision--ECCV 2014},
  pages={33--47},
  year={2014},
  publisher={Springer International Publishing}
}

@inproceedings{ziebart2008maximum,
   author = {Brian D. Ziebart and Andrew Maas 
            and J. Andrew Bagnell and Anind K. Dey},
   title = {Maximum Entropy Inverse Reinforcement Learning},
   year = {2008},
   booktitle = {Proc. AAAI},
   pages = {1433--1438}
}

@article{weiss2012structured,
  title={Structured prediction cascades},
  author={Weiss, David and Sapp, Benjamin and Taskar, Ben},
  journal={arXiv preprint arXiv:1208.3279},
  year={2012}
}

@inproceedings{heitz2009cascaded,
  title={Cascaded classification models: Combining models for holistic scene understanding},
  author={Heitz, Geremy and Gould, Stephen and Saxena, Ashutosh and Koller, Daphne},
  booktitle={Advances in Neural Information Processing Systems},
  pages={641--648},
  year={2009}
}

@article{DBLP:journals/corr/SadeghianAS17,
  author    = {Amir Sadeghian and
               Alexandre Alahi and
               Silvio Savarese},
  title     = {Tracking The Untrackable: Learning To Track Multiple Cues with Long-Term
               Dependencies},
  journal   = {CoRR},
  volume    = {abs/1701.01909},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.01909},
  timestamp = {Wed, 07 Jun 2017 14:40:23 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/SadeghianAS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article {depthadaptive,
author = {Ying, Chris and Fragkiadaki, Katerina},
title = {Depth-Adaptive  Computational Policies for Efficient
Visual Tracking},
journal = {EMMCVPR},
year = {2017}
}

@article{DBLP:journals/corr/LiuAESR15,
  author    = {Wei Liu and
               Dragomir Anguelov and
               Dumitru Erhan and
               Christian Szegedy and
               Scott E. Reed and
               Cheng{-}Yang Fu and
               Alexander C. Berg},
  title     = {{SSD:} Single Shot MultiBox Detector},
  journal   = {CoRR},
  volume    = {abs/1512.02325},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.02325},
  archivePrefix = {arXiv},
  eprint    = {1512.02325},
  timestamp = {Wed, 07 Jun 2017 14:42:54 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LiuAESR15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/ChangFGHHLSSSSX15,
  author    = {Angel X. Chang and
               Thomas A. Funkhouser and
               Leonidas J. Guibas and
               Pat Hanrahan and
               Qi{-}Xing Huang and
               Zimo Li and
               Silvio Savarese and
               Manolis Savva and
               Shuran Song and
               Hao Su and
               Jianxiong Xiao and
               Li Yi and
               Fisher Yu},
  title     = {ShapeNet: An Information-Rich 3D Model Repository},
  journal   = {CoRR},
  volume    = {abs/1512.03012},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.03012},
  archivePrefix = {arXiv},
  eprint    = {1512.03012},
  timestamp = {Wed, 07 Jun 2017 14:41:05 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/ChangFGHHLSSSSX15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{DBLP:journals/corr/RedmonF16,
  author    = {Joseph Redmon and
               Ali Farhadi},
  title     = {{YOLO9000:} Better, Faster, Stronger},
  journal   = {CoRR},
  volume    = {abs/1612.08242},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.08242},
  archivePrefix = {arXiv},
  eprint    = {1612.08242},
  timestamp = {Wed, 07 Jun 2017 14:40:20 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/RedmonF16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/KumarGTL16,
  author    = {Vikash Kumar and
               Abhishek Gupta and
               Emanuel Todorov and
               Sergey Levine},
  title     = {Learning Dexterous Manipulation Policies from Experience and Imitation},
  journal   = {CoRR},
  volume    = {abs/1611.05095},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.05095},
  archivePrefix = {arXiv},
  eprint    = {1611.05095},
  timestamp = {Wed, 07 Jun 2017 14:40:28 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/KumarGTL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@incollection{NIPS2014_5421,
title = {Deep Learning for Real-Time Atari Game Play Using Offline Monte-Carlo Tree Search Planning},
author = {Guo, Xiaoxiao and Singh, Satinder and Lee, Honglak and Lewis, Richard L and Wang, Xiaoshi},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {3338--3346},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5421-deep-learning-for-real-time-atari-game-play-using-offline-monte-carlo-tree-search-planning.pdf}
}


@article{DBLP:journals/corr/abs-1710-06542,
  author    = {Lerrel Pinto and
               Marcin Andrychowicz and
               Peter Welinder and
               Wojciech Zaremba and
               Pieter Abbeel},
  title     = {Asymmetric Actor Critic for Image-Based Robot Learning},
  journal   = {CoRR},
  volume    = {abs/1710.06542},
  year      = {2017},
  url       = {http://arxiv.org/abs/1710.06542},
  archivePrefix = {arXiv},
  eprint    = {1710.06542},
  timestamp = {Wed, 01 Nov 2017 19:05:43 +0100},
  biburl    = {http://dblp.org/rec/bib/journals/corr/abs-1710-06542},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article {TOPS:TOPS12155,
author = {Lupyan, Gary and Bergen, Benjamin},
title = {How Language Programs the Mind},
journal = {Topics in Cognitive Science},
volume = {8},
number = {2},
issn = {1756-8765},
url = {http://dx.doi.org/10.1111/tops.12155},
doi = {10.1111/tops.12155},
pages = {408--424},
keywords = {Language, Language and thought, Embodiment, Categorization, Language evolution},
year = {2016},
}

@article{anonymous2018zero-shot,
  title={Zero-Shot Visual Imitation},
  author={Anonymous},
  journal={International Conference on Learning Representations},
  year={2018},
  url={https://openreview.net/forum?id=BkisuzWRW}
}

@article{DBLP:journals/corr/MnihBMGLHSK16,
  author    = {Volodymyr Mnih and
               Adri{\`{a}} Puigdom{\`{e}}nech Badia and
               Mehdi Mirza and
               Alex Graves and
               Timothy P. Lillicrap and
               Tim Harley and
               David Silver and
               Koray Kavukcuoglu},
  title     = {Asynchronous Methods for Deep Reinforcement Learning},
  journal   = {CoRR},
  volume    = {abs/1602.01783},
  year      = {2016},
  url       = {http://arxiv.org/abs/1602.01783},
  archivePrefix = {arXiv},
  eprint    = {1602.01783},
  timestamp = {Wed, 07 Jun 2017 14:43:09 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/MnihBMGLHSK16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{interactive,
  author    = {https://simons.berkeley.edu/workshops/machinelearning2017-1},
  year      = {2017}
}

@article{DBLP:journals/corr/RahmatizadehAB16,
  author    = {Rouhollah Rahmatizadeh and
               Pooya Abolghasemi and
               Ladislau B{\"{o}}l{\"{o}}ni},
  title     = {Learning Manipulation Trajectories Using Recurrent Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1603.03833},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.03833},
  archivePrefix = {arXiv},
  eprint    = {1603.03833},
  timestamp = {Wed, 07 Jun 2017 14:40:59 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/RahmatizadehAB16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/SermanetXL16,
  author    = {Pierre Sermanet and
               Kelvin Xu and
               Sergey Levine},
  title     = {Unsupervised Perceptual Rewards for Imitation Learning},
  journal   = {CoRR},
  volume    = {abs/1612.06699},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.06699},
  archivePrefix = {arXiv},
  eprint    = {1612.06699},
  timestamp = {Wed, 07 Jun 2017 14:42:07 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/SermanetXL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{MullingKKP2012_2,
  title = {Learning to Select and Generalize Striking Movements in Robot Table Tennis},
  author = {M{\"u}lling, K. and Kober, J. and Kroemer, O. and Peters, J.},
  journal = {International Journal of Robotics Research},
  volume = {32},
  number = {3},
  pages = {263-279},
  year = {2013}
}



@article {CDEP:CDEP12032,
author = {Waxman, Sandra and Fu, Xiaolan and Arunachalam, Sudha and Leddon, Erin and Geraghty, Kathleen and Song, Hyun-joo},
title = {Are Nouns Learned Before Verbs? Infants Provide Insight Into a Long-Standing Debate},
journal = {Child Development Perspectives},
volume = {7},
number = {3},
issn = {1750-8606},
url = {http://dx.doi.org/10.1111/cdep.12032},
doi = {10.1111/cdep.12032},
pages = {155--159},
keywords = {language development, cognitive development, cross-linguistic studies, infancy},
year = {2013},
}


@InProceedings{Su_2015_ICCV,
    Title={Render for CNN: Viewpoint Estimation in Images Using CNNs Trained with Rendered 3D Model Views},
    Author={Su, Hao and Qi, Charles R. and Li, Yangyan and Guibas, Leonidas J.},
    Booktitle={The IEEE International Conference on Computer Vision (ICCV)},
    month = {December},
    Year= {2015}
}

@article{nowozin2011structured,
  title={Structured learning and prediction in computer vision},
  author={Nowozin, Sebastian and Lampert, Christoph H},
  journal={Foundations and Trends{\textregistered} in Computer Graphics and Vision},
  volume={6},
  number={3--4},
  pages={185--365},
  year={2011},
  publisher={Now Publishers Inc.}
}

@inproceedings{stollenga2014deep,
  title={Deep networks with internal selective attention through feedback connections},
  author={Stollenga, Marijn F and Masci, Jonathan and Gomez, Faustino and Schmidhuber, J{\"u}rgen},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3545--3553},
  year={2014}
}

@article{pinheiro2013recurrent,
  title={Recurrent convolutional neural networks for scene parsing},
  author={Pinheiro, Pedro HO and Collobert, Ronan},
  journal={arXiv preprint arXiv:1306.2795},
  year={2013}
}

@article{kass1988snakes,
  title={Snakes: Active contour models},
  author={Kass, Michael and Witkin, Andrew and Terzopoulos, Demetri},
  journal={International journal of computer vision},
  volume={1},
  number={4},
  pages={321--331},
  year={1988},
  publisher={Springer}
}

@article{cootes1995active,
  title={Active shape models-their training and application},
  author={Cootes, Timothy F and Taylor, Christopher J and Cooper, David H and Graham, Jim},
  journal={Computer vision and image understanding},
  volume={61},
  number={1},
  pages={38--59},
  year={1995},
  publisher={Elsevier}
}

@article{felzenszwalb2010object,
  title={Object detection with discriminatively trained part-based models},
  author={Felzenszwalb, Pedro F and Girshick, Ross B and McAllester, David and Ramanan, Deva},
  journal={Pattern Analysis and Machine Intelligence, IEEE Transactions on},
  volume={32},
  number={9},
  pages={1627--1645},
  year={2010},
  publisher={IEEE}
}

@inproceedings{xiong2013supervised,
  title={Supervised descent method and its applications to face alignment},
  author={Xiong, Xuehan and De la Torre, Fernando},
  booktitle={Computer Vision and Pattern Recognition (CVPR), 2013 IEEE Conference on},
  pages={532--539},
  year={2013},
  organization={IEEE}
}


@article{Hochreiter:1997:LSM:1246443.1246450,
 author = {Hochreiter, Sepp and Schmidhuber, J\"{u}rgen},
 title = {Long Short-Term Memory},
 journal = {Neural Comput.},
 issue_date = {November 15, 1997},
 volume = {9},
 number = {8},
 year = {1997},
 issn = {0899-7667},
 pages = {1735--1780},
 numpages = {46},
 url = {http://dx.doi.org/10.1162/neco.1997.9.8.1735},
 doi = {10.1162/neco.1997.9.8.1735},
 acmid = {1246450},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 

@article{DBLP:journals/corr/Graves13,
  author    = {Alex Graves},
  title     = {Generating Sequences With Recurrent Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1308.0850},
  year      = {2013},
  url       = {http://arxiv.org/abs/1308.0850},
  timestamp = {Tue, 10 Dec 2013 12:03:02 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/Graves13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@techreport{Welch:1995:IKF:897831,
 author = {Welch, Greg and Bishop, Gary},
 title = {An Introduction to the Kalman Filter},
 year = {1995},
 publisher = {University of North Carolina at Chapel Hill},
 address = {Chapel Hill, NC, USA},
} 

@article{Vincent:2010:SDA:1756006.1953039,
 author = {Vincent, Pascal and Larochelle, Hugo and Lajoie, Isabelle and Bengio, Yoshua and Manzagol, Pierre-Antoine},
 title = {Stacked Denoising Autoencoders: Learning Useful Representations in a Deep Network with a Local Denoising Criterion},
 journal = {J. Mach. Learn. Res.},
 issue_date = {3/1/2010},
 volume = {11},
 year = {2010},
 issn = {1532-4435},
 pages = {3371--3408},
 numpages = {38},
 url = {http://dl.acm.org/citation.cfm?id=1756006.1953039},
 acmid = {1953039},
 publisher = {JMLR.org},
} 


@article{Mayne20142967,
title = "Model predictive control: Recent developments and future promise ",
journal = "Automatica ",
volume = "50",
number = "12",
pages = "2967 - 2986",
year = "2014",
note = "",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/j.automatica.2014.10.128",
url = "http://www.sciencedirect.com/science/article/pii/S0005109814005160",
author = "David Q. Mayne",
keywords = "Model predictive control ",
abstract = "Abstract This paper recalls a few past achievements in Model Predictive Control, gives an overview of some current developments and suggests a few avenues for future research. "
}

@inproceedings{DBLP:journals/corr/MisraZH16,
  author    = {Ishan Misra and
               C. Lawrence Zitnick and
               Martial Hebert},
  title     = {Unsupervised Learning using Sequential Verification for Action Recognition},
  booktitle={ECCV},
  year      = {2016},
}



@inproceedings{DBLP:journals/corr/WangG15a,
  author    = {Xiaolong Wang and
               Abhinav Gupta},
  title     = {Unsupervised Learning of Visual Representations using Videos},
  booktitle = {ICCV},
  year      = {2015}
}

@article{Wiskott:2002:SFA:638940.638941,
 author = {Wiskott, Laurenz and Sejnowski, Terrence J.},
 title = {Slow Feature Analysis: Unsupervised Learning of Invariances},
 journal = {Neural Comput.},
 issue_date = {April 2002},
 volume = {14},
 number = {4},
 year = {2002},
 issn = {0899-7667},
 pages = {715--770},
 numpages = {56},
 url = {http://dx.doi.org/10.1162/089976602317318938},
 doi = {10.1162/089976602317318938},
 acmid = {638941},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 


@inproceedings{DBLP:conf/icml/BellemareVT14,
  author    = {Marc G. Bellemare and
               Joel Veness and
               Erik Talvitie},
  title     = {Skip Context Tree Switching},
  booktitle = {Proceedings of the 31th International Conference on Machine Learning,
               {ICML} 2014, Beijing, China, 21-26 June 2014},
  pages     = {1458--1466},
  year      = {2014},
  crossref  = {DBLP:conf/icml/2014},
  url       = {http://jmlr.org/proceedings/papers/v32/bellemare14.html},
  timestamp = {Fri, 07 Nov 2014 20:42:30 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icml/BellemareVT14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{DBLP:conf/icmla/KietzmannR09,
  author    = {Tim C. Kietzmann and
               Martin A. Riedmiller},
  title     = {The Neuro Slot Car Racer: Reinforcement Learning in a Real World Setting},
  booktitle = {International Conference on Machine Learning and Applications, {ICMLA}
               2009, Miami Beach, Florida, USA, December 13-15, 2009},
  pages     = {311--316},
  year      = {2009},
  crossref  = {DBLP:conf/icmla/2009},
  url       = {http://dx.doi.org/10.1109/ICMLA.2009.15},
  doi       = {10.1109/ICMLA.2009.15},
  timestamp = {Wed, 06 May 2015 16:20:33 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icmla/KietzmannR09},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}





@article{googlespeech,
  author    = {https://cloud.google.com/speech/}
}



@article{DBLP:journals/corr/MnihKSGAWR13,
  author    = {Volodymyr Mnih and
               Koray Kavukcuoglu and
               David Silver and
               Alex Graves and
               Ioannis Antonoglou and
               Daan Wierstra and
               Martin A. Riedmiller},
  title     = {Playing Atari with Deep Reinforcement Learning},
  journal   = {CoRR},
  volume    = {abs/1312.5602},
  year      = {2013},
  url       = {http://arxiv.org/abs/1312.5602},
  timestamp = {Wed, 01 Apr 2015 20:06:15 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MnihKSGAWR13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{DBLP:conf/icra/BootsBF14,
  author    = {Byron Boots and
               Arunkumar Byravan and
               Dieter Fox},
  title     = {Learning predictive models of a depth camera {\&} manipulator
               from raw execution traces},
  booktitle = {2014 {IEEE} International Conference on Robotics and Automation, {ICRA}
               2014, Hong Kong, China, May 31 - June 7, 2014},
  pages     = {4021--4028},
  year      = {2014},
  crossref  = {DBLP:conf/icra/2014},
  url       = {http://dx.doi.org/10.1109/ICRA.2014.6907443},
  doi       = {10.1109/ICRA.2014.6907443},
  timestamp = {Tue, 07 Oct 2014 13:28:58 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icra/BootsBF14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/LevineFDA15,
  author    = {Sergey Levine and
               Chelsea Finn and
               Trevor Darrell and
               Pieter Abbeel},
  title     = {End-to-End Training of Deep Visuomotor Policies},
  journal   = {CoRR},
  volume    = {abs/1504.00702},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.00702},
  timestamp = {Sat, 02 May 2015 17:50:32 +0200},
  biburl    = {http://dblp2.uni-trier.de/rec/bib/journals/corr/LevineFDA15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{lenz_deepMPC_2015,
  title={DeepMPC: Learning Deep Latent Features for Model Predictive Control},
  author={Ian Lenz and Ross Knepper and Ashutosh Saxena},
  year={2015},
  booktitle={RSS}
}



@article{DBLP:journals/corr/DonahueHGRVSD14,
  author    = {Jeff Donahue and
               Lisa Anne Hendricks and
               Sergio Guadarrama and
               Marcus Rohrbach and
               Subhashini Venugopalan and
               Kate Saenko and
               Trevor Darrell},
  title     = {Long-term Recurrent Convolutional Networks for Visual Recognition
               and Description},
  journal   = {CoRR},
  year      = {2014},
}



@INPROCEEDINGS{4408986, 
author={A. Rabinovich and A. Vedaldi and C. Galleguillos and E. Wiewiora and S. Belongie}, 
booktitle={2007 IEEE 11th International Conference on Computer Vision}, 
title={Objects in Context}, 
year={2007}, 
pages={1-8}, 
keywords={image representation;image segmentation;object recognition;optimisation;conditional random field;contextual relevance;image representation;image segmentation;object label agreement;object recognition;semantic object context;visual object categorization;Computer science;Computer vision;Context modeling;Electrical capacitance tomography;Image segmentation;Layout;Object recognition;Psychology;Statistics;Training data}, 
doi={10.1109/ICCV.2007.4408986}, 
ISSN={1550-5499}, 
month={Oct},}



@article{DBLP:journals/corr/VinyalsTBE14,
  author    = {Oriol Vinyals and
               Alexander Toshev and
               Samy Bengio and
               Dumitru Erhan},
  title     = {Show and Tell: {A} Neural Image Caption Generator},
  journal   = {CoRR},
  volume    = {abs/1411.4555},
  year      = {2014},
  url       = {http://arxiv.org/abs/1411.4555},
  timestamp = {Mon, 01 Dec 2014 14:32:13 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/VinyalsTBE14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{citeulike:11039228,
    abstract = {{Predictions of the near future can optimize the accuracy and speed of sensory processing as well as of behavioral responses. Previous experience and contextual cues are essential elements in the generation of a subjective prediction. Using a blocked fMRI paradigm, we investigated the pattern of neural activation in anticipation of a sensory stimulus and during the processing of the somatosensory stimulus itself. Tickling was chosen as the somatosensory stimulus rather than simple touch in order to increase the probability to get a high degree of anticipation. The location and nature of the stimulus were well defined to the subject. The state of anticipation was initiated by attributing an uncertainty regarding the time of stimulus onset. The network of activation and deactivation during anticipation of the expected stimulus was similar to that engaged during the actual sensory stimulation. The areas that were activated during both states included the contralateral primary sensory cortex, bilateral areas in the inferior parietal lobules, the putative area SII, the right anterior cingulate cortex and areas in the right prefrontal cortex. Similarly, common decreases were observed in areas of sensorimotor cortex located outside the area representing the target of stimulus, i.e., areas that process information which is irrelevant to the attended process. The overlapping pattern of change, during the somatosensory stimulation and the anticipation, furthers the idea that predictions are subserved by a neuronal network similar to that which subserves the processing of actual sensory input. Moreover, this study indicates that activation of primary somatosensory cortex can be obtained without intra-modal sensory input. These findings suggest that anticipation may invoke a tonic top-down regulation of neural activity}},
    author = {Carlsson, K. and Petrovic, P. and Skare, S. and Petersson, K. M. and Ingvar, M.},
    citeulike-article-id = {11039228},
    citeulike-linkout-0 = {\#},
    comment = {UI - 20396805 DA - 20000918},
    journal = {J.Cogn Neurosci.},
    keywords = {adult, anatomy, cinguli, cognition, comparative, conduction, cortex, cues, defense, female, gyrus, histology, human, imaging, lobe, magnetic, male, nerve, net, neural, parietal, perception, perceptual, physical, physiology, prefrontal, probability, resonance, rest, somatosensory, stimulation, study, supportnon-usgovt, touch},
    location = {Karolinska Institute/Karolinska Hospital, Sweden},
    month = jul,
    number = {0898-929X LA - eng PT - Clinical Trial PT - Journal Article},
    pages = {691--703},
    posted-at = {2012-08-10 15:13:09},
    priority = {2},
    title = {{Tickling expectations: neural processing in anticipation of a sensory stimulus}},
    url = {\#},
    volume = {12},
    year = {2000}
}


@article{citeulike:13324644,
    abstract = {{An essential aspect of episodic memory is the formation of associations between neutral sensory cues in the environment. In light of recent evidence that this critical aspect of learning does not require the hippocampus, we tested the involvement of the retrosplenial cortex (RSC) in this process using a chemogenetic approach that allowed us to temporarily silence neurons along the entire rostrocaudal extent of the RSC. A viral vector containing the gene for a synthetic inhibitory G-protein-coupled receptor (hM4Di) was infused into RSC. When the receptor was later activated by systemic injection of clozapine-N-oxide, neural activity in RSC was transiently silenced (confirmed using a patch-clamp procedure). Rats expressing hM4Di and control rats were trained in a sensory preconditioning procedure in which a tone and light were paired on some trials and a white noise stimulus was presented alone on the other trials during the Preconditioning phase. Thus, rats were given the opportunity to form an association between a tone and a light in the absence of reinforcement. Later, the light was paired with food. During the test phase when the auditory cues were presented alone, controls exhibited more conditioned responding during presentation of the tone compared with the white noise reflecting the prior formation of a tone-light association. Silencing RSC neurons during the Preconditioning phase prevented the formation of an association between the tone and light and eliminated the sensory preconditioning effect. These findings indicate that RSC may contribute to episodic memory formation by linking essential sensory stimuli during learning.}},
    author = {Robinson, Siobhan and Todd, Travis P. and Pasternak, Anna R. and Luikart, Bryan W. and Skelton, Patrick D. and Urban, Daniel J. and Bucci, David J.},
    citeulike-article-id = {13324644},
    citeulike-linkout-0 = {http://dx.doi.org/10.1523/jneurosci.1349-14.2014},
    citeulike-linkout-1 = {http://www.jneurosci.org/content/34/33/10982.abstract},
    citeulike-linkout-2 = {http://www.jneurosci.org/content/34/33/10982.full.pdf},
    day = {13},
    doi = {10.1523/jneurosci.1349-14.2014},
    issn = {1529-2401},
    journal = {The Journal of Neuroscience},
    keywords = {genetics},
    number = {33},
    pages = {10982--10988},
    posted-at = {2014-08-13 18:35:53},
    priority = {2},
    publisher = {Society for Neuroscience},
    title = {{Chemogenetic Silencing of Neurons in Retrosplenial Cortex Disrupts Sensory Preconditioning}},
    url = {http://dx.doi.org/10.1523/jneurosci.1349-14.2014},
    volume = {34},
    year = {2014}
}


@article{DBLP:journals/corr/abs-1301-3781,
  author    = {Tomas Mikolov and
               Kai Chen and
               Greg Corrado and
               Jeffrey Dean},
  title     = {Efficient Estimation of Word Representations in Vector Space},
  journal   = {CoRR},
  volume    = {abs/1301.3781},
  year      = {2013},
  url       = {http://arxiv.org/abs/1301.3781},
  timestamp = {Mon, 18 Feb 2013 20:50:59 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/abs-1301-3781},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{citeulike:778023,
       author = {Hinton, G. E. and Salakhutdinov, R. R.},
       journal = {Science},
    keywords = {algorithm, compexity, computation, data, neural\_networks},
    month = jul,
    number = {5786},
    pages = {504--507},
    pmid = {16873662},
    posted-at = {2008-02-27 22:55:12},
    priority = {2},
    publisher = {American Association for the Advancement of Science},
    title = {{Reducing the Dimensionality of Data with Neural Networks}},
    url = {http://dx.doi.org/10.1126/science.1127647},
    volume = {313},
    year = {2006}
}


@article{Vincent:2010:SDA:1756006.1953039,
 author = {Vincent, Pascal and Larochelle, Hugo and Lajoie, Isabelle and Bengio, Yoshua and Manzagol, Pierre-Antoine},
 title = {Stacked Denoising Autoencoders: Learning Useful Representations in a Deep Network with a Local Denoising Criterion},
 journal = {J. Mach. Learn. Res.},
 issue_date = {3/1/2010},
 volume = {11},
 year = {2010},
 issn = {1532-4435},
 pages = {3371--3408},
 numpages = {38},
 url = {http://dl.acm.org/citation.cfm?id=1756006.1953039},
 acmid = {1953039},
 publisher = {JMLR.org},
} 


@inproceedings{DBLP:journals/jmlr/Maaten09,
  author    = {Laurens van der Maaten},
  title     = {Learning a Parametric Embedding by Preserving Local Structure},
  booktitle = {AISTATS},
  year      = {2009}
}

@inproceedings{DBLP:conf/interspeech/MikolovKBCK10,
  author    = {Tomas Mikolov and
               Martin Karafi{\'{a}}t and
               Luk{\'{a}}s Burget and
               Jan Cernock{\'{y}} and
               Sanjeev Khudanpur},
  title     = {Recurrent neural network based language model},
  booktitle = {{INTERSPEECH} 2010, 11th Annual Conference of the International Speech
               Communication Association, Makuhari, Chiba, Japan, September 26-30,
               2010},
  pages     = {1045--1048},
  year      = {2010},
  crossref  = {DBLP:conf/interspeech/2010},
  url       = {http://www.isca-speech.org/archive/interspeech_2010/i10_1045.html},
  timestamp = {Thu, 09 Apr 2015 14:27:21 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/interspeech/MikolovKBCK10},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Brooks:1979:AMV:1624861.1624890,
 author = {Brooks, Rodney A. and Creiner, Russell and Binford, Thomas O.},
 title = {The ACRONYM Model-based Vision System},
 booktitle = {Proceedings of the 6th International Joint Conference on Artificial Intelligence - Volume 1},
 series = {IJCAI'79},
 year = {1979},
 isbn = {0-934613-47-8},
 location = {Tokyo, Japan},
 pages = {105--113},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=1624861.1624890},
 acmid = {1624890},
 publisher = {Morgan Kaufmann Publishers Inc.},
 address = {San Francisco, CA, USA},
} 




@inproceedings{DBLP:conf/slt/MikolovZ12,
  author    = {Tomas Mikolov and
               Geoffrey Zweig},
  title     = {Context dependent recurrent neural network language model},
  booktitle = {2012 {IEEE} Spoken Language Technology Workshop (SLT), Miami, FL,
               USA, December 2-5, 2012},
  pages     = {234--239},
  year      = {2012},
  crossref  = {DBLP:conf/slt/2012},
  url       = {http://dx.doi.org/10.1109/SLT.2012.6424228},
  doi       = {10.1109/SLT.2012.6424228},
  timestamp = {Tue, 12 Feb 2013 15:35:36 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/slt/MikolovZ12},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@MISC{Williams95gradient-basedlearning,
    author = {Ronald J. Williams and David Zipser},
    title = {Gradient-Based Learning Algorithms for Recurrent Networks and Their Computational Complexity},
    year = {1995}
}
@article{Bengio:2003:NPL:944919.944966,
 author = {Bengio, Yoshua and Ducharme, R{\'e}jean and Vincent, Pascal and Janvin, Christian},
 title = {A Neural Probabilistic Language Model},
 journal = {J. Mach. Learn. Res.},
 issue_date = {3/1/2003},
 volume = {3},
 year = {2003},
 issn = {1532-4435},
 pages = {1137--1155},
 numpages = {19},
 url = {http://dl.acm.org/citation.cfm?id=944919.944966},
 acmid = {944966},
 publisher = {JMLR.org},
} 

@inproceedings{Efros03, 
  title = {Recognizing Action at a Distance}, 
  author = {Alexei A. Efros and Alexander C. Berg and Greg Mori and
Jitendra Malik}, 
  booktitle = {ICCV}, 
  year = 2003 }
  
@inproceedings{DBLP:conf/interspeech/KombrinkMKB11,
  author    = {Stefan Kombrink and
               Tomas Mikolov and
               Martin Karafi{\'{a}}t and
               Luk{\'{a}}s Burget},
  title     = {Recurrent Neural Network Based Language Modeling in Meeting Recognition},
  booktitle = {INTERSPEECH},
  year      = {2011},
}

@ARTICLE{Brown92class-basedn-gram,
    author = {Peter F. Brown and Peter V. deSouza and Robert L. Mercer and Vincent J. Della Pietra and Jenifer C. Lai},
    title = {Class-Based n-gram Models of Natural Language},
    journal = {Computational Linguistics},
    year = {1992},
    volume = {18},
    pages = {467--479}
}

@InProceedings{ICML2011Sutskever_524,
  author =    {Ilya Sutskever and James Martens and Geoffrey Hinton},
  title =     {Generating Text with Recurrent Neural Networks },
  booktitle = {ICML},
  year =      {2011}
}
@article{Hochreiter:1997:LSM:1246443.1246450,
 author = {Hochreiter, Sepp and Schmidhuber, J\"{u}rgen},
 title = {Long Short-Term Memory},
 journal = {Neural Comput.},
 issue_date = {November 15, 1997},
 volume = {9},
 number = {8},
 year = {1997},
 issn = {0899-7667},
 pages = {1735--1780},
 numpages = {46},
 url = {http://dx.doi.org/10.1162/neco.1997.9.8.1735},
 doi = {10.1162/neco.1997.9.8.1735},
 acmid = {1246450},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 

@inproceedings{DBLP:conf/icml/GravesJ14,
  author    = {Alex Graves and
               Navdeep Jaitly},
  title     = {Towards End-To-End Speech Recognition with Recurrent Neural Networks},
  booktitle = {Proceedings of the 31th International Conference on Machine Learning,
               {ICML} 2014, Beijing, China, 21-26 June 2014},
  pages     = {1764--1772},
  year      = {2014},
  crossref  = {DBLP:conf/icml/2014},
  url       = {http://jmlr.org/proceedings/papers/v32/graves14.html},
  timestamp = {Fri, 07 Nov 2014 20:42:30 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icml/GravesJ14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/Graves13,
  author    = {Alex Graves},
  title     = {Generating Sequences With Recurrent Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1308.0850},
  year      = {2013},
  url       = {http://arxiv.org/abs/1308.0850},
  timestamp = {Tue, 10 Dec 2013 12:03:02 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/Graves13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@book{DBLP:series/sci/2012-385,
  author    = {Alex Graves},
  title     = {Supervised Sequence Labelling with Recurrent Neural Networks},
  series    = {Studies in Computational Intelligence},
  volume    = {385},
  publisher = {Springer},
  year      = {2012},
  url       = {http://dx.doi.org/10.1007/978-3-642-24797-2},
  doi       = {10.1007/978-3-642-24797-2},
  isbn      = {978-3-642-24796-5},
  timestamp = {Tue, 20 Mar 2012 09:00:13 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/series/sci/2012-385},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/CarreiraAFM15,
  author    = {Jo{\~{a}}o Carreira and
               Pulkit Agrawal and
               Katerina Fragkiadaki and
               Jitendra Malik},
  title     = {Human Pose Estimation with Iterative Error Feedback},
  journal   = {CoRR},
  volume    = {abs/1507.06550},
  year      = {2015},
  url       = {http://arxiv.org/abs/1507.06550},
  archivePrefix = {arXiv},
  eprint    = {1507.06550},
  timestamp = {Wed, 07 Jun 2017 14:42:58 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/CarreiraAFM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@misc{Authors14,
 author = {Authors},
 title = {The frobnicatable foo filter},
 note = {Face and Gesture  submission ID 324. Supplied as additional material {\tt fg324.pdf}},
 year = 2014
}


@inproceedings{bh-sm-00,
 author = {Brand, Matthew and Hertzmann, Aaron},
 title = {Style Machines},
 series = {SIGGRAPH},
 year = {2000}
}

@article{hpp-sthm-05,
 author = {Hsu, Eugene and Pulli, Kari and Popovi\'{c}, Jovan},
 title = {Style Translation for Human Motion},
 journal = {ACM Transactions on Graphics},
 issue_date = {July 2005},
 volume = {24},
 number = {3},
 month = jul,
 year = {2005},
 pages = {1082--1089},
 numpages = {8},
 publisher = {ACM Press},
 address = {New York, NY, USA},
}

@inproceedings{prm-lslmh-00,
author = "Pavlovic, Vladimir and James M. Rehg and John MacCormick",

booktitle = "Neural Information Processing Systems (NIPS)",

title = "Learning switching linear models of human motion",
year = "2000",
}


@inproceedings{Urtasun:2006:PTG:1153170.1153448,
 author = {Urtasun, Raquel and Fleet, David J. and Fua, Pascal},
 title = {3D People Tracking with Gaussian Process Dynamical Models},
 booktitle = {CVPR},
 year = {2006}
} 


@article{Fox:IEEESPM2010,
title={Bayesian Nonparametric Methods for Learning {M}arkov Switching Processes},
author={Fox, E.B. and Sudderth, E.B. and Jordan, M.I. and Willsky, A.S.},
journal={Signal Processing Magazine, IEEE},
volume={27},
number={6},
pages={43--54},
year={2010},
}


@article{wfh-gpdmh-08,
 author = {Wang, Jack M. and Fleet, David J. and Hertzmann, Aaron},
 title = {Gaussian Process Dynamical Models for Human Motion},
 journal = {TPAMI},
 volume = {30},
 year = {2008}
} 

@inproceedings{wfh-mgpms-07,
 author = {Wang, Jack M. and Fleet, David J. and Hertzmann, Aaron},
 title = {Multifactor Gaussian Process Models for Style-content Separation},
 booktitle = {ICML},
 year = {2007}
}

@inproceedings{ufgpd-tclvm-08,
  author    = {Raquel Urtasun and
               David J. Fleet and
               Andreas Geiger and
               Jovan Popovic and
               Trevor Darrell and
               Neil D. Lawrence},
  title     = {Topologically-constrained latent variable models},
  booktitle = {ICML},
  year      = {2008}
}

@inProceedings{vpsKpsTulsianiM14,
author    = {Shubham Tulsiani and Jitendra Malik},
title     = {Viewpoints and Keypoints},
year={2015},
booktitle={CVPR}
}

@inproceedings{thr-mhmub-06,
  author    = {Graham W. Taylor and
               Geoffrey E. Hinton and
               Sam T. Roweis},
  title     = {Modeling Human Motion Using Binary Latent Variables},
  booktitle = {NIPS},
  year      = {2006}
}

@inproceedings{th-fcrbm-09,
  author    = {Graham W. Taylor and
               Geoffrey E. Hinton},
  title     = {Factored conditional restricted Boltzmann Machines for modeling motion
               style},
  booktitle = {ICML},
  year      = {2009}
}


@article{h36m_pami,
author = {Ionescu, Catalin and Papava, Dragos and Olaru, Vlad and Sminchisescu,  Cristian},
title = {Human3.6M: Large Scale Datasets and Predictive Methods for 3D Human Sensing in Natural Environments},
journal = {TPAMI},
volume = {36},
number = {7},
year = {2014}
}


@inproceedings{sht-rtrbm-08,
  author    = {Ilya Sutskever and
               Geoffrey E. Hinton and
               Graham W. Taylor},
  title     = {The Recurrent Temporal Restricted Boltzmann Machine},
  booktitle = {NIPS},
  year      = {2008}
}


@misc{Authors14b,
 author = {Authors},
 title = {Frobnication tutorial},
 note = {Supplied as additional material {\tt tr.pdf}},
 year = 2014
}

@article{Alpher02,
author = {A. Alpher},
title = {Frobnication},
journal = {Journal of Foo},
volume = 12, 
number = 1, 
pages = {234--778}, 
year = 2002
}

@article{Alpher03,
author = {A. Alpher and  J.~P.~N. Fotheringham-Smythe},
title = {Frobnication revisited},
journal = {Journal of Foo},
volume = 13, 
number = 1, 
pages = {234--778}, 
year = 2003
}


@article{Sigal:2012:LPE:2205801.2205829,
 author = {Sigal, Leonid and Isard, Michael and Haussecker, Horst and Black, Michael J.},
 title = {Loose-limbed People: Estimating {3D} Human Pose and Motion Using Non-parametric Belief Propagation},
 journal = {IJCV},
 volume = {98},
 year = {2012}
}

@inproceedings{conf/cvpr/SappWT11,
  added-at = {2011-08-23T00:00:00.000+0200},
  author = {Sapp, Benjamin and Weiss, David and Taskar, Ben},
  booktitle = {CVPR},
  title = {Parsing human motion with stretchable models.},
  year = 2011
}

@inproceedings{Ramakrishna:2012:RHP:2404742.2404786,
 author = {Ramakrishna, Varun and Kanade, Takeo and Sheikh, Yaser},
 title = {Reconstructing 3D Human Pose from 2D Image Landmarks},
 booktitle = {ECCV},
 year = {2012}
} 


@inproceedings{MODEC,
  author    = {Ben Sapp and
               Ben Taskar},
  title     = {MODEC:Multimodal Decomposable Models for Human Pose Estimation},
  booktitle = {CVPR},
  year      = {2013}
}


@article{Alpher04,
author = {A. Alpher and J.~P.~N. Fotheringham-Smythe and G. Gamow},
title = {Can a machine frobnicate?},
journal = {Journal of Foo},
volume = 14, 
number = 1, 
pages = {234--778}, 
year = 2004
}


  @article{Wang94representingmoving,
      author = {Y. A. Wang and H. Adelson},
      title = {Representing Moving Images with Layers},
      journal = {TIP},
      year = {1994},
  }

@article{10.1109/CVPR.1997.609375,
  author = {Yair Weiss},
  title = {Smoothness in Layers: Motion segmentation using nonparametric mixture estimation.},
  journal ={CVPR},
  year={1997},

  }
  
  @article{DBLP:journals/corr/SimonyanVZ13,
  author    = {Karen Simonyan and
               Andrea Vedaldi and
               Andrew Zisserman},
  title     = {Deep Inside Convolutional Networks: Visualising Image Classification
               Models and Saliency Maps},
  journal   = {CoRR},
  volume    = {abs/1312.6034},
  year      = {2013},
  ee        = {http://arxiv.org/abs/1312.6034},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

  @article{DBLP:journals/corr/GirshickDDM13,
  author    = {Ross B. Girshick and
               Jeff Donahue and
               Trevor Darrell and
               Jitendra Malik},
  title     = {Rich feature hierarchies for accurate object detection and
               semantic segmentation},
  journal   = {CoRR},
  volume    = {abs/1311.2524},
  year      = {2013},
  ee        = {http://arxiv.org/abs/1311.2524},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}
  
    @incollection{NIPS2012_0534,
    Title = {ImageNet Classification with Deep Convolutional Neural Networks},
    Booktitle = {NIPS},
    Author = {Alex Krizhevsky and Ilya Sutskever and Geoffrey E. Hinton},
      Year = {2012},
   } 

   @inproceedings{Zuffi:ICCV:2013,
  title = {Estimating Human Pose with Flowing Puppets},
  author = {Zuffi, Silvia and Romero, Javier and Schmid, Cordelia and Black, Michael J},
  booktitle = {IEEE International Conference on Computer Vision (ICCV)},
  pages = {3312-3319},
  year = {2013}
}


@article{DBLP:journals/corr/abs-2103-10429,
  author    = {Despoina Paschalidou and
               Angelos Katharopoulos and
               Andreas Geiger and
               Sanja Fidler},
  title     = {Neural Parts: Learning Expressive 3D Shape Abstractions with Invertible
               Neural Networks},
  journal   = {CoRR},
  volume    = {abs/2103.10429},
  year      = {2021},
  url       = {https://arxiv.org/abs/2103.10429},
  eprinttype = {arXiv},
  eprint    = {2103.10429},
  timestamp = {Wed, 24 Mar 2021 15:50:40 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2103-10429.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


  @inproceedings{DBLP:conf/eccv/VedaldiZ12,
  author    = {Andrea Vedaldi and
               Andrew Zisserman},
  title     = {Self-similar Sketch},
  booktitle = {ECCV (2)},
  year      = {2012},
  pages     = {87-100},
  ee        = {http://dx.doi.org/10.1007/978-3-642-33709-3_7},
  crossref  = {DBLP:conf/eccv/2012-2},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

  @inproceedings{RenMalik07,
	  author = "Xiaofeng Ren and Jitendra Malik",
	  title = "Tracking as Repeated Figure/Ground Segmentation",
	  booktitle = {CVPR},
	  year = "2007"
	  }

  @article{ncut,
  author = {Jianbo Shi and Jitendra Malik},
  title = {Normalized Cuts and Image Segmentation},
  journal = {TPAMI},
  year = {2000},
  }


  @article{10.1109/TPAMI.2005.202,
  author = {Jiangjian Xiao and Mubarak Shah},
  title = {Motion Layer Extraction in the Presence of Occlusion Using Graph Cuts},
  journal ={TPAMI},
  year = {2005},
  }

  @article{1340323,
  author = {Pawan Kumar, M. and Torr, P. H. and Zisserman, A.},
  title = {Learning Layered Motion Segmentations of Video},
  journal = {IJCV},
  volume = {76},
  year = {2008},
  }

  @article{10.1109/CVPR.1997.609375,
  author = {Yair Weiss},
  title = {Smoothness in Layers: Motion segmentation using nonparametric mixture estimation.},
  journal ={CVPR},
  year={1997},

  }
@inproceedings{DBLP:conf/eccv/FabletB02,
  author    = {Ronan Fablet and
               Michael J. Black},
  title     = {Automatic Detection and Tracking of Human Motion with a
               View-Based Representation},
  booktitle = {ECCV},
  year      = {2002}
}
@inproceedings{Shi_1994_3266,
   author = "Jianbo Shi and Carlo Tomasi",
   title = "Good Features to Track",
   booktitle = "CVPR",
   year = "1994",
}

@inproceedings{Rehg:1995:MTS:839277.840114,
 author = {Rehg, J. M. and Kanade, T.},
 title = {Model-based tracking of self-occluding articulated objects},
 booktitle = {ICCV},
 series = {ICCV},
 year = {1995},
}
@inproceedings{DBLP:conf/cvpr/FossatiDLF07,
  author    = {Andrea Fossati and
               Miodrag Dimitrijevic and
               Vincent Lepetit and
               Pascal Fua},
  title     = {Bridging the Gap between Detection and Tracking for 3D Monocular
               Video-Based Motion Capture},
  booktitle = {CVPR},
  year      = {2007},
  ee        = {http://dx.doi.org/10.1109/CVPR.2007.383297},
  crossref  = {DBLP:conf/cvpr/2007},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}
@inproceedings{DBLP:conf/eccv/SidenbladhBF00,
  author    = {Hedvig Sidenbladh and
               Michael J. Black and
               David J. Fleet},
  title     = {Stochastic Tracking of 3D Human Figures Using 2D Image Motion},
  booktitle = {ECCV},
  year      = {2000}
}



@inproceedings{HuayanWang:2011:MIR:2191740.2191905,
 author = {Huayan Wang and Koller, D.},
 title = {Multi-level inference by relaxed dual decomposition for human pose segmentation},
 booktitle = {CVPR},
 year = {2011}}



@INPROCEEDINGS{Johnson_combiningdiscriminative,
    author = {Sam Johnson and Mark Everingham},
    title = {Combining discriminative appearance and segmentation cues for articulated human pose estimation},
    booktitle = {MLVMA},
    year = {2009}
}


@INPROCEEDINGS{Sminchisescu05discriminativedensity,
    author = {Cristian Sminchisescu and Atul Kanaujia and Zhiguo Li and Dimitris Metaxas},
    title = {Discriminative Density Propagation for {3D} Human Motion Estimation},
    booktitle = {In CVPR},
    year = {2005}
}

@book{Gibson1979-GIBTEA,
	author = {James J. Gibson},
	publisher = {Houghton Mifflin},
	year = {1979},
	title = {The Ecological Approach to Visual Perception}
}

@INPROCEEDINGS{motionperception,
    author = {Gunnar Johansson},
    title = {Visual perception of biological motion and a model for its analysis},
    booktitle = {Percept. Psychophys.},
    year = {1973},
    volume={14},
    pages = {201--211}
}




@article{DBLP:journals/cacm/ShottonSKFFBCM13,
  author    = {Jamie Shotton and
               Toby Sharp and
               Alex Kipman and
               Andrew W. Fitzgibbon and
               Mark Finocchio and
               Andrew Blake and
               Mat Cook and
               Richard Moore},
  title     = {Real-time human pose recognition in parts from single depth
               images},
  journal   = {Commun. ACM},
  volume    = {56},
  number    = {1},
  year      = {2013},
  pages     = {116-124},
  ee        = {http://doi.acm.org/10.1145/2398356.2398381},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@article{10.1109/CVPR.2004.303,
author = {Jiang Gao and Robert T. Collins and Alexander G. Hauptmann and Howard D. Wactlar},
title = {Articulated Motion Modeling for Activity Analysis},
journal ={2012 IEEE Computer Society Conference on Computer Vision and Pattern Recognition Workshops},
volume = {1},
issn = {1063-6919},
year = {2004},
pages = {20},
doi = {http://doi.ieeecomputersociety.org/10.1109/CVPR.2004.303},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}


@INPROCEEDINGS{609381,
author={Black, M.J. and Yacoob, Y. and Jepson, A.D. and Fleet, D.J.},
booktitle={CVPR},
title={Learning parameterized models of image motion},
year={1997}}


@inproceedings{DBLP:conf/nips/WuBGBSSD02,
  author    = {Wei Wu and
               Michael J. Black and
               Yun Gao and
               Elie Bienenstock and
               Mijail Serruya and
               A. Shaikhouni and
               John P. Donoghue},
  title     = {Neural Decoding of Cursor Motion Using a Kalman Filter},
  booktitle = {NIPS},
  year      = {2002},
  pages     = {117-124},
  ee        = {http://books.nips.cc/papers/files/nips15/NS03.pdf},
  crossref  = {DBLP:conf/nips/2002},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


  @inproceedings{DBLP:conf/cvpr/AndrilukaRS08,
    author    = {Mykhaylo Andriluka and
		Stefan Roth and
		Bernt Schiele},
    title     = {People-tracking-by-detection and people-detection-by-tracking},
    booktitle = {CVPR},
    year      = {2008},
    ee        = {http://dx.doi.org/10.1109/CVPR.2008.4587583},
    crossref  = {DBLP:conf/cvpr/2008},
    bibsource = {DBLP, http://dblp.uni-trier.de}
  }
  @inproceedings{RenMalik07,
	  author = "Xiaofeng Ren and Jitendra Malik",
	  title = "Tracking as Repeated Figure/Ground Segmentation",
	  booktitle = {CVPR},
	  year = "2007"
	  }

  @article{ncut,
  author = {Jianbo Shi and Jitendra Malik},
  title = {Normalized Cuts and Image Segmentation},
  journal = {TPAMI},
  year = {2000},
  }
@inproceedings{DBLP:conf/cvpr/FragkiadakiZS12,
  author    = {Katerina Fragkiadaki and
               Geng Zhang and
               Jianbo Shi},
  title     = {Video segmentation by tracing discontinuities in a trajectory
               embedding},
  booktitle = {CVPR},
  year      = {2012}
}


  @article{10.1109/TPAMI.2005.202,
  author = {Jiangjian Xiao and Mubarak Shah},
  title = {Motion Layer Extraction in the Presence of Occlusion Using Graph Cuts},
  journal ={TPAMI},
  year = {2005},
  }

  @article{1340323,
  author = {Pawan Kumar, M. and Torr, P. H. and Zisserman, A.},
  title = {Learning Layered Motion Segmentations of Video},
  journal = {IJCV},
  volume = {76},
  year = {2008},
  }





  @InProceedings{Fradet09a,
    author = {Fradet, Matthieu and Robert, Philippe and P\'{e}rez, Patrick},
    Title = {Clustering point trajectories with various life-spans},
    BookTitle = {CVMP},
  year={2009}
  }





  @article{10.1109/ICCV.2001.10061,
  author = {Stella X. Yu and Jianbo Shi},
  title = {Segmentation with Pairwise Attraction and Repulsion},
  journal ={ICCV},
  Volume={75},
  year = {2001},
  }

  @article{1286005,
  author = {Wu, Bo and Nevatia, Ram},
  title = {Detection and Tracking of Multiple, Partially Occluded Humans by Bayesian Combination of Edgelet based Part Detectors},
  journal = {IJCV},
  year = {2007},
  }

  @inproceedings{bibbyeccv08,
    author = {C. Bibby and I. Reid},
    title = {Robust Real-Time Visual Tracking using Pixel-Wise Posteriors},
    booktitle={ECCV},
    year = "2008",
  }


  @InProceedings{BroxSegmentationCVPR11,
    author       = "Thomas Brox and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Object Segmentation by Alignment of Poselet Activations to Image Contours",
    booktitle    = "CVPR",
    year         = "2011"
  }

  @article{10.1109/ICCV.1995.466815,
  author = {J. Costeira and T. Kanade},
  title = {A multi-body factorization method for motion analysis},
  journal ={ICCV},
  year = {1995},
  }

  @inproceedings{Efros_2006_5395,
    author = "Bryan C. Russell and AlexeiA. Efros and Josef Sivic and William T. Freeman and Andrew Zisserman",
    title = "Using Multiple Segmentations to Discover Objects and their Extent in Image Collections",
    booktitle = "CVPR",
    year = "2006",
  }

  @inproceedings{malisiewicz-bmvc07,
    Author =	 {Tomasz Malisiewicz and Alexei A. Efros},
    Booktitle =	 {BMVC},
    Title =	 {Improving Spatial Support for Objects via Multiple Segmentations},
    Year =	 2007
  }

  @ARTICLE{1273918,
  author={Martin, D.R. and Fowlkes, C.C. and Malik, J.},
  journal={TPAMI},
  title={Learning to detect natural image boundaries using local brightness, color, and texture cues},
  year={2004},
  volume={26}
  }
@INPROCEEDINGS{Brox04highaccuracy,
    author = {Thomas Brox and Andrï¿œs Bruhn and Nils Papenberg and Joachim Weickert},
    title = {High Accuracy Optical Flow Estimation Based on a Theory for Warping},
    booktitle = {},
    year = {2004},
    pages = {25--36},
    publisher = {Springer}
}




  @INPROCEEDINGS{5539818,
  author={Bibby, C. and Reid, I.},
  booktitle={CVPR},
  title={Real-time tracking of multiple occluding objects using level sets},
  year={2010}}


  @inproceedings{Mitzel:2010:MTS:1886063.1886094,
  author = {Mitzel, Dennis and Horbert, Esther and Ess, Andreas and Leibe, Bastian},
  title = {Multi-person tracking with sparse detection and continuous segmentation},
  booktitle = {ECCV},
  year={2010}
  }

  @inproceedings{Mitzel:2011:MTS:1886063.1886094,
  author = {Mitzel, Dennis and Horbert, Esther and Ess, Andreas and Leibe, Bastian},
  title = {Level-Set Person Segmentation and Tracking with Multi-Region Appearemnce Models and Top-Down Shape Information},
  booktitle = {ICCV},
  series = {2011}
  }


  @InProceedings{lezama11,
    author = {Lezama, J. and Alahari, K. and Sivic, J. and Laptev, I.},
    title = {Track to the Future: Spatio-temporal Video Segmentation with Long-range Motion Cues},
    booktitle = {CVPR},
    year = {2011}
  }
  @InProceedings{shuwang2,
    author = {Shu Wang and Huchuan Lu and Fan Yang and Ming-Hsuan Yang},
    title = {Superpixel Tracking},
    booktitle = {ICCV},
    year = {2011}
  }
  @InProceedings{OB11,
    author       = "P. Ochs and T. Brox",
    title        = "Object segmentation in video: a hierarchical variational approach for turning point trajectories into dense regions",
    booktitle    = "ICCV",
    year         = "2011"}
  @incollection {springerlink:10.1007/978-3-642-15555-0_27,
    author = {Rahtu, Esa and Kannala, Juho and Salo, Mikko and Heikkilï¿œ, Janne},
    affiliation = {Machine Vision Group, University of Oulu, Finland},
    title = {Segmenting Salient Objects from Images and Videos},
    booktitle = {ECCV},
    year={2010},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }

  @Article{19146246,
  TITLE = {On the plausibility of the discriminant center-surround hypothesis for visual saliency.},
  AUTHOR = {Gao, Dashan and Mahadevan, Vijay and Vasconcelos, Nuno},
  journal = {Journal of vision},
  volume = {8},
  year = {2008}
  }


  @Article{Mahadevan10spatiotemporalsaliency,
      author = {Vijay Mahadevan and Nuno Vasconcelos},
      title = {Spatiotemporal Saliency in Dynamic Scenes},
      journal = {TPAMI},
      volume = {32},
      year = {2010},
  }

@article{DBLP:journals/corr/abs-1711-03129,
  author    = {Jiajun Wu and
               Yifan Wang and
               Tianfan Xue and
               Xingyuan Sun and
               William T. Freeman and
               Joshua B. Tenenbaum},
  title     = {MarrNet: 3D Shape Reconstruction via 2.5D Sketches},
  journal   = {CoRR},
  volume    = {abs/1711.03129},
  year      = {2017},
  url       = {http://arxiv.org/abs/1711.03129},
  archivePrefix = {arXiv},
  eprint    = {1711.03129},
  timestamp = {Fri, 01 Dec 2017 14:22:24 +0100},
  biburl    = {http://dblp.org/rec/bib/journals/corr/abs-1711-03129},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @InProceedings{background_subtraction_free_camera,
    author = {Yaser Sheikh, Omar Javed, and Takeo Kanade},
    title = {Background Subtraction for Freely Moving Cameras},
    booktitle = {ICCV},
    year = {2009},
  }
  @conference{vondrick2010,
    title={Efficiently Scaling Up Video Annotation with Crowdsourced Marketplaces},
    author={Carl Vondrick and Deva Ramanan and Donald Patterson},
    booktitle={ECCV},
    year = {2010},
  }

  @conference{StellaRepulsion,
      author = {Stella X. Yu and Jianbo Shi},
      title = {Understanding Popout through Repulsion},
      booktitle= {CVPR},
      year={2001},
  }

  @article{10.1109/TPAMI.2009.167,
  author = {Pedro F. Felzenszwalb and Ross B. Girshick and David McAllester and Deva Ramanan},
  title = {Object Detection with Discriminatively Trained Part-Based Models},
  journal ={TPAMI},
    year = {2010},
  volume={32},
  }

  @INPROCEEDINGS{Avidan05ensembletracking,
      author = {Shai Avidan},
      title = {Ensemble Tracking},
      booktitle = {CVPR},
      year = {2005},
  }

  @INPROCEEDINGS{planningtracking,
      author = {Haifeng Gong and Jack Simy and Maxim Likhachev and Jianbo Shi},
      title = {Multi-hypothesis Motion Planning for Visual Object Tracking},
      booktitle = {ICCV},
      year = {2011},
  }

  @incollection {SLIC,
    title={SLIC Superpixels},
    author={Radhakrishna Achanta and Appu Shaji and Kevin Smith and Aurelien Lucchi and Pascal Fua and Sabine Susstrunk},
    booktitle={EPFL Technical Report no. 149300, June 2010},
  }


@inproceedings{DBLP:conf/cvpr/UrtasunD08,
  author    = {Raquel Urtasun and
               Trevor Darrell},
  title     = {Sparse probabilistic regression for activity-independent
               human pose inference},
  booktitle = {CVPR},
  year      = {2008},
  ee        = {http://dx.doi.org/10.1109/CVPR.2008.4587360},
  crossref  = {DBLP:conf/cvpr/2008},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{DBLP:journals/pami/XuJM12,
  author    = {Li Xu and
               Jiaya Jia and
               Yasuyuki Matsushita},
  title     = {Motion Detail Preserving Optical Flow Estimation},
  journal   = {TPAMI},
  volume    = {34},
  year      = {2012},
}

  @incollection {springerlink:10.1007/978-3-540-88688-4_58,
    author = {Huang, Chang and Wu, Bo and Nevatia, Ramakant},
    title = {Robust Object Tracking by Hierarchical Association of Detection Responses},
    booktitle = {ECCV},
    year={2008},
  }
  
  @article{DBLP:journals/corr/RenHG015,
  author    = {Shaoqing Ren and
               Kaiming He and
               Ross B. Girshick and
               Jian Sun},
  title     = {Faster {R-CNN:} Towards Real-Time Object Detection with Region Proposal
               Networks},
  journal   = {CoRR},
  volume    = {abs/1506.01497},
  year      = {2015},
  url       = {http://arxiv.org/abs/1506.01497},
  timestamp = {Wed, 07 Jun 2017 14:42:40 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RenHG015},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @inproceedings{DBLP:conf/cvpr/CechS07,
    author    = {Jan Cech and Radim S{\'a}ra},
    title     = {Efficient Sampling of Disparity Space for Fast And Accurate Matching},
    booktitle = {CVPR},
    year      = {2007}
  }
  @inproceedings{DBLP:conf/iccv/PellegriniESG09,
    author    = {Stefano Pellegrini and
		Andreas Ess and
		Konrad Schindler and
		Luc J. Van Gool},
    title     = {You'll never walk alone: Modeling social behavior for multi-target
		tracking},
    booktitle = {ICCV},
    year      = {2009}
  }

@article{hindside,
  author    = {Marcin Andrychowicz and
               Filip Wolski and
               Alex Ray and
               Jonas Schneider and
               Rachel Fong and
               Peter Welinder and
               Bob McGrew and
               Josh Tobin and
               Pieter Abbeel and
               Wojciech Zaremba},
  title     = {Hindsight Experience Replay},
  journal   = {CoRR},
  volume    = {abs/1707.01495},
  year      = {2017},
  url       = {http://arxiv.org/abs/1707.01495},
  archivePrefix = {arXiv},
  eprint    = {1707.01495},
  timestamp = {Sat, 05 Aug 2017 14:56:09 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/AndrychowiczWRS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

  @InProceedings{eth_biwi_00483,
    author = {B. Leibe and N. Cornelis and K. Cornelis and L. Van Gool},
    title = {Dynamic 3D Scene Analysis from a Moving Vehicle},
    booktitle = {CVPR},
    year = {2007},
  }

  @article{10.1109/TPAMI.2010.143,
  author = {Thomas Brox and Jitendra Malik},
  title = {Large Displacement Optical Flow: Descriptor Matching in Variational Motion Estimation},
  journal ={TPAMI},
  year = {2010},
  }
  
  
  @article{DBLP:journals/corr/HeZRS15,
  author    = {Kaiming He and
               Xiangyu Zhang and
               Shaoqing Ren and
               Jian Sun},
  title     = {Deep Residual Learning for Image Recognition},
  journal   = {CoRR},
  volume    = {abs/1512.03385},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.03385},
  timestamp = {Wed, 07 Jun 2017 14:41:17 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/HeZRS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/SrivastavaLM17,
  author    = {Shashank Srivastava and
               Igor Labutov and
               Tom M. Mitchell},
  title     = {Joint Concept Learning and Semantic Parsing from Natural Language
               Explanations},
  booktitle = {Proceedings of the 2017 Conference on Empirical Methods in Natural
               Language Processing, {EMNLP} 2017, Copenhagen, Denmark, September
               9-11, 2017},
  pages     = {1528--1537},
  year      = {2017},
  crossref  = {DBLP:conf/emnlp/2017},
  url       = {http://aclanthology.info/papers/D17-1161/d17-1161},
  timestamp = {Fri, 15 Sep 2017 17:29:54 +0200},
  biburl    = {http://dblp.org/rec/bib/conf/emnlp/SrivastavaLM17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@Article{dm-elav-86, 
author = "Gerald Dejong and Raymond Mooney", 
year = "1986", 
title = "Explanation-Based Learning: An Alternative View", 
journal = "Machine Learning", 
volume = "1", 
pages = "145--176", 
publisher = "Kluwer", 
} 
Hide BibTex Record


@inproceedings{Perazzi2016,
  author = {F. Perazzi and J. Pont-Tuset and B. McWilliams and L. {Van Gool} and M. Gross and A. Sorkine-Hornung},
  title = {A Benchmark Dataset and Evaluation Methodology for Video Object Segmentation},
  booktitle = {Computer Vision and Pattern Recognition},
  year = {2016}
}
  
  @article{DBLP:journals/corr/HeGDG17,
  author    = {Kaiming He and
               Georgia Gkioxari and
               Piotr Doll{\'{a}}r and
               Ross B. Girshick},
  title     = {Mask {R-CNN}},
  journal   = {CoRR},
  volume    = {abs/1703.06870},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.06870},
  timestamp = {Wed, 07 Jun 2017 14:42:32 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/HeGDG17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @inproceedings{citeulike:9244127,
      author = {Li, Yuan and Huang, Chang and Nevatia, R.},
    booktitle = {CVPR},
      title = {Learning to associate: HybridBoosted multi-target tracker for crowded scene},
      year = {2009}
  }


@InProceedings{Johnson_2015_CVPR,
author = {Johnson, Justin and Krishna, Ranjay and Stark, Michael and Li, Li-Jia and Shamma, David and Bernstein, Michael and Fei-Fei, Li},
title = {Image Retrieval Using Scene Graphs},
booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2015}
}


@article{Hofsten19971799,
title = "Development of smooth pursuit tracking in young infants ",
journal = "Vision Research ",
volume = "37",
number = "13",
pages = "1799 - 1810",
year = "1997",
note = "",
issn = "0042-6989",
doi = "http://dx.doi.org/10.1016/S0042-6989(96)00332-X",
url = "http://www.sciencedirect.com/science/article/pii/S004269899600332X",
author = "Claes Von Hofsten and Kerstin Rosander",
keywords = "Eye movements",
keywords = "Infants",
keywords = "Smooth pursuit",
keywords = "Saccades",
keywords = "Head movements "
}


  @article {springerlink:10.1007/s11263-008-0136-6,
  title = {Particle Video: Long-Range Motion Estimation Using Point Trajectories},
    author = {Sand, Peter and Teller, Seth},
    affiliation = {MIT Computer Science and Artificial Intelligence Laboratory Cambridge MA 02139 USA},
    journal = {IJCV},
    year = {2008}
  }
  @INPROCEEDINGS{Dalal05histogramsof,
      author = {Navneet Dalal and Bill Triggs},
      title = {Histograms of Oriented Gradients for Human Detection},
      booktitle = {CVPR},
      year = {2005}
  }

  @InProceedings{yma,
    author = { Rao, S. and Tron, R. and Vidal, R. and Ma, Y. },
    title = {Motion segmentation via robust subspace separation in the presence of outlying, incomplete, or corrupted trajectories.},
    booktitle = {CVPR},
    year={2008},
  }
  
  

@inproceedings{Diuk:2008:ORE:1390156.1390187,
 author = {Diuk, Carlos and Cohen, Andre and Littman, Michael L.},
 title = {An Object-oriented Representation for Efficient Reinforcement Learning},
 booktitle = {Proceedings of the 25th International Conference on Machine Learning},
 series = {ICML '08},
 year = {2008},
 isbn = {978-1-60558-205-4},
 location = {Helsinki, Finland},
 pages = {240--247},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/1390156.1390187},
 doi = {10.1145/1390156.1390187},
 acmid = {1390187},
 publisher = {ACM},
 address = {New York, NY, USA},
} 


  
  @article{DBLP:journals/corr/abs-1708-04225,
  author    = {Coline Devin and
               Pieter Abbeel and
               Trevor Darrell and
               Sergey Levine},
  title     = {Deep Object-Centric Representations for Generalizable Robot Learning},
  journal   = {CoRR},
  volume    = {abs/1708.04225},
  year      = {2017},
  url       = {http://arxiv.org/abs/1708.04225},
  archivePrefix = {arXiv},
  eprint    = {1708.04225},
  timestamp = {Tue, 05 Sep 2017 10:03:46 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/abs-1708-04225},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}




  @inproceedings{Grabner:2008:SOB:1478392.1478414,
  author = {Grabner, Helmut and Leistner, Christian and Bischof, Horst},
  title = {Semi-supervised On-Line Boosting for Robust Tracking},
  booktitle = {ECCV},
  year = {2008},
  }


  @inproceedings{citeulike:2085974,
      author = {Grabner , H. and Bischof, H.},
    title = {Online Boosting and Vision},
      booktitle = {CVPR},
      year = {2006}
  }

  @INPROCEEDINGS{5573752,
  author={Zhang Tao and Fei Shumin and Hu Gang},
  booktitle={Control Conference (CCC)},
  title={Target tracking with particle filter based on multiple cues fusion},
  year={2010}}

  @INPROCEEDINGS{Okuma04aboosted,
      author = {Kenji Okuma and Ali Taleghani and Nando De Freitas and O De Freitas and James J. Little and David G. Lowe},
      title = {A Boosted Particle Filter: Multitarget Detection and Tracking},
      booktitle = {ECCV},
      year = {2004},
  }


  @InProceedings{sparsesubsp,
    author = {Elhamifar, E. and Vidal, R.},
    title = {Sparse subspace clustering},
    booktitle = {CVPR},
    year = {2009}
  }




  @INPROCEEDINGS{BrostowCipollaCVPR2006,
    AUTHOR       = {Gabriel J. Brostow and Roberto Cipolla},
    TITLE        = {Unsupervised Bayesian Detection of Independent Motion in Crowds},
    BOOKTITLE    = {CVPR},
    YEAR         = {2006},
  }
  @article{GrundmannKwatra2010,
    author = {Matthias Grundmann and Vivek Kwatra and Mei Han and Irfan Essa},
    title = {Efficient Hierarchical Graph Based Video Segmentation},
    journal = {CVPR},
    year = {2010},
  }



  @incollection {mhvs,
    author = {Amelio Vazquez-Reina and Shai Avidan and Hanspeter Pfister and Eric Miller},
    title = {Multiple Hypothesis Video Segmentation from Superpixel Flows},
    booktitle = {ECCV},
  year={2010},
  }



  @article{phycho,
    author = {H. C. Nothdurft},
    title = {Feature analysis and the role of similarity in preattentive vision},
    journal = {Perception and Psychophysics},
    volume={52},
    year = {1992},
  }




  @INPROCEEDINGS{5206727,
  author={Chunhui Gu and Lim, J.J. and Arbelaez, P. and Malik, J.},
  booktitle={CVPR},
  year={2009},
  title={Recognition using regions},
  }
  @InProceedings{citeulike:942103,
      title = {Bottom-up/top-down image parsing by attribute graph grammar},
      author = {Han, Feng and Zhu, Song-Chun},
      journal = {ICCV},
  year={ 2005},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {CVPR},
  year={2009},
  }
@InProceedings{eth_biwi_00555,
  author = {S. Gammeter and A. Ess and T. Jaeggli and K. Schindler and B. Leibe and and L. van Gool},
  title = {Articulated Multibody Tracking Under Egomotion},
  booktitle = {ECCV},
  year = {2008}
}


@INPROCEEDINGS{unified,
author={Xiangyang Lan and Huttenlocher, D.P.},
booktitle={CVPR},
title={A unified spatio-temporal articulated model for tracking},
year={2004},
volume={1}}


  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }

  @InProceedings{Yan06general,
    title     = {A General Framework for Motion Segmentation: Independent, Articulated, Rigid, Non-rigid, Degenerate and Non-degenerate.},
    author = {J. Yan and M. Pollefeys},
    booktitle = {ECCV},
  year={ 2006},
  }

  @InProceedings{Ayer,
    title     = {Layered representation of motion video using robust maximum-likelihood estimation of mixture models and MDL encoding},
    author = {S. Ayer and H. S. Sawhney},
    booktitle = {ICCV},
  year={ 1995},
  }

  @article{10.1109/CVPR.2005.335,
  author = {Deva Ramanan and D. A. Forsyth and Andrew Zisserman},
  title = {Strike a Pose: Tracking People by Finding Stylized Poses},
  journal ={CVPR},
  year = {2005},
  }
  
  @article{citeulike:13375196,
    author = {Tompson, Jonathan and Stein, Murphy and Lecun, Yann and Perlin, Ken},
    journal = {ACM Trans. Graph.},
    title = {{Real-Time Continuous Pose Recovery of Human Hands Using Convolutional Networks}},
    year = {2014}
}



  @inproceedings{DBLP:conf/nips/TompsonJLB14,
  author    = {Jonathan J. Tompson and
               Arjun Jain and
               Yann LeCun and
               Christoph Bregler},
  title     = {Joint Training of a Convolutional Network and a Graphical Model for
               Human Pose Estimation},
  booktitle = {NIPS},
  year      = {2014}
  }
  
  @inproceedings{Sapp:2010:CMA:1888028.1888060,
 author = {Sapp, Benjamin and Toshev, Alexander and Taskar, Ben},
 title = {Cascaded Models for Articulated Pose Estimation},
 booktitle = {Proceedings of the 11th European Conference on Computer Vision: Part II},
 series = {ECCV'10},
 year = {2010},
 isbn = {3-642-15551-0, 978-3-642-15551-2},
 location = {Heraklion, Crete, Greece},
 pages = {406--420},
 numpages = {15},
 url = {http://dl.acm.org/citation.cfm?id=1888028.1888060},
 acmid = {1888060},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 
  
  
  
@article{DBLP:journals/corr/ToshevS13,
  author    = {Alexander Toshev and
               Christian Szegedy},
  title     = {DeepPose: Human Pose Estimation via Deep Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1312.4659},
  year      = {2013},
  ee        = {http://arxiv.org/abs/1312.4659},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}



  @inproceedings{DBLP:conf/eccv/SappTT10,
  author    = {Benjamin Sapp and
               Alexander Toshev and
               Ben Taskar},
  title     = {Cascaded Models for Articulated Pose Estimation},
  booktitle = {ECCV (2)},
  year      = {2010},
  pages     = {406-420},
  ee        = {http://dx.doi.org/10.1007/978-3-642-15552-9_30},
  crossref  = {DBLP:conf/eccv/2010-2},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{10.1109/TPAMI.2008.35,
author = {Mun Wai Lee and Ramakant Nevatia},
title = {Human Pose Tracking in Monocular Sequence Using Multilevel Structured Models},
journal ={IEEE Transactions on Pattern Analysis and Machine Intelligence},
volume = {31},
number = {1},
issn = {0162-8828},
year = {2009},
pages = {27-38},
doi = {http://doi.ieeecomputersociety.org/10.1109/TPAMI.2008.35},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}



@inproceedings{tellex11,
  address = {San Francisco, CA},
  author = {Stefanie Tellex and Thomas Kollar and Steven Dickerson and Matthew R. Walter and Ashish G. Banerjee and Seth Teller and Nicholas Roy},
  booktitle = {Proceedings of the National Conference on Artificial Intelligence (AAAI)},
  month = {August},
  pages = {1507--1514},
  title = {Understanding Natural Language Commands for Robotic Navigation and Mobile Manipulation},
  year = {2011},
}




  @inproceedings{DBLP:conf/iccv/CheriyadatR09,
    author    = {Anil Cheriyadat and
		Richard J. Radke},
    title     = {Non-negative matrix factorization of partial track data
		for motion segmentation},
    booktitle = {ICCV},
    year      = {2009}
  }

@inproceedings{Kuo:2015:DLO:2919332.2919793,
 author = {Kuo, Weicheng and Hariharan, Bharath and Malik, Jitendra},
 title = {DeepBox: Learning Objectness with Convolutional Networks},
 booktitle = {Proceedings of the 2015 IEEE International Conference on Computer Vision (ICCV)},
 series = {ICCV '15},
 year = {2015},
 isbn = {978-1-4673-8391-2},
 pages = {2479--2487},
 numpages = {9},
 url = {http://dx.doi.org/10.1109/ICCV.2015.285},
 doi = {10.1109/ICCV.2015.285},
 acmid = {2919793},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
} 



@Inbook{Xiang2016,
author="Xiang, Yu
and Kim, Wonhui
and Chen, Wei
and Ji, Jingwei
and Choy, Christopher
and Su, Hao
and Mottaghi, Roozbeh
and Guibas, Leonidas
and Savarese, Silvio",
editor="Leibe, Bastian
and Matas, Jiri
and Sebe, Nicu
and Welling, Max",
title="ObjectNet3D: A Large Scale Database for 3D Object Recognition",
bookTitle="Computer Vision -- ECCV 2016: 14th European Conference, Amsterdam, The Netherlands, October 11-14, 2016, Proceedings, Part VIII",
year="2016",
publisher="Springer International Publishing",
address="Cham",
pages="160--176",
abstract="We contribute a large scale database for 3D object recognition, named ObjectNet3D, that consists of 100 categories, 90,127 images, 201,888 objects in these images and 44,147 3D shapes. Objects in the 2D images in our database are aligned with the 3D shapes, and the alignment provides both accurate 3D pose annotation and the closest 3D shape annotation for each 2D object. Consequently, our database is useful for recognizing the 3D pose and 3D shape of objects from 2D images. We also provide baseline experiments on four tasks: region proposal generation, 2D object detection, joint 2D detection and 3D object pose estimation, and image-based 3D shape retrieval, which can serve as baselines for future research using our database. Our database is available online at                     http://cvgl.stanford.edu/projects/objectnet3d                                      .",
isbn="978-3-319-46484-8",
doi="10.1007/978-3-319-46484-8_10",
url="https://doi.org/10.1007/978-3-319-46484-8_10"
}

@Inbook{Kuettel2012,
author="Kuettel, Daniel
and Guillaumin, Matthieu
and Ferrari, Vittorio",
editor="Fitzgibbon, Andrew
and Lazebnik, Svetlana
and Perona, Pietro
and Sato, Yoichi
and Schmid, Cordelia",
title="Segmentation Propagation in ImageNet",
bookTitle="Computer Vision -- ECCV 2012: 12th European Conference on Computer Vision, Florence, Italy, October 7-13, 2012, Proceedings, Part VII",
year="2012",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="459--473",
abstract="ImageNet is a large-scale hierarchical database of object classes. We propose to automatically populate it with pixelwise segmentations, by leveraging existing manual annotations in the form of class labels and bounding-boxes. The key idea is to recursively exploit images segmented so far to guide the segmentation of new images. At each stage this propagation process expands into the images which are easiest to segment at that point in time, e.g. by moving to the semantically most related classes to those segmented so far. The propagation of segmentation occurs both (a) at the image level, by transferring existing segmentations to estimate the probability of a pixel to be foreground, and (b) at the class level, by jointly segmenting images of the same class and by importing the appearance models of classes that are already segmented. Through an experiment on 577 classes and 500k images we show that our technique (i) annotates a wide range of classes with accurate segmentations; (ii) effectively exploits the hierarchical structure of ImageNet; (iii) scales efficiently; (iv) outperforms a baseline GrabCut [1] initialized on the image center, as well as our recent segmentation transfer technique [2] on which this paper is based. Moreover, our method also delivers state-of-the-art results on the recent iCoseg dataset for co-segmentation.",
isbn="978-3-642-33786-4",
doi="10.1007/978-3-642-33786-4_34",
url="https://doi.org/10.1007/978-3-642-33786-4_34"
}


@article{DBLP:journals/corr/SukhbaatarSWF15,
  author    = {Sainbayar Sukhbaatar and
               Arthur Szlam and
               Jason Weston and
               Rob Fergus},
  title     = {Weakly Supervised Memory Networks},
  journal   = {CoRR},
  volume    = {abs/1503.08895},
  year      = {2015},
  url       = {http://arxiv.org/abs/1503.08895},
  archivePrefix = {arXiv},
  eprint    = {1503.08895},
  timestamp = {Wed, 07 Jun 2017 14:40:08 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/SukhbaatarSWF15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/AndorAWSPGPC16,
  author    = {Daniel Andor and
               Chris Alberti and
               David Weiss and
               Aliaksei Severyn and
               Alessandro Presta and
               Kuzman Ganchev and
               Slav Petrov and
               Michael Collins},
  title     = {Globally Normalized Transition-Based Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1603.06042},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.06042},
  archivePrefix = {arXiv},
  eprint    = {1603.06042},
  timestamp = {Wed, 07 Jun 2017 14:42:37 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/AndorAWSPGPC16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/SwayamdiptaBDS16,
  author    = {Swabha Swayamdipta and
               Miguel Ballesteros and
               Chris Dyer and
               Noah A. Smith},
  title     = {Greedy, Joint Syntactic-Semantic Parsing with Stack LSTMs},
  journal   = {CoRR},
  volume    = {abs/1606.08954},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.08954},
  archivePrefix = {arXiv},
  eprint    = {1606.08954},
  timestamp = {Wed, 07 Jun 2017 14:40:31 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/SwayamdiptaBDS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{DBLP:journals/corr/TaiSM15,
  author    = {Kai Sheng Tai and
               Richard Socher and
               Christopher D. Manning},
  title     = {Improved Semantic Representations From Tree-Structured Long Short-Term
               Memory Networks},
  journal   = {CoRR},
  volume    = {abs/1503.00075},
  year      = {2015},
  url       = {http://arxiv.org/abs/1503.00075},
  archivePrefix = {arXiv},
  eprint    = {1503.00075},
  timestamp = {Wed, 07 Jun 2017 14:43:13 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/TaiSM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Krishnamurthy2014JointSA,
  title={Joint Syntactic and Semantic Parsing with Combinatory Categorial Grammar},
  author={Jayant Krishnamurthy and Tom M. Mitchell},
  booktitle={ACL},
  year={2014}
}

@inproceedings{AAA,
author = {Socher, Richard and Bauer, John and Manning, Christoper and Andrew Y., Ng},
year = {2013},
month = {08},
pages = {455-465},
title = {Parsing with Compositional Vector Grammars},
volume = {1},
booktitle = {ACL 2013 - 51st Annual Meeting of the Association for Computational Linguistics, Proceedings of the Conference}
}



@article{Bahdanau2014NeuralMT,
  title={Neural Machine Translation by Jointly Learning to Align and Translate},
  author={Dzmitry Bahdanau and Kyunghyun Cho and Yoshua Bengio},
  journal={CoRR},
  year={2014},
  volume={abs/1409.0473}
}


@article{DBLP:journals/corr/DosovitskiyK16,
  author    = {Alexey Dosovitskiy and
               Vladlen Koltun},
  title     = {Learning to Act by Predicting the Future},
  journal   = {CoRR},
  volume    = {abs/1611.01779},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.01779},
  archivePrefix = {arXiv},
  eprint    = {1611.01779},
  timestamp = {Wed, 07 Jun 2017 14:43:00 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/DosovitskiyK16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/LevinePKQ16,
  author    = {Sergey Levine and
               Peter Pastor and
               Alex Krizhevsky and
               Deirdre Quillen},
  title     = {Learning Hand-Eye Coordination for Robotic Grasping with Deep Learning
               and Large-Scale Data Collection},
  journal   = {CoRR},
  volume    = {abs/1603.02199},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.02199},
  archivePrefix = {arXiv},
  eprint    = {1603.02199},
  timestamp = {Wed, 07 Jun 2017 14:41:34 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LevinePKQ16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@INPROCEEDINGS{1544874, 
author={E. B. Sudderth and A. Torralba and W. T. Freeman and A. S. Willsky}, 
booktitle={Tenth IEEE International Conference on Computer Vision (ICCV'05) Volume 1}, 
title={Learning hierarchical models of scenes, objects, and parts}, 
year={2005}, 
volume={2}, 
pages={1331-1338 Vol. 2}, 
keywords={feature extraction;natural scenes;object detection;object recognition;feature detection;hierarchical probabilistic model;image database;low-level interest operator;natural scenes;object centered coordinate frame;object detection;object recognition;Computer science;Computer vision;Dictionaries;Graphical models;Image databases;Layout;Object detection;Random variables;Spatial databases;Visual databases}, 
doi={10.1109/ICCV.2005.137}, 
ISSN={1550-5499}, 
month={Oct},}



@INPROCEEDINGS{Carlson10towardan,
    author = {Andrew Carlson and Justin Betteridge and Bryan Kisiel and Burr Settles and Estevam R. Hruschka and Tom M. Mitchell},
    title = {Toward an architecture for never-ending language learning},
    booktitle = {In AAAI},
    year = {2010}
}


@INPROCEEDINGS{6751285, 
author={X. Chen and A. Shrivastava and A. Gupta}, 
booktitle={2013 IEEE International Conference on Computer Vision}, 
title={NEIL: Extracting Visual Knowledge from Web Data}, 
year={2013}, 
pages={1409-1416}, 
keywords={Internet;knowledge acquisition;NEIL;Web data;common sense relationships;never ending image learner;semi-supervised learning algorithm;visual knowledge extraction;Computers;Data mining;Detectors;Knowledge based systems;Semantics;Semisupervised learning;Visualization;attributes;common sense relationships;macro vision;never ending learning;object detection;scene classification;semi-supervised learning;visual knowledge base}, 
doi={10.1109/ICCV.2013.178}, 
ISSN={1550-5499}, 
month={Dec},}



  @Article{ Perse2009612,
  title = "A trajectory-based analysis of coordinated team activity in a basketball game",
  journal = "Computer Vision and Image Understanding",
  volume = "113",
  year = "2009",
  }

  @inproceedings{morariu11eventstructure,
    author    = {Vlad I. Morariu and Larry S. Davis},
    title     = {Multi-agent event recognition in structured scenarios.},
    booktitle = {CVPR},
    year      = {2011}
  }


  @inproceedings{storyline,
    author    = {Abhinav Gupta and Praveen Srinivasan and Jianbo Shi and Larry S. Davis},
    title     = {Understanding videos, constructing plots learning a visually grounded storyline model from annotated videos},
    booktitle = {CVPR},
    year      = {2009}
  }

  @inproceedings{benfold2011stable,
	  author = {Benfold, Ben and Reid, Ian},
	  title = {Stable Multi-Target Tracking in Real-Time Surveillance Video},
	  booktitle = {CVPR},
	  year = {2011}
  }


  @ARTICLE{790429,
  author={Wilson, A.D. and Bobick, A.F.},
  journal={TPAMI},
  title={Parametric hidden Markov models for gesture recognition},
  year={1999},
  volume={21}
  }



  @article{experts,
  author = {Terence D. Sanger and Robert A. Jacobs and Steven J. Nowlan and Geoffrey E. Hinton},
  title = {Adaptive Mixtures of Local Experts},
  journal = {Neural Computation},
  volume = {3},
  year = {1991}
  }


  @INPROCEEDINGS{lips,
  author={Bregler, C. and Omohundro, S.M.},
  booktitle={ICCV},
  title={Nonlinear manifold learning for visual speech recognition},
  year={1995}
  }



  @inproceedings{BN,
  author = {Shaogang Gong and Tao Xiang},
  title = {Recognition of Group Activities using Dynamic Probabilistic Networks},
  booktitle = {ICCV},
  year={2003}
  }


  @article{HMMMO,
  author = {Aaron F. Bobick and Andrew D. Wilson},
  title = {A State-Based Approach to the Representation and Recognition of Gesture},
  journal = {TPAMI},
  volume = {19}
  }

  @inproceedings{Brand:1997:CHM:794189.794420,
  author = {Brand, M. and Oliver, N. and Pentland, A.},
  title = {Coupled hidden Markov models for complex action recognition},
  booktitle = {CVPR},
  year = {1997}
  }

  @article{Ghahramani:1997:FHM:274158.274165,
  author = {Ghahramani, Zoubin and Jordan, Michael I.},
  title = {Factorial Hidden Markov Models},
  journal = {Mach. Learn.},
  volume = {29},
  year = {1997}
  }


  @INPROCEEDINGS{4270099,
  author={Laxton, B. and Jongwoo Lim and Kriegman, D.},
  booktitle={CVPR},
  title={Leveraging temporal, contextual and ordering constraints for recognizing complex activities in video},
  year={2007}
  }


  @article{DBLP:journals/jmlr/SiracusaF09,
    author    = {Michael Siracusa and John Fisher},
    title     = {Tractable Bayesian Inference of Time-Series Dependence Structure},
    journal   = {Journal of Machine Learning Research - Proceedings Track},
    volume    = {5},
    year      = {2009}
  }



  @article{parametrized,
  author = {Yaser Yacoob and Michael J. Black},
  title = {Parameterized Modeling and Recognition of Activities},
  journal = {Computer Vision and Image Understanding},
  volume = {73},
  year = {1999}
  }




  @inproceedings{Bobick:1995:STS:839277.840051,
  author = {Bobick, A. F. and Wilson, A. D.},
  title = {A state-based technique for the summarization and recognition of gesture},
  booktitle = {ICCV},
  year = {1995}
  }


  @inproceedings{Niebles:2010:MTS:1888028.1888059,
  author = {Niebles, Juan Carlos and Chen, Chih-Wei and Fei-Fei, Li},
  title = {Modeling temporal structure of decomposable motion segments for activity classification},
  booktitle = {ECCV},
  year = {2010}
  }



  @inproceedings{NCA,
  author = {Jacob Goldberger and Sam T. Roweis and Geoffrey E. Hinton and Ruslan Salakhutdinov},
  title = {Neighbourhood Components Analysis},
  booktitle = {Neural Information Processing Systems},
  year = {2004}
  }

  @article{Hakeem:2007:LDR:1265999.1266287,
  author = {Hakeem, Asaad and Shah, Mubarak},
  title = {Learning, detection and representation of multi-agent events in videos},
  journal = {Artif. Intell.},
  volume = {171},
  year = {2007}
  }



  @INPROCEEDINGS{Zelnik-manor01event-basedanalysis,
      author = {Lihi Zelnik-manor and Michal Irani},
      title = {Event-based analysis of video},
      booktitle = {CVPR},
      year = {2001}
  }

  @inproceedings{Jebara:2007:SCE:1421665.1421685,
  author = {Jebara, Tony and Song, Yingbo and Thadani, Kapil},
  title = {Spectral Clustering and Embedding with Hidden Markov Models},
  booktitle = {European conference on Machine Learning},
  year = {2007}
  }
  @article{10.1109/CVPR.1997.609375,
  author = {Yair Weiss},
  title = {Smoothness in Layers: Motion segmentation using nonparametric mixture estimation.},
  journal ={CVPR},
  year={1997},

  }

  @article{ncut,
  author = {Jianbo Shi and Jitendra Malik},
  title = {Normalized Cuts and Image Segmentation},
  journal = {TPAMI},
  year = {2000},
  }


  @article{10.1109/TPAMI.2005.202,
  author = {Jiangjian Xiao and Mubarak Shah},
  title = {Motion Layer Extraction in the Presence of Occlusion Using Graph Cuts},
  journal ={TPAMI},
  year = {2005},
  }

  @article{1340323,
  author = {Pawan Kumar, M. and Torr, P. H. and Zisserman, A.},
  title = {Learning Layered Motion Segmentations of Video},
  journal = {IJCV},
  volume = {76},
  year = {2008},
  }



  @ARTICLE{Wang94representingmoving,
      author = {Y. A. Wang and H. Adelson},
      title = {Representing Moving Images with Layers},
      journal = {TIP},
      year = {1994},
  }

  @InProceedings{Fradet09a,
    author = {Fradet, Matthieu and Robert, Philippe and P\'{e}rez, Patrick},
    Title = {Clustering point trajectories with various life-spans},
    BookTitle = {CVMP},
  year={2009}
  }





  @article{10.1109/ICCV.2001.10061,
  author = {Stella X. Yu and Jianbo Shi},
  title = {Segmentation with Pairwise Attraction and Repulsion},
  journal ={ICCV},
  Volume={75},
  year = {2001},
  }

  @article{1286005,
  author = {Wu, Bo and Nevatia, Ram},
  title = {Detection and Tracking of Multiple, Partially Occluded Humans by Bayesian Combination of Edgelet based Part Detectors},
  journal = {IJCV},
  year = {2007},
  }


  @inproceedings{DBLP:conf/iccv/CheriyadatR09,
    author    = {Anil Cheriyadat and
		Richard J. Radke},
    title     = {Non-negative matrix factorization of partial track data
		for motion segmentation},
    booktitle = {ICCV},
    year      = {2009},
    pages     = {865-872},
    ee        = {http://dx.doi.org/10.1109/ICCV.2009.5459311},
    crossref  = {DBLP:conf/iccv/2009},
    bibsource = {DBLP, http://dblp.uni-trier.de}
  }

  @article{Canny86,
      author = {Canny, J.},
      journal = {TPAMI},
      title = {{A Computational Approach to Edge Detection}},
      url = {http://dx.doi.org/10.1109/TPAMI.1986.4767851},
      volume = {PAMI-8},
      year = {1986}
  }

  @article{10.1109/ICCV.1995.466815,
  author = {J. Costeira and T. Kanade},
  title = {A multi-body factorization method for motion analysis},
  journal ={ICCV},
  year = {1995},
  }

  @ARTICLE{1273918,
  author={Martin, D.R. and Fowlkes, C.C. and Malik, J.},
  journal={TPAMI},
  title={Learning to detect natural image boundaries using local brightness, color, and texture cues},
  year={2004},
  volume={26}
  }

  @INPROCEEDINGS{139492,
  author={Perona, P. and Malik, J.},
  booktitle={ICCV},
  title={Detecting and localizing edges composed of steps, peaks and roofs },
  year={1990}
  }

  @incollection {springerlink:10.1007/978-3-642-15555-0_21,
    author = {Brox, Thomas and Malik, Jitendra},
    affiliation = {University of California at Berkeley},
    title = {Object Segmentation by Long Term Analysis of Point Trajectories},
    booktitle = {ECCV},
    year={2010}
  }

  @incollection {springerlink:10.1007/978-3-642-15555-0_27,
    author = {Rahtu, Esa and Kannala, Juho and Salo, Mikko and Heikkilï¿œ, Janne},
    affiliation = {Machine Vision Group, University of Oulu, Finland},
    title = {Segmenting Salient Objects from Images and Videos},
    booktitle = {ECCV},
    year={2010},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }

  @Article{19146246,
  TITLE = {On the plausibility of the discriminant center-surround hypothesis for visual saliency.},
  AUTHOR = {Gao, Dashan and Mahadevan, Vijay and Vasconcelos, Nuno},
  journal = {Journal of vision},
  volume = {8},
  year = {2008}
  }


  @Article{Mahadevan10spatiotemporalsaliency,
      author = {Vijay Mahadevan and Nuno Vasconcelos},
      title = {Spatiotemporal Saliency in Dynamic Scenes},
      journal = {TPAMI},
      volume = {32},
      year = {2010},
  }


  @InProceedings{background_subtraction_free_camera,
    author = {Yaser Sheikh, Omar Javed, and Takeo Kanade},
    title = {Background Subtraction for Freely Moving Cameras},
    booktitle = {ICCV},
    year = {2009},
  }
  @conference{vondrick2010,
    title={Efficiently Scaling Up Video Annotation with Crowdsourced Marketplaces},
    author={Carl Vondrick and Deva Ramanan and Donald Patterson},
    booktitle={ECCV},
    year = {2010},
  }

@article{DBLP:journals/corr/PatrauceanHC15,
  author    = {Viorica Patraucean and
               Ankur Handa and
               Roberto Cipolla},
  title     = {Spatio-temporal video autoencoder with differentiable memory},
  journal   = {CoRR},
  volume    = {abs/1511.06309},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.06309},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/PatrauceanHC15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @conference{StellaRepulsion,
      author = {Stella X. Yu and Jianbo Shi},
      title = {Understanding Popout through Repulsion},
      booktitle= {CVPR},
      year={2001},
  }

  @article{10.1109/TPAMI.2009.167,
  author = {Pedro F. Felzenszwalb and Ross B. Girshick and David McAllester and Deva Ramanan},
  title = {Object Detection with Discriminatively Trained Part-Based Models},
  journal ={TPAMI},
    year = {2010},
  volume={32},
  }

  @inproceedings{Datta_2008_6037,
   author = "Ankur Datta and Yaser Ajmal Sheikh and Takeo Kanade",
   title = "Linear Motion Estimation for Systems of Articulated Planes",
   booktitle = "CVPR",
   month = "June",
   year = "2008",
}

@inproceedings{DBLP:conf/cvpr/FragkiadakiHS13,
  author    = {Katerina Fragkiadaki and
               Han Hu and
               Jianbo Shi},
  title     = {Pose from Flow and Flow from Pose},
  booktitle = {CVPR},
  year      = {2013},
}

@inproceedings{DBLP:conf/cvpr/LadickyTZ13,
  author    = {Lubor Ladicky and
               Philip H. S. Torr and
               Andrew Zisserman},
  title     = {Human Pose Estimation Using a Joint Pixel-wise and Part-wise
               Formulation},
  booktitle = {CVPR},
  year      = {2013}
}

@inproceedings{Zuffi:ICCV:2013,
  title = {Estimating Human Pose with Flowing Puppets},
  author = {Zuffi, Silvia and Romero, Javier and Schmid, Cordelia and Black, Michael J},
  booktitle = {ICCV},
   year = {2013}
}

@ARTICLE{1542030,
author={Agarwal, A. and Triggs, B.},
journal={Pattern Analysis and Machine Intelligence, IEEE Transactions on}, title={Recovering 3D human pose from monocular images},
year={2006},
volume={28},
number={1},
pages={44-58},
keywords={computer vision;image motion analysis;image sequences;learning (artificial intelligence);regression analysis;support vector machines;3D human pose;histogram-of-shape-contexts descriptors;human motion estimation;image silhouettes;learning-based method;monocular image sequences;nonlinear regression;relevance vector machine regression;ridge regression;shape descriptor vectors;silhouette shape;support vector machine regression;Biological system modeling;Humans;Image segmentation;Image sequences;Kernel;Labeling;Learning systems;Robustness;Shape;Support vector machines;Index Terms- Computer vision;human motion estimation;machine learning;multivariate regression.;Algorithms;Artificial Intelligence;Humans;Image Interpretation, Computer-Assisted;Imaging, Three-Dimensional;Joints;Pattern Recognition, Automated;Photography;Posture;Reproducibility of Results;Sensitivity and Specificity;Subtraction Technique},
doi={10.1109/TPAMI.2006.21},
ISSN={0162-8828},}



@inproceedings {420,
	title = {Monocular 3D Pose Estimation and Tracking by Detection},
	booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	year = {2010},
	month = {06/2010},
	address = {San Francisco, USA},
	author = {Mykhaylo Andriluka and Stefan Roth and Schiele, Bernt}
}

@inproceedings{DBLP:conf/cvpr/PirsiavashR12,
  author    = {Hamed Pirsiavash and
               Deva Ramanan},
  title     = {Detecting activities of daily living in first-person camera
               views},
  booktitle = {CVPR},
  year      = {2012},
  pages     = {2847-2854},
  ee        = {http://doi.ieeecomputersociety.org/10.1109/CVPR.2012.6248010},
  crossref  = {DBLP:conf/cvpr/2012},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@inproceedings{Sun:CVPR:10,
  title = {Secrets of optical flow estimation and their principles},
  author = {Sun, D. and Roth, S. and Black, M. J.},
  booktitle = {CVPR},
  year = {2010}
}



@inproceedings{DBLP:conf/eccv/DesaiR12,
  author    = {Chaitanya Desai and
               Deva Ramanan},
  title     = {Detecting Actions, Poses, and Objects with Relational Phraselets},
  booktitle = {ECCV},
  year      = {2012}
}


@INPROCEEDINGS{Sigal06measurelocally,
    author = {Leonid Sigal and Michael J. Black},
    title = {Measure locally, reason globally: Occlusion-sensitive articulated pose estimation},
    booktitle = {CVPR},
    year = {2006}
}

@article{DBLP:journals/pami/Memisevic13,
  author    = {Roland Memisevic},
  title     = {Learning to Relate Images},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {35},
  number    = {8},
  pages     = {1829--1846},
  year      = {2013},
  url       = {http://doi.ieeecomputersociety.org/10.1109/TPAMI.2013.53},
  doi       = {10.1109/TPAMI.2013.53},
  timestamp = {Tue, 25 Jun 2013 20:04:57 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/pami/Memisevic13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@incollection{springerlink:10.1007/978-3-642-15549-9_17,
    author = {Eichner, Marcin and Ferrari, Vittorio},
    booktitle = {ECCV},
    title = {{We Are Family: Joint Pose Estimation of Multiple Persons}},
    year = {2010}
}


@inproceedings{DBLP:conf/nips/MichalskiMK14,
  author    = {Vincent Michalski and
               Roland Memisevic and
               Kishore Reddy Konda},
  title     = {Modeling Deep Temporal Dependencies with Recurrent Grammar Cells""},
  booktitle = {Advances in Neural Information Processing Systems 27: Annual Conference
               on Neural Information Processing Systems 2014, December 8-13 2014,
               Montreal, Quebec, Canada},
  pages     = {1925--1933},
  year      = {2014},
  crossref  = {DBLP:conf/nips/2014},
  url       = {http://papers.nips.cc/paper/5549-modeling-deep-temporal-dependencies-with-recurrent-grammar-cells},
  timestamp = {Wed, 10 Dec 2014 21:34:12 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/nips/MichalskiMK14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@INCOLLECTION{ferrariprogressive,
author = {V. Ferrari and M.J. MarÃ­n-JimÃ©nez and A. Zisserman},
title = {{2D} Human Pose Estimation in {TV} Shows},
booktitle = {Statistical and Geometrical Approaches to Visual Motion Analysis},
year = {2009}}
@inproceedings{pressigout:inria-00351874,
    hal_id = {inria-00351874},
    url = {http://hal.inria.fr/inria-00351874},
    title = {{Hybrid tracking approach using optical flow and pose estimation}},
    author = {Pressigout, Muriel and Marchand, Eric and Memin, Etienne},
    abstract = {{This paper proposes an hybrid approach to estimate the 3D pose of an object. The integration of texture information based on image intensities in a more classical non-linear edge-based pose estimation computation has proven to highly increase the reliability of the tracker. We propose in this work to exploit the data provided by an optical flow algorithm for a similar purpose. The advantage of using the optical flow is that it does not require any a priori knowledge on the object appearance. The registration of 2D and 3D cues for monocular tracking is performed by a non linear minimization. Results obtained show that using optical flow enables to perform robust 3D hybrid tracking even without any texture model}},
    language = {Anglais},
    affiliation = {Institut d'Electronique et de T{\'e}l{\'e}communications de Rennes - IETR , LAGADIC - INRIA - IRISA , VISTA - INRIA - IRISA},
    booktitle = {{IEEE Int. Conf. on Image Processing, ICIP'08}},
    address = {San Diego, California, France},
    audience = {internationale },
    year = {2008},
    pdf = {http://hal.inria.fr/inria-00351874/PDF/2008\_icip\_pressigout.pdf},
}







  @inproceedings{conf/cvpr/BreglerM98,
  author = {Bregler, Christoph and Malik, Jitendra},
  booktitle = {CVPR},
  title = {Tracking People with Twists and Exponential Maps.},
  year = 1998
}
@InProceedings{Bro06k,
  author       = "T. Brox and B. Rosenhahn and D. Cremers and H.-P. Seidel",
  title        = "High accuracy optical flow serves 3-D pose tracking: exploiting contour and flow based constraints",
  booktitle    = "ECCV",
  year         = "2006"
}

@article{DBLP:journals/corr/RusuRDSKKPH16,
  author    = {Andrei A. Rusu and
               Neil C. Rabinowitz and
               Guillaume Desjardins and
               Hubert Soyer and
               James Kirkpatrick and
               Koray Kavukcuoglu and
               Razvan Pascanu and
               Raia Hadsell},
  title     = {Progressive Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1606.04671},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.04671},
  timestamp = {Wed, 07 Jun 2017 14:40:25 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RusuRDSKKPH16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@InProceedings{Ferrari08,
  author       = "Ferrari, V. and Marin-Jimenez, M. and Zisserman, A.",
  title        = "Progressive Search Space Reduction for Human Pose Estimation",
  booktitle    = "IEEE Conference on Computer Vision and Pattern Recognition",
  year         = "2008",
}


  @incollection {SLIC,
    title={SLIC Superpixels},
    author={Radhakrishna Achanta and Appu Shaji and Kevin Smith and Aurelien Lucchi and Pascal Fua and Sabine Susstrunk},
    booktitle={EPFL Technical Report no. 149300, June 2010},
  }
  @incollection {springerlink:10.1007/978-3-642-15549-9_32,
    author = {Sundaram, Narayanan and Brox, Thomas and Keutzer, Kurt},
    title = {Dense Point Trajectories by {GPU}-Accelerated Large Displacement Optical Flow},
    booktitle = {ECCV},
    year={2010},

  }
  @incollection {springerlink:10.1007/978-3-540-88688-4_58,
    author = {Huang, Chang and Wu, Bo and Nevatia, Ramakant},
    title = {Robust Object Tracking by Hierarchical Association of Detection Responses},
    booktitle = {ECCV},
    year={2008},
  }

  @InProceedings{eth_biwi_00483,
    author = {B. Leibe and N. Cornelis and K. Cornelis and L. Van Gool},
    title = {Dynamic 3D Scene Analysis from a Moving Vehicle},
    booktitle = {CVPR},
    year = {2007},
  }

  @article{10.1109/TPAMI.2010.143,
  author = {Thomas Brox and Jitendra Malik},
  title = {Large Displacement Optical Flow: Descriptor Matching in Variational Motion Estimation},
  journal ={TPAMI},
  year = {2010},

  }


  @article {springerlink:10.1007/s11263-008-0136-6,
  title = {Particle Video: Long-Range Motion Estimation Using Point Trajectories},
    author = {Sand, Peter and Teller, Seth},
    affiliation = {MIT Computer Science and Artificial Intelligence Laboratory Cambridge MA 02139 USA},
    journal = {IJCV},
    year = {2008}
  }

  @InProceedings{yma,
    author = { Rao, S. and Tron, R. and Vidal, R. and Ma, Y. },
    title = {Motion segmentation via robust subspace separation in the presence of outlying, incomplete, or corrupted trajectories.},
    booktitle = {CVPR},
  year={2008},
  }



  @InProceedings{sparsesubsp,
    author = {Elhamifar, E. and Vidal, R.},
    title = {Sparse subspace clustering},
    booktitle = {CVPR},
    year = {2009}
  }




  @INPROCEEDINGS{BrostowCipollaCVPR2006,
    AUTHOR       = {Gabriel J. Brostow and Roberto Cipolla},
    TITLE        = {Unsupervised Bayesian Detection of Independent Motion in Crowds},
    BOOKTITLE    = {CVPR},
    YEAR         = {2006},
  }
  @article{GrundmannKwatra2010,
    author = {Matthias Grundmann and Vivek Kwatra and Mei Han and Irfan Essa},
    title = {Efficient Hierarchical Graph Based Video Segmentation},
    journal = {CVPR},
    year = {2010},
  }



  @incollection {mhvs,
    author = {Amelio Vazquez-Reina and Shai Avidan and Hanspeter Pfister and Eric Miller},
    title = {Multiple Hypothesis Video Segmentation from Superpixel Flows},
    booktitle = {ECCV},
  year={2010},
  }
  @INPROCEEDINGS{4761133,
  author={Izadi, M. and Saeedi, P.},
  booktitle={Pattern Recognition, 2008. ICPR 2008. 19th International Conference on},
  title={Robust region-based background subtraction and shadow removing using color and gradient information},
  year={2008}
  }

  @INPROCEEDINGS{784637,
  author={Stauffer, C. and Grimson, W.E.L.},
  booktitle={CVPR},
  title={Adaptive background mixture models for real-time tracking},
  year={1999}}


  @inproceedings{Zivkovic:2004:IAG:1018428.1020644,
  author = {Zivkovic, Zoran},
  title = {Improved Adaptive Gaussian Mixture Model for Background Subtraction},
  booktitle = {ICPR},
  year = {2004}
  }


  @article{Felzenszwalb:2004:EGI:981793.981796,
  author = {Felzenszwalb, Pedro F. and Huttenlocher, Daniel P.},
  title = {Efficient Graph-Based Image Segmentation},
  journal = {IJCV},
  volume = {59},
  year = {2004}
  }

  @article{phycho,
    author = {H. C. Nothdurft},
    title = {Feature analysis and the role of similarity in preattentive vision},
    journal = {Perception and Psychophysics},
    volume={52},
    year = {1992},
  }

  @inproceedings{DBLP:conf/eccv/Ren08,
    author    = {Xiaofeng Ren},
    title     = {Multi-scale Improves Boundary Detection in Natural Images},
    booktitle = {ECCV (3)},
    year      = {2008},
    pages     = {533-545},
    ee        = {http://dx.doi.org/10.1007/978-3-540-88690-7_40},
    crossref  = {DBLP:conf/eccv/2008-3},
    bibsource = {DBLP, http://dblp.uni-trier.de}
  }



  @INPROCEEDINGS{5206727,
  author={Chunhui Gu and Lim, J.J. and Arbelaez, P. and Malik, J.},
  booktitle={CVPR},
  year={2009},
  title={Recognition using regions}
  }
  @InProceedings{citeulike:942103,
      title = {Bottom-up/top-down image parsing by attribute graph grammar},
      author = {Han, Feng and Zhu, Song-Chun},
      journal = {ICCV},
  year={ 2005}
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {CVPR},
  year={2009},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }

  @InProceedings{Yan06general,
    title     = {A General Framework for Motion Segmentation: Independent, Articulated, Rigid, Non-rigid, Degenerate and Non-degenerate.},
    author = {J. Yan and M. Pollefeys},
    booktitle = {ECCV},
  year={ 2006},
  }

  @InProceedings{Ayer,
    title     = {Layered representation of motion video using robust maximum-likelihood estimation of mixture models and MDL encoding},
    author = {S. Ayer and H. S. Sawhney},
    booktitle = {ICCV},
  year={ 1995},
  }

  @article{10.1109/CVPR.2005.335,
  author = {Deva Ramanan and D. A. Forsyth and Andrew Zisserman},
  title = {Strike a Pose: Tracking People by Finding Stylized Poses},
  journal ={CVPR},
  year = {2005},
  }
  
    @incollection{NIPS2012_0534,
    Title = {ImageNet Classification with Deep Convolutional Neural Networks},
    Url = {http://books.nips.cc/papers/files/nips25/NIPS2012_0534.pdf},
    Booktitle = {Advances in Neural Information Processing Systems 25},
    Author = {Alex Krizhevsky and Ilya Sutskever and Geoffrey E. Hinton},
    Editor = {P. Bartlett and F.c.n. Pereira and C.j.c. Burges and L. Bottou and K.q. Weinberger},
    Year = {2012},
    Pages = {1106--1114}
   } 
   
@inproceedings{DBLP:conf/iccv/ParkR11,
  author    = {Dennis Park and Deva Ramanan},
  title     = {N-best maximal decoders for part models},
  booktitle = {ICCV},
  year      = {2011},
  pages     = {2627-2634},
  ee        = {http://dx.doi.org/10.1109/ICCV.2011.6126552},
  crossref  = {DBLP:conf/iccv/2011},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Batra:2012:DMS:2403138.2403140,
 author = {Batra, Dhruv and Yadollahpour, Payman and Guzman-Rivera, Abner and Shakhnarovich, Gregory},
 title = {Diverse "M"-best solutions in markov random fields},
 booktitle = {ECCV},
 year = {2012}
} 


@inproceedings{Batra:2012:DMS:2403138.2403140,
 author = {Batra, Dhruv and Yadollahpour, Payman and Guzman-Rivera, Abner and Shakhnarovich, Gregory},
 title = {Diverse M-best solutions in markov random fields},
 booktitle = {Proceedings of the 12th European conference on Computer Vision - Volume Part V},
 series = {ECCV'12},
 year = {2012},
 isbn = {978-3-642-33714-7},
 location = {Florence, Italy},
 pages = {1--16},
 numpages = {16},
 url = {http://dx.doi.org/10.1007/978-3-642-33715-4_1},
 doi = {10.1007/978-3-642-33715-4_1},
 acmid = {2403140},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
}


@InProceedings{Weiss_2013_ICCV,
author = {David Weiss and Benjamin Sapp and Ben Taskar},
title = {Dynamic Structured Model Selection},
booktitle = {ICCv},
month = {December},
year = {2013}
} 


@inproceedings{DBLP:conf/iros/KoppulaS13,
  author    = {Hema Swetha Koppula and
               Ashutosh Saxena},
  title     = {Anticipating human activities for reactive robotic response},
  booktitle = {2013 {IEEE/RSJ} International Conference on Intelligent Robots and
               Systems, Tokyo, Japan, November 3-7, 2013},
  pages     = {2071},
  year      = {2013},
  crossref  = {DBLP:conf/iros/2013},
  url       = {http://dx.doi.org/10.1109/IROS.2013.6696634},
  doi       = {10.1109/IROS.2013.6696634},
  timestamp = {Fri, 10 Jan 2014 20:22:57 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/iros/KoppulaS13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{YangR_CVPR_2011,
    author = "Yang, Yi and Ramanan, Deva",
    booktitle = "CVPR",
    year = "2011",
    title = "Articulated pose estimation with flexible mixtures-of-parts"
}

@INPROCEEDINGS{Felzenszwalb00efficientmatching,
    author = {Pedro F. Felzenszwalb and Daniel P. Huttenlocher},
    title = {Efficient Matching of Pictorial Structures},
    booktitle = {CVPR},
    year = {2000},
}

@inproceedings{YangWang:2011:LHP:2191740.2192189,
 author = {Yang Wang and Duan Tran and Zicheng Liao},
 title = {Learning hierarchical poselets for human parsing},
 booktitle = {Proceedings of the 2011 IEEE Conference on Computer Vision and Pattern Recognition},
 series = {CVPR '11},
 year = {2011},
 isbn = {978-1-4577-0394-2},
 pages = {1705--1712},
 numpages = {8},
 url = {http://dx.doi.org/10.1109/CVPR.2011.5995519},
 doi = {10.1109/CVPR.2011.5995519},
 acmid = {2192189},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
 keywords = {max-margin framework, hierarchical poselets, human parsing, part-based model, rigid parts, human anatomy, structured model},
}

@article{Grady:2006:RWI:1175896.1176220,
 author = {Grady, Leo},
 title = {Random Walks for Image Segmentation},
 journal = {IEEE Trans. Pattern Anal. Mach. Intell.},
 issue_date = {November 2006},
 volume = {28},
 number = {11},
 month = nov,
 year = {2006},
 issn = {0162-8828},
 pages = {1768--1783},
 numpages = {16},
 url = {http://dx.doi.org/10.1109/TPAMI.2006.233},
 doi = {10.1109/TPAMI.2006.233},
 acmid = {1176220},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
 keywords = {Image segmentation, Image segmentation, interactive segmentation, graph theory, random walks, combinatorial Dirichlet problem, harmonic functions, Laplace equation, graph cuts, boundary completion., Laplace equation, boundary completion., combinatorial Dirichlet problem, graph cuts, graph theory, harmonic functions, interactive segmentation, random walks},
} 



@inproceedings{DBLP:conf/cvpr/JohnsonE11,
  author    = {Sam Johnson and
               Mark Everingham},
  title     = {Learning effective human pose estimation from inaccurate
               annotation},
  booktitle = {CVPR},
  year      = {2011}
}

@misc{Jia13caffe,
   Author = {Yangqing Jia},
   Title = { {Caffe}: An Open Source Convolutional Architecture for Fast Feature Embedding},
   Year  = {2013}
}

@inproceedings{MODEC,
  author    = {Ben Sapp and
               Ben Taskar},
  title     = {MODEC:Multimodal Decomposable Models for Human Pose Estimation},
  booktitle = {CVPR},
  year      = {2013}
}


















  @Article{ Perse2009612,
  title = "A trajectory-based analysis of coordinated team activity in a basketball game",
  journal = "Computer Vision and Image Understanding",
  volume = "113",
  year = "2009",
  }

  @inproceedings{morariu11eventstructure,
    author    = {Vlad I. Morariu and Larry S. Davis},
    title     = {Multi-agent event recognition in structured scenarios.},
    booktitle = {CVPR},
    year      = {2011}
  }


  @inproceedings{storyline,
    author    = {Abhinav Gupta and Praveen Srinivasan and Jianbo Shi and Larry S. Davis},
    title     = {Understanding videos, constructing plots learning a visually grounded storyline model from annotated videos},
    booktitle = {CVPR},
    year      = {2009}
  }


  @ARTICLE{790429,
  author={Wilson, A.D. and Bobick, A.F.},
  journal={TPAMI},
  title={Parametric hidden Markov models for gesture recognition},
  year={1999},
  volume={21}
  }



  @article{experts,
  author = {Terence D. Sanger and Robert A. Jacobs and Steven J. Nowlan and Geoffrey E. Hinton},
  title = {Adaptive Mixtures of Local Experts},
  journal = {Neural Computation},
  volume = {3},
  year = {1991}
  }


  @INPROCEEDINGS{lips,
  author={Bregler, C. and Omohundro, S.M.},
  booktitle={ICCV},
  title={Nonlinear manifold learning for visual speech recognition},
  year={1995}
  }



  @inproceedings{BN,
  author = {Shaogang Gong and Tao Xiang},
  title = {Recognition of Group Activities using Dynamic Probabilistic Networks},
  booktitle = {ICCV},
  year={2003}
  }


  @article{HMMMO,
  author = {Aaron F. Bobick and Andrew D. Wilson},
  title = {A State-Based Approach to the Representation and Recognition of Gesture},
  journal = {TPAMI},
  volume = {19}
  }

  @inproceedings{Brand:1997:CHM:794189.794420,
  author = {Brand, M. and Oliver, N. and Pentland, A.},
  title = {Coupled hidden Markov models for complex action recognition},
  booktitle = {CVPR},
  year = {1997}
  }

  @article{Ghahramani:1997:FHM:274158.274165,
  author = {Ghahramani, Zoubin and Jordan, Michael I.},
  title = {Factorial Hidden Markov Models},
  journal = {Mach. Learn.},
  volume = {29},
  year = {1997}
  }


  @INPROCEEDINGS{4270099,
  author={Laxton, B. and Jongwoo Lim and Kriegman, D.},
  booktitle={CVPR},
  title={Leveraging temporal, contextual and ordering constraints for recognizing complex activities in video},
  year={2007}
  }


  @article{DBLP:journals/jmlr/SiracusaF09,
    author    = {Michael Siracusa and John Fisher},
    title     = {Tractable Bayesian Inference of Time-Series Dependence Structure},
    journal   = {Journal of Machine Learning Research - Proceedings Track},
    volume    = {5},
    year      = {2009}
  }



  @article{parametrized,
  author = {Yaser Yacoob and Michael J. Black},
  title = {Parameterized Modeling and Recognition of Activities},
  journal = {Computer Vision and Image Understanding},
  volume = {73},
  year = {1999}
  }




  @inproceedings{Bobick:1995:STS:839277.840051,
  author = {Bobick, A. F. and Wilson, A. D.},
  title = {A state-based technique for the summarization and recognition of gesture},
  booktitle = {ICCV},
  year = {1995}
  }

  @inproceedings{Xu:2008:SBV:1478392.1478446,
  author = {Xu, Li and Chen, Jianing and Jia, Jiaya},
  title = {A Segmentation Based Variational Model for Accurate Optical Flow Estimation},
  booktitle = {ECCV},
  year = {2008}
  }

  @inproceedings{Niebles:2010:MTS:1888028.1888059,
  author = {Niebles, Juan Carlos and Chen, Chih-Wei and Fei-Fei, Li},
  title = {Modeling temporal structure of decomposable motion segments for activity classification},
  booktitle = {ECCV},
  year = {2010}
  }

  @InProceedings{Bro11c,
    author       = "P. Sundberg and T. Brox and M. Maire and P. Arbelaez and J. Malik",
    title        = "Occlusion boundary detection and figure/ground assignment from optical flow",
    booktitle    = "CVPR",
    year         = "2011"
  }

  @inproceedings{Stein_2007_5836,
    author = "Andrew Stein and Derek Hoiem and Martial Hebert",
    title = "Learning to Find Object Boundaries Using Motion Cues",
    booktitle = "IEEE International Conference on Computer Vision (ICCV)",
    month = "October",
    year = "2007",
    Notes = "Dataset available from http://www.cs.cmu.edu/~stein/occlusion_data"
  }


  @article{Hakeem:2007:LDR:1265999.1266287,
  author = {Hakeem, Asaad and Shah, Mubarak},
  title = {Learning, detection and representation of multi-agent events in videos},
  journal = {Artif. Intell.},
  volume = {171},
  year = {2007}
  }


  @INPROCEEDINGS{Zelnik-manor01event-basedanalysis,
      author = {Lihi Zelnik-manor and Michal Irani},
      title = {Event-based analysis of video},
      booktitle = {CVPR},
      year = {2001}
  }

  @inproceedings{Jebara:2007:SCE:1421665.1421685,
  author = {Jebara, Tony and Song, Yingbo and Thadani, Kapil},
  title = {Spectral Clustering and Embedding with Hidden Markov Models},
  booktitle = {European conference on Machine Learning},
  year = {2007}
  }

  @article{Jebara:2004:PPK:1005332.1016786,
  author = {Jebara, Tony and Kondor, Risi and Howard, Andrew},
  title = {Probability Product Kernels},
  journal = {J. Mach. Learn. Res.},
  volume = {5},
  year = {2004}
  }

  @INPROCEEDINGS{Gong99recognitionof,
      author = {Shaogang Gong and Michael Walter},
      title = {Recognition of Temporal Structures: Learning Prior and Propagating Observation Augmented Densities via Hidden Markov States},
      booktitle = {ICCV},
      year = {1999},
  }

  @article{Brand:2000:DSA:351581.351608,
  author = {Brand, Matthew and Kettnaker, Vera},
  title = {Discovery and Segmentation of Activities in Video},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }


  @INPROCEEDINGS{Brown01productsof,
      author = {Andrew D. Brown and Andrew D. Brown and Geoffrey E. Hinton and Geoffrey E. Hinton},
      title = {Products of Hidden Markov Models},
      booktitle = {In Proceedings of Artificial Intelligence and Statistics},
      year = {2001},
  }


  @inproceedings{malisiewicz-nips09,
    Author =	 {Tomasz Malisiewicz and Alexei A. Efros},
    Booktitle =	 {NIPS},
    Title =	 {Beyond Categories: The Visual Memex Model for Reasoning About Object Relationships},
    Year =	 2009
  }


  @inproceedings{yamato,
  author = {J. Yamato and J. Ohya and K. Ishii},
  title = {Recognizing human action in time-sequential images using a hidden Markov model},
  booktitle = {CVPR},
  year = {1994},
  }



  @INPROCEEDINGS{Elgammal04separatingstyle,
      author = {Ahmed Elgammal and Chan-su Lee},
      title = {Separating style and content on a nonlinear manifold},
      booktitle = {CVPR},
      year = {2004}
  }

  @INPROCEEDINGS{Tenenbaum97separatingstyle,
      author = {Joshua B. Tenenbaum and William T. Freeman},
      title = {Separating style and content},
      booktitle = {In Advances in neural},
      year = {1997}
  }

@article{DBLP:journals/corr/LeeKP016,
  author    = {Kenton Lee and
               Tom Kwiatkowski and
               Ankur P. Parikh and
               Dipanjan Das},
  title     = {Learning Recurrent Span Representations for Extractive Question Answering},
  journal   = {CoRR},
  volume    = {abs/1611.01436},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.01436},
  archivePrefix = {arXiv},
  eprint    = {1611.01436},
  timestamp = {Wed, 07 Jun 2017 14:41:54 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LeeKP016},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/LiuAESR15,
  author    = {Wei Liu and
               Dragomir Anguelov and
               Dumitru Erhan and
               Christian Szegedy and
               Scott E. Reed and
               Cheng{-}Yang Fu and
               Alexander C. Berg},
  title     = {{SSD:} Single Shot MultiBox Detector},
  journal   = {CoRR},
  volume    = {abs/1512.02325},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.02325},
  timestamp = {Wed, 07 Jun 2017 14:42:54 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LiuAESR15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @inproceedings{DBLP:conf/cvpr/LvN07,
    author    = {Fengjun Lv and
		Ramakant Nevatia},
    title     = {Single View Human Action Recognition using Key Pose Matching and Viterbi Path Searching},
    booktitle = {CVPR},
    year      = {2007}
  }


  @inproceedings { 158,
	  title = {Linear Embeddings in Non-Rigid Structure From Motion},
	  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	  year = {2009},
	  address = {Miami, FL},
	  author = {Vincent Rabaud and Serge Belongie}
  }



  @INPROCEEDINGS{4270260,
  author={Goh, A. and Vidal, R.},
  booktitle={CVPR},
  title={Segmenting Motions of Different Types by Unsupervised Manifold Clustering},
  year={2007},
  }


  @incollection {springerlink:10.1007/11551188_37,
    author = {Wang, Fei and Zhang, Changshui},
    title = {Spectral Clustering for Time Series},
    booktitle = {Pattern Recognition and Data Mining},
    volume = {3686},
    year = {2005}
  }

  @INPROCEEDINGS{4587385,
  author={Xiaozhe Wang and Liang Wang and Wirth, A.},
  booktitle={CVPR},
  title={Pattern discovery in motion time series via structure-based spectral clustering},
  year={2008}
  }


  @article{Stauffer:2000:LPA:351581.351588,
  author = {Stauffer, Chris and Grimson, W. Eric L.},
  title = {Learning Patterns of Activity Using Real-Time Tracking},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }

  @incollection{Nanopoulos:2001:FCT:766914.766918,
  author = {Nanopoulos, Alex and Alcock, Rob and Manolopoulos, Yannis},
  title = {Information processing and technology},
  year = {2001},
  }

  BibTeX | EndNote | ACM Ref

  @inproceedings{Shi:2006:LTS:1153171.1153641,
  author = {Shi, Yifan and Bobick, Aaron and Essa, Irfan},
  title = {Learning Temporal Sequence Model from Partially Labeled Data},
  booktitle = {CVPR},
  year = {2006}
  }


  @article{Murase,
  author = {Murase, Hiroshi and Nayar, Shree K.},
  title = {Visual learning and recognition of 3-D objects from appearance},
  journal = {IJCV},
  volume = {14},
  year = {1995}
  }


  @INPROCEEDINGS{698609,
  author={Bobick, A.F. and Ivanov, Y.A.},
  booktitle={CVPR},
  title={Action recognition using probabilistic parsing},
  year={1998}
  }

  @inproceedings{Ryoo:2006:RCH:1153171.1153651,
  author = {Ryoo, M. S. and Aggarwal, J. K.},
  title = {Recognition of Composite Human Activities through Context-Free Grammar Based Representation},
  booktitle = {CVPR},
  year = {2006}
  }


  @INPROCEEDINGS{Hadsell06dimensionalityreduction,
      author = {Raia Hadsell and Sumit Chopra and Yann Lecun},
      title = {Dimensionality reduction by learning an invariant mapping},
      booktitle = {CVPR},
      year = {2006}
  }


  @incollection{NIPS2010_0893,
  title = {Pose-Sensitive Embedding by Nonlinear NCA Regression},
  author = {Graham Taylor and Rob Fergus and George Williams and Ian Spiro and Christoph Bregler},
  booktitle = {NIPS},
  year = {2010}
  }
  @InProceedings{lezama11,
    author = {Lezama, J. and Alahari, K. and Sivic, J. and Laptev, I.},
    title = {Track to the Future: Spatio-temporal Video Segmentation with Long-range Motion Cues},
    booktitle = {CVPR},
    year = {2011}
  }
  @InProceedings{shuwang2,
    author = {Shu Wang and Huchuan Lu and Fan Yang and Ming-Hsuan Yang},
    title = {Superpixel Tracking},
    booktitle = {ICCV},
    year = {2011}
  }
  @InProceedings{OB11,
    author       = "P. Ochs and T.Brox",
    title        = "Object segmentation in video: a hierarchical variational approach for turning point trajectories into dense regions",
    booktitle    = "ICCV",
    year         = "2011",
    url          = "http://lmb.informatik.uni-freiburg.de/Publications/2011/OB11"
  }

  @InProceedings{raptisS10,
    author = 	{Raptis, M. and Soatto, S.},
    title = 	{Tracklet Descriptors for Action Modeling and Video Analysis},
    booktitle = 	{ECCV},
    year = 	{2010}
  }


  @book{Fukunaga:1990:ISP:92131,
  author = {Fukunaga, Keinosuke},
  title = {Introduction to statistical pattern recognition (2nd ed.)},
  year = {1990}
  }


  @ARTICLE{Roweis00nonlineardimensionality,
      author = {Sam T. Roweis and Lawrence K. Saul},
      title = {Nonlinear dimensionality reduction by locally linear embedding},
      journal = {SCIENCE},
      year = {2000},
      volume = {290}
  }

  @article{Turk_Pentland_1991,
  title={Face recognition using eigenfaces},
  journal={CVPR},
  year={1991}
  }


  @INPROCEEDINGS{Laptev03space-timeinterest,
      author = {Ivan Laptev and Tony Lindeberg},
      title = {Space-time Interest Points},
      booktitle = {ICCV},
      year = {2003}
  }


  @INPROCEEDINGS{Kim07r.:tensor,
      author = {Tae-kyun Kim and Shu-fai Wong and Roberto Cipolla},
      title = {Tensor Canonical Correlation Analysis for Action Classification},
      booktitle = {CVPR},
      year = {2007}
  }


  @inproceedings{Fragkiadaki:topology,
  author = {Fragkiadaki, Katerina and Shi, Jianbo},
  title = {Exploiting Motion and Topology for Segmenting and tracking Under Entanglement.},
  booktitle = {CVPR},
  year = {2011},
  }

  @INPROCEEDINGS{Jianbo03multiclassspectral,
      author = {Yu,Stella and Shi, Jianbo},
      title = {Multiclass Spectral Clustering},
      booktitle = {ICCV},
      year = {2003}
  }



  @INPROCEEDINGS{lu_cvpr2011,
      author = {Wei-Lwun Lu and Jo-Anne Ting and Kevin P. Murphy and James J. Little},
      booktitle = {Identifying Players in Broadcast Sports Videos using Conditional Random Fields},
      journal = {Proceedings of the 2011 IEEE Conference on Computer Vision and Pattern Recognition},
      year = {2011}
  }

  @article{DBLP:journals/pami/BoykovVZ01,
    author    = {Yuri Boykov and Olga Veksler and Ramin Zabih},
    title     = {Fast Approximate Energy Minimization via Graph Cuts},
    journal   = {TPAMI},
    volume    = {23},
    year      = {2001}
  }

  @article{GEAN:GEAN31,
  author = {Matula, David W. and Sokal, Robert R.},
  title = {Properties of Gabriel Graphs Relevant to Geographic Variation Research and the Clustering of Points in the Plane},
  journal = {Geographical Analysis},
  volume = {12},
  year = {1980}
  }


  @INPROCEEDINGS{global_Pb,
  AUTHOR = {Michael Maire and Pablo Arbelaez and Charless Fowlkes and Jitendra Malik},
  TITLE = {Using contours to detect and localize junctions in natural images.},
  booktitle = {CVPR},
  YEAR = {2008}
  }


  @inproceedings{Yu:2010:AIO:1873951.1874105,
  author = {Yu, Haonan and Li, Jia and Tian, Yonghong and Huang, Tiejun},
  title = {Automatic interesting object extraction from images using complementary saliency maps},
  booktitle = {Proceedings of the international conference on Multimedia},
  year = {2010}
  }
  @inproceedings{DBLP:conf/accv/DonoserRB09,
    author    = {Michael Donoser and Hayko Riemenschneider and  Horst Bischof},
    title     = {Efficient Partial Shape Matching of Outer Contours},
    booktitle = {ACCV},
    year      = {2009}
  }

  @inproceedings{RenFM05a,
	  author = "Xiaofeng Ren and Charless C. Fowlkes and Jitendra Malik",
	  title = "Scale-invariant contour completion using conditional random fields",
	  booktitle = {ICCV},
	  year = "2005"
	  }
@INPROCEEDINGS{Xiao06bilateralfiltering-based,
    author = {Jiangjian Xiao and Hui Cheng and Harpreet Sawhney and Cen Rao and Michael Isnardi and Sarnoff Corporation},
    title = {Bilateral filtering-based optical flow estimation with occlusion detection},
    booktitle = {ECCV},
    year = {2006},
}

  @TechReport{RenFM05tech,
	  author = "Xiaofeng Ren and Charless C. Fowlkes and Jitendra Malik",
	  title = "Mid-level cues improve boundary detection",
	  institution =  {UC Berkeley},
	  number =       {UCB//CSD-05-1382},
	  year =         {2005}
	  }

  @InProceedings{BroxSegmentationCVPR11,
    author       = "Thomas Brox and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Object Segmentation by Alignment of Poselet Activations to Image Contours",
    booktitle    = "IEEE International Conference on Computer Vision and Pattern Recognition (CVPR)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }
  @InProceedings{HariharanSemanticContoursICCV11,
    author       = "Bharath Hariharan and Pablo Arbelaez and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Semantic Contours from Inverse Detectors",
    booktitle    = "International Conference on Computer Vision (ICCV)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }
  @inproceedings{DBLP:conf/eccv/RiemenschneiderDB10,
    author    = {Hayko Riemenschneider and Michael Donoser and Horst Bischof},
    title     = {Using Partial Edge Contour Matches for Efficient Object
		Category Localization},
    booktitle = {ECCV},
    year      = {2010}
  }

  


  @inproceedings{MoriREM04,
	  author = "Greg Mori and Xiaofeng Ren and Alexei A. Efros and Jitendra Malik",
	  title = "Recovering human body configurations: combining segmentation and recognition.",
	  booktitle = {Proc. IEEE Conf. Comput. Vision and Pattern Recogn.},
	  volume = 2,
	  pages = "326-333",
	  year = "2004",
	  }



  @inproceedings{Latecki2010,
    author    = {Tianyang Ma and Longin Jan Latecki},
    title     = { From Partial Shape Matching through Local Deformation to Robust Global Shape Similarity for Object Detection},
    booktitle = {CVPR},
    year      = {2011}
  }
  @article{Jebara:2004:PPK:1005332.1016786,
  author = {Jebara, Tony and Kondor, Risi and Howard, Andrew},
  title = {Probability Product Kernels},
  journal = {J. Mach. Learn. Res.},
  volume = {5},
  year = {2004}
  }

  @INPROCEEDINGS{Gong99recognitionof,
      author = {Shaogang Gong and Michael Walter},
      title = {Recognition of Temporal Structures: Learning Prior and Propagating Observation Augmented Densities via Hidden Markov States},
      booktitle = {ICCV},
      year = {1999},
  }

  @article{Brand:2000:DSA:351581.351608,
  author = {Brand, Matthew and Kettnaker, Vera},
  title = {Discovery and Segmentation of Activities in Video},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }


  @INPROCEEDINGS{Brown01productsof,
      author = {Andrew D. Brown and Andrew D. Brown and Geoffrey E. Hinton and Geoffrey E. Hinton},
      title = {Products of Hidden Markov Models},
      booktitle = {In Proceedings of Artificial Intelligence and Statistics},
      year = {2001},
  }


  @inproceedings{malisiewicz-nips09,
    Author =	 {Tomasz Malisiewicz and Alexei A. Efros},
    Booktitle =	 {NIPS},
    Title =	 {Beyond Categories: The Visual Memex Model for Reasoning About Object Relationships},
    Year =	 2009
  }


  @inproceedings{yamato,
  author = {J. Yamato and J. Ohya and K. Ishii},
  title = {Recognizing human action in time-sequential images using a hidden Markov model},
  booktitle = {CVPR},
  year = {1994},
  }



  @INPROCEEDINGS{Elgammal04separatingstyle,
      author = {Ahmed Elgammal and Chan-su Lee},
      title = {Separating style and content on a nonlinear manifold},
      booktitle = {CVPR},
      year = {2004}
  }

  @INPROCEEDINGS{Tenenbaum97separatingstyle,
      author = {Joshua B. Tenenbaum and William T. Freeman},
      title = {Separating style and content},
      booktitle = {In Advances in neural},
      year = {1997}
  }

  @inproceedings{DBLP:conf/cvpr/LvN07,
    author    = {Fengjun Lv and
		Ramakant Nevatia},
    title     = {Single View Human Action Recognition using Key Pose Matching and Viterbi Path Searching},
    booktitle = {CVPR},
    year      = {2007}
  }


  @inproceedings { 158,
	  title = {Linear Embeddings in Non-Rigid Structure From Motion},
	  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	  year = {2009},
	  address = {Miami, FL},
	  author = {Vincent Rabaud and Serge Belongie}
  }



  @INPROCEEDINGS{4270260,
  author={Goh, A. and Vidal, R.},
  booktitle={CVPR},
  title={Segmenting Motions of Different Types by Unsupervised Manifold Clustering},
  year={2007},
  }


  @incollection {springerlink:10.1007/11551188_37,
    author = {Wang, Fei and Zhang, Changshui},
    title = {Spectral Clustering for Time Series},
    booktitle = {Pattern Recognition and Data Mining},
    volume = {3686},
    year = {2005}
  }


@INPROCEEDINGS{Wang06gaussianprocess,
    author = {Jack M. Wang and David J. Fleet and Aaron Hertzmann},
    title = {Gaussian process dynamical models},
    booktitle = {In NIPS},
    year = {2006},
    pages = {1441--1448},
    publisher = {MIT Press}
}


  @INPROCEEDINGS{4587385,
  author={Xiaozhe Wang and Liang Wang and Wirth, A.},
  booktitle={CVPR},
  title={Pattern discovery in motion time series via structure-based spectral clustering},
  year={2008}
  }


  @article{Stauffer:2000:LPA:351581.351588,
  author = {Stauffer, Chris and Grimson, W. Eric L.},
  title = {Learning Patterns of Activity Using Real-Time Tracking},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }

  @incollection{Nanopoulos:2001:FCT:766914.766918,
  author = {Nanopoulos, Alex and Alcock, Rob and Manolopoulos, Yannis},
  title = {Information processing and technology},
  year = {2001},
  }

  BibTeX | EndNote | ACM Ref

  @inproceedings{Shi:2006:LTS:1153171.1153641,
  author = {Shi, Yifan and Bobick, Aaron and Essa, Irfan},
  title = {Learning Temporal Sequence Model from Partially Labeled Data},
  booktitle = {CVPR},
  year = {2006}
  }


  @article{Murase,
  author = {Murase, Hiroshi and Nayar, Shree K.},
  title = {Visual learning and recognition of 3-D objects from appearance},
  journal = {IJCV},
  volume = {14},
  year = {1995}
  }


  @INPROCEEDINGS{698609,
  author={Bobick, A.F. and Ivanov, Y.A.},
  booktitle={CVPR},
  title={Action recognition using probabilistic parsing},
  year={1998}
  }

  @inproceedings{Ryoo:2006:RCH:1153171.1153651,
  author = {Ryoo, M. S. and Aggarwal, J. K.},
  title = {Recognition of Composite Human Activities through Context-Free Grammar Based Representation},
  booktitle = {CVPR},
  year = {2006}
  }


  @INPROCEEDINGS{Hadsell06dimensionalityreduction,
      author = {Raia Hadsell and Sumit Chopra and Yann Lecun},
      title = {Dimensionality reduction by learning an invariant mapping},
      booktitle = {CVPR},
      year = {2006}
  }


  @incollection{NIPS2010_0893,
  title = {Pose-Sensitive Embedding by Nonlinear NCA Regression},
  author = {Graham Taylor and Rob Fergus and George Williams and Ian Spiro and Christoph Bregler},
  booktitle = {NIPS},
  year = {2010}
  }
  @InProceedings{BroxSegmentationCVPR11,
    author       = "Thomas Brox and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Object Segmentation by Alignment of Poselet Activations to Image Contours",
    booktitle    = "IEEE International Conference on Computer Vision and Pattern Recognition (CVPR)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }
  @InProceedings{HariharanSemanticContoursICCV11,
    author       = "Bharath Hariharan and Pablo Arbelaez and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Semantic Contours from Inverse Detectors",
    booktitle    = "International Conference on Computer Vision (ICCV)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }

  @InProceedings{raptisS10,
    author = 	{Raptis, M. and Soatto, S.},
    title = 	{Tracklet Descriptors for Action Modeling and Video Analysis},
    booktitle = 	{ECCV},
    year = 	{2010}
  }


  @book{Fukunaga:1990:ISP:92131,
  author = {Fukunaga, Keinosuke},
  title = {Introduction to statistical pattern recognition (2nd ed.)},
  year = {1990}
  }


  @ARTICLE{Roweis00nonlineardimensionality,
      author = {Sam T. Roweis and Lawrence K. Saul},
      title = {Nonlinear dimensionality reduction by locally linear embedding},
      journal = {SCIENCE},
      year = {2000},
      volume = {290}
  }

  @article{Turk_Pentland_1991,
  title={Face recognition using eigenfaces},
  journal={CVPR},
  year={1991}
  }


  @INPROCEEDINGS{Laptev03space-timeinterest,
      author = {Ivan Laptev and Tony Lindeberg},
      title = {Space-time Interest Points},
      booktitle = {ICCV},
      year = {2003}
  }


  @INPROCEEDINGS{Kim07r.:tensor,
      author = {Tae-kyun Kim and Shu-fai Wong and Roberto Cipolla},
      title = {Tensor Canonical Correlation Analysis for Action Classification},
      booktitle = {CVPR},
      year = {2007}
  }

  @ARTICLE{Shao_trackingalgorithm,
      author = {Jie Shao and Shaohua Kevin Zhou},
      title = {Tracking Algorithm Using Background-Foreground Motion Models and Multiple Cues},
      journal = {ICASSP}
  }
  @INPROCEEDINGS{Taylor03fusionof,
      author = {Geoffrey Taylor and Lindsay Kleeman},
      title = {Fusion of Multimodal Visual Cues for Model-Based Object Tracking},
      booktitle = {ACRA},
      year = {2003}
  }

  @inproceedings{DBLP:conf/accv/KumarBD07,
    author    = {Pankaj Kumar and
		Michael J. Brooks and
		Anthony R. Dick},
    title     = {Adaptive Multiple Object Tracking Using Colour and Segmentation
		Cues},
    booktitle = {ACCV},
    year      = {2007}
  }

  @InProceedings{rodriguez11b,
    author = "Rodriguez, M. and Sivic, J. and Laptev, I. and Audibert, J.-Y.",
    title = "Density-aware person detection and tracking in crowds",
    booktitle = "ICCV",
    year = "2011"
  }

  @inproceedings{Fragkiadaki:topology,
  author = {Fragkiadaki, Katerina and Shi, Jianbo},
  title = {Exploiting Motion and Topology for Segmenting and tracking Under Entanglement.},
  booktitle = {CVPR},
  year = {2011},
  }



@inproceedings{DBLP:conf/eccv/WangM08,
  author    = {Yang Wang and
               Greg Mori},
  title     = {Multiple Tree Models for Occlusion and Spatial Constraints
               in Human Pose Estimation},
  booktitle = {ECCV},
  year      = {2008}
}



  @InProceedings{BourdevPoseletsECCV10,
    author       = "Lubomir Bourdev and Subhransu Maji and Thomas Brox and Jitendra Malik",
    title        = "Detecting People Using Mutually Consistent Poselet Activations",
    booktitle    = "ECCV",
    year         = "2010",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }

  @inproceedings{partsagain,
  author = {Michael Maire and Stella Yu and Pietro Perona},
  title = {Object Detection and Segmentation from Joint Embedding of Parts and Pixels},
  booktitle = {ICCV},
  year = {2011},
  }

  @INPROCEEDINGS{Jianbo03multiclassspectral,
      author = {Yu,Stella and Shi, Jianbo},
      title = {Multiclass Spectral Clustering},
      booktitle = {ICCV},
      year = {2003}
  }



  @INPROCEEDINGS{lu_cvpr2011,
      author = {Wei-Lwun Lu and Jo-Anne Ting and Kevin P. Murphy and James J. Little},
      booktitle = {Identifying Players in Broadcast Sports Videos using Conditional Random Fields},
      journal = {Proceedings of the 2011 IEEE Conference on Computer Vision and Pattern Recognition},
      year = {2011}
  }

  @article{DBLP:journals/pami/BoykovVZ01,
    author    = {Yuri Boykov and Olga Veksler and Ramin Zabih},
    title     = {Fast Approximate Energy Minimization via Graph Cuts},
    journal   = {TPAMI},
    volume    = {23},
    year      = {2001}
  }

  @article{GEAN:GEAN31,
  author = {Matula, David W. and Sokal, Robert R.},
  title = {Properties of Gabriel Graphs Relevant to Geographic Variation Research and the Clustering of Points in the Plane},
  journal = {Geographical Analysis},
  volume = {12},
  year = {1980}
  }


  @INPROCEEDINGS{global_Pb,
  AUTHOR = {Michael Maire and Pablo Arbelaez and Charless Fowlkes and Jitendra Malik},
  TITLE = {Using contours to detect and localize junctions in natural images.},
  booktitle = {CVPR},
  YEAR = {2008}
  }


  @inproceedings{Yu:2010:AIO:1873951.1874105,
  author = {Yu, Haonan and Li, Jia and Tian, Yonghong and Huang, Tiejun},
  title = {Automatic interesting object extraction from images using complementary saliency maps},
  booktitle = {Proceedings of the international conference on Multimedia},
  year = {2010}
  }
  @inproceedings{DBLP:conf/accv/DonoserRB09,
    author    = {Michael Donoser and Hayko Riemenschneider and  Horst Bischof},
    title     = {Efficient Partial Shape Matching of Outer Contours},
    booktitle = {ACCV},
    year      = {2009}
  }

  @inproceedings{DBLP:conf/eccv/RiemenschneiderDB10,
    author    = {Hayko Riemenschneider and Michael Donoser and Horst Bischof},
    title     = {Using Partial Edge Contour Matches for Efficient Object
		Category Localization},
    booktitle = {ECCV},
    year      = {2010}
  }

  @inproceedings{Latecki2010,
    author    = {Tianyang Ma and Longin Jan Latecki},
    title     = { From Partial Shape Matching through Local Deformation to Robust Global Shape Similarity for Object Detection},
    booktitle = {CVPR},
    year      = {2011}
  }



  @ARTICLE{Wang94representingmoving,
      author = {Y. A. Wang and H. Adelson},
      title = {Representing Moving Images with Layers},
      journal = {TIP},
      year = {1994},
  }

  @InProceedings{Fradet09a,
    author = {Fradet, Matthieu and Robert, Philippe and P\'{e}rez, Patrick},
    Title = {Clustering point trajectories with various life-spans},
    BookTitle = {CVMP},
  year={2009}
  }





  @article{10.1109/ICCV.2001.10061,
  author = {Stella X. Yu and Jianbo Shi},
  title = {Segmentation with Pairwise Attraction and Repulsion},
  journal ={ICCV},
  Volume={75},
  year = {2001},
  }

  @article{1286005,
  author = {Wu, Bo and Nevatia, Ram},
  title = {Detection and Tracking of Multiple, Partially Occluded Humans by Bayesian Combination of Edgelet based Part Detectors},
  journal = {IJCV},
  year = {2007},
  }

  @inproceedings{bibbyeccv08,
    author = {C. Bibby and I. Reid},
    title = {Robust Real-Time Visual Tracking using Pixel-Wise Posteriors},
    booktitle={ECCV},
    year = "2008",
  }

  ]
  @InProceedings{BroxSegmentationCVPR11,
    author       = "Thomas Brox and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Object Segmentation by Alignment of Poselet Activations to Image Contours",
    booktitle    = "CVPR",
    year         = "2011"
  }

  @article{10.1109/ICCV.1995.466815,
  author = {J. Costeira and T. Kanade},
  title = {A multi-body factorization method for motion analysis},
  journal ={ICCV},
  year = {1995},
  }

  @inproceedings{Efros_2006_5395,
    author = "Bryan C. Russell and AlexeiA. Efros and Josef Sivic and William T. Freeman and Andrew Zisserman",
    title = "Using Multiple Segmentations to Discover Objects and their Extent in Image Collections",
    booktitle = "CVPR",
    year = "2006",
  }

  @inproceedings{malisiewicz-bmvc07,
    Author =	 {Tomasz Malisiewicz and Alexei A. Efros},
    Booktitle =	 {BMVC},
    Title =	 {Improving Spatial Support for Objects via Multiple Segmentations},
    Year =	 2007
  }

  @ARTICLE{1273918,
  author={Martin, D.R. and Fowlkes, C.C. and Malik, J.},
  journal={TPAMI},
  title={Learning to detect natural image boundaries using local brightness, color, and texture cues},
  year={2004},
  volume={26}
  }
@INPROCEEDINGS{Brox04highaccuracy,
    author = {Thomas Brox and Andrï¿œs Bruhn and Nils Papenberg and Joachim Weickert},
    title = {High Accuracy Optical Flow Estimation Based on a Theory for Warping},
    booktitle = {},
    year = {2004},
    pages = {25--36},
    publisher = {Springer}
}

 


  @INPROCEEDINGS{5539818,
  author={Bibby, C. and Reid, I.},
  booktitle={CVPR},
  title={Real-time tracking of multiple occluding objects using level sets},
  year={2010}}


  @inproceedings{Mitzel:2010:MTS:1886063.1886094,
  author = {Mitzel, Dennis and Horbert, Esther and Ess, Andreas and Leibe, Bastian},
  title = {Multi-person tracking with sparse detection and continuous segmentation},
  booktitle = {ECCV},
  year={2010}
  }

  @inproceedings{Mitzel:2011:MTS:1886063.1886094,
  author = {Mitzel, Dennis and Horbert, Esther and Ess, Andreas and Leibe, Bastian},
  title = {Level-Set Person Segmentation and Tracking with Multi-Region Appearemnce Models and Top-Down Shape Information},
  booktitle = {ICCV},
  series = {2011}
  }


  @InProceedings{lezama11,
    author = {Lezama, J. and Alahari, K. and Sivic, J. and Laptev, I.},
    title = {Track to the Future: Spatio-temporal Video Segmentation with Long-range Motion Cues},
    booktitle = {CVPR},
    year = {2011}
  }
  @InProceedings{shuwang2,
    author = {Shu Wang and Huchuan Lu and Fan Yang and Ming-Hsuan Yang},
    title = {Superpixel Tracking},
    booktitle = {ICCV},
    year = {2011}
  }
  @InProceedings{OB11,
    author       = "P.Ochs and T.Brox",
    title        = "Object segmentation in video: a hierarchical variational approach for turning point trajectories into dense regions",
    booktitle    = "ICCV",
    year         = "2011"}
  @incollection {springerlink:10.1007/978-3-642-15555-0_27,
    author = {Rahtu, Esa and Kannala, Juho and Salo, Mikko and Heikkilï¿œ, Janne},
    affiliation = {Machine Vision Group, University of Oulu, Finland},
    title = {Segmenting Salient Objects from Images and Videos},
    booktitle = {ECCV},
    year={2010},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }
@INPROCEEDINGS{Gall09motioncapture,
    author = {Juergen Gall and Carsten Stoll and Edilson De Aguiar and Christian Theobalt and Bodo Rosenhahn and Hans-peter Seidel and Mpi Informatik},
    title = {Motion capture using joint skeleton tracking and surface estimation},
    booktitle = {In IEEE Conf. on Computer Vision and Pattern Recognition},
    year = {2009}
}

  @Article{19146246,
  TITLE = {On the plausibility of the discriminant center-surround hypothesis for visual saliency.},
  AUTHOR = {Gao, Dashan and Mahadevan, Vijay and Vasconcelos, Nuno},
  journal = {Journal of vision},
  volume = {8},
  year = {2008}
  }


  @Article{Mahadevan10spatiotemporalsaliency,
      author = {Vijay Mahadevan and Nuno Vasconcelos},
      title = {Spatiotemporal Saliency in Dynamic Scenes},
      journal = {TPAMI},
      volume = {32},
      year = {2010},
  }


  @InProceedings{background_subtraction_free_camera,
    author = {Yaser Sheikh, Omar Javed, and Takeo Kanade},
    title = {Background Subtraction for Freely Moving Cameras},
    booktitle = {ICCV},
    year = {2009},
  }
  @conference{vondrick2010,
    title={Efficiently Scaling Up Video Annotation with Crowdsourced Marketplaces},
    author={Carl Vondrick and Deva Ramanan and Donald Patterson},
    booktitle={ECCV},
    year = {2010},
  }

  @conference{StellaRepulsion,
      author = {Stella X. Yu and Jianbo Shi},
      title = {Understanding Popout through Repulsion},
      booktitle= {CVPR},
      year={2001},
  }

  
  
  @article{DBLP:journals/corr/RanzatoSBMCC14,
  author    = {Marc'Aurelio Ranzato and
               Arthur Szlam and
               Joan Bruna and
               Micha{\"{e}}l Mathieu and
               Ronan Collobert and
               Sumit Chopra},
  title     = {Video (language) modeling: a baseline for generative models of natural
               videos},
  journal   = {CoRR},
  volume    = {abs/1412.6604},
  year      = {2014},
  url       = {http://arxiv.org/abs/1412.6604},
  timestamp = {Thu, 01 Jan 2015 19:51:08 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RanzatoSBMCC14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @article{10.1109/TPAMI.2009.167,
  author = {Pedro F. Felzenszwalb and Ross B. Girshick and David McAllester and Deva Ramanan},
  title = {Object Detection with Discriminatively Trained Part-Based Models},
  journal ={TPAMI},
    year = {2010},
  volume={32},
  }

@inproceedings{DBLP:conf/iccv/GirshickSKCF11,
  author    = {Ross B. Girshick and
               Jamie Shotton and
               Pushmeet Kohli and
               Antonio Criminisi and
               Andrew W. Fitzgibbon},
  title     = {Efficient regression of general-activity human poses from
               depth images},
  booktitle = {ICCV},
  year      = {2011},
  pages     = {415-422},
  ee        = {http://dx.doi.org/10.1109/ICCV.2011.6126270},
  crossref  = {DBLP:conf/iccv/2011},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


  @INPROCEEDINGS{Avidan05ensembletracking,
      author = {Shai Avidan},
      title = {Ensemble Tracking},
      booktitle = {CVPR},
      year = {2005},
  }

  @INPROCEEDINGS{planningtracking,
      author = {Haifeng Gong and Jack Simy and Maxim Likhachev and Jianbo Shi},
      title = {Multi-hypothesis Motion Planning for Visual Object Tracking},
      booktitle = {ICCV},
      year = {2011},
  }

  @incollection {SLIC,
    title={SLIC Superpixels},
    author={Radhakrishna Achanta and Appu Shaji and Kevin Smith and Aurelien Lucchi and Pascal Fua and Sabine Susstrunk},
    booktitle={EPFL Technical Report no. 149300, June 2010},
  }

  @incollection {springerlink:10.1007/978-3-540-88688-4_58,
    author = {Huang, Chang and Wu, Bo and Nevatia, Ramakant},
    title = {Robust Object Tracking by Hierarchical Association of Detection Responses},
    booktitle = {ECCV},
    year={2008},
  }

  @inproceedings{DBLP:conf/cvpr/CechS07,
    author    = {Jan Cech and Radim S{\'a}ra},
    title     = {Efficient Sampling of Disparity Space for Fast And Accurate Matching},
    booktitle = {CVPR},
    year      = {2007}
  }
  @inproceedings{DBLP:conf/iccv/PellegriniESG09,
    author    = {Stefano Pellegrini and
		Andreas Ess and
		Konrad Schindler and
		Luc J. Van Gool},
    title     = {You'll never walk alone: Modeling social behavior for multi-target
		tracking},
    booktitle = {ICCV},
    year      = {2009}
  }
  @INPROCEEDINGS{Yu02concurrentobject,
      author = {Stella X. Yu and Ralph Gross and Jianbo Shi},
      title = {Concurrent Object Recognition and Segmentation by Graph Partitioning},
      booktitle = {NIPS},
      year = {2002}
  }

  @InProceedings{eth_biwi_00483,
    author = {B. Leibe and N. Cornelis and K. Cornelis and L. Van Gool},
    title = {Dynamic 3D Scene Analysis from a Moving Vehicle},
    booktitle = {CVPR},
    year = {2007},
  }
@inproceedings{DBLP:conf/eccv/Black92,
  author    = {Michael J. Black},
  title     = {Combining Intensity and Motion for Incremental Segmentation
               and Tracking Over Long Image Sequences},
  booktitle = {ECCV},
  year      = {1992},
  pages     = {485-493},
  ee        = {http://dx.doi.org/10.1007/3-540-55426-2_54},
  crossref  = {DBLP:conf/eccv/1992},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}
  @article{10.1109/TPAMI.2010.143,
  author = {Thomas Brox and Jitendra Malik},
  title = {Large Displacement Optical Flow: Descriptor Matching in Variational Motion Estimation},
  journal ={TPAMI},
  year = {2010},

  }
  @inproceedings{citeulike:9244127,
      author = {Li, Yuan and Huang, Chang and Nevatia, R.},
    booktitle = {CVPR},
      title = {Learning to associate: HybridBoosted multi-target tracker for crowded scene},
      year = {2009}
  }


  @article {springerlink:10.1007/s11263-008-0136-6,
  title = {Particle Video: Long-Range Motion Estimation Using Point Trajectories},
    author = {Sand, Peter and Teller, Seth},
    affiliation = {MIT Computer Science and Artificial Intelligence Laboratory Cambridge MA 02139 USA},
    journal = {IJCV},
    year = {2008}
  }
  @INPROCEEDINGS{Dalal05histogramsof,
      author = {Navneet Dalal and Bill Triggs},
      title = {Histograms of Oriented Gradients for Human Detection},
      booktitle = {CVPR},
      year = {2005}
  }

  @InProceedings{yma,
    author = { Rao, S. and Tron, R. and Vidal, R. and Ma, Y. },
    title = {Motion segmentation via robust subspace separation in the presence of outlying, incomplete, or corrupted trajectories.},
    booktitle = {CVPR},
  year={2008},
  }

  @inproceedings{Grabner:2008:SOB:1478392.1478414,
  author = {Grabner, Helmut and Leistner, Christian and Bischof, Horst},
  title = {Semi-supervised On-Line Boosting for Robust Tracking},
  booktitle = {ECCV},
  year = {2008},
  }


  @inproceedings{citeulike:2085974,
      author = {Grabner , H. and Bischof, H.},
    title = {Online Boosting and Vision},
      booktitle = {CVPR},
      year = {2006}
  }

  @INPROCEEDINGS{5573752,
  author={Zhang Tao and Fei Shumin and Hu Gang},
  booktitle={Control Conference (CCC)},
  title={Target tracking with particle filter based on multiple cues fusion},
  year={2010}}

  @INPROCEEDINGS{Okuma04aboosted,
      author = {Kenji Okuma and Ali Taleghani and Nando De Freitas and O De Freitas and James J. Little and David G. Lowe},
      title = {A Boosted Particle Filter: Multitarget Detection and Tracking},
      booktitle = {ECCV},
      year = {2004},
  }


  @InProceedings{sparsesubsp,
    author = {Elhamifar, E. and Vidal, R.},
    title = {Sparse subspace clustering},
    booktitle = {CVPR},
    year = {2009}
  }




  @INPROCEEDINGS{BrostowCipollaCVPR2006,
    AUTHOR       = {Gabriel J. Brostow and Roberto Cipolla},
    TITLE        = {Unsupervised Bayesian Detection of Independent Motion in Crowds},
    BOOKTITLE    = {CVPR},
    YEAR         = {2006},
  }
  @article{GrundmannKwatra2010,
    author = {Matthias Grundmann and Vivek Kwatra and Mei Han and Irfan Essa},
    title = {Efficient Hierarchical Graph Based Video Segmentation},
    journal = {CVPR},
    year = {2010},
  }



  @incollection {mhvs,
    author = {Amelio Vazquez-Reina and Shai Avidan and Hanspeter Pfister and Eric Miller},
    title = {Multiple Hypothesis Video Segmentation from Superpixel Flows},
    booktitle = {ECCV},
  year={2010},
  }



  @article{phycho,
    author = {H. C. Nothdurft},
    title = {Feature analysis and the role of similarity in preattentive vision},
    journal = {Perception and Psychophysics},
    volume={52},
    year = {1992},
  }




  @article{commonfate,
    author = {M. Wertheimer},
    title = {Laws of organization in perceptual forms},
    journal = {A Sourcebook of Gestalt Psycycholgy (Partial translation)},
    year = {1938},
  }

  @INPROCEEDINGS{5206727,
  author={Chunhui Gu and Lim, J.J. and Arbelaez, P. and Malik, J.},
  booktitle={CVPR},
  year={2009},
  title={Recognition using regions},
  }
  @InProceedings{citeulike:942103,
      title = {Bottom-up/top-down image parsing by attribute graph grammar},
      author = {Han, Feng and Zhu, Song-Chun},
      journal = {ICCV},
  year={ 2005},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {CVPR},
    year={2009}
  }



  @InProceedings{Yan06general,
    title     = {A General Framework for Motion Segmentation: Independent, Articulated, Rigid, Non-rigid, Degenerate and Non-degenerate.},
    author = {J. Yan and M. Pollefeys},
    booktitle = {ECCV},
  year={2006},
  }

  @InProceedings{Ayer,
    title     = {Layered representation of motion video using robust maximum-likelihood estimation of mixture models and MDL encoding},
    author = {S. Ayer and H. S. Sawhney},
    booktitle = {ICCV},
  year={1995},
  }

  @article{101109CVPR2005335,
  author = {Deva Ramanan and D. A. Forsyth and Andrew Zisserman},
  title = {Strike a Pose: Tracking People by Finding Stylized Poses},
  journal ={CVPR},
  year = {2005},
  }

  @inproceedings{DBLP:conf/iccv/CheriyadatR09,
    author    = {Anil Cheriyadat and
		Richard J. Radke},
    title     = {Non-negative matrix factorization of partial track data
		for motion segmentation},
    booktitle = {ICCV},
    year      = {2009}
  }




  @inproceedings{Hoiem_2006_5467,
    author = "Derek Hoiem and Alexei Efros and Martial Hebert",
    title = "Putting Objects in Perspective",
    booktitle = "CVPR",
    year = "2006",
  }


  @Article{ Perse2009612,
  title = "A trajectory-based analysis of coordinated team activity in a basketball game",
  journal = "Computer Vision and Image Understanding",
  volume = "113",
  year = "2009",
  }

  @inproceedings{morariu11eventstructure,
    author    = {Vlad I. Morariu and Larry S. Davis},
    title     = {Multi-agent event recognition in structured scenarios.},
    booktitle = {CVPR},
    year      = {2011}
  }


  @inproceedings{storyline,
    author    = {Abhinav Gupta and Praveen Srinivasan and Jianbo Shi and Larry S. Davis},
    title     = {Understanding videos, constructing plots learning a visually grounded storyline model from annotated videos},
    booktitle = {CVPR},
    year      = {2009}
  }

  @inproceedings{benfold2011stable,
	  author = {Benfold, Ben and Reid, Ian},
	  title = {Stable Multi-Target Tracking in Real-Time Surveillance Video},
	  booktitle = {CVPR},
	  year = {2011}
  }


  @ARTICLE{790429,
  author={Wilson, A.D. and Bobick, A.F.},
  journal={TPAMI},
  title={Parametric hidden Markov models for gesture recognition},
  year={1999},
  volume={21}
  }



  @article{experts,
  author = {Terence D. Sanger and Robert A. Jacobs and Steven J. Nowlan and Geoffrey E. Hinton},
  title = {Adaptive Mixtures of Local Experts},
  journal = {Neural Computation},
  volume = {3},
  year = {1991}
  }


  @INPROCEEDINGS{lips,
  author={Bregler, C. and Omohundro, S.M.},
  booktitle={ICCV},
  title={Nonlinear manifold learning for visual speech recognition},
  year={1995}
  }



  @inproceedings{BN,
  author = {Shaogang Gong and Tao Xiang},
  title = {Recognition of Group Activities using Dynamic Probabilistic Networks},
  booktitle = {ICCV},
  year={2003}
  }


  @article{HMMMO,
  author = {Aaron F. Bobick and Andrew D. Wilson},
  title = {A State-Based Approach to the Representation and Recognition of Gesture},
  journal = {TPAMI},
  volume = {19}
  }

  @inproceedings{Brand:1997:CHM:794189.794420,
  author = {Brand, M. and Oliver, N. and Pentland, A.},
  title = {Coupled hidden Markov models for complex action recognition},
  booktitle = {CVPR},
  year = {1997}
  }

  @article{Ghahramani:1997:FHM:274158.274165,
  author = {Ghahramani, Zoubin and Jordan, Michael I.},
  title = {Factorial Hidden Markov Models},
  journal = {Mach. Learn.},
  volume = {29},
  year = {1997}
  }


  @INPROCEEDINGS{4270099,
  author={Laxton, B. and Jongwoo Lim and Kriegman, D.},
  booktitle={CVPR},
  title={Leveraging temporal, contextual and ordering constraints for recognizing complex activities in video},
  year={2007}
  }


  @article{DBLP:journals/jmlr/SiracusaF09,
    author    = {Michael Siracusa and John Fisher},
    title     = {Tractable Bayesian Inference of Time-Series Dependence Structure},
    journal   = {Journal of Machine Learning Research - Proceedings Track},
    volume    = {5},
    year      = {2009}
  }



  @article{parametrized,
  author = {Yaser Yacoob and Michael J. Black},
  title = {Parameterized Modeling and Recognition of Activities},
  journal = {Computer Vision and Image Understanding},
  volume = {73},
  year = {1999}
  }




  @inproceedings{Bobick:1995:STS:839277.840051,
  author = {Bobick, A. F. and Wilson, A. D.},
  title = {A state-based technique for the summarization and recognition of gesture},
  booktitle = {ICCV},
  year = {1995}
  }


  @inproceedings{Niebles:2010:MTS:1888028.1888059,
  author = {Niebles, Juan Carlos and Chen, Chih-Wei and Fei-Fei, Li},
  title = {Modeling temporal structure of decomposable motion segments for activity classification},
  booktitle = {ECCV},
  year = {2010}
  }


  @article{Hakeem:2007:LDR:1265999.1266287,
  author = {Hakeem, Asaad and Shah, Mubarak},
  title = {Learning, detection and representation of multi-agent events in videos},
  journal = {Artif. Intell.},
  volume = {171},
  year = {2007}
  }



  @INPROCEEDINGS{Zelnik-manor01event-basedanalysis,
      author = {Lihi Zelnik-manor and Michal Irani},
      title = {Event-based analysis of video},
      booktitle = {CVPR},
      year = {2001}
  }

  @inproceedings{Jebara:2007:SCE:1421665.1421685,
  author = {Jebara, Tony and Song, Yingbo and Thadani, Kapil},
  title = {Spectral Clustering and Embedding with Hidden Markov Models},
  booktitle = {European conference on Machine Learning},
  year = {2007}
  }
  @article{10.1109/CVPR.1997.609375,
  author = {Yair Weiss},
  title = {Smoothness in Layers: Motion segmentation using nonparametric mixture estimation.},
  journal ={CVPR},
  year={1997},

  }

  @article{ncut,
  author = {Jianbo Shi and Jitendra Malik},
  title = {Normalized Cuts and Image Segmentation},
  journal = {TPAMI},
  year = {2000},
  }


  @article{10.1109/TPAMI.2005.202,
  author = {Jiangjian Xiao and Mubarak Shah},
  title = {Motion Layer Extraction in the Presence of Occlusion Using Graph Cuts},
  journal ={TPAMI},
  year = {2005},
  }

  @article{1340323,
  author = {Pawan Kumar, M. and Torr, P. H. and Zisserman, A.},
  title = {Learning Layered Motion Segmentations of Video},
  journal = {IJCV},
  volume = {76},
  year = {2008},
  }



  @ARTICLE{Wang94representingmoving,
      author = {Y. A. Wang and H. Adelson},
      title = {Representing Moving Images with Layers},
      journal = {TIP},
      year = {1994},
  }

  @InProceedings{Fradet09a,
    author = {Fradet, Matthieu and Robert, Philippe and P\'{e}rez, Patrick},
    Title = {Clustering point trajectories with various life-spans},
    BookTitle = {CVMP},
  year={2009}
  }

@incollection{has,
year={2012},
booktitle={ECCV},
title={Has My Algorithm Succeeded? An Evaluator for Human Pose Estimators},
author={Jammalamadaka, Nataraj and Zisserman, Andrew and Eichner, Marcin and Ferrari, Vittorio and Jawahar, C.V.},

}




  @article{10.1109/ICCV.2001.10061,
  author = {Stella X. Yu and Jianbo Shi},
  title = {Segmentation with Pairwise Attraction and Repulsion},
  journal ={ICCV},
  Volume={75},
  year = {2001},
  }

  @article{1286005,
  author = {Wu, Bo and Nevatia, Ram},
  title = {Detection and Tracking of Multiple, Partially Occluded Humans by Bayesian Combination of Edgelet based Part Detectors},
  journal = {IJCV},
  year = {2007},
  }


  @inproceedings{DBLP:conf/iccv/CheriyadatR09,
    author    = {Anil Cheriyadat and
		Richard J. Radke},
    title     = {Non-negative matrix factorization of partial track data
		for motion segmentation},
    booktitle = {ICCV},
    year      = {2009},
    pages     = {865-872},
    ee        = {http://dx.doi.org/10.1109/ICCV.2009.5459311},
    crossref  = {DBLP:conf/iccv/2009},
    bibsource = {DBLP, http://dblp.uni-trier.de}
  }

  @article{Canny86,
      author = {Canny, J.},
      journal = {TPAMI},
      title = {{A Computational Approach to Edge Detection}},
      url = {http://dx.doi.org/10.1109/TPAMI.1986.4767851},
      volume = {PAMI-8},
      year = {1986}
  }

  @article{10.1109/ICCV.1995.466815,
  author = {J. Costeira and T. Kanade},
  title = {A multi-body factorization method for motion analysis},
  journal ={ICCV},
  year = {1995},
  }

  @ARTICLE{1273918,
  author={Martin, D.R. and Fowlkes, C.C. and Malik, J.},
  journal={TPAMI},
  title={Learning to detect natural image boundaries using local brightness, color, and texture cues},
  year={2004},
  volume={26}
  }

  @INPROCEEDINGS{139492,
  author={Perona, P. and Malik, J.},
  booktitle={ICCV},
  title={Detecting and localizing edges composed of steps, peaks and roofs },
  year={1990}
  }

 

  @incollection {springerlink:10.1007/978-3-642-15555-0_27,
    author = {Rahtu, Esa and Kannala, Juho and Salo, Mikko and Heikkilï¿œ, Janne},
    affiliation = {Machine Vision Group, University of Oulu, Finland},
    title = {Segmenting Salient Objects from Images and Videos},
    booktitle = {ECCV},
    year={2010},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }

  @Article{19146246,
  TITLE = {On the plausibility of the discriminant center-surround hypothesis for visual saliency.},
  AUTHOR = {Gao, Dashan and Mahadevan, Vijay and Vasconcelos, Nuno},
  journal = {Journal of vision},
  volume = {8},
  year = {2008}
  }


  @Article{Mahadevan10spatiotemporalsaliency,
      author = {Vijay Mahadevan and Nuno Vasconcelos},
      title = {Spatiotemporal Saliency in Dynamic Scenes},
      journal = {TPAMI},
      volume = {32},
      year = {2010},
  }


  @InProceedings{background_subtraction_free_camera,
    author = {Yaser Sheikh, Omar Javed, and Takeo Kanade},
    title = {Background Subtraction for Freely Moving Cameras},
    booktitle = {ICCV},
    year = {2009},
  }
  @conference{vondrick2010,
    title={Efficiently Scaling Up Video Annotation with Crowdsourced Marketplaces},
    author={Carl Vondrick and Deva Ramanan and Donald Patterson},
    booktitle={ECCV},
    year = {2010},
  }

  @conference{StellaRepulsion,
      author = {Stella X. Yu and Jianbo Shi},
      title = {Understanding Popout through Repulsion},
      booktitle= {CVPR},
      year={2001},
  }

  @article{10.1109/TPAMI.2009.167,
  author = {Pedro F. Felzenszwalb and Ross B. Girshick and David McAllester and Deva Ramanan},
  title = {Object Detection with Discriminatively Trained Part-Based Models},
  journal ={TPAMI},
    year = {2010},
  volume={32},
  }

  @inproceedings{Datta_2008_6037,
   author = "Ankur Datta and Yaser Ajmal Sheikh and Takeo Kanade",
   title = "Linear Motion Estimation for Systems of Articulated Planes",
   booktitle = "IEEE Conference on Computer Vision and Pattern Recognition",
   month = "June",
   year = "2008",
}

@INPROCEEDINGS{motionperception,
    author = {Gunnar Johansson},
    title = {Visual perception of biological motion and a model for its analysis},
    booktitle = {Percept. Psychophys.},
    year = {1973},
    volume={14},
    pages = {201--211}
}

@article{Sigal:2012:LPE:2205801.2205829,
 author = {Sigal, Leonid and Isard, Michael and Haussecker, Horst and Black, Michael J.},
 title = {Loose-limbed People: Estimating {3D} Human Pose and Motion Using Non-parametric Belief Propagation},
 journal = {IJCV},
 volume = {98},
 year = {2012}
}
@inproceedings{conf/cvpr/SappWT11,
  added-at = {2011-08-23T00:00:00.000+0200},
  author = {Sapp, Benjamin and Weiss, David and Taskar, Ben},
  booktitle = {CVPR},
  title = {Parsing human motion with stretchable models.},
  year = 2011
}





@inproceedings{DBLP:conf/fgr/JuBY96,
  author    = {Shanon X. Ju and
               Michael J. Black and
               Yaser Yacoob},
  title     = {Cardboard People: A Parameterized Model of Articulated Image
               Motion},
  booktitle = {FG},
  year      = {1996},
}

@InProceedings{Bro06k,
  author       = "T. Brox and B. Rosenhahn and D. Cremers and H.-P. Seidel",
  title        = "High accuracy optical flow serves 3-D pose tracking: exploiting contour and flow based constraints",
  booktitle    = "ECCV",
  year         = "2006"
}

  @incollection {SLIC,
    title={SLIC Superpixels},
    author={Radhakrishna Achanta and Appu Shaji and Kevin Smith and Aurelien Lucchi and Pascal Fua and Sabine Susstrunk},
    booktitle={EPFL Technical Report no. 149300, June 2010},
  }

  @incollection {springerlink:10.1007/978-3-540-88688-4_58,
    author = {Huang, Chang and Wu, Bo and Nevatia, Ramakant},
    title = {Robust Object Tracking by Hierarchical Association of Detection Responses},
    booktitle = {ECCV},
    year={2008},
  }

  @InProceedings{eth_biwi_00483,
    author = {B. Leibe and N. Cornelis and K. Cornelis and L. Van Gool},
    title = {Dynamic 3D Scene Analysis from a Moving Vehicle},
    booktitle = {CVPR},
    year = {2007},
  }

  @article{10.1109/TPAMI.2010.143,
  author = {Thomas Brox and Jitendra Malik},
  title = {Large Displacement Optical Flow: Descriptor Matching in Variational Motion Estimation},
  journal ={TPAMI},
  year = {2010},

  }


  @article {springerlink:10.1007/s11263-008-0136-6,
  title = {Particle Video: Long-Range Motion Estimation Using Point Trajectories},
    author = {Sand, Peter and Teller, Seth},
    affiliation = {MIT Computer Science and Artificial Intelligence Laboratory Cambridge MA 02139 USA},
    journal = {IJCV},
    year = {2008}
  }

  @InProceedings{yma,
    author = { Rao, S. and Tron, R. and Vidal, R. and Ma, Y. },
    title = {Motion segmentation via robust subspace separation in the presence of outlying, incomplete, or corrupted trajectories.},
    booktitle = {CVPR},
  year={2008},
  }



  @InProceedings{sparsesubsp,
    author = {Elhamifar, E. and Vidal, R.},
    title = {Sparse subspace clustering},
    booktitle = {CVPR},
    year = {2009}
  }




  @INPROCEEDINGS{BrostowCipollaCVPR2006,
    AUTHOR       = {Gabriel J. Brostow and Roberto Cipolla},
    TITLE        = {Unsupervised Bayesian Detection of Independent Motion in Crowds},
    BOOKTITLE    = {CVPR},
    YEAR         = {2006},
  }
  @article{GrundmannKwatra2010,
    author = {Matthias Grundmann and Vivek Kwatra and Mei Han and Irfan Essa},
    title = {Efficient Hierarchical Graph Based Video Segmentation},
    journal = {CVPR},
    year = {2010},
  }



  @incollection {mhvs,
    author = {Amelio Vazquez-Reina and Shai Avidan and Hanspeter Pfister and Eric Miller},
    title = {Multiple Hypothesis Video Segmentation from Superpixel Flows},
    booktitle = {ECCV},
  year={2010},
  }
  @INPROCEEDINGS{4761133,
  author={Izadi, M. and Saeedi, P.},
  booktitle={Pattern Recognition, 2008. ICPR 2008. 19th International Conference on},
  title={Robust region-based background subtraction and shadow removing using color and gradient information},
  year={2008}
  }

  @INPROCEEDINGS{784637,
  author={Stauffer, C. and Grimson, W.E.L.},
  booktitle={CVPR},
  title={Adaptive background mixture models for real-time tracking},
  year={1999}}


  @inproceedings{Zivkovic:2004:IAG:1018428.1020644,
  author = {Zivkovic, Zoran},
  title = {Improved Adaptive Gaussian Mixture Model for Background Subtraction},
  booktitle = {ICPR},
  year = {2004}
  }


  @article{Felzenszwalb:2004:EGI:981793.981796,
  author = {Felzenszwalb, Pedro F. and Huttenlocher, Daniel P.},
  title = {Efficient Graph-Based Image Segmentation},
  journal = {IJCV},
  volume = {59},
  year = {2004}
  }

  @article{phycho,
    author = {H. C. Nothdurft},
    title = {Feature analysis and the role of similarity in preattentive vision},
    journal = {Perception and Psychophysics},
    volume={52},
    year = {1992},
  }

  @inproceedings{DBLP:conf/eccv/Ren08,
    author    = {Xiaofeng Ren},
    title     = {Multi-scale Improves Boundary Detection in Natural Images},
    booktitle = {ECCV (3)},
    year      = {2008},
    pages     = {533-545},
    ee        = {http://dx.doi.org/10.1007/978-3-540-88690-7_40},
    crossref  = {DBLP:conf/eccv/2008-3},
    bibsource = {DBLP, http://dblp.uni-trier.de}
  }


@article{DBLP:journals/corr/BalogGBNT16,
  author    = {Matej Balog and
               Alexander L. Gaunt and
               Marc Brockschmidt and
               Sebastian Nowozin and
               Daniel Tarlow},
  title     = {DeepCoder: Learning to Write Programs},
  journal   = {CoRR},
  volume    = {abs/1611.01989},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.01989},
  archivePrefix = {arXiv},
  eprint    = {1611.01989},
  timestamp = {Wed, 07 Jun 2017 14:43:01 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/BalogGBNT16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @INPROCEEDINGS{5206727,
  author={Chunhui Gu and Lim, J.J. and Arbelaez, P. and Malik, J.},
  booktitle={CVPR},
  year={2009},
  title={Recognition using regions},
  }
  @InProceedings{citeulike:942103,
      title = {Bottom-up/top-down image parsing by attribute graph grammar},
      author = {Han, Feng and Zhu, Song-Chun},
      journal = {ICCV},
  year={ 2005},
  }

  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }

  @InProceedings{Yan06general,
    title     = {A General Framework for Motion Segmentation: Independent, Articulated, Rigid, Non-rigid, Degenerate and Non-degenerate.},
    author = {J. Yan and M. Pollefeys},
    booktitle = {ECCV},
  year={ 2006},
  }
@inproceedings{Datta_2008_6037,
   author = "Ankur Datta and Yaser Ajmal Sheikh and Takeo Kanade",
   title = "Linear Motion Estimation for Systems of Articulated Planes",
   booktitle = "IEEE Conference on Computer Vision and Pattern Recognition",
   month = "June",
   year = "2008",
}

  @InProceedings{Ayer,
    title     = {Layered representation of motion video using robust maximum-likelihood estimation of mixture models and MDL encoding},
    author = {S. Ayer and H. S. Sawhney},
    booktitle = {ICCV},
  year={ 1995}
  }

  @article{10.1109/CVPR.2005.335,
  author = {Deva Ramanan and D. A. Forsyth and Andrew Zisserman},
  title = {Strike a Pose: Tracking People by Finding Stylized Poses},
  journal ={CVPR},
  year = {2005}
  }









@inproceedings{SheikhNIPS2008,
   author = "Ijaz Akhter and Yaser Ajmal Sheikh and Sohaib Khan and Takeo Kanade",
   title = "Nonrigid Structure from Motion in Trajectory Space",
   booktitle = "NIPS",
   year = "2008"
} 


  @Article{ Perse2009612,
  title = "A trajectory-based analysis of coordinated team activity in a basketball game",
  journal = "Computer Vision and Image Understanding",
  volume = "113",
  year = "2009"
  }

  @inproceedings{morariu11eventstructure,
    author    = {Vlad I. Morariu and Larry S. Davis},
    title     = {Multi-agent event recognition in structured scenarios.},
    booktitle = {CVPR},
    year      = {2011}
  }


  @inproceedings{storyline,
    author    = {Abhinav Gupta and Praveen Srinivasan and Jianbo Shi and Larry S. Davis},
    title     = {Understanding videos, constructing plots learning a visually grounded storyline model from annotated videos},
    booktitle = {CVPR},
    year      = {2009}
  }


  @ARTICLE{790429,
  author={Wilson, A.D. and Bobick, A.F.},
  journal={TPAMI},
  title={Parametric hidden Markov models for gesture recognition},
  year={1999},
  volume={21}
  }



  @article{experts,
  author = {Terence D. Sanger and Robert A. Jacobs and Steven J. Nowlan and Geoffrey E. Hinton},
  title = {Adaptive Mixtures of Local Experts},
  journal = {Neural Computation},
  volume = {3},
  year = {1991}
  }

@article{anonymous2018zero-shot,
  title={Zero-Shot Visual Imitation},
  author={Anonymous},
  journal={International Conference on Learning Representations},
  year={2018},
  url={https://openreview.net/forum?id=BkisuzWRW}
}


  @INPROCEEDINGS{lips,
  author={Bregler, C. and Omohundro, S.M.},
  booktitle={ICCV},
  title={Nonlinear manifold learning for visual speech recognition},
  year={1995}
  }



  @inproceedings{BN,
  author = {Shaogang Gong and Tao Xiang},
  title = {Recognition of Group Activities using Dynamic Probabilistic Networks},
  booktitle = {ICCV},
  year={2003}
  }


  @article{HMMMO,
  author = {Aaron F. Bobick and Andrew D. Wilson},
  title = {A State-Based Approach to the Representation and Recognition of Gesture},
  journal = {TPAMI},
  volume = {19}
  }

  @inproceedings{Brand:1997:CHM:794189.794420,
  author = {Brand, M. and Oliver, N. and Pentland, A.},
  title = {Coupled hidden Markov models for complex action recognition},
  booktitle = {CVPR},
  year = {1997}
  }

  @article{Ghahramani:1997:FHM:274158.274165,
  author = {Ghahramani, Zoubin and Jordan, Michael I.},
  title = {Factorial Hidden Markov Models},
  journal = {Mach. Learn.},
  volume = {29},
  year = {1997}
  }


  @INPROCEEDINGS{4270099,
  author={Laxton, B. and Jongwoo Lim and Kriegman, D.},
  booktitle={CVPR},
  title={Leveraging temporal, contextual and ordering constraints for recognizing complex activities in video},
  year={2007}
  }


  @article{DBLP:journals/jmlr/SiracusaF09,
    author    = {Michael Siracusa and John Fisher},
    title     = {Tractable Bayesian Inference of Time-Series Dependence Structure},
    journal   = {Journal of Machine Learning Research - Proceedings Track},
    volume    = {5},
    year      = {2009}
  }



  @article{parametrized,
  author = {Yaser Yacoob and Michael J. Black},
  title = {Parameterized Modeling and Recognition of Activities},
  journal = {Computer Vision and Image Understanding},
  volume = {73},
  year = {1999}
  }




  @inproceedings{Bobick:1995:STS:839277.840051,
  author = {Bobick, A. F. and Wilson, A. D.},
  title = {A state-based technique for the summarization and recognition of gesture},
  booktitle = {ICCV},
  year = {1995}
  }

  @inproceedings{Xu:2008:SBV:1478392.1478446,
  author = {Xu, Li and Chen, Jianing and Jia, Jiaya},
  title = {A Segmentation Based Variational Model for Accurate Optical Flow Estimation},
  booktitle = {ECCV},
  year = {2008}
  }

  @inproceedings{Niebles:2010:MTS:1888028.1888059,
  author = {Niebles, Juan Carlos and Chen, Chih-Wei and Fei-Fei, Li},
  title = {Modeling temporal structure of decomposable motion segments for activity classification},
  booktitle = {ECCV},
  year = {2010}
  }

  @InProceedings{Bro11c,
    author       = "P. Sundberg and T. Brox and M. Maire and P. Arbelaez and J. Malik",
    title        = "Occlusion boundary detection and figure/ground assignment from optical flow",
    booktitle    = "CVPR",
    year         = "2011"
  }

  @inproceedings{Stein_2007_5836,
    author = "Andrew Stein and Derek Hoiem and Martial Hebert",
    title = "Learning to Find Object Boundaries Using Motion Cues",
    booktitle = "IEEE International Conference on Computer Vision (ICCV)",
    month = "October",
    year = "2007",
    Notes = "Dataset available from http://www.cs.cmu.edu/~stein/occlusion_data"
  }
  
  @inproceedings{Zhou2015EndtoendLO,
  title={End-to-end learning of semantic role labeling using recurrent neural networks},
  author={Jie Zhou and Wei Xu},
  booktitle={ACL},
  year={2015}
}


  @article{Hakeem:2007:LDR:1265999.1266287,
  author = {Hakeem, Asaad and Shah, Mubarak},
  title = {Learning, detection and representation of multi-agent events in videos},
  journal = {Artif. Intell.},
  volume = {171},
  year = {2007}
  }


  
  @INPROCEEDINGS{Zelnik-manor01event-basedanalysis,
      author = {Lihi Zelnik-manor and Michal Irani},
      title = {Event-based analysis of video},
      booktitle = {CVPR},
      year = {2001}
  }

  @inproceedings{Jebara:2007:SCE:1421665.1421685,
  author = {Jebara, Tony and Song, Yingbo and Thadani, Kapil},
  title = {Spectral Clustering and Embedding with Hidden Markov Models},
  booktitle = {European conference on Machine Learning},
  year = {2007}
  }

  @article{Jebara:2004:PPK:1005332.1016786,
  author = {Jebara, Tony and Kondor, Risi and Howard, Andrew},
  title = {Probability Product Kernels},
  journal = {J. Mach. Learn. Res.},
  volume = {5},
  year = {2004}
  }

  @INPROCEEDINGS{Gong99recognitionof,
      author = {Shaogang Gong and Michael Walter},
      title = {Recognition of Temporal Structures: Learning Prior and Propagating Observation Augmented Densities via Hidden Markov States},
      booktitle = {ICCV},
      year = {1999},
  }

  @article{Brand:2000:DSA:351581.351608,
  author = {Brand, Matthew and Kettnaker, Vera},
  title = {Discovery and Segmentation of Activities in Video},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }


  @INPROCEEDINGS{Brown01productsof,
      author = {Andrew D. Brown and Andrew D. Brown and Geoffrey E. Hinton and Geoffrey E. Hinton},
      title = {Products of Hidden Markov Models},
      booktitle = {In Proceedings of Artificial Intelligence and Statistics},
      year = {2001},
  }


  @inproceedings{malisiewicz-nips09,
    Author =	 {Tomasz Malisiewicz and Alexei A. Efros},
    Booktitle =	 {NIPS},
    Title =	 {Beyond Categories: The Visual Memex Model for Reasoning About Object Relationships},
    Year =	 2009
  }


  @inproceedings{yamato,
  author = {J. Yamato and J. Ohya and K. Ishii},
  title = {Recognizing human action in time-sequential images using a hidden Markov model},
  booktitle = {CVPR},
  year = {1994},
  }



  @INPROCEEDINGS{Elgammal04separatingstyle,
      author = {Ahmed Elgammal and Chan-su Lee},
      title = {Separating style and content on a nonlinear manifold},
      booktitle = {CVPR},
      year = {2004}
  }

  @INPROCEEDINGS{Tenenbaum97separatingstyle,
      author = {Joshua B. Tenenbaum and William T. Freeman},
      title = {Separating style and content},
      booktitle = {In Advances in neural},
      year = {1997}
  }

  @inproceedings{DBLP:conf/cvpr/LvN07,
    author    = {Fengjun Lv and
		Ramakant Nevatia},
    title     = {Single View Human Action Recognition using Key Pose Matching and Viterbi Path Searching},
    booktitle = {CVPR},
    year      = {2007}
  }


  @inproceedings { 158,
	  title = {Linear Embeddings in Non-Rigid Structure From Motion},
	  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	  year = {2009},
	  address = {Miami, FL},
	  author = {Vincent Rabaud and Serge Belongie}
  }



  @INPROCEEDINGS{4270260,
  author={Goh, A. and Vidal, R.},
  booktitle={CVPR},
  title={Segmenting Motions of Different Types by Unsupervised Manifold Clustering},
  year={2007},
  }


  @incollection {springerlink:10.1007/11551188_37,
    author = {Wang, Fei and Zhang, Changshui},
    title = {Spectral Clustering for Time Series},
    booktitle = {Pattern Recognition and Data Mining},
    volume = {3686},
    year = {2005}
  }

  @INPROCEEDINGS{4587385,
  author={Xiaozhe Wang and Liang Wang and Wirth, A.},
  booktitle={CVPR},
  title={Pattern discovery in motion time series via structure-based spectral clustering},
  year={2008}
  }


  @article{Stauffer:2000:LPA:351581.351588,
  author = {Stauffer, Chris and Grimson, W. Eric L.},
  title = {Learning Patterns of Activity Using Real-Time Tracking},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }

  @incollection{Nanopoulos:2001:FCT:766914.766918,
  author = {Nanopoulos, Alex and Alcock, Rob and Manolopoulos, Yannis},
  title = {Information processing and technology},
  year = {2001},
  }

  BibTeX | EndNote | ACM Ref

  @inproceedings{Shi:2006:LTS:1153171.1153641,
  author = {Shi, Yifan and Bobick, Aaron and Essa, Irfan},
  title = {Learning Temporal Sequence Model from Partially Labeled Data},
  booktitle = {CVPR},
  year = {2006}
  }


  @article{Murase,
  author = {Murase, Hiroshi and Nayar, Shree K.},
  title = {Visual learning and recognition of 3-D objects from appearance},
  journal = {IJCV},
  volume = {14},
  year = {1995}
  }


  @INPROCEEDINGS{698609,
  author={Bobick, A.F. and Ivanov, Y.A.},
  booktitle={CVPR},
  title={Action recognition using probabilistic parsing},
  year={1998}
  }

  @inproceedings{Ryoo:2006:RCH:1153171.1153651,
  author = {Ryoo, M. S. and Aggarwal, J. K.},
  title = {Recognition of Composite Human Activities through Context-Free Grammar Based Representation},
  booktitle = {CVPR},
  year = {2006}
  }


  @INPROCEEDINGS{Hadsell06dimensionalityreduction,
      author = {Raia Hadsell and Sumit Chopra and Yann Lecun},
      title = {Dimensionality reduction by learning an invariant mapping},
      booktitle = {CVPR},
      year = {2006}
  }


  @incollection{NIPS2010_0893,
  title = {Pose-Sensitive Embedding by Nonlinear NCA Regression},
  author = {Graham Taylor and Rob Fergus and George Williams and Ian Spiro and Christoph Bregler},
  booktitle = {NIPS},
  year = {2010}
  }
  @InProceedings{lezama11,
    author = {Lezama, J. and Alahari, K. and Sivic, J. and Laptev, I.},
    title = {Track to the Future: Spatio-temporal Video Segmentation with Long-range Motion Cues},
    booktitle = {CVPR},
    year = {2011}
  }
  @InProceedings{shuwang2,
    author = {Shu Wang and Huchuan Lu and Fan Yang and Ming-Hsuan Yang},
    title = {Superpixel Tracking},
    booktitle = {ICCV},
    year = {2011}
  }
  @InProceedings{OB11,
    author       = "P.Ochs and T.Brox",
    title        = "Object segmentation in video: a hierarchical variational approach for turning point trajectories into dense regions",
    booktitle    = "IEEE International Conference on Computer Vision (ICCV)",
    year         = "2011",
    url          = "http://lmb.informatik.uni-freiburg.de/Publications/2011/OB11"
  }

  @InProceedings{raptisS10,
    author = 	{Raptis, M. and Soatto, S.},
    title = 	{Tracklet Descriptors for Action Modeling and Video Analysis},
    booktitle = 	{ECCV},
    year = 	{2010}
  }


  @book{Fukunaga:1990:ISP:92131,
  author = {Fukunaga, Keinosuke},
  title = {Introduction to statistical pattern recognition (2nd ed.)},
  year = {1990}
  }


  @ARTICLE{Roweis00nonlineardimensionality,
      author = {Sam T. Roweis and Lawrence K. Saul},
      title = {Nonlinear dimensionality reduction by locally linear embedding},
      journal = {SCIENCE},
      year = {2000},
      volume = {290}
  }

  @article{Turk_Pentland_1991,
  title={Face recognition using eigenfaces},
  journal={CVPR},
  year={1991}
  }


  @INPROCEEDINGS{Laptev03space-timeinterest,
      author = {Ivan Laptev and Tony Lindeberg},
      title = {Space-time Interest Points},
      booktitle = {ICCV},
      year = {2003}
  }


  @INPROCEEDINGS{Kim07r.:tensor,
      author = {Tae-kyun Kim and Shu-fai Wong and Roberto Cipolla},
      title = {Tensor Canonical Correlation Analysis for Action Classification},
      booktitle = {CVPR},
      year = {2007}
  }


  @inproceedings{Fragkiadaki:topology,
  author = {Fragkiadaki, Katerina and Shi, Jianbo},
  title = {Exploiting Motion and Topology for Segmenting and tracking Under Entanglement.},
  booktitle = {CVPR},
  year = {2011},
  }

  @INPROCEEDINGS{Jianbo03multiclassspectral,
      author = {Yu,Stella and Shi, Jianbo},
      title = {Multiclass Spectral Clustering},
      booktitle = {ICCV},
      year = {2003}
  }



  @INPROCEEDINGS{lu_cvpr2011,
      author = {Wei-Lwun Lu and Jo-Anne Ting and Kevin P. Murphy and James J. Little},
      booktitle = {Identifying Players in Broadcast Sports Videos using Conditional Random Fields},
      journal = {Proceedings of the 2011 IEEE Conference on Computer Vision and Pattern Recognition},
      year = {2011}
  }

  @article{DBLP:journals/pami/BoykovVZ01,
    author    = {Yuri Boykov and Olga Veksler and Ramin Zabih},
    title     = {Fast Approximate Energy Minimization via Graph Cuts},
    journal   = {TPAMI},
    volume    = {23},
    year      = {2001}
  }

  @article{GEAN:GEAN31,
  author = {Matula, David W. and Sokal, Robert R.},
  title = {Properties of Gabriel Graphs Relevant to Geographic Variation Research and the Clustering of Points in the Plane},
  journal = {Geographical Analysis},
  volume = {12},
  year = {1980}
  }


  @INPROCEEDINGS{global_Pb,
  AUTHOR = {Michael Maire and Pablo Arbelaez and Charless Fowlkes and Jitendra Malik},
  TITLE = {Using contours to detect and localize junctions in natural images.},
  booktitle = {CVPR},
  YEAR = {2008}
  }


  @inproceedings{Yu:2010:AIO:1873951.1874105,
  author = {Yu, Haonan and Li, Jia and Tian, Yonghong and Huang, Tiejun},
  title = {Automatic interesting object extraction from images using complementary saliency maps},
  booktitle = {Proceedings of the international conference on Multimedia},
  year = {2010}
  }
  @inproceedings{DBLP:conf/accv/DonoserRB09,
    author    = {Michael Donoser and Hayko Riemenschneider and  Horst Bischof},
    title     = {Efficient Partial Shape Matching of Outer Contours},
    booktitle = {ACCV},
    year      = {2009}
  }

  @inproceedings{RenFM05a,
	  author = "Xiaofeng Ren and Charless C. Fowlkes and Jitendra Malik",
	  title = "Scale-invariant contour completion using conditional random fields",
	  booktitle = {ICCV},
	  year = "2005"
	  }
@inproceedings{RenMalik07,
        author = "Xiaofeng Ren and Jitendra Malik",
        title = "Tracking as Repeated Figure/Ground Segmentation",
        booktitle = {Proc. IEEE Conf. Comput. Vision and Pattern Recogn.},
        year = "2007"
        }

@InProceedings{Buehler08,
   author = "Buehler, P. and Everingham, M. and Huttenlocher, D.~P. and Zisserman, A.",
   title = "Long Term Arm and Hand Tracking for Continuous Sign Language {TV} Broadcasts",
   booktitle = "Proceedings of the British Machine Vision Conference",
   year = "2008",
}


@inproceedings{DBLP:conf/iccv/IonescuLS11,
  author    = {Catalin Ionescu and
               Fuxin Li and
               Cristian Sminchisescu},
  title     = {Latent structured models for human pose estimation},
  booktitle = {ICCV},
  year      = {2011}
}

@inproceedings{Bray:2006:PSS:2168483.2168541,
 author = {Bray, Matthieu and Kohli, Pushmeet and Torr, Philip H. S.},
 title = {POSECUT: simultaneous segmentation and 3D pose estimation of humans using dynamic graph-cuts},
 booktitle = {ECCV},
 year = {2006}
}
@inproceedings{Dalal:2006:HDU:2168483.2168522,
 author = {Dalal, Navneet and Triggs, Bill and Schmid, Cordelia},
 title = {Human detection using oriented histograms of flow and appearance},
 series = {ECCV},
 year = {2006}
} 


@inproceedings{DBLP:conf/cvpr/GkioxariABM13,
  author    = {Georgia Gkioxari and
               Pablo Arbelaez and
               Lubomir D. Bourdev and
               Jitendra Malik},
  title     = {Articulated Pose Estimation Using Discriminative Armlet
               Classifiers},
  booktitle = {CVPR},
  year      = {2013}
}
@inproceedings {Pishchulin2013cvpr,
	title = {Poselet Conditioned Pictorial Structures},
	booktitle = {CVPR},
	year = {2013},
	author = {Leonid Pishchulin and Mykhaylo Andriluka and Peter Gehler and Schiele, Bernt}
}


@INPROCEEDINGS{5540232,
author={Karlinsky, L. and Dinerstein, M. and Harari, D. and Ullman, S.},
booktitle={CVPR},
title={The chains model for detecting parts by their context},
year={2010}}
@article{DBLP:journals/pami/FelzenszwalbGMR10,
  author    = {Pedro F. Felzenszwalb and
               Ross B. Girshick and
               David A. McAllester and
               Deva Ramanan},
  title     = {Object Detection with Discriminatively Trained Part-Based
               Models},
  journal   = {IEEE Trans. Pattern Anal. Mach. Intell.},
  volume    = {32},
  number    = {9},
  year      = {2010},
  pages     = {1627-1645},
  ee        = {http://doi.ieeecomputersociety.org/10.1109/TPAMI.2009.167},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Gaidon:Virtual:CVPR2016,
    author = {Gaidon, A and Wang, Q and Cabon, Y and Vig, E},
    title = {Virtual Worlds as Proxy for Multi-Object Tracking Analysis},
    booktitle = {CVPR},
    year = {2016}
}


@inproceedings{parkhi11truth,
  Author    = {O. M. Parkhi and A. Vedaldi and C. V. Jawahar and A. Zisserman},
  Title     = {The Truth About Cats and Dogs},
  Booktitle = {Proceedings of the International
               Conference on Computer Vision ({ICCV})},
  Year      = {2011}}

@INPROCEEDINGS{6248070,
author={Qieyun Dai and Hoiem, D.},
booktitle={Computer Vision and Pattern Recognition (CVPR), 2012 IEEE Conference on}, title={Learning to localize detected objects},
year={2012},
pages={3322-3329},
keywords={image segmentation;learning (artificial intelligence);object detection;bounding box overlap;color models;edge cues;initial detector;learned graph cut segmentation;learning;object detection localization;pixel assignment;structural bounding box prediction;Color;Computational modeling;Detectors;Image color analysis;Image edge detection;Shape;Training},
doi={10.1109/CVPR.2012.6248070},
ISSN={1063-6919},}

@inproceedings{Karlinsky:2012:ULF:24030722403098,
 author = {Karlinsky, Leonid and Ullman, Shimon},
 title = {Using linking features in learning non-parametric part models},
 booktitle = {Proceedings of the 12th European conference on Computer Vision - Volume Part III},
 series = {ECCV'12},
 year = {2012},
 isbn = {978-3-642-33711-6},
 location = {Florence, Italy},
 pages = {326--339},
 numpages = {14},
 url = {http://dx.doi.org/10.1007/978-3-642-33712-3_24},
 doi = {10.1007/978-3-642-33712-3_24},
 acmid = {2403098},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
 keywords = {FLPM model, linking features, parts detection},
}




  @TechReport{RenFM05tech,
	  author = "Xiaofeng Ren and Charless C. Fowlkes and Jitendra Malik",
	  title = "Mid-level cues improve boundary detection",
	  institution =  {UC Berkeley},
	  number =       {UCB//CSD-05-1382},
	  year =         {2005}
	  }

  @InProceedings{BroxSegmentationCVPR11,
    author       = "Thomas Brox and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Object Segmentation by Alignment of Poselet Activations to Image Contours",
    booktitle    = "IEEE International Conference on Computer Vision and Pattern Recognition (CVPR)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }
  @InProceedings{HariharanSemanticContoursICCV11,
    author       = "Bharath Hariharan and Pablo Arbelaez and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Semantic Contours from Inverse Detectors",
    booktitle    = "International Conference on Computer Vision (ICCV)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }
  @inproceedings{DBLP:conf/eccv/RiemenschneiderDB10,
    author    = {Hayko Riemenschneider and Michael Donoser and Horst Bischof},
    title     = {Using Partial Edge Contour Matches for Efficient Object
		Category Localization},
    booktitle = {ECCV},
    year      = {2010}
  }

  @inproceedings{ArbelaezMFM_CVPR_2009,
      author = "Arbelaez, Pablo and Maire, Michael and Fowlkes, Charless C. and Malik, Jitendra",
      booktitle = "CVPR",
      year = "2009",
      title = "From Contours to Regions: An Empirical Evaluation"
  }

@incollection{NIPS2014_5349,
title = {Learning Deep Features for Scene Recognition using Places Database},
author = {Zhou, Bolei and Lapedriza, Agata and Xiao, Jianxiong and Torralba, Antonio and Oliva, Aude},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {487--495},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5349-learning-deep-features-for-scene-recognition-using-places-database.pdf}
}

  @inproceedings{MoriREM04,
	  author = "Greg Mori and Xiaofeng Ren and Alexei A. Efros and Jitendra Malik",
	  title = "Recovering human body configurations: combining segmentation and recognition.",
	  booktitle = {Proc. IEEE Conf. Comput. Vision and Pattern Recogn.},
	  volume = 2,
	  pages = "326-333",
	  year = "2004",
	  }



  @inproceedings{Latecki2010,
    author    = {Tianyang Ma and Longin Jan Latecki},
    title     = { From Partial Shape Matching through Local Deformation to Robust Global Shape Similarity for Object Detection},
    booktitle = {CVPR},
    year      = {2011}
  }
  @article{Jebara:2004:PPK:1005332.1016786,
  author = {Jebara, Tony and Kondor, Risi and Howard, Andrew},
  title = {Probability Product Kernels},
  journal = {J. Mach. Learn. Res.},
  volume = {5},
  year = {2004}
  }

  @INPROCEEDINGS{Gong99recognitionof,
      author = {Shaogang Gong and Michael Walter},
      title = {Recognition of Temporal Structures: Learning Prior and Propagating Observation Augmented Densities via Hidden Markov States},
      booktitle = {ICCV},
      year = {1999},
  }

  @article{Brand:2000:DSA:351581.351608,
  author = {Brand, Matthew and Kettnaker, Vera},
  title = {Discovery and Segmentation of Activities in Video},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }


  @INPROCEEDINGS{Brown01productsof,
      author = {Andrew D. Brown and Andrew D. Brown and Geoffrey E. Hinton and Geoffrey E. Hinton},
      title = {Products of Hidden Markov Models},
      booktitle = {In Proceedings of Artificial Intelligence and Statistics},
      year = {2001},
  }


  @inproceedings{malisiewicz-nips09,
    Author =	 {Tomasz Malisiewicz and Alexei A. Efros},
    Booktitle =	 {NIPS},
    Title =	 {Beyond Categories: The Visual Memex Model for Reasoning About Object Relationships},
    Year =	 2009
  }


  @inproceedings{yamato,
  author = {J. Yamato and J. Ohya and K. Ishii},
  title = {Recognizing human action in time-sequential images using a hidden Markov model},
  booktitle = {CVPR},
  year = {1994},
  }

 @inproceedings{Kuniyoshi,
  author = {Kuniyoshi Y.},
  title = {Learning from Examples: Imitation Learning and Emerging Cognition},
  booktitle = {Humanoid Robotics and Neuroscience: Science, Engineering and Society. },
  year = {2015},
  }
  
  
  @inproceedings{icml2015_schulman15, 
   Publisher = {JMLR Workshop and Conference Proceedings}, 
   title="Trust Region Policy Optimization", 
   Author={Schulman, John and Levine, Sergey and Abbeel, Pieter and Jordan, Michael and Moritz, Philipp}, 
   year="2015", 
   Booktitle="Proceedings of the 32nd International Conference on Machine Learning (ICML-15)", 
   Editor={David Blei and Francis Bach}, 
   pages="1889-1897", 
   url="http://jmlr.org/proceedings/papers/v37/schulman15.pdf" 
   }
  
  
  @article{DBLP:journals/corr/HasseltGS15,
  author    = {Hado van Hasselt and
               Arthur Guez and
               David Silver},
  title     = {Deep Reinforcement Learning with Double Q-learning},
  journal   = {CoRR},
  volume    = {abs/1509.06461},
  year      = {2015},
  url       = {http://arxiv.org/abs/1509.06461},
  archivePrefix = {arXiv},
  eprint    = {1509.06461},
  timestamp = {Wed, 07 Jun 2017 14:40:43 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/HasseltGS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @INPROCEEDINGS{Elgammal04separatingstyle,
      author = {Ahmed Elgammal and Chan-su Lee},
      title = {Separating style and content on a nonlinear manifold},
      booktitle = {CVPR},
      year = {2004}
  }

  @INPROCEEDINGS{Tenenbaum97separatingstyle,
      author = {Joshua B. Tenenbaum and William T. Freeman},
      title = {Separating style and content},
      booktitle = {In Advances in neural},
      year = {1997}
  }

  @inproceedings{DBLP:conf/cvpr/LvN07,
    author    = {Fengjun Lv and
		Ramakant Nevatia},
    title     = {Single View Human Action Recognition using Key Pose Matching and Viterbi Path Searching},
    booktitle = {CVPR},
    year      = {2007}
  }


  @inproceedings { 158,
	  title = {Linear Embeddings in Non-Rigid Structure From Motion},
	  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	  year = {2009},
	  address = {Miami, FL},
	  author = {Vincent Rabaud and Serge Belongie}
  }



  @INPROCEEDINGS{4270260,
  author={Goh, A. and Vidal, R.},
  booktitle={CVPR},
  title={Segmenting Motions of Different Types by Unsupervised Manifold Clustering},
  year={2007},
  }

@incollection{cycle,
year={2008},
isbn={978-3-540-88689-1},
booktitle={ECCV},
volume={5304},
series={Lecture Notes in Computer Science},
editor={Forsyth, David and Torr, Philip and Zisserman, Andrew},
doi={10.1007/978-3-540-88690-7_60},
title={Beyond Loose LP-Relaxations: Optimizing MRFs by Repairing Cycles},
url={http://dx.doi.org/10.1007/978-3-540-88690-7_60},
publisher={Springer Berlin Heidelberg},
author={Komodakis, Nikos and Paragios, Nikos},
pages={806-820}
}


  @incollection {springerlink:10.1007/11551188_37,
    author = {Wang, Fei and Zhang, Changshui},
    title = {Spectral Clustering for Time Series},
    booktitle = {Pattern Recognition and Data Mining},
    volume = {3686},
    year = {2005}
  }

  @INPROCEEDINGS{4587385,
  author={Xiaozhe Wang and Liang Wang and Wirth, A.},
  booktitle={CVPR},
  title={Pattern discovery in motion time series via structure-based spectral clustering},
  year={2008}
  }


  @article{Stauffer:2000:LPA:351581.351588,
  author = {Stauffer, Chris and Grimson, W. Eric L.},
  title = {Learning Patterns of Activity Using Real-Time Tracking},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }

  @incollection{Nanopoulos:2001:FCT:766914.766918,
  author = {Nanopoulos, Alex and Alcock, Rob and Manolopoulos, Yannis},
  title = {Information processing and technology},
  year = {2001},
  }

  BibTeX | EndNote | ACM Ref

  @inproceedings{Shi:2006:LTS:1153171.1153641,
  author = {Shi, Yifan and Bobick, Aaron and Essa, Irfan},
  title = {Learning Temporal Sequence Model from Partially Labeled Data},
  booktitle = {CVPR},
  year = {2006}
  }


  @article{Murase,
  author = {Murase, Hiroshi and Nayar, Shree K.},
  title = {Visual learning and recognition of 3-D objects from appearance},
  journal = {IJCV},
  volume = {14},
  year = {1995}
  }


  @INPROCEEDINGS{698609,
  author={Bobick, A.F. and Ivanov, Y.A.},
  booktitle={CVPR},
  title={Action recognition using probabilistic parsing},
  year={1998}
  }

  @inproceedings{Ryoo:2006:RCH:1153171.1153651,
  author = {Ryoo, M. S. and Aggarwal, J. K.},
  title = {Recognition of Composite Human Activities through Context-Free Grammar Based Representation},
  booktitle = {CVPR},
  year = {2006}
  }
  
  @article{Williams:1989:LAC:1351124.1351135,
 author = {Williams, Ronald J. and Zipser, David},
 title = {A Learning Algorithm for Continually Running Fully Recurrent Neural Networks},
 journal = {Neural Comput.},
 volume = {1},
 number = {2},
 year = {1989}
} 

  @article{Elman,
 author = {Rodriguez, P. and Wiles, J and Elman, J.},
 title = {A recurrent neural network that learns to count},
 journal = {. Connection Science},
 volume = {1},
 year = {1999}
} 


  
  @INPROCEEDINGS{Cun90handwrittendigit,
    author = {Le Cun and B. Boser and J. S. Denker and D. Henderson and R. E. Howard and W. Hubbard and L. D. Jackel},
    title = {Handwritten Digit Recognition with a Back-Propagation Network},
    booktitle = {NIPS},
    year = {1990}
}



  @INPROCEEDINGS{Hadsell06dimensionalityreduction,
      author = {Raia Hadsell and Sumit Chopra and Yann Lecun},
      title = {Dimensionality reduction by learning an invariant mapping},
      booktitle = {CVPR},
      year = {2006}
  }
  
   @INPROCEEDINGS{LupBer15,
      author = {Gary Lupyan and Benjamin Bergen},
      title = {How Language Programs the Mind},
      booktitle = {Topics in Cognitive Science},
      year = {2015}
  }

@misc{googlespeech,
  title = {Google Cloud Platform( Speech API - Speech Recognition)},
  howpublished = {\url{https://cloud.google.com/speech/}},
  
}
  
  
  @inproceedings{MovieQA,
author = {Makarand Tapaswi and Yukun Zhu and Rainer Stiefelhagen and Antonio Torralba and Raquel Urtasun and Sanja Fidler},
title = {MovieQA: Understanding Stories in Movies through Question-Answering},
booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
year = {2016}
}
  
    @inproceedings{chen2014fast,
    title={A Fast and Accurate Dependency Parser using Neural Networks},
    author={Chen, Danqi and Manning, Christopher D},
    booktitle={Empirical Methods in Natural Language Processing (EMNLP)},
    year={2014}
  }
  
  @article{DBLP:journals/corr/HuangRSZKFFWSG016,
  author    = {Jonathan Huang and
               Vivek Rathod and
               Chen Sun and
               Menglong Zhu and
               Anoop Korattikara and
               Alireza Fathi and
               Ian Fischer and
               Zbigniew Wojna and
               Yang Song and
               Sergio Guadarrama and
               Kevin Murphy},
  title     = {Speed/accuracy trade-offs for modern convolutional object detectors},
  journal   = {CoRR},
  volume    = {abs/1611.10012},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.10012},
  archivePrefix = {arXiv},
  eprint    = {1611.10012},
  timestamp = {Wed, 07 Jun 2017 14:41:50 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/HuangRSZKFFWSG016},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @incollection{NIPS2010_0893,
  title = {Pose-Sensitive Embedding by Nonlinear NCA Regression},
  author = {Graham Taylor and Rob Fergus and George Williams and Ian Spiro and Christoph Bregler},
  booktitle = {NIPS},
  year = {2010}
  }
  
  @InProceedings{BroxSegmentationCVPR11,
    author       = "Thomas Brox and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Object Segmentation by Alignment of Poselet Activations to Image Contours",
    booktitle    = "IEEE International Conference on Computer Vision and Pattern Recognition (CVPR)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }
  @InProceedings{HariharanSemanticContoursICCV11,
    author       = "Bharath Hariharan and Pablo Arbelaez and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Semantic Contours from Inverse Detectors",
    booktitle    = "International Conference on Computer Vision (ICCV)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }

  @InProceedings{raptisS10,
    author = 	{Raptis, M. and Soatto, S.},
    title = 	{Tracklet Descriptors for Action Modeling and Video Analysis},
    booktitle = 	{ECCV},
    year = 	{2010}
  }


  @book{Fukunaga:1990:ISP:92131,
  author = {Fukunaga, Keinosuke},
  title = {Introduction to statistical pattern recognition (2nd ed.)},
  year = {1990}
  }


  @ARTICLE{Roweis00nonlineardimensionality,
      author = {Sam T. Roweis and Lawrence K. Saul},
      title = {Nonlinear dimensionality reduction by locally linear embedding},
      journal = {SCIENCE},
      year = {2000},
      volume = {290}
  }

  @article{Turk_Pentland_1991,
  title={Face recognition using eigenfaces},
  journal={CVPR},
  year={1991}
  }


  @INPROCEEDINGS{Laptev03space-timeinterest,
      author = {Ivan Laptev and Tony Lindeberg},
      title = {Space-time Interest Points},
      booktitle = {ICCV},
      year = {2003}
  }


  @INPROCEEDINGS{Kim07r.:tensor,
      author = {Tae-kyun Kim and Shu-fai Wong and Roberto Cipolla},
      title = {Tensor Canonical Correlation Analysis for Action Classification},
      booktitle = {CVPR},
      year = {2007}
  }

  
  @article{Taylor:2000:RAO:364058.364079,
 author = {Taylor, Camillo J.},
 title = {Reconstruction of Articulated Objects from Point Correspondences in a Single Uncalibrated Image},
 journal = {CVIU},
 volume = {80},
 year = {2000}
} 


  @ARTICLE{Shao_trackingalgorithm,
      author = {Jie Shao and Shaohua Kevin Zhou},
      title = {Tracking Algorithm Using Background-Foreground Motion Models and Multiple Cues},
      journal = {ICASSP}
  }
  @INPROCEEDINGS{Taylor03fusionof,
      author = {Geoffrey Taylor and Lindsay Kleeman},
      title = {Fusion of Multimodal Visual Cues for Model-Based Object Tracking},
      booktitle = {ACRA},
      year = {2003}
  }

  @inproceedings{DBLP:conf/accv/KumarBD07,
    author    = {Pankaj Kumar and
		Michael J. Brooks and
		Anthony R. Dick},
    title     = {Adaptive Multiple Object Tracking Using Colour and Segmentation
		Cues},
    booktitle = {ACCV},
    year      = {2007}
  }

@InProceedings{Kumar05,
   author = "Kumar, M.~P. and Torr, P.~H.~S. and Zisserman, A.",
   title = "{OBJ} {CUT}",
   booktitle = "CVPR",
   year = "2005"
}
@inproceedings{DBLP:conf/eccv/FragkiadakiZZS12,
  author    = {Katerina Fragkiadaki and
               Weiyu Zhang and
               Geng Zhang and
               Jianbo Shi},
  title     = {Two-Granularity Tracking: Mediating Trajectory and Detection
               Graphs for Tracking under Occlusions},
  booktitle = {ECCV},
  year      = {2012}
}


  @InProceedings{rodriguez11b,
    author = "Rodriguez, M. and Sivic, J. and Laptev, I. and Audibert, J.-Y.",
    title = "Density-aware person detection and tracking in crowds",
    booktitle = "ICCV",
    year = "2011"
  }
@inproceedings{DBLP:conf/iccv/Jiang09,
 author    = {Hao Jiang},
 title     = {Human pose estimation using consistent max-covering},
 booktitle = {ICCV},
 year      = {2009}
}

  @inproceedings{Fragkiadaki:topology,
  author = {Fragkiadaki, Katerina and Shi, Jianbo},
  title = {Exploiting Motion and Topology for Segmenting and tracking Under Entanglement.},
  booktitle = {CVPR},
  year = {2011},
  }
@INPROCEEDINGS{Ferrari092dhuman,
    author = {Vittorio Ferrari and Manuel Marín-jiménez and Andrew Zisserman},
    title = {{2D} human pose estimation in {TV} shows},
    booktitle = {In Dagstuhl post-proceedings},
    year = {2009}
}


  @inproceedings{partsagain,
  author = {Michael Maire and Stella Yu and Pietro Perona},
  title = {Object Detection and Segmentation from Joint Embedding of Parts and Pixels},
  booktitle = {ICCV},
  year = {2011},
  }

  @INPROCEEDINGS{Jianbo03multiclassspectral,
      author = {Yu,Stella and Shi, Jianbo},
      title = {Multiclass Spectral Clustering},
      booktitle = {ICCV},
      year = {2003}
  }



  @INPROCEEDINGS{lu_cvpr2011,
      author = {Wei-Lwun Lu and Jo-Anne Ting and Kevin P. Murphy and James J. Little},
      booktitle = {Identifying Players in Broadcast Sports Videos using Conditional Random Fields},
      journal = {Proceedings of the 2011 IEEE Conference on Computer Vision and Pattern Recognition},
      year = {2011}
  }

  @article{DBLP:journals/pami/BoykovVZ01,
    author    = {Yuri Boykov and Olga Veksler and Ramin Zabih},
    title     = {Fast Approximate Energy Minimization via Graph Cuts},
    journal   = {TPAMI},
    volume    = {23},
    year      = {2001}
  }

  @article{GEAN:GEAN31,
  author = {Matula, David W. and Sokal, Robert R.},
  title = {Properties of Gabriel Graphs Relevant to Geographic Variation Research and the Clustering of Points in the Plane},
  journal = {Geographical Analysis},
  volume = {12},
  year = {1980}
  }

@proceedings{citeulike:3504535,
    abstract = {{This paper addresses human pose recognition from video sequences by formulating it as a classification problem. Unlike much previous work we do not make any assumptions on the availability of clean segmentation. The first step of this work consists in a novel method of aligning the training images using 3D Mocap data. Next we define classes by discretizing a 2D manifold whose two dimensions are camera viewpoint and actions. Our main contribution is a pose detection algorithm based on random forests. A bottom-up approach is followed to build a decision tree by recursively clustering and merging the classes at each level. For each node of the decision tree we build a list of potentially discriminative features using the alignment of training images; in this paper we consider Histograms of Orientated Gradient (HOG). We finally grow an ensemble of trees by randomly sampling one of the selected HOG blocks at each node. Our proposed approach gives promising results with both fixed and moving cameras.}},
    author = {Rogez, G. and Rihan, J. and Ramalingam, S. and Orrite, C. and Torr, P. H. S.},
    booktitle = {Computer Vision and Pattern Recognition, 2008. CVPR 2008. IEEE Conference on},
    citeulike-article-id = {3504535},
    citeulike-linkout-0 = {http://dx.doi.org/10.1109/cvpr.2008.4587617},
    citeulike-linkout-1 = {http://ieeexplore.ieee.org/xpls/abs\_all.jsp?arnumber=4587617},
    doi = {10.1109/cvpr.2008.4587617},
    journal = {Computer Vision and Pattern Recognition, 2008. CVPR 2008. IEEE Conference on},
    keywords = {detection, exemplar-based, pose, random, trees},
    pages = {1--8},
    posted-at = {2008-11-11 22:03:40},
    priority = {2},
    title = {{Randomized trees for human pose detection}},
    url = {http://dx.doi.org/10.1109/cvpr.2008.4587617},
    year = {2008}
}




  @INPROCEEDINGS{global_Pb,
  AUTHOR = {Michael Maire and Pablo Arbelaez and Charless Fowlkes and Jitendra Malik},
  TITLE = {Using contours to detect and localize junctions in natural images.},
  booktitle = {CVPR},
  YEAR = {2008}
  }


  @inproceedings{Yu:2010:AIO:1873951.1874105,
  author = {Yu, Haonan and Li, Jia and Tian, Yonghong and Huang, Tiejun},
  title = {Automatic interesting object extraction from images using complementary saliency maps},
  booktitle = {Proceedings of the international conference on Multimedia},
  year = {2010}
  }
  @inproceedings{DBLP:conf/accv/DonoserRB09,
    author    = {Michael Donoser and Hayko Riemenschneider and  Horst Bischof},
    title     = {Efficient Partial Shape Matching of Outer Contours},
    booktitle = {ACCV},
    year      = {2009}
  }

  @inproceedings{DBLP:conf/eccv/RiemenschneiderDB10,
    author    = {Hayko Riemenschneider and Michael Donoser and Horst Bischof},
    title     = {Using Partial Edge Contour Matches for Efficient Object
		Category Localization},
    booktitle = {ECCV},
    year      = {2010}
  }
@article{DBLP:journals/cacm/ShottonSKFFBCM13,
  author    = {Jamie Shotton and
               Toby Sharp and
               Alex Kipman and
               Andrew W. Fitzgibbon and
               Mark Finocchio and
               Andrew Blake and
               Mat Cook and
               Richard Moore},
  title     = {Real-time human pose recognition in parts from single depth
               images},
  journal   = {Commun. ACM},
  volume    = {56},
  number    = {1},
  year      = {2013},
  pages     = {116-124},
  ee        = {http://doi.acm.org/10.1145/2398356.2398381},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@inproceedings{DBLP:conf/cvpr/SunKS12,
  author    = {Min Sun and
               Pushmeet Kohli and
               Jamie Shotton},
  title     = {Conditional regression forests for human pose estimation},
  booktitle = {CVPR},
  year      = {2012},
  pages     = {3394-3401},
  ee        = {http://doi.ieeecomputersociety.org/10.1109/CVPR.2012.6248079},
  crossref  = {DBLP:conf/cvpr/2012},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@article{Rogez:2012:FHP:2317226.2317274,
 author = {Rogez, Gr{\'e}gory and Rihan, Jonathan and Orrite-Uru\~{n}uela, Carlos and Torr, Philip H.},
 title = {Fast Human Pose Detection Using Randomized Hierarchical Cascades of Rejectors},
 journal = {Int. J. Comput. Vision},
 issue_date = {August    2012},
 volume = {99},
 number = {1},
 month = aug,
 year = {2012},
 issn = {0920-5691},
 pages = {25--52},
 numpages = {28},
 url = {http://dx.doi.org/10.1007/s11263-012-0516-9},
 doi = {10.1007/s11263-012-0516-9},
 acmid = {2317274},
 publisher = {Kluwer Academic Publishers},
 address = {Hingham, MA, USA},
 keywords = {Cascade classifiers, Human detection, Pose estimation},
}


  @inproceedings{Latecki2010,
    author    = {Tianyang Ma and Longin Jan Latecki},
    title     = { From Partial Shape Matching through Local Deformation to Robust Global Shape Similarity for Object Detection},
    booktitle = {CVPR},
    year      = {2011}
  }

@INPROCEEDINGS{Sigal03attractivepeople:,
    author = {Leonid Sigal and Michael Isard and Benjamin H. Sigelman and Michael J. Black},
    title = {Attractive People: Assembling Loose-Limbed Models Using Non-parametric Belief Propagation},
    booktitle = {in NIPS},
    year = {2003},
    pages = {1539--1546},
    publisher = {MIT Press}
}

@InProceedings{Richter_2016_ECCV,
author = {Stephan R. Richter and Vibhav Vineet and Stefan Roth and Vladlen Koltun},
title = {Playing for Data: Ground Truth from Computer Games},
booktitle = {European Conference on Computer Vision (ECCV)},
year = {2016},
editor = {Bastian Leibe and Jiri Matas and Nicu Sebe and Max Welling},
series = {LNCS}, 
volume = {9906}, 
publisher = {Springer International Publishing},
pages = {102--118}
}

@inproceedings{DBLP:conf/nips/SutskeverVL14,
  author    = {Ilya Sutskever and
               Oriol Vinyals and
               Quoc V. Le},
  title     = {Sequence to Sequence Learning with Neural Networks},
  booktitle = {NIPS},
  year      = {2014}
}



@article{Weng:2006:VOT:1223195.1223208,
 author = {Weng, Shiuh-Ku and Kuo, Chung-Ming and Tu, Shu-Kang},
 title = {Video Object Tracking Using Adaptive Kalman Filter},
 journal = {J. Vis. Comun. Image Represent.},
 issue_date = {December, 2006},
 volume = {17},
 number = {6},
 year = {2006},
 issn = {1047-3203},
 pages = {1190--1208},
 numpages = {19},
 url = {http://dx.doi.org/10.1016/j.jvcir.2006.03.004},
 doi = {10.1016/j.jvcir.2006.03.004},
 acmid = {1223208},
 publisher = {Academic Press, Inc.},
 address = {Orlando, FL, USA},
 keywords = {Adaptive Kalman filter, HSI color space, Occlusion ratio},
} 



@incollection{Smith88a,
    abstract = {{The Austrian philosopher Christian von Ehrenfels published his essay "On 'Gestalt Qualities'" in 1890. The essay initiated a current of thought which enjoyed a powerful position in the philosophy and psychology of the first half of this century and has more recently enjoyed a minor resurgence of interest in the area of cognitive science, above all in criticisms of the so-called 'strong programme' in artificial intelligence. The theory of Gestalt is of course associated most specifically with psychologists of the Berlin school such as Max Wertheimer, Wolfgang Kohler and Kurt Koffka. We shall see in what follows, however, that an adequate philosophical understanding of the Gestalt idea and of Ehrenfels' achievement will require a close examination not merely of the work of the Berlin school but also of a much wider tradition in Austrian and German philosophy in general.}},
    author = {Smith, Barry},
    booktitle = {Foundations of Gestalt Theory},
    citeulike-article-id = {13114130},
    day = {31},
    editor = {Smith, Barry},
    keywords = {gestalt\_theory},
    month = dec,
    pages = {11--81},
    posted-at = {2014-03-22 09:53:37},
    priority = {2},
    publisher = {Philosophia Verlag},
    title = {{Gestalt Theory: An Essay in Philosophy}},
    year = {1988}
}

@article{DBLP:journals/corr/IsolaZZE16,
  author    = {Phillip Isola and
               Jun{-}Yan Zhu and
               Tinghui Zhou and
               Alexei A. Efros},
  title     = {Image-to-Image Translation with Conditional Adversarial Networks},
  journal   = {CoRR},
  volume    = {abs/1611.07004},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.07004},
  timestamp = {Thu, 01 Dec 2016 19:32:08 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/IsolaZZE16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/HandaBPSMD16,
  author    = {Ankur Handa and
               Michael Bl{\"{o}}sch and
               Viorica Patraucean and
               Simon Stent and
               John McCormac and
               Andrew J. Davison},
  title     = {gvnn: Neural Network Library for Geometric Computer Vision},
  journal   = {CoRR},
  volume    = {abs/1607.07405},
  year      = {2016},
  url       = {http://arxiv.org/abs/1607.07405},
  timestamp = {Tue, 02 Aug 2016 12:59:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/HandaBPSMD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{IEF2015human,
 author = {Carreira, Joao and Agrawal, Pulkit and Fragkiadaki, Katerina and Malik, Jitendra},
 title = {Human Pose Estimation with Iterative Error Feedback},
 journal={arXiv preprint arXiv:1507.06550},
 Year = {2015}}
 
@article{tijmen,
  title={Optimizing neural networks that generate images},
  author={Tijmen Tieleman},
  journal={Ph.D. Thesis},
  year={2014}
}



@Article{Regolin1995,
author="Regolin, Lucia
and Vallortigara, Giorgio",
title="Perception of partly occluded objects by young chicks",
journal="Perception {\&} Psychophysics",
year="1995",
volume="57",
number="7",
pages="971--976",
abstract="Completion of partly occluded objects is a ubiquitous phenomenon in human visual perception. It is unclear, however, whether it occurs at all in other species: Studies on visual discrimination learning have revealed that animals usually attend to parts and features of the discriminative stimuli rather than to global object properties. We provide here the first demonstration of recognition of partly occluded objects in a bird species, the domestic chickGallus gallus, using the naturalistic setting made available by filial imprinting, a process whereby young birds form attachments to their mothers or some artificial substitute. In Experiment 1, newborn chicks were reared singly with a red cardboard triangle, to which they rapidly imprinted and therefore treated as a social partner. On Day 3 of life, the chicks were presented with pairs of objects composed of either isolated fragments or occluded parts of the imprinting stimulus. Chicks consistently chose to associate with complete or with partly occluded versions of the imprinting object rather than with separate fragments of it. Similarly, in Experiment 2, chicks reared with a partly occluded triangle chose to associate with a complete triangle rather than with a fragmented one, whereas chicks reared with a fragmented triangle chose to associate with a fragmented triangle and not with a complete one. Newborn chicks thus appear to behave as if they could experience amodal completion.",
issn="1532-5962",
doi="10.3758/BF03205456",
url="http://dx.doi.org/10.3758/BF03205456"
}
@inproceedings{Kong:ECCV:2014,
  title = {Intrinsic Video},
  author = {Kong, Naejin and Gehler, Peter V. and Black, Michael J.},
  booktitle = {Computer Vision -- ECCV 2014},
  volume = {8690},
  pages = {360--375},
  series = {Lecture Notes in Computer Science},
  editors = {D. Fleet  and T. Pajdla and B. Schiele  and T. Tuytelaars },
  publisher = {Springer International Publishing},
  month = sep,
  year = {2014}
}

@article{DBLP:journals/pami/YangHRF12,
  author    = {Yi Yang and
               Sam Hallman and
               Deva Ramanan and
               Charless C. Fowlkes},
  title     = {Layered Object Models for Image Segmentation},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {34},
  number    = {9},
  pages     = {1731--1743},
  year      = {2012},
  url       = {http://dx.doi.org/10.1109/TPAMI.2011.208},
  doi       = {10.1109/TPAMI.2011.208},
  timestamp = {Sat, 12 Mar 2016 09:04:20 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/pami/YangHRF12},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Tomasi:1992:SMI:144398.144403,
 author = {Tomasi, Carlo and Kanade, Takeo},
 title = {Shape and Motion from Image Streams Under Orthography: A Factorization Method},
 journal = {Int. J. Comput. Vision},
 issue_date = {Nov. 1992},
 volume = {9},
 number = {2},
 month = nov,
 year = {1992},
 issn = {0920-5691},
 pages = {137--154},
 numpages = {18},
 url = {http://dx.doi.org/10.1007/BF00129684},
 doi = {10.1007/BF00129684},
 acmid = {144403},
 publisher = {Kluwer Academic Publishers},
 address = {Hingham, MA, USA},
} 


@techreport{Barron:EECS-2013-117,
    Author = {Barron, Jonathan and Malik, Jitendra},
    Title = {Shape, Illumination, and Reflectance from Shading},
    Institution = {EECS Department, University of California, Berkeley},
    Year = {2013},
    Month = {May},
    URL = {http://www2.eecs.berkeley.edu/Pubs/TechRpts/2013/EECS-2013-117.html},
    Number = {UCB/EECS-2013-117},
    Abstract = {A fundamental problem in computer vision is that of inferring the intrinsic, 3D structure of the world from flat, 2D images of that world. Traditional methods for recovering scene properties such as shape, reflectance, or illumination rely on multiple observations of the same scene to overconstrain the problem. Recovering these same properties from a single image seems almost impossible in comparison --- there are an infinite number of shapes, paint, and lights that exactly reproduce a single image. However, certain explanations are more likely than others: surfaces tend to be smooth, paint tends to be uniform, and illumination tends to be natural. We therefore pose this problem as one of statistical inference, and define an optimization problem that searches for the most likely explanation of a single image. Our technique can be viewed as a superset of several classic computer vision problems (shape-from-shading, intrinsic images, color constancy, illumination estimation, etc) and outperforms all previous solutions to those constituent problems.}
}
@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={770--778},
  year={2016}
}



@article{DBLP:journals/corr/PintoG15,
  author    = {Lerrel Pinto and
               Abhinav Gupta},
  title     = {Supersizing Self-supervision: Learning to Grasp from 50K Tries and
               700 Robot Hours},
  journal   = {CoRR},
  volume    = {abs/1509.06825},
  year      = {2015},
  url       = {http://arxiv.org/abs/1509.06825},
  timestamp = {Wed, 07 Jun 2017 14:41:22 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/PintoG15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@inproceedings{rohrbach2012database,
  title={A Database for Fine Grained Activity Detection of Cooking Activities},
  author={Rohrbach, Marcus and Amin, Sikandar and Andriluka, Mykhaylo and Schiele, Bernt},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2012},
  organization={IEEE}
}

@inproceedings{rohrbach2013translating,
  title={Translating Video Content to Natural Language Descriptions},
  author={Rohrbach, Marcus and Wei, Qiu and Titov, Ivan and Thater, Stefan and Pinkal, Manfred and Schiele, Bernt},
  booktitle={IEEE International Conference on Computer Vision (ICCV)},
  year={2013}
}


@article{DBLP:journals/corr/HuARDS17,
  author    = {Ronghang Hu and
               Jacob Andreas and
               Marcus Rohrbach and
               Trevor Darrell and
               Kate Saenko},
  title     = {Learning to Reason: End-to-End Module Networks for Visual Question
               Answering},
  journal   = {CoRR},
  volume    = {abs/1704.05526},
  year      = {2017},
  url       = {http://arxiv.org/abs/1704.05526},
  archivePrefix = {arXiv},
  eprint    = {1704.05526},
  timestamp = {Wed, 07 Jun 2017 14:40:24 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/HuARDS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{malinowski2015ask,
  title={Ask Your Neurons: A Neural-based Approach to Answering Questions about Images},
  author={Malinowski, Mateusz and Rohrbach, Marcus and Fritz, Mario},
  booktitle={IEEE International Conference on Computer Vision (ICCV)},
  year={2015}
}

@InProceedings{VQA, 
author = {Stanislaw Antol and Aishwarya Agrawal and Jiasen Lu and Margaret Mitchell and Dhruv Batra and C. Lawrence Zitnick and Devi Parikh}, 
title = {{VQA}: {V}isual {Q}uestion {A}nswering}, 
booktitle = {International Conference on Computer Vision (ICCV)}, 
year = {2015}, 
}

@inproceedings{andreas2016learning,
  title={Learning to Compose Neural Networks for Question Answering},
  author={Andreas, Jacob and Rohrbach, Marcus and Darrell, Trevor and Klein, Dan},
  booktitle={North American Chapter of the Association for Computational Linguistics: Human Language Technologies (NAACL)},
  year={2016}
}

@inproceedings{fukui2016multimodal,
  title={Multimodal Compact Bilinear Pooling for Visual Question Answering and Visual Grounding},
  author={Fukui, Akira and Park, Dong Huk and Yang, Daylen and Rohrbach, Anna and Darrell, Trevor and Rohrbach, Marcus},
  booktitle={Conference on Empirical Methods in Natural Language Processing (EMNLP)},
  year={2016}
}
@InProceedings{Das_2013_CVPR,
author = {Das, Pradipto and Xu, Chenliang and Doell, Richard F. and Corso, Jason J.},
title = {A Thousand Frames in Just a Few Words: Lingual Description of Videos through Latent Topics and Sparse Object Stitching},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2013}
}

@article{DBLP:journals/corr/abs-1710-04615,
  author    = {Tianhao Zhang and
               Zoe McCarthy and
               Owen Jow and
               Dennis Lee and
               Ken Goldberg and
               Pieter Abbeel},
  title     = {Deep Imitation Learning for Complex Manipulation Tasks from Virtual
               Reality Teleoperation},
  journal   = {CoRR},
  volume    = {abs/1710.04615},
  year      = {2017},
  url       = {http://arxiv.org/abs/1710.04615},
  archivePrefix = {arXiv},
  eprint    = {1710.04615},
  timestamp = {Wed, 01 Nov 2017 19:05:43 +0100},
  biburl    = {http://dblp.org/rec/bib/journals/corr/abs-1710-04615},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{DBLP:journals/corr/NeelakantanLAMA16,
  author    = {Arvind Neelakantan and
               Quoc V. Le and
               Mart{\'{\i}}n Abadi and
               Andrew McCallum and
               Dario Amodei},
  title     = {Learning a Natural Language Interface with Neural Programmer},
  journal   = {CoRR},
  volume    = {abs/1611.08945},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.08945},
  archivePrefix = {arXiv},
  eprint    = {1611.08945},
  timestamp = {Wed, 07 Jun 2017 14:42:36 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/NeelakantanLAMA16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@INPROCEEDINGS{6619231, 
author={C. L. Zitnick and D. Parikh}, 
booktitle={2013 IEEE Conference on Computer Vision and Pattern Recognition}, 
title={Bringing Semantics into Focus Using Visual Abstraction}, 
year={2013}, 
pages={3009-3016}, 
keywords={image processing;abstract images;abstract scenes;complex visual information;high level semantic information;image hand labeling;linguistic semantic similarity;visual abstraction;Abstracts;Art;Feature extraction;Mutual information;Semantics;Speech;Visualization;abstract scenes;semantic understanding}, 
doi={10.1109/CVPR.2013.387}, 
ISSN={1063-6919}, 
month={June},}


@inproceedings{rohrbach2015dataset,
  title={A Dataset for Movie Description},
  author={Rohrbach, Anna and Rohrbach, Marcus and Tandon, Niket and Schiele, Bernt},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2015}
}

@inproceedings{rohrbach2012script,
  title={Script Data for Attribute-based Recognition of Composite Activities},
  author={Rohrbach, Marcus and Regneri, Michaela and Andriluka, Micha and Amin, Sikandar and Pinkal, Manfred and Schiele, Bernt},
  booktitle={ECCV 2012 : 12th European Conference on Computer Vision},
  year={2012},
  organization={Springer}
}

@inproceedings{rohrbach2016grounding,
  title={Grounding of Textual Phrases in Images by Reconstruction},
  author={Rohrbach, Anna and Rohrbach, Marcus and Hu, Ronghang and Darrell, Trevor and Schiele, Bernt},
  booktitle={European Conference on Computer Vision (ECCV)},
  year={2016}
}

@inproceedings{rohrbach2014coherent,
  title={Coherent Multi-Sentence Video Description with Variable Level of Detail},
  author={Rohrbach, Anna and Rohrbach, Marcus and Qiu, Wei and Friedrich, Annemarie and Pinkal, Manfred and Schiele, Bernt},
  booktitle={German Conference on Pattern Recognition (GCPR)},
  year={2014}
}

@inproceedings{hendricks2016generating,
  title={Generating Visual Explanations},
  author={Hendricks, Lisa Anne and Akata, Zeynep and Rohrbach, Marcus and Donahue, Jeff and Schiele, Bernt and Darrell, Trevor},
  booktitle={European Conference on Computer Vision (ECCV)},
  year={2016}
}

@inproceedings{venugopalan2017captioning,
  title={Captioning Images with Diverse Objects},
  author={Venugopalan, Subhashini and Hendricks, Lisa Anne and Rohrbach, Marcus and Mooney, Raymond and Darrell, Trevor and Saenko, Kate},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017}
}

@inproceedings{hu2017learning,
  title={Learning to Reason: End-to-End Module Networks for Visual Question Answering},
  author={Hu, Ronghang and Andreas, Jacob and Rohrbach, Marcus and Darrell, Trevor and Saenko, Kate},
  booktitle={IEEE International Conference on Computer Vision (ICCV)},
  year={2017}
}

@article{DBLP:journals/corr/AlemiCISU16,
  author    = {Alexander A. Alemi and
               Fran{\c{c}}ois Chollet and
               Geoffrey Irving and
               Christian Szegedy and
               Josef Urban},
  title     = {DeepMath - Deep Sequence Models for Premise Selection},
  journal   = {CoRR},
  volume    = {abs/1606.04442},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.04442},
  timestamp = {Wed, 07 Jun 2017 14:40:07 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/AlemiCISU16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{45942,
title = {Collective Robot Reinforcement Learning with Distributed Asynchronous Guided Policy Search},
author  = {Ali Yahya and Adrian Li and Mrinal Kalakrishnan and Yevgen Chebotar and Sergey Levine},
year  = {2017},
URL = {https://arxiv.org/abs/1610.00673}
}

@article{DBLP:journals/corr/AndrychowiczWRS17,
  author    = {Marcin Andrychowicz and
               Filip Wolski and
               Alex Ray and
               Jonas Schneider and
               Rachel Fong and
               Peter Welinder and
               Bob McGrew and
               Josh Tobin and
               Pieter Abbeel and
               Wojciech Zaremba},
  title     = {Hindsight Experience Replay},
  journal   = {CoRR},
  volume    = {abs/1707.01495},
  year      = {2017},
  url       = {http://arxiv.org/abs/1707.01495},
  archivePrefix = {arXiv},
  eprint    = {1707.01495},
  timestamp = {Sat, 05 Aug 2017 14:56:09 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/AndrychowiczWRS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/DuanASHSSAZ17,
  author    = {Yan Duan and
               Marcin Andrychowicz and
               Bradly C. Stadie and
               Jonathan Ho and
               Jonas Schneider and
               Ilya Sutskever and
               Pieter Abbeel and
               Wojciech Zaremba},
  title     = {One-Shot Imitation Learning},
  journal   = {CoRR},
  volume    = {abs/1703.07326},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.07326},
  archivePrefix = {arXiv},
  eprint    = {1703.07326},
  timestamp = {Wed, 07 Jun 2017 14:43:13 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/DuanASHSSAZ17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/FinnL16,
  author    = {Chelsea Finn and
               Sergey Levine},
  title     = {Deep Visual Foresight for Planning Robot Motion},
  journal   = {CoRR},
  volume    = {abs/1610.00696},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.00696},
  archivePrefix = {arXiv},
  eprint    = {1610.00696},
  timestamp = {Wed, 07 Jun 2017 14:42:20 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/FinnL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/NairCAIAML17,
  author    = {Ashvin Nair and
               Dian Chen and
               Pulkit Agrawal and
               Phillip Isola and
               Pieter Abbeel and
               Jitendra Malik and
               Sergey Levine},
  title     = {Combining Self-Supervised Learning and Imitation for Vision-Based
               Rope Manipulation},
  journal   = {CoRR},
  volume    = {abs/1703.02018},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.02018},
  archivePrefix = {arXiv},
  eprint    = {1703.02018},
  timestamp = {Wed, 07 Jun 2017 14:41:24 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/NairCAIAML17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/abs-1709-04905,
  author    = {Chelsea Finn and
               Tianhe Yu and
               Tianhao Zhang and
               Pieter Abbeel and
               Sergey Levine},
  title     = {One-Shot Visual Imitation Learning via Meta-Learning},
  journal   = {CoRR},
  volume    = {abs/1709.04905},
  year      = {2017},
  url       = {http://arxiv.org/abs/1709.04905},
  archivePrefix = {arXiv},
  eprint    = {1709.04905},
  timestamp = {Thu, 05 Oct 2017 09:42:52 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/abs-1709-04905},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{Xiao:2017:LAA:3131944.3133941,
 author = {Xiao, Jianxiong},
 title = {Learning Affordance for Autonomous Driving},
 booktitle = {Proceedings of the 2Nd ACM International Workshop on Smart, Autonomous, and Connected Vehicular Systems and Services},
 series = {CarSys '17},
 year = {2017},
 isbn = {978-1-4503-5146-1},
 location = {Snowbird, Utah, USA},
 pages = {1--1},
 numpages = {1},
 url = {http://doi.acm.org/10.1145/3131944.3133941},
 doi = {10.1145/3131944.3133941},
 acmid = {3133941},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {autonomous driving, self-driving car},
} 


@article{DBLP:journals/corr/PintoG15,
  author    = {Lerrel Pinto and
               Abhinav Gupta},
  title     = {Supersizing Self-supervision: Learning to Grasp from 50K Tries and
               700 Robot Hours},
  journal   = {CoRR},
  volume    = {abs/1509.06825},
  year      = {2015},
  url       = {http://arxiv.org/abs/1509.06825},
  archivePrefix = {arXiv},
  eprint    = {1509.06825},
  timestamp = {Wed, 07 Jun 2017 14:41:22 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/PintoG15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@INPROCEEDINGS{Andrews03supportvector,
    author = {Stuart Andrews and Ioannis Tsochantaridis and Thomas Hofmann},
    title = {Support vector machines for multiple-instance learning},
    booktitle = {Advances in Neural Information Processing Systems 15},
    year = {2003},
    pages = {561--568},
    publisher = {MIT Press}
}


@article{modularreferential,
author = {Hu, Ronghang and Rohrbach, Marcus and Andreas, Jacob and Darrell, Trevor and Saenko, Kate},
year = {2016},
month = {11},
pages = {},
title = {Modeling Relationships in Referential Expressions with Compositional Modular Networks}
}



@article{DBLP:journals/corr/MaLH16,
  author    = {Xuezhe Ma and
               Zhengzhong Liu and
               Eduard H. Hovy},
  title     = {Unsupervised Ranking Model for Entity Coreference Resolution},
  journal   = {CoRR},
  volume    = {abs/1603.04553},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.04553},
  timestamp = {Wed, 07 Jun 2017 14:42:20 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MaLH16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{shetty2017speaking,
  title={Speaking the Same Language: Matching Machine to Human Captions by Adversarial Training},
  author={Shetty, Rakshith and Rohrbach, Marcus and Hendricks, Lisa Anne and Fritz, Mario and Schiele, Bernt},
  booktitle={IEEE International Conference on Computer Vision (ICCV)},
  year={2017}
}

@inproceedings{rohrbach2017generating,
  title={Generating descriptions with grounded and co-referenced people},
  author={Rohrbach, Anna and Rohrbach, Marcus and Tang, Siyu and Oh, Seong Joon and Schiele, Bernt},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017}
}



@article{DBLP:journals/corr/YangHGDS15,
  author    = {Zichao Yang and
               Xiaodong He and
               Jianfeng Gao and
               Li Deng and
               Alexander J. Smola},
  title     = {Stacked Attention Networks for Image Question Answering},
  journal   = {CoRR},
  volume    = {abs/1511.02274},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.02274},
  timestamp = {Wed, 07 Jun 2017 14:41:59 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/YangHGDS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{karpathy2015deep,
  title={Deep visual-semantic alignments for generating image descriptions},
  author={Karpathy, Andrej and Fei-Fei, Li},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3128--3137},
  year={2015}
}

@article{DBLP:journals/corr/LinMBHPRDZ14,
  author    = {Tsung{-}Yi Lin and
               Michael Maire and
               Serge J. Belongie and
               Lubomir D. Bourdev and
               Ross B. Girshick and
               James Hays and
               Pietro Perona and
               Deva Ramanan and
               Piotr Doll{\'{a}}r and
               C. Lawrence Zitnick},
  title     = {Microsoft {COCO:} Common Objects in Context},
  journal   = {CoRR},
  volume    = {abs/1405.0312},
  year      = {2014},
  url       = {http://arxiv.org/abs/1405.0312},
  timestamp = {Wed, 07 Jun 2017 14:41:35 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LinMBHPRDZ14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/SermanetXL16,
  author    = {Pierre Sermanet and
               Kelvin Xu and
               Sergey Levine},
  title     = {Unsupervised Perceptual Rewards for Imitation Learning},
  journal   = {CoRR},
  volume    = {abs/1612.06699},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.06699},
  archivePrefix = {arXiv},
  eprint    = {1612.06699},
  timestamp = {Wed, 07 Jun 2017 14:42:07 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/SermanetXL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{bullet,
 title = {http://bulletphysics.org/wordpress/},
} 



@article{Liang:2016:LES:2991470.2866568,
 author = {Liang, Percy},
 title = {Learning Executable Semantic Parsers for Natural Language Understanding},
 journal = {Commun. ACM},
 issue_date = {September 2016},
 volume = {59},
 number = {9},
 month = aug,
 year = {2016},
 issn = {0001-0782},
 pages = {68--76},
 numpages = {9},
 url = {http://doi.acm.org/10.1145/2866568},
 doi = {10.1145/2866568},
 acmid = {2866568},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@article{DBLP:journals/corr/LocascioNDKB16,
  author    = {Nicholas Locascio and
               Karthik Narasimhan and
               Eduardo DeLeon and
               Nate Kushman and
               Regina Barzilay},
  title     = {Neural Generation of Regular Expressions from Natural Language with
               Minimal Domain Knowledge},
  journal   = {CoRR},
  volume    = {abs/1608.03000},
  year      = {2016},
  url       = {http://arxiv.org/abs/1608.03000},
  archivePrefix = {arXiv},
  eprint    = {1608.03000},
  timestamp = {Wed, 07 Jun 2017 14:40:18 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LocascioNDKB16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{DBLP:conf/acl/WangBL15,
  author    = {Yushi Wang and
               Jonathan Berant and
               Percy Liang},
  title     = {Building a Semantic Parser Overnight},
  booktitle = {Proceedings of the 53rd Annual Meeting of the Association for Computational
               Linguistics and the 7th International Joint Conference on Natural
               Language Processing of the Asian Federation of Natural Language Processing,
               {ACL} 2015, July 26-31, 2015, Beijing, China, Volume 1: Long Papers},
  pages     = {1332--1342},
  year      = {2015},
  crossref  = {DBLP:conf/acl/2015-1},
  url       = {http://aclweb.org/anthology/P/P15/P15-1129.pdf},
  timestamp = {Sun, 02 Aug 2015 19:26:07 +0200},
  biburl    = {http://dblp.org/rec/bib/conf/acl/WangBL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/acl/IyerKCKZ17,
  author    = {Srinivasan Iyer and
               Ioannis Konstas and
               Alvin Cheung and
               Jayant Krishnamurthy and
               Luke Zettlemoyer},
  title     = {Learning a Neural Semantic Parser from User Feedback},
  booktitle = {Proceedings of the 55th Annual Meeting of the Association for Computational
               Linguistics, {ACL} 2017, Vancouver, Canada, July 30 - August 4, Volume
               1: Long Papers},
  pages     = {963--973},
  year      = {2017},
  crossref  = {DBLP:conf/acl/2017-1},
  url       = {https://doi.org/10.18653/v1/P17-1089},
  doi       = {10.18653/v1/P17-1089},
  timestamp = {Fri, 04 Aug 2017 16:38:24 +0200},
  biburl    = {http://dblp.org/rec/bib/conf/acl/IyerKCKZ17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/IyerKCKZ17,
  author    = {Srinivasan Iyer and
               Ioannis Konstas and
               Alvin Cheung and
               Jayant Krishnamurthy and
               Luke Zettlemoyer},
  title     = {Learning a Neural Semantic Parser from User Feedback},
  journal   = {CoRR},
  volume    = {abs/1704.08760},
  year      = {2017},
  url       = {http://arxiv.org/abs/1704.08760},
  archivePrefix = {arXiv},
  eprint    = {1704.08760},
  timestamp = {Wed, 07 Jun 2017 14:40:09 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/IyerKCKZ17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/MisraLA17,
  author    = {Dipendra Kumar Misra and
               John Langford and
               Yoav Artzi},
  title     = {Mapping Instructions and Visual Observations to Actions with Reinforcement
               Learning},
  journal   = {CoRR},
  volume    = {abs/1704.08795},
  year      = {2017},
  url       = {http://arxiv.org/abs/1704.08795},
  archivePrefix = {arXiv},
  eprint    = {1704.08795},
  timestamp = {Wed, 07 Jun 2017 14:42:37 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/MisraLA17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}




@Inbook{Matuszek2013,
author="Matuszek, Cynthia
and Herbst, Evan
and Zettlemoyer, Luke
and Fox, Dieter",
editor="Desai, Jaydev P.
and Dudek, Gregory
and Khatib, Oussama
and Kumar, Vijay",
title="Learning to Parse Natural Language Commands to a Robot Control System",
bookTitle="Experimental Robotics: The 13th International Symposium on Experimental Robotics",
year="2013",
publisher="Springer International Publishing",
address="Heidelberg",
pages="403--415",
abstract="As robots become more ubiquitous and capable of performing complex tasks, the importance of enabling untrained users to interact with them has increased. In response, unconstrained natural-language interaction with robots has emerged as a significant research area. We discuss the problem of parsing natural language commands to actions and control structures that can be readily implemented in a robot execution system. Our approach learns a parser based on example pairs of English commands and corresponding control language expressions. We evaluate this approach in the context of following route instructions through an indoor environment, and demonstrate that our system can learn to translate English commands into sequences of desired actions, while correctly capturing the semantic intent of statements involving complex control structures. The procedural nature of our formal representation allows a robot to interpret route instructions online while moving through a previously unknown environment.",
isbn="978-3-319-00065-7",
doi="10.1007/978-3-319-00065-7_28",
url="https://doi.org/10.1007/978-3-319-00065-7_28"
}

@article{DBLP:journals/corr/LeeHLZ17,
  author    = {Kenton Lee and
               Luheng He and
               Mike Lewis and
               Luke Zettlemoyer},
  title     = {End-to-end Neural Coreference Resolution},
  journal   = {CoRR},
  volume    = {abs/1707.07045},
  year      = {2017},
  url       = {http://arxiv.org/abs/1707.07045},
  archivePrefix = {arXiv},
  eprint    = {1707.07045},
  timestamp = {Sat, 05 Aug 2017 14:56:20 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LeeHLZ17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/BahdanauCB14,
  author    = {Dzmitry Bahdanau and
               Kyunghyun Cho and
               Yoshua Bengio},
  title     = {Neural Machine Translation by Jointly Learning to Align and Translate},
  journal   = {CoRR},
  volume    = {abs/1409.0473},
  year      = {2014},
  url       = {http://arxiv.org/abs/1409.0473},
  archivePrefix = {arXiv},
  eprint    = {1409.0473},
  timestamp = {Wed, 07 Jun 2017 14:40:19 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/BahdanauCB14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{doi:10.1177/0278364915602060,
author = {Dipendra K. Misra and Jaeyong Sung and Kevin Lee and Ashutosh Saxena},
title ={Tell me Dave: Context-sensitive grounding of natural language to manipulation           instructions},
journal = {The International Journal of Robotics Research},
volume = {35},
number = {1-3},
pages = {281-300},
year = {2016},
doi = {10.1177/0278364915602060},

URL = { 
        https://doi.org/10.1177/0278364915602060
    
},
eprint = { 
        https://doi.org/10.1177/0278364915602060
    
}
,
    abstract = { It is important for a robot to be able to interpret natural language commands given by a human. In this paper, we consider performing a sequence of mobile manipulation tasks with instructions described in natural language. Given a new environment, even a simple task such as boiling water would be performed quite differently depending on the presence, location and state of the objects. We start by collecting a dataset of task descriptions in free-form natural language and the corresponding grounded task-logs of the tasks performed in an online robot simulator. We then build a library of verb–environment instructions that represents the possible instructions for each verb in that environment, these may or may not be valid for a different environment and task context. We present a model that takes into account the variations in natural language and ambiguities in grounding them to robotic instructions with appropriate environment context and task constraints. Our model also handles incomplete or noisy natural language instructions. It is based on an energy function that encodes such properties in a form isomorphic to a conditional random field. We evaluate our model on tasks given in a robotic simulator and show that it successfully outperforms the state of the art with 61.8\% accuracy. We also demonstrate a grounded robotic instruction sequence on a PR2 robot using the Learning from Demonstration approach. }
}

@inproceedings{Branavan:2009:RLM:1687878.1687892,
 author = {Branavan, S. R. K. and Chen, Harr and Zettlemoyer, Luke S. and Barzilay, Regina},
 title = {Reinforcement Learning for Mapping Instructions to Actions},
 booktitle = {Proceedings of the Joint Conference of the 47th Annual Meeting of the ACL and the 4th International Joint Conference on Natural Language Processing of the AFNLP: Volume 1 - Volume 1},
 series = {ACL '09},
 year = {2009},
 isbn = {978-1-932432-45-9},
 location = {Suntec, Singapore},
 pages = {82--90},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=1687878.1687892},
 acmid = {1687892},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
}




@inproceedings{mei16,
  address = {Phoenix, AZ},
  author = {Hongyuan Mei and Mohit Bansal and Matthew R. Walter},
  booktitle = {Proceedings of the National Conference on Artificial Intelligence (AAAI)},
  month = {February},
  pages = {2772--2778},
  title = {Listen, Attend, and Walk: Neural Mapping of Navigational Instructions to Action Sequences},
  year = {2016},
}



@InProceedings{zelle:aaai96,
title={Learning to Parse Database Queries using Inductive Logic Programming},
author={John M. Zelle and Raymond J. Mooney},
booktitle={AAAI/IAAI},
month={August},
address={Portland, OR},
publisher={AAAI Press/MIT Press},
pages={1050-1055},
url="http://www.cs.utexas.edu/users/ai-lab/?zelle:aaai96",
year={1996}

@article{DBLP:journals/corr/abs-1207-1420,
  author    = {Luke S. Zettlemoyer and
               Michael Collins},
  title     = {Learning to Map Sentences to Logical Form: Structured Classification
               with Probabilistic Categorial Grammars},
  journal   = {CoRR},
  volume    = {abs/1207.1420},
  year      = {2012},
  url       = {http://arxiv.org/abs/1207.1420},
  archivePrefix = {arXiv},
  eprint    = {1207.1420},
  timestamp = {Wed, 07 Jun 2017 14:41:47 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/abs-1207-1420},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{Clarke:2010:DSP:1870568.1870571,
 author = {Clarke, James and Goldwasser, Dan and Chang, Ming-Wei and Roth, Dan},
 title = {Driving Semantic Parsing from the World's Response},
 booktitle = {Proceedings of the Fourteenth Conference on Computational Natural Language Learning},
 series = {CoNLL '10},
 year = {2010},
 isbn = {978-1-932432-83-1},
 location = {Uppsala, Sweden},
 pages = {18--27},
 numpages = {10},
 url = {http://dl.acm.org/citation.cfm?id=1870568.1870571},
 acmid = {1870571},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
} 


@article{DBLP:journals/corr/HuMLHX16,
  author    = {Zhiting Hu and
               Xuezhe Ma and
               Zhengzhong Liu and
               Eduard H. Hovy and
               Eric P. Xing},
  title     = {Harnessing Deep Neural Networks with Logic Rules},
  journal   = {CoRR},
  volume    = {abs/1603.06318},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.06318},
  timestamp = {Wed, 07 Jun 2017 14:42:52 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/HuMLHX16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/ChenFLVGDZ15,
  author    = {Xinlei Chen and
               Hao Fang and
               Tsung{-}Yi Lin and
               Ramakrishna Vedantam and
               Saurabh Gupta and
               Piotr Doll{\'{a}}r and
               C. Lawrence Zitnick},
  title     = {Microsoft {COCO} Captions: Data Collection and Evaluation Server},
  journal   = {CoRR},
  volume    = {abs/1504.00325},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.00325},
  timestamp = {Wed, 07 Jun 2017 14:41:06 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/ChenFLVGDZ15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{antol2015vqa,
  title={Vqa: Visual question answering},
  author={Antol, Stanislaw and Agrawal, Aishwarya and Lu, Jiasen and Mitchell, Margaret and Batra, Dhruv and Lawrence Zitnick, C and Parikh, Devi},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={2425--2433},
  year={2015}
}

@inproceedings{fang2015captions,
  title={From captions to visual concepts and back},
  author={Fang, Hao and Gupta, Saurabh and Iandola, Forrest and Srivastava, Rupesh K and Deng, Li and Doll{\'a}r, Piotr and Gao, Jianfeng and He, Xiaodong and Mitchell, Margaret and Platt, John C and others},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1473--1482},
  year={2015}
}

@article{tenenbaumetal2006,
    abstract = {{Inductive inference allows humans to make powerful generalizations from sparse data when learning about word meanings, unobserved properties, causal relationships, and many other aspects of the world. Traditional accounts of induction emphasize either the power of statistical learning, or the importance of strong constraints from structured domain knowledge, intuitive theories or schemas. We argue that both components are necessary to explain the nature, use and acquisition of human knowledge, and we introduce a theory-based Bayesian framework for modeling inductive learning and reasoning as statistical inferences over structured knowledge representations.}},
    author = {Tenenbaum, Joshua B. and Griffiths, Thomas L. and Kemp, Charles},
    citeulike-article-id = {715656},
    citeulike-linkout-0 = {http://dx.doi.org/10.1016/j.tics.2006.05.009},
    citeulike-linkout-1 = {http://view.ncbi.nlm.nih.gov/pubmed/16797219},
    citeulike-linkout-2 = {http://www.hubmed.org/display.cgi?uids=16797219},
    citeulike-linkout-3 = {http://www.sciencedirect.com/science/article/B6VH9-4K7NHVY-1/2/04b4431587598b181b73ee9b39bdcb72},
    doi = {10.1016/j.tics.2006.05.009},
    issn = {1364-6613},
    journal = {Trends in cognitive sciences},
    keywords = {bayesian, human\_reasoning, probabilistic-inference, probabilistic-reasoning},
    month = jul,
    number = {7},
    pages = {309--318},
    pmid = {16797219},
    posted-at = {2010-07-26 00:18:39},
    priority = {2},
    title = {{Theory-based Bayesian models of inductive learning and reasoning.}},
    url = {http://dx.doi.org/10.1016/j.tics.2006.05.009},
    volume = {10},
    year = {2006}
}



@inproceedings{mitchell2012midge,
  title={Midge: Generating image descriptions from computer vision detections},
  author={Mitchell, Margaret and Han, Xufeng and Dodge, Jesse and Mensch, Alyssa and Goyal, Amit and Berg, Alex and Yamaguchi, Kota and Berg, Tamara and Stratos, Karl and Daum{\'e} III, Hal},
  booktitle={Proceedings of the 13th Conference of the European Chapter of the Association for Computational Linguistics},
  pages={747--756},
  year={2012},
  organization={Association for Computational Linguistics}
}

@article{sordoni2015neural,
  title={A neural network approach to context-sensitive generation of conversational responses},
  author={Sordoni, Alessandro and Galley, Michel and Auli, Michael and Brockett, Chris and Ji, Yangfeng and Mitchell, Margaret and Nie, Jian-Yun and Gao, Jianfeng and Dolan, Bill},
  journal={arXiv preprint arXiv:1506.06714},
  year={2015}
}

@article{devlin2015language,
  title={Language models for image captioning: The quirks and what works},
  author={Devlin, Jacob and Cheng, Hao and Fang, Hao and Gupta, Saurabh and Deng, Li and He, Xiaodong and Zweig, Geoffrey and Mitchell, Margaret},
  journal={arXiv preprint arXiv:1505.01809},
  year={2015}
}

@article{DBLP:journals/corr/BattagliaPLRK16,
  author    = {Peter W. Battaglia and
               Razvan Pascanu and
               Matthew Lai and
               Danilo Jimenez Rezende and
               Koray Kavukcuoglu},
  title     = {Interaction Networks for Learning about Objects, Relations and Physics},
  journal   = {CoRR},
  volume    = {abs/1612.00222},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.00222},
  archivePrefix = {arXiv},
  eprint    = {1612.00222},
  timestamp = {Wed, 07 Jun 2017 14:42:45 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/BattagliaPLRK16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/FinnGL16,
  author    = {Chelsea Finn and
               Ian J. Goodfellow and
               Sergey Levine},
  title     = {Unsupervised Learning for Physical Interaction through Video Prediction},
  journal   = {CoRR},
  volume    = {abs/1605.07157},
  year      = {2016},
  url       = {http://arxiv.org/abs/1605.07157},
  timestamp = {Wed, 07 Jun 2017 14:42:02 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/FinnGL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@InProceedings{Yatskar_2016_CVPR,
author = {Yatskar, Mark and Zettlemoyer, Luke and Farhadi, Ali},
title = {Situation Recognition: Visual Semantic Role Labeling for Image Understanding },
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2016}
}

@article{DBLP:journals/corr/GuptaM15,
  author    = {Saurabh Gupta and
               Jitendra Malik},
  title     = {Visual Semantic Role Labeling},
  journal   = {CoRR},
  volume    = {abs/1505.04474},
  year      = {2015},
  url       = {http://arxiv.org/abs/1505.04474},
  timestamp = {Wed, 07 Jun 2017 14:42:30 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/GuptaM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/HuangLLN17,
  author    = {De{-}An Huang and
               Joseph J. Lim and
               Fei{-}Fei Li and
               Juan Carlos Niebles},
  title     = {Unsupervised Visual-Linguistic Reference Resolution in Instructional
               Videos},
  journal   = {CoRR},
  volume    = {abs/1703.02521},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.02521},
  timestamp = {Wed, 07 Jun 2017 14:40:45 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/HuangLLN17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{Schaal_TCS_1999,
  title = {Is imitation learning the route to humanoid robots?},
  author = {Schaal, S.},
  booktitle = {Trends in Cognitive Sciences},
  volume = {3},
  number = {6},
  pages = {233-242},
  year = {1999},
  note = {},
  crossref = {p1246},
  url = {http://www-clmc.usc.edu/publications/S/schaal-TICS1999.pdf; http://www-clmc.usc.edu/publications/S/schaal-TICS1999-rep.pdf}
}


@inproceedings{densecap,
  title={DenseCap: Fully Convolutional Localization Networks for Dense Captioning},
  author={Johnson, Justin and Karpathy, Andrej and Fei-Fei, Li},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and 
             Pattern Recognition},
  year={2016}
}

@InProceedings{Alayrac16unsupervised,
    author      = "Alayrac, Jean-Baptiste and Bojanowski, Piotr and Agrawal, Nishant and Laptev, Ivan and Sivic, Josef and Lacoste-Julien, Simon",
    title       = "Unsupervised learning from Narrated Instruction Videos",
    booktitle   = "Computer Vision and Pattern Recognition (CVPR)",
    year        = "2016"
}

}
@inproceedings{krishnavisualgenome,
  title={Visual Genome: Connecting Language and Vision Using Crowdsourced Dense Image Annotations},
  author={Krishna, Ranjay and Zhu, Yuke and Groth, Oliver and Johnson, Justin and Hata, Kenji and Kravitz, Joshua and Chen, Stephanie and Kalanditis, Yannis and Li, Li-Jia and Shamma, David A and Bernstein, Michael and Fei-Fei, Li},
  year = {2016},
}

@inproceedings{Patterson2012SunAttributes,    
Author    = {Genevieve Patterson and James Hays},    
Title     = {SUN Attribute Database:
Discovering, Annotating, and Recognizing Scene Attributes},    
Booktitle = {Proceeding of the 25th Conference on Computer Vision and Pattern Recognition (CVPR)},    
Year      = {2012},  
}

@article{DBLP:journals/corr/JiaL16,
  author    = {Robin Jia and
               Percy Liang},
  title     = {Data Recombination for Neural Semantic Parsing},
  journal   = {CoRR},
  volume    = {abs/1606.03622},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.03622},
  timestamp = {Wed, 07 Jun 2017 14:40:39 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/JiaL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/StadieAS17,
  author    = {Bradly C. Stadie and
               Pieter Abbeel and
               Ilya Sutskever},
  title     = {Third-Person Imitation Learning},
  journal   = {CoRR},
  volume    = {abs/1703.01703},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.01703},
  timestamp = {Wed, 07 Jun 2017 14:40:15 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/StadieAS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@incollection{Nehaniv:2002:CP:762896.762899,
 author = {Nehaniv, Chrystopher L. and Dautenhahn, Kerstin},
 chapter = {The Correspondence Problem},
 title = {Imitation in Animals and Artifacts},
 editor = {Dautenhahn, Kerstin and Nehaniv, Chrystopher L.},
 year = {2002},
 isbn = {0-262-04203-7},
 pages = {41--61},
 numpages = {21},
 url = {http://dl.acm.org/citation.cfm?id=762896.762899},
 acmid = {762899},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 



@article{DBLP:journals/corr/FragkiadakiHAVR17,
  author    = {Katerina Fragkiadaki and
               Jonathan Huang and
               Alex Alemi and
               Sudheendra Vijayanarasimhan and
               Susanna Ricco and
               Rahul Sukthankar},
  title     = {Motion Prediction Under Multimodality with Conditional Stochastic
               Networks},
  journal   = {CoRR},
  volume    = {abs/1705.02082},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.02082},
  timestamp = {Wed, 07 Jun 2017 14:41:48 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/FragkiadakiHAVR17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{Argall:2009:SRL:1523530.1524008,
 author = {Argall, Brenna D. and Chernova, Sonia and Veloso, Manuela and Browning, Brett},
 title = {A Survey of Robot Learning from Demonstration},
 journal = {Robot. Auton. Syst.},
 issue_date = {May, 2009},
 volume = {57},
 number = {5},
 month = may,
 year = {2009},
 issn = {0921-8890},
 pages = {469--483},
 numpages = {15},
 url = {http://dx.doi.org/10.1016/j.robot.2008.10.024},
 doi = {10.1016/j.robot.2008.10.024},
 acmid = {1524008},
 publisher = {North-Holland Publishing Co.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 keywords = {Autonomous systems, Learning from demonstration, Machine learning, Robotics},
} 



@article{Hussein:2017:ILS:3071073.3054912,
 author = {Hussein, Ahmed and Gaber, Mohamed Medhat and Elyan, Eyad and Jayne, Chrisina},
 title = {Imitation Learning: A Survey of Learning Methods},
 journal = {ACM Comput. Surv.},
 issue_date = {June 2017},
 volume = {50},
 number = {2},
 month = apr,
 year = {2017},
 issn = {0360-0300},
 pages = {21:1--21:35},
 articleno = {21},
 numpages = {35},
 url = {http://doi.acm.org/10.1145/3054912},
 doi = {10.1145/3054912},
 acmid = {3054912},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Imitation learning, deep learning, feature representations, intelligent agents, learning from demonstrations, learning from experience, reinforcement learning, robotics, self-improvement},
} 


@article{DBLP:journals/corr/JiaL16,
  author    = {Robin Jia and
               Percy Liang},
  title     = {Data Recombination for Neural Semantic Parsing},
  journal   = {CoRR},
  volume    = {abs/1606.03622},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.03622},
  timestamp = {Wed, 07 Jun 2017 14:40:39 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/JiaL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Zhou2015EndtoendLO,
  title={End-to-end learning of semantic role labeling using recurrent neural networks},
  author={Jie Zhou and Wei Xu},
  booktitle={ACL},
  year={2015}
}


@InProceedings{vedantamLinICCV15,
author = {Ramakrishna Vedantam and Xiao Lin and Tanmay Batra and C. Lawrence Zitnick and Devi Parikh},
title = {Learning Common Sense Through Visual Abstraction},
booktitle = {International Conference on Computer Vision (ICCV)},
year = {2015}
}

@InProceedings{P15-1096,
  author = 	"Misra, Kumar Dipendra
		and Tao, Kejia
		and Liang, Percy
		and Saxena, Ashutosh",
  title = 	"Environment-Driven Lexicon Induction for High-Level Instructions",
  booktitle = 	"Proceedings of the 53rd Annual Meeting of the Association for Computational Linguistics and the 7th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)",
  year = 	"2015",
  publisher = 	"Association for Computational Linguistics",
  pages = 	"992--1002",
  location = 	"Beijing, China",
  doi = 	"10.3115/v1/P15-1096",
  url = 	"http://aclweb.org/anthology/P15-1096"
}



@article{DBLP:journals/corr/AgrawalNAML16,
  author    = {Pulkit Agrawal and
               Ashvin Nair and
               Pieter Abbeel and
               Jitendra Malik and
               Sergey Levine},
  title     = {Learning to Poke by Poking: Experiential Learning of Intuitive Physics},
  journal   = {CoRR},
  volume    = {abs/1606.07419},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.07419},
  timestamp = {Wed, 07 Jun 2017 14:42:59 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/AgrawalNAML16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/McCormacHLD16,
  author    = {John McCormac and
               Ankur Handa and
               Stefan Leutenegger and
               Andrew J. Davison},
  title     = {SceneNet {RGB-D:} 5M Photorealistic Images of Synthetic Indoor Trajectories
               with Ground Truth},
  journal   = {CoRR},
  volume    = {abs/1612.05079},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.05079},
  timestamp = {Wed, 07 Jun 2017 01:00:00 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/McCormacHLD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{sigurdsson2016hollywood,
  author = {Gunnar A. Sigurdsson and G{\"u}l Varol and Xiaolong Wang and Ali Farhadi and Ivan Laptev and Abhinav Gupta},
  title={Hollywood in Homes: Crowdsourcing Data Collection for Activity Understanding},
  booktitle={European Conference on Computer Vision},
  year={2016},
  pdf = {http://arxiv.org/pdf/1604.01753.pdf},
  web = {http://allenai.org/plato/charades/}
}
  
  
@article{Ji:2013:CNN:2412386.2412939,
 author = {Ji, Shuiwang and Xu, Wei and Yang, Ming and Yu, Kai},
 title = {3D Convolutional Neural Networks for Human Action Recognition},
 journal = {IEEE Trans. Pattern Anal. Mach. Intell.},
 issue_date = {January 2013},
 volume = {35},
 number = {1},
 month = jan,
 year = {2013},
 issn = {0162-8828},
 pages = {221--231},
 numpages = {11},
 url = {http://dx.doi.org/10.1109/TPAMI.2012.59},
 doi = {10.1109/TPAMI.2012.59},
 acmid = {2412939},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
 keywords = {Deep learning, convolutional neural networks, 3D convolution, model combination, action recognition},
} 


@inproceedings{Branavan:2012:LHP:2390524.2390543,
 author = {Branavan, S. R. K. and Kushman, Nate and Lei, Tao and Barzilay, Regina},
 title = {Learning High-level Planning from Text},
 booktitle = {Proceedings of the 50th Annual Meeting of the Association for Computational Linguistics: Long Papers - Volume 1},
 series = {ACL '12},
 year = {2012},
 location = {Jeju Island, Korea},
 pages = {126--135},
 numpages = {10},
 url = {http://dl.acm.org/citation.cfm?id=2390524.2390543},
 acmid = {2390543},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
} 


@article{Chu:2015:RLH:2947721.2947949,
 author = {Chu, Vivian and McMahon, Ian and Riano, Lorenzo and McDonald, Craig G. and He, Qin and Martinez Perez-Tejada, Jorge and Arrigo, Michael and Darrell, Trevor and Kuchenbecker, Katherine J.},
 title = {Robotic Learning of Haptic Adjectives Through Physical Interaction},
 journal = {Robot. Auton. Syst.},
 issue_date = {January 2015},
 volume = {63},
 number = {P3},
 month = jan,
 year = {2015},
 issn = {0921-8890},
 pages = {279--292},
 numpages = {14},
 url = {http://dx.doi.org/10.1016/j.robot.2014.09.021},
 doi = {10.1016/j.robot.2014.09.021},
 acmid = {2947949},
 publisher = {North-Holland Publishing Co.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 keywords = {Haptics, Machine learning, Robotic perception, Tactile sensing, Time-series classification},
} 

@inproceedings{conf/emnlp/BerantCFL13,
  added-at = {2013-11-10T00:00:00.000+0100},
  author = {Berant, Jonathan and Chou, Andrew and Frostig, Roy and Liang, Percy},
  biburl = {https://www.bibsonomy.org/bibtex/2b7403aae1579048cfe77e88fb67a4704/dblp},
  booktitle = {EMNLP},
  ee = {http://aclweb.org/anthology//D/D13/D13-1160.pdf},
  interhash = {6f5f5cf4aab75502a5e67454eb6679b4},
  intrahash = {b7403aae1579048cfe77e88fb67a4704},
  isbn = {978-1-937284-97-8},
  keywords = {dblp},
  pages = {1533-1544},
  publisher = {ACL},
  timestamp = {2013-11-12T11:34:07.000+0100},
  title = {Semantic Parsing on Freebase from Question-Answer Pairs.},
  url = {http://dblp.uni-trier.de/db/conf/emnlp/emnlp2013.html#BerantCFL13},
  year = 2013
}

@inproceedings{Branavan:2009:RLM:1687878.1687892,
 author = {Branavan, S. R. K. and Chen, Harr and Zettlemoyer, Luke S. and Barzilay, Regina},
 title = {Reinforcement Learning for Mapping Instructions to Actions},
 booktitle = {Proceedings of the Joint Conference of the 47th Annual Meeting of the ACL and the 4th International Joint Conference on Natural Language Processing of the AFNLP: Volume 1 - Volume 1},
 series = {ACL '09},
 year = {2009},
 isbn = {978-1-932432-45-9},
 location = {Suntec, Singapore},
 pages = {82--90},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=1687878.1687892},
 acmid = {1687892},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
} 


@article{young-etal-2014,
    author = {Young, Peter and Lai, Alice and Hodosh, Micah and Hockenmaier, Julia},
    citeulike-article-id = {13652898},
    journal = {Transactions of the Association for Computational Linguistics},
    keywords = {semantics, vision},
    pages = {67--78},
    posted-at = {2015-06-22 00:30:56},
    priority = {2},
    title = {{From image descriptions to visual denotations: New similarity metrics for semantic inference over event descriptions}},
    volume = {2},
    year = {2014}
}

@inproceedings{Clarke:2010:DSP:1870568.1870571,
 author = {Clarke, James and Goldwasser, Dan and Chang, Ming-Wei and Roth, Dan},
 title = {Driving Semantic Parsing from the World's Response},
 booktitle = {Proceedings of the Fourteenth Conference on Computational Natural Language Learning},
 series = {CoNLL '10},
 year = {2010},
 isbn = {978-1-932432-83-1},
 location = {Uppsala, Sweden},
 pages = {18--27},
 numpages = {10},
 url = {http://dl.acm.org/citation.cfm?id=1870568.1870571},
 acmid = {1870571},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
} 


@inproceedings{conf/emnlp/BerantCFL13,
  added-at = {2013-11-10T00:00:00.000+0100},
  author = {Berant, Jonathan and Chou, Andrew and Frostig, Roy and Liang, Percy},
  biburl = {https://www.bibsonomy.org/bibtex/2b7403aae1579048cfe77e88fb67a4704/dblp},
  booktitle = {EMNLP},
  crossref = {conf/emnlp/2013},
  ee = {http://aclweb.org/anthology//D/D13/D13-1160.pdf},
  interhash = {6f5f5cf4aab75502a5e67454eb6679b4},
  intrahash = {b7403aae1579048cfe77e88fb67a4704},
  isbn = {978-1-937284-97-8},
  keywords = {dblp},
  pages = {1533-1544},
  publisher = {ACL},
  timestamp = {2013-11-12T11:34:07.000+0100},
  title = {Semantic Parsing on Freebase from Question-Answer Pairs.},
  url = {http://dblp.uni-trier.de/db/conf/emnlp/emnlp2013.html#BerantCFL13},
  year = 2013
}




@paper{AAAI1612383,
	author = {Amos Azaria and Jayant Krishnamurthy and Tom Mitchell},
	title = {Instructable Intelligent Personal Agent},
	conference = {AAAI Conference on Artificial Intelligence},
	year = {2016},
	keywords = {Learning by Instructions; Instructable Agent; Learning in Natural Language},
	url = {https://www.aaai.org/ocs/index.php/AAAI/AAAI16/paper/view/12383}
}

@inproceedings{huang2016visual,
  title={Visual Storytelling},
  author={Huang, Ting-Hao K. and Ferraro, Francis and Mostafazadeh, Nasrin and Misra, Ishan and Devlin, Jacob and Agrawal, Aishwarya and Girshick, Ross and He, Xiaodong and Kohli, Pushmeet and Batra, Dhruv and others},
  booktitle={15th Annual Conference of the North American Chapter of the Association for Computational Linguistics (NAACL 2016)},
  year={2016}
}


@inproceedings{DBLP:conf/emnlp/HeLZ15,
  author    = {Luheng He and
               Mike Lewis and
               Luke Zettlemoyer},
  title     = {Question-Answer Driven Semantic Role Labeling: Using Natural Language
               to Annotate Natural Language},
  booktitle = {Proceedings of the 2015 Conference on Empirical Methods in Natural
               Language Processing, {EMNLP} 2015, Lisbon, Portugal, September 17-21,
               2015},
  pages     = {643--653},
  year      = {2015},
  crossref  = {DBLP:conf/emnlp/2015},
  url       = {http://aclweb.org/anthology/D/D15/D15-1076.pdf},
  timestamp = {Wed, 14 Oct 2015 09:56:24 +0200},
  biburl    = {http://dblp.org/rec/bib/conf/emnlp/HeLZ15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/LiangBLFL16,
  author    = {Chen Liang and
               Jonathan Berant and
               Quoc Le and
               Kenneth D. Forbus and
               Ni Lao},
  title     = {Neural Symbolic Machines: Learning Semantic Parsers on Freebase with
               Weak Supervision},
  journal   = {CoRR},
  volume    = {abs/1611.00020},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.00020},
  archivePrefix = {arXiv},
  eprint    = {1611.00020},
  timestamp = {Wed, 07 Jun 2017 14:42:59 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LiangBLFL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{semantic-parsing-via-staged-query-graph-generation-question-answering-with-knowledge-base,
author = {Yih, Scott Wen-tau and Chang, Ming-Wei and He, Xiaodong and Gao, Jianfeng},
title = {Semantic Parsing via Staged Query Graph Generation: Question Answering with Knowledge Base},
booktitle = {},
year = {2015},
month = {July},
publisher = {ACL – Association for Computational Linguistics}
}

@INPROCEEDINGS{Mitchell93explanationbased,
    author = {Tom M. Mitchell},
    title = {Explanation based learning: A comparison of symbolic and neural network approaches},
    booktitle = {Proceedings of the Tenth International Conference on Machine Learning},
    year = {1993},
    pages = {197--204},
    publisher = {Morgan Kaufmann}
}

@inproceedings{zhou2015end,
  title={End-to-end learning of semantic role labeling using recurrent neural networks.},
  author={Zhou, Jie and Xu, Wei},
  booktitle={ACL (1)},
  pages={1127--1137},
  year={2015}
}
@article{DBLP:journals/corr/JohnsonHMHLZG17,
  author    = {Justin Johnson and
               Bharath Hariharan and
               Laurens van der Maaten and
               Judy Hoffman and
               Fei{-}Fei Li and
               C. Lawrence Zitnick and
               Ross B. Girshick},
  title     = {Inferring and Executing Programs for Visual Reasoning},
  journal   = {CoRR},
  volume    = {abs/1705.03633},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.03633},
  timestamp = {Wed, 07 Jun 2017 14:42:58 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/JohnsonHMHLZG17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/HeLZ15,
  author    = {Luheng He and
               Mike Lewis and
               Luke Zettlemoyer},
  title     = {Question-Answer Driven Semantic Role Labeling: Using Natural Language
               to Annotate Natural Language},
  booktitle = {Proceedings of the 2015 Conference on Empirical Methods in Natural
               Language Processing, {EMNLP} 2015, Lisbon, Portugal, September 17-21,
               2015},
  pages     = {643--653},
  year      = {2015},
}

@article{DBLP:journals/corr/RajpurkarZLL16,
  author    = {Pranav Rajpurkar and
               Jian Zhang and
               Konstantin Lopyrev and
               Percy Liang},
  title     = {SQuAD: 100, 000+ Questions for Machine Comprehension of Text},
  journal   = {CoRR},
  volume    = {abs/1606.05250},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.05250},
  timestamp = {Wed, 07 Jun 2017 14:41:34 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RajpurkarZLL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/WestonBCM15,
  author    = {Jason Weston and
               Antoine Bordes and
               Sumit Chopra and
               Tomas Mikolov},
  title     = {Towards AI-Complete Question Answering: {A} Set of Prerequisite Toy
               Tasks},
  journal   = {CoRR},
  volume    = {abs/1502.05698},
  year      = {2015},
  url       = {http://arxiv.org/abs/1502.05698},
  timestamp = {Wed, 07 Jun 2017 14:42:32 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/WestonBCM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/HewlettLJPFHKB16,
  author    = {Daniel Hewlett and
               Alexandre Lacoste and
               Llion Jones and
               Illia Polosukhin and
               Andrew Fandrianto and
               Jay Han and
               Matthew Kelcey and
               David Berthelot},
  title     = {WikiReading: {A} Novel Large-scale Language Understanding Task over
               Wikipedia},
  journal   = {CoRR},
  volume    = {abs/1608.03542},
  year      = {2016},
  url       = {http://arxiv.org/abs/1608.03542},
  timestamp = {Wed, 07 Jun 2017 14:41:20 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/HewlettLJPFHKB16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}




@article{doi:10.1162/1064546053278973,
author = { Linda Smith  and  Michael Gasser },
title = {The Development of Embodied Cognition: Six Lessons from Babies},
journal = {Artificial Life},
volume = {11},
number = {1-2},
pages = {13-29},
year = {2005},
doi = {10.1162/1064546053278973},

URL = { 
        https://doi.org/10.1162/1064546053278973
    
},
eprint = { 
        https://doi.org/10.1162/1064546053278973
    
}
,
    abstract = { The embodiment hypothesis is the idea that intelligence emerges in the interaction of an agent with an environment and as a result of sensorimotor activity. We offer six lessons for developing embodied intelligent agents suggested by research in developmental psychology. We argue that starting as a baby grounded in a physical, social, and linguistic world is crucial to the development of the flexible and inventive intelligence that characterizes humankind. }
}




@article{DBLP:journals/corr/LillicrapHPHETS15,
  author    = {Timothy P. Lillicrap and
               Jonathan J. Hunt and
               Alexander Pritzel and
               Nicolas Heess and
               Tom Erez and
               Yuval Tassa and
               David Silver and
               Daan Wierstra},
  title     = {Continuous control with deep reinforcement learning},
  journal   = {CoRR},
  volume    = {abs/1509.02971},
  year      = {2015},
  url       = {http://arxiv.org/abs/1509.02971},
  archivePrefix = {arXiv},
  eprint    = {1509.02971},
  timestamp = {Wed, 07 Jun 2017 14:40:26 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LillicrapHPHETS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/KanskySMELLDSPG17,
  author    = {Ken Kansky and
               Tom Silver and
               David A. M{\'{e}}ly and
               Mohamed Eldawy and
               Miguel L{\'{a}}zaro{-}Gredilla and
               Xinghua Lou and
               Nimrod Dorfman and
               Szymon Sidor and
               D. Scott Phoenix and
               Dileep George},
  title     = {Schema Networks: Zero-shot Transfer with a Generative Causal Model
               of Intuitive Physics},
  journal   = {CoRR},
  volume    = {abs/1706.04317},
  year      = {2017},
  url       = {http://arxiv.org/abs/1706.04317},
  archivePrefix = {arXiv},
  eprint    = {1706.04317},
  timestamp = {Tue, 04 Jul 2017 09:48:42 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/KanskySMELLDSPG17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/HausmanCSSL17,
  author    = {Karol Hausman and
               Yevgen Chebotar and
               Stefan Schaal and
               Gaurav S. Sukhatme and
               Joseph J. Lim},
  title     = {Multi-Modal Imitation Learning from Unstructured Demonstrations using
               Generative Adversarial Nets},
  journal   = {CoRR},
  volume    = {abs/1705.10479},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.10479},
  archivePrefix = {arXiv},
  eprint    = {1705.10479},
  timestamp = {Sun, 26 Nov 2017 16:54:43 +0100},
  biburl    = {http://dblp.org/rec/bib/journals/corr/HausmanCSSL17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/FinnL16,
  author    = {Chelsea Finn and
               Sergey Levine},
  title     = {Deep Visual Foresight for Planning Robot Motion},
  journal   = {CoRR},
  volume    = {abs/1610.00696},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.00696},
  archivePrefix = {arXiv},
  eprint    = {1610.00696},
  timestamp = {Wed, 07 Jun 2017 14:42:20 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/FinnL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/NairCAIAML17,
  author    = {Ashvin Nair and
               Dian Chen and
               Pulkit Agrawal and
               Phillip Isola and
               Pieter Abbeel and
               Jitendra Malik and
               Sergey Levine},
  title     = {Combining Self-Supervised Learning and Imitation for Vision-Based
               Rope Manipulation},
  journal   = {CoRR},
  volume    = {abs/1703.02018},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.02018},
  archivePrefix = {arXiv},
  eprint    = {1703.02018},
  timestamp = {Wed, 07 Jun 2017 14:41:24 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/NairCAIAML17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/abs-1709-10087,
  author    = {Aravind Rajeswaran and
               Vikash Kumar and
               Abhishek Gupta and
               John Schulman and
               Emanuel Todorov and
               Sergey Levine},
  title     = {Learning Complex Dexterous Manipulation with Deep Reinforcement Learning
               and Demonstrations},
  journal   = {CoRR},
  volume    = {abs/1709.10087},
  year      = {2017},
  url       = {http://arxiv.org/abs/1709.10087},
  archivePrefix = {arXiv},
  eprint    = {1709.10087},
  timestamp = {Thu, 05 Oct 2017 09:43:05 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/abs-1709-10087},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{JMLR:v16:vapnik15b,
  author  = {Vladimir Vapnik and Rauf Izmailov},
  title   = {Learning Using Privileged Information: Similarity Control and Knowledge Transfer},
  journal = {Journal of Machine Learning Research},
  year    = {2015},
  volume  = {16},
  pages   = {2023-2049},
  url     = {http://jmlr.org/papers/v16/vapnik15b.html}
}

@article{DBLP:journals/corr/FinnLA16,
  author    = {Chelsea Finn and
               Sergey Levine and
               Pieter Abbeel},
  title     = {Guided Cost Learning: Deep Inverse Optimal Control via Policy Optimization},
  journal   = {CoRR},
  volume    = {abs/1603.00448},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.00448},
  archivePrefix = {arXiv},
  eprint    = {1603.00448},
  timestamp = {Wed, 07 Jun 2017 14:41:08 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/FinnLA16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Ng:2000:AIR:645529.657801,
 author = {Ng, Andrew Y. and Russell, Stuart J.},
 title = {Algorithms for Inverse Reinforcement Learning},
 booktitle = {Proceedings of the Seventeenth International Conference on Machine Learning},
 series = {ICML '00},
 year = {2000},
 isbn = {1-55860-707-2},
 pages = {663--670},
 numpages = {8},
 url = {http://dl.acm.org/citation.cfm?id=645529.657801},
 acmid = {657801},
 publisher = {Morgan Kaufmann Publishers Inc.},
 address = {San Francisco, CA, USA},
} 




@article{DBLP:journals/corr/ChenFLVGDZ15,
  author    = {Xinlei Chen and
               Hao Fang and
               Tsung{-}Yi Lin and
               Ramakrishna Vedantam and
               Saurabh Gupta and
               Piotr Doll{\'{a}}r and
               C. Lawrence Zitnick},
  title     = {Microsoft {COCO} Captions: Data Collection and Evaluation Server},
  journal   = {CoRR},
  volume    = {abs/1504.00325},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.00325},
  archivePrefix = {arXiv},
  eprint    = {1504.00325},
  timestamp = {Wed, 07 Jun 2017 14:41:06 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/ChenFLVGDZ15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/GuHLL16,
  author    = {Shixiang Gu and
               Ethan Holly and
               Timothy P. Lillicrap and
               Sergey Levine},
  title     = {Deep Reinforcement Learning for Robotic Manipulation},
  journal   = {CoRR},
  volume    = {abs/1610.00633},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.00633},
  archivePrefix = {arXiv},
  eprint    = {1610.00633},
  timestamp = {Wed, 07 Jun 2017 14:40:31 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/GuHLL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/KroemerS16,
  author    = {Oliver Kroemer and
               Gaurav S. Sukhatme},
  title     = {Learning Relevant Features for Manipulation Skills using Meta-Level
               Priors},
  journal   = {CoRR},
  volume    = {abs/1605.04439},
  year      = {2016},
  url       = {http://arxiv.org/abs/1605.04439},
  archivePrefix = {arXiv},
  eprint    = {1605.04439},
  timestamp = {Wed, 07 Jun 2017 14:42:29 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/KroemerS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Akgun:2012:TKK:2157689.2157815,
 author = {Akgun, Baris and Cakmak, Maya and Yoo, Jae Wook and Thomaz, Andrea Lockerd},
 title = {Trajectories and Keyframes for Kinesthetic Teaching: A Human-robot Interaction Perspective},
 booktitle = {Proceedings of the Seventh Annual ACM/IEEE International Conference on Human-Robot Interaction},
 series = {HRI '12},
 year = {2012},
 isbn = {978-1-4503-1063-5},
 location = {Boston, Massachusetts, USA},
 pages = {391--398},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/2157689.2157815},
 doi = {10.1145/2157689.2157815},
 acmid = {2157815},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {learning from demonstration},
} 



@article{DBLP:journals/corr/SungJS15,
  author    = {Jaeyong Sung and
               Seok Hyun Jin and
               Ashutosh Saxena},
  title     = {Robobarista: Object Part based Transfer of Manipulation Trajectories
               from Crowd-sourcing in 3D Pointclouds},
  journal   = {CoRR},
  volume    = {abs/1504.03071},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.03071},
  archivePrefix = {arXiv},
  eprint    = {1504.03071},
  timestamp = {Wed, 07 Jun 2017 14:42:19 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/SungJS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/RahmatizadehABL17,
  author    = {Rouhollah Rahmatizadeh and
               Pooya Abolghasemi and
               Ladislau B{\"{o}}l{\"{o}}ni and
               Sergey Levine},
  title     = {Vision-Based Multi-Task Manipulation for Inexpensive Robots Using
               End-To-End Learning from Demonstration},
  journal   = {CoRR},
  volume    = {abs/1707.02920},
  year      = {2017},
  url       = {http://arxiv.org/abs/1707.02920},
  archivePrefix = {arXiv},
  eprint    = {1707.02920},
  timestamp = {Sat, 05 Aug 2017 14:56:06 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/RahmatizadehABL17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{DBLP:journals/corr/LiuGAL17,
  author    = {Yuxuan Liu and
               Abhishek Gupta and
               Pieter Abbeel and
               Sergey Levine},
  title     = {Imitation from Observation: Learning to Imitate Behaviors from Raw
               Video via Context Translation},
  journal   = {CoRR},
  volume    = {abs/1707.03374},
  year      = {2017},
  url       = {http://arxiv.org/abs/1707.03374},
  archivePrefix = {arXiv},
  eprint    = {1707.03374},
  timestamp = {Sat, 05 Aug 2017 14:56:08 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LiuGAL17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{PatrauceanHC16,
  author    = {Viorica P{\u a}tr{\u a}ucean and
               Ankur Handa and
               Roberto Cipolla},
  title     = {Spatio-temporal video autoencoder with differentiable memory},
  booktitle = {International Conference on Learning Representations (ICLR) Workshop},
  year      = {2016}
}


@article{DBLP:journals/corr/SadeghianAS17,
  author    = {Amir Sadeghian and
               Alexandre Alahi and
               Silvio Savarese},
  title     = {Tracking The Untrackable: Learning To Track Multiple Cues with Long-Term
               Dependencies},
  journal   = {CoRR},
  volume    = {abs/1701.01909},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.01909},
  timestamp = {Wed, 07 Jun 2017 14:40:23 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/SadeghianAS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/McCormacHDL16,
  author    = {John McCormac and
               Ankur Handa and
               Andrew J. Davison and
               Stefan Leutenegger},
  title     = {SemanticFusion: Dense 3D Semantic Mapping with Convolutional Neural
               Networks},
  journal   = {CoRR},
  volume    = {abs/1609.05130},
  year      = {2016},
  url       = {http://arxiv.org/abs/1609.05130},
  timestamp = {Wed, 07 Jun 2017 14:42:17 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/McCormacHDL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/MalmaudHRJRM15,
  author    = {Jonathan Malmaud and
               Jonathan Huang and
               Vivek Rathod and
               Nick Johnston and
               Andrew Rabinovich and
               Kevin Murphy},
  title     = {What's Cookin'? Interpreting Cooking Videos using Text, Speech and
               Vision},
  journal   = {CoRR},
  volume    = {abs/1503.01558},
  year      = {2015},
  url       = {http://arxiv.org/abs/1503.01558},
  timestamp = {Wed, 07 Jun 2017 14:42:04 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MalmaudHRJRM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/RedmonF16,
  author    = {Joseph Redmon and
               Ali Farhadi},
  title     = {{YOLO9000:} Better, Faster, Stronger},
  journal   = {CoRR},
  volume    = {abs/1612.08242},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.08242},
  timestamp = {Wed, 07 Jun 2017 14:40:20 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RedmonF16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/LongSD14,
  author    = {Jonathan Long and
               Evan Shelhamer and
               Trevor Darrell},
  title     = {Fully Convolutional Networks for Semantic Segmentation},
  journal   = {CoRR},
  volume    = {abs/1411.4038},
  year      = {2014},
  url       = {http://arxiv.org/abs/1411.4038},
  timestamp = {Wed, 07 Jun 2017 14:42:28 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LongSD14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@ARTICLE{SilverHuangEtAl16nature,
  author = {Silver, David and Huang, Aja and Maddison, Chris J. and Guez, Arthur and Sifre, Laurent and van den Driessche, George and Schrittwieser, Julian and Antonoglou, Ioannis and Panneershelvam, Veda and Lanctot, Marc and Dieleman, Sander and Grewe, Dominik and Nham, John and Kalchbrenner, Nal and Sutskever, Ilya and Lillicrap, Timothy and Leach, Madeleine and Kavukcuoglu, Koray and Graepel, Thore and Hassabis, Demis},
  journal = {Nature},
  title = {Mastering the Game of Go with Deep Neural Networks and Tree Search},
  volume = {529},
  year = {2016}
}

@inproceedings{Hasselt:2016:DRL:3016100.3016191,
 author = {Hasselt, Hado van and Guez, Arthur and Silver, David},
 title = {Deep Reinforcement Learning with Double Q-Learning},
 booktitle = {Proceedings of the Thirtieth AAAI Conference on Artificial Intelligence},
 series = {AAAI'16},
 year = {2016},
 location = {Phoenix, Arizona},
 pages = {2094--2100},
 numpages = {7},
 url = {http://dl.acm.org/citation.cfm?id=3016100.3016191},
 acmid = {3016191},
 publisher = {AAAI Press},
} 


@inproceedings{cao2017realtime,
  author = {Zhe Cao and Tomas Simon and Shih-En Wei and Yaser Sheikh},
  booktitle = {CVPR},
  title = {Realtime Multi-Person 2D Pose Estimation using Part Affinity Fields},
  year = {2017}
}

@inproceedings{simon2017hand,
  author = {Tomas Simon and Hanbyul Joo and Iain Matthews and Yaser Sheikh},
  booktitle = {CVPR},
  title = {Hand Keypoint Detection in Single Images using Multiview Bootstrapping},
  year = {2017}
}

@inproceedings{wei2016cpm,
  author = {Shih-En Wei and Varun Ramakrishna and Takeo Kanade and Yaser Sheikh},
  booktitle = {CVPR},
  title = {Convolutional pose machines},
  year = {2016}
}

@article{DBLP:journals/corr/PathakAED17,
  author    = {Deepak Pathak and
               Pulkit Agrawal and
               Alexei A. Efros and
               Trevor Darrell},
  title     = {Curiosity-driven Exploration by Self-supervised Prediction},
  journal   = {CoRR},
  volume    = {abs/1705.05363},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.05363},
  archivePrefix = {arXiv},
  eprint    = {1705.05363},
  timestamp = {Wed, 07 Jun 2017 14:41:47 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/PathakAED17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@ARTICLE{Browne2012,
  ABSTRACT = {Monte Carlo Tree Search (MCTS) is a recently proposed search method that combines the precision of tree search with the generality of random sampling. It has received considerable interest due to its spectacular success in the difficult problem of computer Go, but has also proved beneficial in a range of other domains. This paper is a survey of the literature to date, intended to provide a snapshot of the state of the art after the first five years of MCTS research. We outline the core algorithm’s derivation, impart some structure on the many variations and enhancements that have been proposed, and summarise the results from the key game and non-game domains to which MCTS methods have been applied. A number of open research questions indicate that the field is ripe for future work.},
  AUTHOR   = {Browne, Cb and Powley, Edward},
  DOI      = {10.1109/TCIAIG.2012.2186810},
  FILE     = {http://bib.unthinkingdepths.fr/seb/pdf/Browne, Powley_2012_A survey of monte carlo tree search methods.pdf},
  ISSN     = {1943-068X},
  JOURNAL  = {Intelligence and AI},
  NUMBER   = {1},
  PAGES    = {1--49},
  TITLE    = {{A survey of monte carlo tree search methods}},
  URL      = {http://ieeexplore.ieee.org/xpls/abs_all.jsp?arnumber=6145622},
  VOLUME   = {4},
  YEAR     = {2012},
}


@article{DBLP:journals/corr/KhorevaBIBS17,
  author    = {Anna Khoreva and
               Rodrigo Benenson and
               Eddy Ilg and
               Thomas Brox and
               Bernt Schiele},
  title     = {Lucid Data Dreaming for Object Tracking},
  journal   = {CoRR},
  volume    = {abs/1703.09554},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.09554},
  timestamp = {Wed, 07 Jun 2017 14:43:15 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KhorevaBIBS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@INPROCEEDINGS{Whelan-RSS-15, 
    AUTHOR    = {Thomas Whelan AND Stefan Leutenegger AND Renato Salas Moreno AND Ben Glocker AND Andrew Davison}, 
    TITLE     = {ElasticFusion: Dense SLAM Without A Pose Graph}, 
    BOOKTITLE = {Proceedings of Robotics: Science and Systems}, 
    YEAR      = {2015}, 
    ADDRESS   = {Rome, Italy}, 
    MONTH     = {July},
    DOI       = {10.15607/RSS.2015.XI.001} 
} 
  
  
@article{DBLP:journals/corr/RitchieHG16,
  author    = {Daniel Ritchie and
               Paul Horsfall and
               Noah D. Goodman},
  title     = {Deep Amortized Inference for Probabilistic Programs},
  journal   = {CoRR},
  volume    = {abs/1610.05735},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.05735},
  timestamp = {Wed, 07 Jun 2017 14:42:26 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RitchieHG16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@misc{ceres-solver,
  author = "Sameer Agarwal and Keir Mierle and Others",
  title = "Ceres Solver",
  howpublished = "\url{http://ceres-solver.org}",
}

@article{DBLP:journals/corr/CarreiraAFM15,
  author    = {Jo{\~{a}}o Carreira and
               Pulkit Agrawal and
               Katerina Fragkiadaki and
               Jitendra Malik},
  title     = {Human Pose Estimation with Iterative Error Feedback},
  journal   = {CoRR},
  volume    = {abs/1507.06550},
  year      = {2015},
}

@article{DBLP:journals/corr/FischerDIHHGSCB15,
  author    = {Philipp Fischer and
               Alexey Dosovitskiy and
               Eddy Ilg and
               Philip H{\"{a}}usser and
               Caner Hazirbas and
               Vladimir Golkov and
               Patrick van der Smagt and
               Daniel Cremers and
               Thomas Brox},
  title     = {FlowNet: Learning Optical Flow with Convolutional Networks},
  journal   = {CoRR},
  volume    = {abs/1504.06852},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.06852},
  timestamp = {Wed, 07 Jun 2017 14:41:04 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/FischerDIHHGSCB15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@incollection{NIPS2014_5421,
title = {Deep Learning for Real-Time Atari Game Play Using Offline Monte-Carlo Tree Search Planning},
author = {Guo, Xiaoxiao and Singh, Satinder and Lee, Honglak and Lewis, Richard L and Wang, Xiaoshi},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {3338--3346},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5421-deep-learning-for-real-time-atari-game-play-using-offline-monte-carlo-tree-search-planning.pdf}
}

@inproceedings{Silberer2013ModelsOS,
  title={Models of Semantic Representation with Visual Attributes},
  author={Carina Silberer and Vittorio Ferrari and Mirella Lapata},
  booktitle={ACL},
  year={2013}
}

@article{carreira2017quo,
  title={Quo Vadis, Action Recognition? A New Model and the Kinetics Dataset},
  author={Carreira, Joao and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1705.07750},
  year={2017}
}

@article{DBLP:journals/corr/WestonCB14,
  author    = {Jason Weston and
               Sumit Chopra and
               Antoine Bordes},
  title     = {Memory Networks},
  journal   = {CoRR},
  volume    = {abs/1410.3916},
  year      = {2014},
  url       = {http://arxiv.org/abs/1410.3916},
  timestamp = {Wed, 07 Jun 2017 14:41:04 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/WestonCB14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@incollection{NIPS2015_5945,
title = {Teaching Machines to Read and Comprehend},
author = {Hermann, Karl Moritz and Kocisky, Tomas and Grefenstette, Edward and Espeholt, Lasse and Kay, Will and Suleyman, Mustafa and Blunsom, Phil},
booktitle = {Advances in Neural Information Processing Systems 28},
editor = {C. Cortes and N. D. Lawrence and D. D. Lee and M. Sugiyama and R. Garnett},
pages = {1693--1701},
year = {2015},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5945-teaching-machines-to-read-and-comprehend.pdf}
}

@article{DBLP:journals/corr/KadlecSBK16,
  author    = {Rudolf Kadlec and
               Martin Schmid and
               Ondrej Bajgar and
               Jan Kleindienst},
  title     = {Text Understanding with the Attention Sum Reader Network},
  journal   = {CoRR},
  volume    = {abs/1603.01547},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.01547},
  timestamp = {Wed, 07 Jun 2017 14:41:38 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KadlecSBK16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Article:00:Glenberg:hallsa,
    author = {Glenberg, A. and Robertson, D.},
    citeulike-article-id = {850491},
    citeulike-linkout-0 = {http://psych.wisc.edu/glenberg/},
    journal = {Journal of {M}emory and {L}anguage},
    keywords = {bibtex-import},
    posted-at = {2006-09-20 03:18:45},
    priority = {0},
    title = {Symbol grounding and meaning: {A} comparison of high-dimensional and embodied theories of meaning.},
    url = {http://psych.wisc.edu/glenberg/},
    year = {2000}
}



@article{DBLP:journals/corr/DhingraLCS16,
  author    = {Bhuwan Dhingra and
               Hanxiao Liu and
               William W. Cohen and
               Ruslan Salakhutdinov},
  title     = {Gated-Attention Readers for Text Comprehension},
  journal   = {CoRR},
  volume    = {abs/1606.01549},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.01549},
  timestamp = {Wed, 07 Jun 2017 14:42:11 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/DhingraLCS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/SeoKFH16,
  author    = {Min Joon Seo and
               Aniruddha Kembhavi and
               Ali Farhadi and
               Hannaneh Hajishirzi},
  title     = {Bidirectional Attention Flow for Machine Comprehension},
  journal   = {CoRR},
  volume    = {abs/1611.01603},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.01603},
  timestamp = {Wed, 07 Jun 2017 14:41:03 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/SeoKFH16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}







@inproceedings{donahue2015long,
  title={Long-term Recurrent Convolutional Networks for Visual Recognition and Description},
  author={Donahue, Jeff and Hendricks, Lisa Anne and Guadarrama, Sergio and Rohrbach, Marcus and Venugopalan, Subhashini and Saenko, Kate and Darrell, Trevor},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2015}
}



@inproceedings{kazemi2014one,
  title={One Millisecond Face Alignment with an Ensemble of Regression Trees},
  author={Kazemi, Vahid and Sullivan, Josephine},
  booktitle={CVPR},
  year={2014}
}

@article{DBLP:journals/corr/KimLL15a,
  author    = {Jiwon Kim and
               Jung Kwon Lee and
               Kyoung Mu Lee},
  title     = {Deeply-Recursive Convolutional Network for Image Super-Resolution},
  journal   = {CoRR},
  volume    = {abs/1511.04491},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.04491},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KimLL15a},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{pennington2014glove,
  author = {Jeffrey Pennington and Richard Socher and Christopher D. Manning},
  booktitle = {Empirical Methods in Natural Language Processing (EMNLP)},
  title = {GloVe: Global Vectors for Word Representation},
  year = {2014},
  pages = {1532--1543},
  url = {http://www.aclweb.org/anthology/D14-1162},
}

@article{Gupta:2015:ISU:2750551.2750559,
 author = {Gupta, Saurabh and Arbel\'{a}ez, Pablo and Girshick, Ross and Malik, Jitendra},
 title = {Indoor Scene Understanding with RGB-D Images: Bottom-up Segmentation, Object Detection and Semantic Segmentation},
 journal = {Int. J. Comput. Vision},
 issue_date = {April     2015},
 volume = {112},
 number = {2},
 month = apr,
 year = {2015},
 issn = {0920-5691},
 pages = {133--149},
 numpages = {17},
 url = {http://dx.doi.org/10.1007/s11263-014-0777-6},
 doi = {10.1007/s11263-014-0777-6},
 acmid = {2750559},
 publisher = {Kluwer Academic Publishers},
 address = {Hingham, MA, USA},
 keywords = {RGB-D contour detection, RGB-D image segmentation, RGB-D object detection, RGB-D scene classification, RGB-D semantic segmentation},
} 

@article{DBLP:journals/corr/TungHSF17,
  author    = {Hsiao{-}Yu Fish Tung and
               Adam Harley and
               William Seto and
               Katerina Fragkiadaki},
  title     = {Adversarial Inversion: Inverse Graphics with Adversarial Priors},
  journal   = {CoRR},
  volume    = {abs/1705.11166},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.11166},
  timestamp = {Wed, 07 Jun 2017 14:41:13 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/TungHSF17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{mocap,
  author    = {Hsiao{-}Yu Fish Tung and
               Wei Tung and
               Ersin Yumer and
               Katerina Fragkiadaki},
  title     = {Self-supervised learning of Motion Capture},
  journal   = {under submission},
  year      = {2017}
}

@inproceedings{andriluka14cvpr,
               author = {Mykhaylo Andriluka and Leonid Pishchulin and Peter Gehler and Schiele, Bernt},
               title = {2D Human Pose Estimation: New Benchmark and State of the Art Analysis},
               booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
               year = {2014},
               month = {June}
}
@article{inversionearlier,
  author    = {Fish Tung and Katerina Fragkiadaki},
  title     = {Inverse Problems in Computer Vision with Adversarial Imagination Priors},
  journal   = {openreview},
  year      = {2016}
}




@article{deeppaint,
  author    = {Kushagr Gupta and
               Suleman Kazi and
               Terry Kong},
  title     = {DeepPaint: A Tool for Image Inpainting},
  journal   = {tech. report},
  year      = {2016}
}

@article{DBLP:journals/corr/DongNWG17,
  author    = {Hao Dong and
               Paarth Neekhara and
               Chao Wu and
               Yike Guo},
  title     = {Unsupervised Image-to-Image Translation with Generative Adversarial
               Networks},
  journal   = {CoRR},
  volume    = {abs/1701.02676},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.02676},
  timestamp = {Wed, 01 Feb 2017 17:47:56 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/DongNWG17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/YanYSL15,
  author    = {Xinchen Yan and
               Jimei Yang and
               Kihyuk Sohn and
               Honglak Lee},
  title     = {Attribute2Image: Conditional Image Generation from Visual Attributes},
  journal   = {CoRR},
  volume    = {abs/1512.00570},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.00570},
  timestamp = {Sat, 02 Jan 2016 11:38:49 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/YanYSL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{DBLP:journals/corr/LedigTHCATTWS16,
  author    = {Christian Ledig and
               Lucas Theis and
               Ferenc Huszar and
               Jose Caballero and
               Andrew P. Aitken and
               Alykhan Tejani and
               Johannes Totz and
               Zehan Wang and
               Wenzhe Shi},
  title     = {Photo-Realistic Single Image Super-Resolution Using a Generative Adversarial
               Network},
  journal   = {CoRR},
  volume    = {abs/1609.04802},
  year      = {2016},
  url       = {http://arxiv.org/abs/1609.04802},
  timestamp = {Tue, 04 Oct 2016 08:10:36 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LedigTHCATTWS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/cvpr/MaoHTCY016,
  author    = {Junhua Mao and
               Jonathan Huang and
               Alexander Toshev and
               Oana Camburu and
               Alan L. Yuille and
               Kevin Murphy},
  title     = {Generation and Comprehension of Unambiguous Object Descriptions},
  booktitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016},
  pages     = {11--20},
  year      = {2016},
  crossref  = {DBLP:conf/cvpr/2016},
  url       = {https://doi.org/10.1109/CVPR.2016.9},
  doi       = {10.1109/CVPR.2016.9},
  timestamp = {Thu, 25 May 2017 00:41:21 +0200},
  biburl    = {http://dblp.org/rec/bib/conf/cvpr/MaoHTCY016},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/BrunaSL15,
  author    = {Joan Bruna and
               Pablo Sprechmann and
               Yann LeCun},
  title     = {Super-Resolution with Deep Convolutional Sufficient Statistics},
  journal   = {CoRR},
  volume    = {abs/1511.05666},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.05666},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/BrunaSL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}












@article{ramakrishna2012reconstructing,
  title={{Reconstructing 3d Human Pose from 2d Image Landmarks}},
  author={Ramakrishna, V. and Kanade, T. and Sheikh, Y.},
  journal={Computer Vision--ECCV 2012},
  pages={573--586},
  year={2012},
  publisher={Springer}
}

@article{DBLP:journals/corr/ChenR16a,
  author    = {Ching{-}Hang Chen and
               Deva Ramanan},
  title     = {3D Human Pose Estimation = 2D Pose Estimation + Matching},
  journal   = {CoRR},
  volume    = {abs/1612.06524},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.06524},
  timestamp = {Mon, 02 Jan 2017 11:09:15 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/ChenR16a},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/icra/JaeglePD16,
  author    = {Andrew Jaegle and
               Stephen Phillips and
               Kostas Daniilidis},
  title     = {Fast, robust, continuous monocular egomotion computation},
  booktitle = {2016 {IEEE} International Conference on Robotics and Automation, {ICRA}
               2016, Stockholm, Sweden, May 16-21, 2016},
  pages     = {773--780},
  year      = {2016},
  crossref  = {DBLP:conf/icra/2016},
  url       = {http://dx.doi.org/10.1109/ICRA.2016.7487206},
  doi       = {10.1109/ICRA.2016.7487206},
  timestamp = {Tue, 14 Jun 2016 19:35:07 +0200},
  biburl    = {http://dblp2.uni-trier.de/rec/bib/conf/icra/JaeglePD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/RogezS16,
  author    = {Gr{\'{e}}gory Rogez and
               Cordelia Schmid},
  title     = {MoCap-guided Data Augmentation for 3D Pose Estimation in the Wild},
  journal   = {CoRR},
  volume    = {abs/1607.02046},
  year      = {2016},
  url       = {http://arxiv.org/abs/1607.02046},
  timestamp = {Tue, 02 Aug 2016 12:59:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RogezS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}
@article{DBLP:journals/corr/ZhouZPLDD17,
  author    = {Xiaowei Zhou and
               Menglong Zhu and
               Georgios Pavlakos and
               Spyridon Leonardos and
               Konstantinos G. Derpanis and
               Kostas Daniilidis},
  title     = {MonoCap: Monocular Human Motion Capture using a {CNN} Coupled with
               a Geometric Prior},
  journal   = {CoRR},
  volume    = {abs/1701.02354},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.02354},
  timestamp = {Wed, 01 Feb 2017 17:47:56 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/ZhouZPLDD17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/PavlakosZDD16,
  author    = {Georgios Pavlakos and
               Xiaowei Zhou and
               Konstantinos G. Derpanis and
               Kostas Daniilidis},
  title     = {Coarse-to-Fine Volumetric Prediction for Single-Image 3D Human Pose},
  journal   = {CoRR},
  volume    = {abs/1611.07828},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.07828},
  timestamp = {Thu, 01 Dec 2016 19:32:08 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/PavlakosZDD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/TomeRA17,
  author    = {Denis Tom{\`{e}} and
               Chris Russell and
               Lourdes Agapito},
  title     = {Lifting from the Deep: Convolutional 3D Pose Estimation from a Single
               Image},
  journal   = {CoRR},
  volume    = {abs/1701.00295},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.00295},
  timestamp = {Wed, 01 Feb 2017 17:47:56 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/TomeRA17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{liu2015faceattributes,
 author = {Ziwei Liu and Ping Luo and Xiaogang Wang and Xiaoou Tang},
 title = {Deep Learning Face Attributes in the Wild},
 booktitle = {Proceedings of International Conference on Computer Vision (ICCV)},
 month = December,
 year = {2015} 
}





@incollection{Bengio+chapter2007,
author = {Bengio, Yoshua and LeCun, Yann},
booktitle = {Large Scale Kernel Machines},
publisher = {MIT Press},
title = {Scaling Learning Algorithms Towards {AI}},
year = {2007}
}

@article{Hinton06,
author = {Hinton, Geoffrey E. and Osindero, Simon and Teh, Yee Whye},
journal = {Neural Computation},
pages = {1527--1554},
title = {A Fast Learning Algorithm for Deep Belief Nets},
volume = {18},
year = {2006}
}

@article{DBLP:journals/corr/UmmenhoferZUMID16,
  author    = {Benjamin Ummenhofer and
               Huizhong Zhou and
               Jonas Uhrig and
               Nikolaus Mayer and
               Eddy Ilg and
               Alexey Dosovitskiy and
               Thomas Brox},
  title     = {DeMoN: Depth and Motion Network for Learning Monocular Stereo},
  journal   = {CoRR},
  volume    = {abs/1612.02401},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.02401},
  timestamp = {Wed, 07 Jun 2017 14:41:36 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/UmmenhoferZUMID16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@misc{45166,
title = {TensorFlow: Large-Scale Machine Learning on Heterogeneous Distributed Systems},
author  = {Martín Abadi and Ashish Agarwal and Paul Barham and Eugene Brevdo and Zhifeng Chen and Craig Citro and Greg Corrado and Andy Davis and Jeffrey Dean and Matthieu Devin and Sanjay Ghemawat and Ian Goodfellow and Andrew Harp and Geoffrey Irving and Michael Isard and Yangqing Jia and Rafal Jozefowicz and Lukasz Kaiser and Manjunath Kudlur and Josh Levenberg and Dan Mané and Rajat Monga and Sherry Moore and Derek Murray and Chris Olah and Mike Schuster and Jonathon Shlens and Benoit Steiner and Ilya Sutskever and Kunal Talwar and Paul Tucker and Vincent Vanhoucke and Vijay Vasudevan and Fernanda Viégas and Oriol Vinyals and Pete Warden and Martin Wattenberg and Martin Wicke and Yuan Yu and Xiaoqiang Zheng},
year  = 2015,
URL = {http://download.tensorflow.org/paper/whitepaper2015.pdf}
}



@incollection{NIPS2012_4824,
title = {ImageNet Classification with Deep Convolutional Neural Networks},
author = {Alex Krizhevsky and Sutskever, Ilya and Geoffrey E. Hinton},
booktitle = {Advances in Neural Information Processing Systems 25},
editor = {F. Pereira and C. J. C. Burges and L. Bottou and K. Q. Weinberger},
pages = {1097--1105},
year = {2012},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/4824-imagenet-classification-with-deep-convolutional-neural-networks.pdf}
}


@article{JMLR:v16:vapnik15b,
  author  = {Vladimir Vapnik and Rauf Izmailov},
  title   = {Learning Using Privileged Information: Similarity Control and Knowledge Transfer},
  journal = {Journal of Machine Learning Research},
  year    = {2015},
  volume  = {16},
  pages   = {2023-2049},
  url     = {http://jmlr.org/papers/v16/vapnik15b.html}
}




@article{DBLP:journals/corr/GuHLL16,
  author    = {Shixiang Gu and
               Ethan Holly and
               Timothy P. Lillicrap and
               Sergey Levine},
  title     = {Deep Reinforcement Learning for Robotic Manipulation},
  journal   = {CoRR},
  volume    = {abs/1610.00633},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.00633},
  archivePrefix = {arXiv},
  eprint    = {1610.00633},
  timestamp = {Wed, 07 Jun 2017 14:40:31 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/GuHLL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/KroemerS16,
  author    = {Oliver Kroemer and
               Gaurav S. Sukhatme},
  title     = {Learning Relevant Features for Manipulation Skills using Meta-Level
               Priors},
  journal   = {CoRR},
  volume    = {abs/1605.04439},
  year      = {2016},
  url       = {http://arxiv.org/abs/1605.04439},
  archivePrefix = {arXiv},
  eprint    = {1605.04439},
  timestamp = {Wed, 07 Jun 2017 14:42:29 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/KroemerS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Akgun:2012:TKK:2157689.2157815,
 author = {Akgun, Baris and Cakmak, Maya and Yoo, Jae Wook and Thomaz, Andrea Lockerd},
 title = {Trajectories and Keyframes for Kinesthetic Teaching: A Human-robot Interaction Perspective},
 booktitle = {Proceedings of the Seventh Annual ACM/IEEE International Conference on Human-Robot Interaction},
 series = {HRI '12},
 year = {2012},
 isbn = {978-1-4503-1063-5},
 location = {Boston, Massachusetts, USA},
 pages = {391--398},
 numpages = {8},
 url = {http://doi.acm.org/10.1145/2157689.2157815},
 doi = {10.1145/2157689.2157815},
 acmid = {2157815},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {learning from demonstration},
} 



@article{DBLP:journals/corr/SungJS15,
  author    = {Jaeyong Sung and
               Seok Hyun Jin and
               Ashutosh Saxena},
  title     = {Robobarista: Object Part based Transfer of Manipulation Trajectories
               from Crowd-sourcing in 3D Pointclouds},
  journal   = {CoRR},
  volume    = {abs/1504.03071},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.03071},
  archivePrefix = {arXiv},
  eprint    = {1504.03071},
  timestamp = {Wed, 07 Jun 2017 14:42:19 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/SungJS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/RahmatizadehABL17,
  author    = {Rouhollah Rahmatizadeh and
               Pooya Abolghasemi and
               Ladislau B{\"{o}}l{\"{o}}ni and
               Sergey Levine},
  title     = {Vision-Based Multi-Task Manipulation for Inexpensive Robots Using
               End-To-End Learning from Demonstration},
  journal   = {CoRR},
  volume    = {abs/1707.02920},
  year      = {2017},
  url       = {http://arxiv.org/abs/1707.02920},
  archivePrefix = {arXiv},
  eprint    = {1707.02920},
  timestamp = {Sat, 05 Aug 2017 14:56:06 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/RahmatizadehABL17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{DBLP:journals/corr/LiuGAL17,
  author    = {Yuxuan Liu and
               Abhishek Gupta and
               Pieter Abbeel and
               Sergey Levine},
  title     = {Imitation from Observation: Learning to Imitate Behaviors from Raw
               Video via Context Translation},
  journal   = {CoRR},
  volume    = {abs/1707.03374},
  year      = {2017},
  url       = {http://arxiv.org/abs/1707.03374},
  archivePrefix = {arXiv},
  eprint    = {1707.03374},
  timestamp = {Sat, 05 Aug 2017 14:56:08 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LiuGAL17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{PatrauceanHC16,
  author    = {Viorica P{\u a}tr{\u a}ucean and
               Ankur Handa and
               Roberto Cipolla},
  title     = {Spatio-temporal video autoencoder with differentiable memory},
  booktitle = {International Conference on Learning Representations (ICLR) Workshop},
  year      = {2016}
}


@article{DBLP:journals/corr/SadeghianAS17,
  author    = {Amir Sadeghian and
               Alexandre Alahi and
               Silvio Savarese},
  title     = {Tracking The Untrackable: Learning To Track Multiple Cues with Long-Term
               Dependencies},
  journal   = {CoRR},
  volume    = {abs/1701.01909},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.01909},
  timestamp = {Wed, 07 Jun 2017 14:40:23 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/SadeghianAS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/McCormacHDL16,
  author    = {John McCormac and
               Ankur Handa and
               Andrew J. Davison and
               Stefan Leutenegger},
  title     = {SemanticFusion: Dense 3D Semantic Mapping with Convolutional Neural
               Networks},
  journal   = {CoRR},
  volume    = {abs/1609.05130},
  year      = {2016},
  url       = {http://arxiv.org/abs/1609.05130},
  timestamp = {Wed, 07 Jun 2017 14:42:17 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/McCormacHDL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/MalmaudHRJRM15,
  author    = {Jonathan Malmaud and
               Jonathan Huang and
               Vivek Rathod and
               Nick Johnston and
               Andrew Rabinovich and
               Kevin Murphy},
  title     = {What's Cookin'? Interpreting Cooking Videos using Text, Speech and
               Vision},
  journal   = {CoRR},
  volume    = {abs/1503.01558},
  year      = {2015},
  url       = {http://arxiv.org/abs/1503.01558},
  timestamp = {Wed, 07 Jun 2017 14:42:04 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MalmaudHRJRM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/RedmonF16,
  author    = {Joseph Redmon and
               Ali Farhadi},
  title     = {{YOLO9000:} Better, Faster, Stronger},
  journal   = {CoRR},
  volume    = {abs/1612.08242},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.08242},
  timestamp = {Wed, 07 Jun 2017 14:40:20 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RedmonF16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/LongSD14,
  author    = {Jonathan Long and
               Evan Shelhamer and
               Trevor Darrell},
  title     = {Fully Convolutional Networks for Semantic Segmentation},
  journal   = {CoRR},
  volume    = {abs/1411.4038},
  year      = {2014},
  url       = {http://arxiv.org/abs/1411.4038},
  timestamp = {Wed, 07 Jun 2017 14:42:28 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LongSD14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@ARTICLE{SilverHuangEtAl16nature,
  author = {Silver, David and Huang, Aja and Maddison, Chris J. and Guez, Arthur and Sifre, Laurent and van den Driessche, George and Schrittwieser, Julian and Antonoglou, Ioannis and Panneershelvam, Veda and Lanctot, Marc and Dieleman, Sander and Grewe, Dominik and Nham, John and Kalchbrenner, Nal and Sutskever, Ilya and Lillicrap, Timothy and Leach, Madeleine and Kavukcuoglu, Koray and Graepel, Thore and Hassabis, Demis},
  journal = {Nature},
  title = {Mastering the Game of Go with Deep Neural Networks and Tree Search},
  volume = {529},
  year = {2016}
}

@inproceedings{Hasselt:2016:DRL:3016100.3016191,
 author = {Hasselt, Hado van and Guez, Arthur and Silver, David},
 title = {Deep Reinforcement Learning with Double Q-Learning},
 booktitle = {Proceedings of the Thirtieth AAAI Conference on Artificial Intelligence},
 series = {AAAI'16},
 year = {2016},
 location = {Phoenix, Arizona},
 pages = {2094--2100},
 numpages = {7},
 url = {http://dl.acm.org/citation.cfm?id=3016100.3016191},
 acmid = {3016191},
 publisher = {AAAI Press},
} 


@inproceedings{cao2017realtime,
  author = {Zhe Cao and Tomas Simon and Shih-En Wei and Yaser Sheikh},
  booktitle = {CVPR},
  title = {Realtime Multi-Person 2D Pose Estimation using Part Affinity Fields},
  year = {2017}
}

@inproceedings{simon2017hand,
  author = {Tomas Simon and Hanbyul Joo and Iain Matthews and Yaser Sheikh},
  booktitle = {CVPR},
  title = {Hand Keypoint Detection in Single Images using Multiview Bootstrapping},
  year = {2017}
}

@inproceedings{wei2016cpm,
  author = {Shih-En Wei and Varun Ramakrishna and Takeo Kanade and Yaser Sheikh},
  booktitle = {CVPR},
  title = {Convolutional pose machines},
  year = {2016}
}

@article{DBLP:journals/corr/PathakAED17,
  author    = {Deepak Pathak and
               Pulkit Agrawal and
               Alexei A. Efros and
               Trevor Darrell},
  title     = {Curiosity-driven Exploration by Self-supervised Prediction},
  journal   = {CoRR},
  volume    = {abs/1705.05363},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.05363},
  archivePrefix = {arXiv},
  eprint    = {1705.05363},
  timestamp = {Wed, 07 Jun 2017 14:41:47 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/PathakAED17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@ARTICLE{Browne2012,
  ABSTRACT = {Monte Carlo Tree Search (MCTS) is a recently proposed search method that combines the precision of tree search with the generality of random sampling. It has received considerable interest due to its spectacular success in the difficult problem of computer Go, but has also proved beneficial in a range of other domains. This paper is a survey of the literature to date, intended to provide a snapshot of the state of the art after the first five years of MCTS research. We outline the core algorithm’s derivation, impart some structure on the many variations and enhancements that have been proposed, and summarise the results from the key game and non-game domains to which MCTS methods have been applied. A number of open research questions indicate that the field is ripe for future work.},
  AUTHOR   = {Browne, Cb and Powley, Edward},
  DOI      = {10.1109/TCIAIG.2012.2186810},
  FILE     = {http://bib.unthinkingdepths.fr/seb/pdf/Browne, Powley_2012_A survey of monte carlo tree search methods.pdf},
  ISSN     = {1943-068X},
  JOURNAL  = {Intelligence and AI},
  NUMBER   = {1},
  PAGES    = {1--49},
  TITLE    = {{A survey of monte carlo tree search methods}},
  URL      = {http://ieeexplore.ieee.org/xpls/abs_all.jsp?arnumber=6145622},
  VOLUME   = {4},
  YEAR     = {2012},
}


@article{DBLP:journals/corr/KhorevaBIBS17,
  author    = {Anna Khoreva and
               Rodrigo Benenson and
               Eddy Ilg and
               Thomas Brox and
               Bernt Schiele},
  title     = {Lucid Data Dreaming for Object Tracking},
  journal   = {CoRR},
  volume    = {abs/1703.09554},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.09554},
  timestamp = {Wed, 07 Jun 2017 14:43:15 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KhorevaBIBS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@INPROCEEDINGS{Whelan-RSS-15, 
    AUTHOR    = {Thomas Whelan AND Stefan Leutenegger AND Renato Salas Moreno AND Ben Glocker AND Andrew Davison}, 
    TITLE     = {ElasticFusion: Dense SLAM Without A Pose Graph}, 
    BOOKTITLE = {Proceedings of Robotics: Science and Systems}, 
    YEAR      = {2015}, 
    ADDRESS   = {Rome, Italy}, 
    MONTH     = {July},
    DOI       = {10.15607/RSS.2015.XI.001} 
} 
  
  
@article{DBLP:journals/corr/RitchieHG16,
  author    = {Daniel Ritchie and
               Paul Horsfall and
               Noah D. Goodman},
  title     = {Deep Amortized Inference for Probabilistic Programs},
  journal   = {CoRR},
  volume    = {abs/1610.05735},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.05735},
  timestamp = {Wed, 07 Jun 2017 14:42:26 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RitchieHG16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@misc{ceres-solver,
  author = "Sameer Agarwal and Keir Mierle and Others",
  title = "Ceres Solver",
  howpublished = "\url{http://ceres-solver.org}",
}

@article{DBLP:journals/corr/CarreiraAFM15,
  author    = {Jo{\~{a}}o Carreira and
               Pulkit Agrawal and
               Katerina Fragkiadaki and
               Jitendra Malik},
  title     = {Human Pose Estimation with Iterative Error Feedback},
  journal   = {CoRR},
  volume    = {abs/1507.06550},
  year      = {2015},
}

@article{DBLP:journals/corr/FischerDIHHGSCB15,
  author    = {Philipp Fischer and
               Alexey Dosovitskiy and
               Eddy Ilg and
               Philip H{\"{a}}usser and
               Caner Hazirbas and
               Vladimir Golkov and
               Patrick van der Smagt and
               Daniel Cremers and
               Thomas Brox},
  title     = {FlowNet: Learning Optical Flow with Convolutional Networks},
  journal   = {CoRR},
  volume    = {abs/1504.06852},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.06852},
  timestamp = {Wed, 07 Jun 2017 14:41:04 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/FischerDIHHGSCB15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@incollection{NIPS2014_5421,
title = {Deep Learning for Real-Time Atari Game Play Using Offline Monte-Carlo Tree Search Planning},
author = {Guo, Xiaoxiao and Singh, Satinder and Lee, Honglak and Lewis, Richard L and Wang, Xiaoshi},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {3338--3346},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5421-deep-learning-for-real-time-atari-game-play-using-offline-monte-carlo-tree-search-planning.pdf}
}

@inproceedings{Silberer2013ModelsOS,
  title={Models of Semantic Representation with Visual Attributes},
  author={Carina Silberer and Vittorio Ferrari and Mirella Lapata},
  booktitle={ACL},
  year={2013}
}

@article{carreira2017quo,
  title={Quo Vadis, Action Recognition? A New Model and the Kinetics Dataset},
  author={Carreira, Joao and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1705.07750},
  year={2017}
}

@article{DBLP:journals/corr/WestonCB14,
  author    = {Jason Weston and
               Sumit Chopra and
               Antoine Bordes},
  title     = {Memory Networks},
  journal   = {CoRR},
  volume    = {abs/1410.3916},
  year      = {2014},
  url       = {http://arxiv.org/abs/1410.3916},
  timestamp = {Wed, 07 Jun 2017 14:41:04 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/WestonCB14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@incollection{NIPS2015_5945,
title = {Teaching Machines to Read and Comprehend},
author = {Hermann, Karl Moritz and Kocisky, Tomas and Grefenstette, Edward and Espeholt, Lasse and Kay, Will and Suleyman, Mustafa and Blunsom, Phil},
booktitle = {Advances in Neural Information Processing Systems 28},
editor = {C. Cortes and N. D. Lawrence and D. D. Lee and M. Sugiyama and R. Garnett},
pages = {1693--1701},
year = {2015},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5945-teaching-machines-to-read-and-comprehend.pdf}
}

@article{DBLP:journals/corr/KadlecSBK16,
  author    = {Rudolf Kadlec and
               Martin Schmid and
               Ondrej Bajgar and
               Jan Kleindienst},
  title     = {Text Understanding with the Attention Sum Reader Network},
  journal   = {CoRR},
  volume    = {abs/1603.01547},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.01547},
  timestamp = {Wed, 07 Jun 2017 14:41:38 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KadlecSBK16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Article:00:Glenberg:hallsa,
    author = {Glenberg, A. and Robertson, D.},
    citeulike-article-id = {850491},
    citeulike-linkout-0 = {http://psych.wisc.edu/glenberg/},
    journal = {Journal of {M}emory and {L}anguage},
    keywords = {bibtex-import},
    posted-at = {2006-09-20 03:18:45},
    priority = {0},
    title = {Symbol grounding and meaning: {A} comparison of high-dimensional and embodied theories of meaning.},
    url = {http://psych.wisc.edu/glenberg/},
    year = {2000}
}



@article{DBLP:journals/corr/DhingraLCS16,
  author    = {Bhuwan Dhingra and
               Hanxiao Liu and
               William W. Cohen and
               Ruslan Salakhutdinov},
  title     = {Gated-Attention Readers for Text Comprehension},
  journal   = {CoRR},
  volume    = {abs/1606.01549},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.01549},
  timestamp = {Wed, 07 Jun 2017 14:42:11 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/DhingraLCS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/SeoKFH16,
  author    = {Min Joon Seo and
               Aniruddha Kembhavi and
               Ali Farhadi and
               Hannaneh Hajishirzi},
  title     = {Bidirectional Attention Flow for Machine Comprehension},
  journal   = {CoRR},
  volume    = {abs/1611.01603},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.01603},
  timestamp = {Wed, 07 Jun 2017 14:41:03 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/SeoKFH16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}







@inproceedings{donahue2015long,
  title={Long-term Recurrent Convolutional Networks for Visual Recognition and Description},
  author={Donahue, Jeff and Hendricks, Lisa Anne and Guadarrama, Sergio and Rohrbach, Marcus and Venugopalan, Subhashini and Saenko, Kate and Darrell, Trevor},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2015}
}



@inproceedings{kazemi2014one,
  title={One Millisecond Face Alignment with an Ensemble of Regression Trees},
  author={Kazemi, Vahid and Sullivan, Josephine},
  booktitle={CVPR},
  year={2014}
}

@article{DBLP:journals/corr/KimLL15a,
  author    = {Jiwon Kim and
               Jung Kwon Lee and
               Kyoung Mu Lee},
  title     = {Deeply-Recursive Convolutional Network for Image Super-Resolution},
  journal   = {CoRR},
  volume    = {abs/1511.04491},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.04491},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KimLL15a},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{pennington2014glove,
  author = {Jeffrey Pennington and Richard Socher and Christopher D. Manning},
  booktitle = {Empirical Methods in Natural Language Processing (EMNLP)},
  title = {GloVe: Global Vectors for Word Representation},
  year = {2014},
  pages = {1532--1543},
  url = {http://www.aclweb.org/anthology/D14-1162},
}

@article{Gupta:2015:ISU:2750551.2750559,
 author = {Gupta, Saurabh and Arbel\'{a}ez, Pablo and Girshick, Ross and Malik, Jitendra},
 title = {Indoor Scene Understanding with RGB-D Images: Bottom-up Segmentation, Object Detection and Semantic Segmentation},
 journal = {Int. J. Comput. Vision},
 issue_date = {April     2015},
 volume = {112},
 number = {2},
 month = apr,
 year = {2015},
 issn = {0920-5691},
 pages = {133--149},
 numpages = {17},
 url = {http://dx.doi.org/10.1007/s11263-014-0777-6},
 doi = {10.1007/s11263-014-0777-6},
 acmid = {2750559},
 publisher = {Kluwer Academic Publishers},
 address = {Hingham, MA, USA},
 keywords = {RGB-D contour detection, RGB-D image segmentation, RGB-D object detection, RGB-D scene classification, RGB-D semantic segmentation},
} 

@article{DBLP:journals/corr/TungHSF17,
  author    = {Hsiao{-}Yu Fish Tung and
               Adam Harley and
               William Seto and
               Katerina Fragkiadaki},
  title     = {Adversarial Inverse Graphics Networks: Learning 2D-to-3D Lifting and Image-to-Image Translation with Unpaired Supervision},
  journal   = {ICCV},
  year      = {2017}
}


@article{mocap,
  author    = {Hsiao{-}Yu Fish Tung and
               Wei Tung and
               Ersin Yumer and
               Katerina Fragkiadaki},
  title     = {Self-supervised learning of Motion Capture},
  journal   = {NIPS},
  year      = {2017}
}

@inproceedings{andriluka14cvpr,
               author = {Mykhaylo Andriluka and Leonid Pishchulin and Peter Gehler and Schiele, Bernt},
               title = {2D Human Pose Estimation: New Benchmark and State of the Art Analysis},
               booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
               year = {2014},
               month = {June}
}
@article{inversionearlier,
  author    = {Fish Tung and Katerina Fragkiadaki},
  title     = {Inverse Problems in Computer Vision with Adversarial Imagination Priors},
  journal   = {openreview},
  year      = {2016}
}




@article{deeppaint,
  author    = {Kushagr Gupta and
               Suleman Kazi and
               Terry Kong},
  title     = {DeepPaint: A Tool for Image Inpainting},
  journal   = {tech. report},
  year      = {2016}
}

@article{DBLP:journals/corr/DongNWG17,
  author    = {Hao Dong and
               Paarth Neekhara and
               Chao Wu and
               Yike Guo},
  title     = {Unsupervised Image-to-Image Translation with Generative Adversarial
               Networks},
  journal   = {CoRR},
  volume    = {abs/1701.02676},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.02676},
  timestamp = {Wed, 01 Feb 2017 17:47:56 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/DongNWG17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/YanYSL15,
  author    = {Xinchen Yan and
               Jimei Yang and
               Kihyuk Sohn and
               Honglak Lee},
  title     = {Attribute2Image: Conditional Image Generation from Visual Attributes},
  journal   = {CoRR},
  volume    = {abs/1512.00570},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.00570},
  timestamp = {Sat, 02 Jan 2016 11:38:49 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/YanYSL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{DBLP:journals/corr/LedigTHCATTWS16,
  author    = {Christian Ledig and
               Lucas Theis and
               Ferenc Huszar and
               Jose Caballero and
               Andrew P. Aitken and
               Alykhan Tejani and
               Johannes Totz and
               Zehan Wang and
               Wenzhe Shi},
  title     = {Photo-Realistic Single Image Super-Resolution Using a Generative Adversarial
               Network},
  journal   = {CoRR},
  volume    = {abs/1609.04802},
  year      = {2016},
  url       = {http://arxiv.org/abs/1609.04802},
  timestamp = {Tue, 04 Oct 2016 08:10:36 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LedigTHCATTWS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/cvpr/MaoHTCY016,
  author    = {Junhua Mao and
               Jonathan Huang and
               Alexander Toshev and
               Oana Camburu and
               Alan L. Yuille and
               Kevin Murphy},
  title     = {Generation and Comprehension of Unambiguous Object Descriptions},
  booktitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016},
  pages     = {11--20},
  year      = {2016},
  crossref  = {DBLP:conf/cvpr/2016},
  url       = {https://doi.org/10.1109/CVPR.2016.9},
  doi       = {10.1109/CVPR.2016.9},
  timestamp = {Thu, 25 May 2017 00:41:21 +0200},
  biburl    = {http://dblp.org/rec/bib/conf/cvpr/MaoHTCY016},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/BrunaSL15,
  author    = {Joan Bruna and
               Pablo Sprechmann and
               Yann LeCun},
  title     = {Super-Resolution with Deep Convolutional Sufficient Statistics},
  journal   = {CoRR},
  volume    = {abs/1511.05666},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.05666},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/BrunaSL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}












@article{ramakrishna2012reconstructing,
  title={{Reconstructing 3d Human Pose from 2d Image Landmarks}},
  author={Ramakrishna, V. and Kanade, T. and Sheikh, Y.},
  journal={Computer Vision--ECCV 2012},
  pages={573--586},
  year={2012},
  publisher={Springer}
}

@article{DBLP:journals/corr/ChenR16a,
  author    = {Ching{-}Hang Chen and
               Deva Ramanan},
  title     = {3D Human Pose Estimation = 2D Pose Estimation + Matching},
  journal   = {CoRR},
  volume    = {abs/1612.06524},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.06524},
  timestamp = {Mon, 02 Jan 2017 11:09:15 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/ChenR16a},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/icra/JaeglePD16,
  author    = {Andrew Jaegle and
               Stephen Phillips and
               Kostas Daniilidis},
  title     = {Fast, robust, continuous monocular egomotion computation},
  booktitle = {2016 {IEEE} International Conference on Robotics and Automation, {ICRA}
               2016, Stockholm, Sweden, May 16-21, 2016},
  pages     = {773--780},
  year      = {2016},
  crossref  = {DBLP:conf/icra/2016},
  url       = {http://dx.doi.org/10.1109/ICRA.2016.7487206},
  doi       = {10.1109/ICRA.2016.7487206},
  timestamp = {Tue, 14 Jun 2016 19:35:07 +0200},
  biburl    = {http://dblp2.uni-trier.de/rec/bib/conf/icra/JaeglePD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/RogezS16,
  author    = {Gr{\'{e}}gory Rogez and
               Cordelia Schmid},
  title     = {MoCap-guided Data Augmentation for 3D Pose Estimation in the Wild},
  journal   = {CoRR},
  volume    = {abs/1607.02046},
  year      = {2016},
  url       = {http://arxiv.org/abs/1607.02046},
  timestamp = {Tue, 02 Aug 2016 12:59:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RogezS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}
@article{DBLP:journals/corr/ZhouZPLDD17,
  author    = {Xiaowei Zhou and
               Menglong Zhu and
               Georgios Pavlakos and
               Spyridon Leonardos and
               Konstantinos G. Derpanis and
               Kostas Daniilidis},
  title     = {MonoCap: Monocular Human Motion Capture using a {CNN} Coupled with
               a Geometric Prior},
  journal   = {CoRR},
  volume    = {abs/1701.02354},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.02354},
  timestamp = {Wed, 01 Feb 2017 17:47:56 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/ZhouZPLDD17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/PavlakosZDD16,
  author    = {Georgios Pavlakos and
               Xiaowei Zhou and
               Konstantinos G. Derpanis and
               Kostas Daniilidis},
  title     = {Coarse-to-Fine Volumetric Prediction for Single-Image 3D Human Pose},
  journal   = {CoRR},
  volume    = {abs/1611.07828},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.07828},
  timestamp = {Thu, 01 Dec 2016 19:32:08 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/PavlakosZDD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@incollection{hurley2005perspectives,
  title={Perspectives on Imitation: {F}rom Neuroscience to Social Science. {I}mitation, human development and culture. 2},
  author={Hurley, S. and Chater, N.},
  isbn={9780262582520},
  url={https://books.google.com/books?id=NZA\_ngEACAAJ},
  year={2005},
  publisher={MIT Press}
}



@incollection{POULSON1989271,
title = "Imitation in Infancy: A Critical Review",
editor = "Hayne W. Reese",
series = "Advances in Child Development and Behavior",
publisher = "JAI",
volume = "22",
number = "Supplement C",
pages = "271 - 298",
year = "1989",
issn = "0065-2407",
doi = "https://doi.org/10.1016/S0065-2407(08)60417-6",
url = "http://www.sciencedirect.com/science/article/pii/S0065240708604176",
author = "Claire L. Poulson and Leila Regina de Paula Nunes and Steven F. Warren"
}



@article{DBLP:journals/corr/TomeRA17,
  author    = {Denis Tom{\`{e}} and
               Chris Russell and
               Lourdes Agapito},
  title     = {Lifting from the Deep: Convolutional 3D Pose Estimation from a Single
               Image},
  journal   = {CoRR},
  volume    = {abs/1701.00295},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.00295},
  timestamp = {Wed, 01 Feb 2017 17:47:56 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/TomeRA17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{liu2015faceattributes,
 author = {Ziwei Liu and Ping Luo and Xiaogang Wang and Xiaoou Tang},
 title = {Deep Learning Face Attributes in the Wild},
 booktitle = {Proceedings of International Conference on Computer Vision (ICCV)},
 month = December,
 year = {2015} 
}





@incollection{Bengio+chapter2007,
author = {Bengio, Yoshua and LeCun, Yann},
booktitle = {Large Scale Kernel Machines},
publisher = {MIT Press},
title = {Scaling Learning Algorithms Towards {AI}},
year = {2007}
}

@article{Hinton06,
author = {Hinton, Geoffrey E. and Osindero, Simon and Teh, Yee Whye},
journal = {Neural Computation},
pages = {1527--1554},
title = {A Fast Learning Algorithm for Deep Belief Nets},
volume = {18},
year = {2006}
}

@article{DBLP:journals/corr/UmmenhoferZUMID16,
  author    = {Benjamin Ummenhofer and
               Huizhong Zhou and
               Jonas Uhrig and
               Nikolaus Mayer and
               Eddy Ilg and
               Alexey Dosovitskiy and
               Thomas Brox},
  title     = {DeMoN: Depth and Motion Network for Learning Monocular Stereo},
  journal   = {CoRR},
  volume    = {abs/1612.02401},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.02401},
  timestamp = {Wed, 07 Jun 2017 14:41:36 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/UmmenhoferZUMID16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@misc{45166,
title = {TensorFlow: Large-Scale Machine Learning on Heterogeneous Distributed Systems},
author  = {Martín Abadi and Ashish Agarwal and Paul Barham and Eugene Brevdo and Zhifeng Chen and Craig Citro and Greg Corrado and Andy Davis and Jeffrey Dean and Matthieu Devin and Sanjay Ghemawat and Ian Goodfellow and Andrew Harp and Geoffrey Irving and Michael Isard and Yangqing Jia and Rafal Jozefowicz and Lukasz Kaiser and Manjunath Kudlur and Josh Levenberg and Dan Mané and Rajat Monga and Sherry Moore and Derek Murray and Chris Olah and Mike Schuster and Jonathon Shlens and Benoit Steiner and Ilya Sutskever and Kunal Talwar and Paul Tucker and Vincent Vanhoucke and Vijay Vasudevan and Fernanda Viégas and Oriol Vinyals and Pete Warden and Martin Wattenberg and Martin Wicke and Yuan Yu and Xiaoqiang Zheng},
year  = 2015,
URL = {http://download.tensorflow.org/paper/whitepaper2015.pdf}
}



@incollection{NIPS2012_4824,
title = {ImageNet Classification with Deep Convolutional Neural Networks},
author = {Alex Krizhevsky and Sutskever, Ilya and Geoffrey E. Hinton},
booktitle = {Advances in Neural Information Processing Systems 25},
editor = {F. Pereira and C. J. C. Burges and L. Bottou and K. Q. Weinberger},
pages = {1097--1105},
year = {2012},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/4824-imagenet-classification-with-deep-convolutional-neural-networks.pdf}
}

@inproceedings{imagenet_cvpr09,
        AUTHOR = {Deng, J. and Dong, W. and Socher, R. and Li, L.-J. and Li, K. and Fei-Fei, L.},
        TITLE = {{ImageNet: A Large-Scale Hierarchical Image Database}},
        BOOKTITLE = {CVPR09},
        YEAR = {2009},
        BIBSOURCE = "http://www.image-net.org/papers/imagenet_cvpr09.bib"}
    
    
    
    @inproceedings{Misra2015EnvironmentDrivenLI,
  title={Environment-Driven Lexicon Induction for High-Level Instructions},
  author={Dipendra Kumar Misra and Kejia Tao and Percy Liang and Ashutosh Saxena},
  booktitle={ACL},
  year={2015}
}


  @INPROCEEDINGS{Misra-RSS-14, 
    AUTHOR    = {Dipendra Kumar Misra AND Jaeyong Sung AND Kevin Lee AND Ashutosh Saxena}, 
    TITLE     = {Tell Me Dave: Context-Sensitive Grounding of Natural Language to Manipulation Instructions}, 
    BOOKTITLE = {Proceedings of Robotics: Science and Systems}, 
    YEAR      = {2014}, 
    ADDRESS   = {Berkeley, USA}, 
    MONTH     = {July},
    DOI       = {10.15607/RSS.2014.X.005} 
} 
        
        
@article{DBLP:journals/tacl/ArtziZ13,
  author    = {Yoav Artzi and
               Luke Zettlemoyer},
  title     = {Weakly Supervised Learning of Semantic Parsers for Mapping Instructions
               to Actions},
  journal   = {{TACL}},
  volume    = {1},
  pages     = {49--62},
  year      = {2013},
  url       = {https://tacl2013.cs.columbia.edu/ojs/index.php/tacl/article/view/27},
  timestamp = {Thu, 28 May 2015 17:23:25 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/tacl/ArtziZ13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


        
@article{DBLP:journals/corr/MisraLA17,
  author    = {Dipendra Kumar Misra and
               John Langford and
               Yoav Artzi},
  title     = {Mapping Instructions and Visual Observations to Actions with Reinforcement
               Learning},
  journal   = {CoRR},
  volume    = {abs/1704.08795},
  year      = {2017},
  url       = {http://arxiv.org/abs/1704.08795},
  archivePrefix = {arXiv},
  eprint    = {1704.08795},
  timestamp = {Wed, 07 Jun 2017 14:42:37 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/MisraLA17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


 
@inproceedings{Branavan:2009:RLM:1687878.1687892,
 author = {Branavan, S. R. K. and Chen, Harr and Zettlemoyer, Luke S. and Barzilay, Regina},
 title = {Reinforcement Learning for Mapping Instructions to Actions},
 booktitle = {Proceedings of the Joint Conference of the 47th Annual Meeting of the ACL and the 4th International Joint Conference on Natural Language Processing of the AFNLP: Volume 1 - Volume 1},
 series = {ACL '09},
 year = {2009},
 isbn = {978-1-932432-45-9},
 location = {Suntec, Singapore},
 pages = {82--90},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=1687878.1687892},
 acmid = {1687892},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
} 


   
@inproceedings{Ng:2000:AIR:645529.657801,
 author = {Ng, Andrew Y. and Russell, Stuart J.},
 title = {Algorithms for Inverse Reinforcement Learning},
 booktitle = {Proceedings of the Seventeenth International Conference on Machine Learning},
 series = {ICML '00},
 year = {2000},
 isbn = {1-55860-707-2},
 pages = {663--670},
 numpages = {8},
 url = {http://dl.acm.org/citation.cfm?id=645529.657801},
 acmid = {657801},
 publisher = {Morgan Kaufmann Publishers Inc.},
 address = {San Francisco, CA, USA},
} 




        
@article{mnist,
  added-at = {2010-06-28T21:16:30.000+0200},
  author = {LeCun, Yann and Cortes, Corinna},
  biburl = {http://www.bibsonomy.org/bibtex/2935bad99fa1f65e03c25b315aa3c1032/mhwombat},
  groups = {public},
  howpublished = {http://yann.lecun.com/exdb/mnist/},
  interhash = {21b9d0558bd66279df9452562df6e6f3},
  intrahash = {935bad99fa1f65e03c25b315aa3c1032},
  keywords = {MSc _checked character_recognition mnist network neural},
  lastchecked = {2016-01-14 14:24:11},
  timestamp = {2016-07-12T19:25:30.000+0200},
  title = {{MNIST} handwritten digit database},
  url = {http://yann.lecun.com/exdb/mnist/},
  username = {mhwombat},
  year = 2010
}

@INPROCEEDINGS{grosse09intrinsic,
   AUTHOR = "Roger Grosse and Micah K. Johnson and Edward H. Adelson and William T. Freeman",
    TITLE = "Ground-truth dataset and baseline evaluations for intrinsic image algorithms",
    PAGES = "2335--2342",
     YEAR = "2009",
BOOKTITLE = "International Conference on Computer Vision",
      DOI = "http://dx.doi.org/10.1109/ICCV.2009.5459428"
}

@article{DBLP:journals/corr/TomeRA17,
  author    = {Denis Tom{\`{e}} and
               Chris Russell and
               Lourdes Agapito},
  title     = {Lifting from the Deep: Convolutional 3D Pose Estimation from a Single
               Image},
  journal   = {CoRR},
  volume    = {abs/1701.00295},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.00295},
  timestamp = {Wed, 01 Feb 2017 17:47:56 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/TomeRA17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/WangWLYG14,
  author    = {Chunyu Wang and
               Yizhou Wang and
               Zhouchen Lin and
               Alan L. Yuille and
               Wen Gao},
  title     = {Robust Estimation of 3D Human Poses from a Single Image},
  journal   = {CoRR},
  volume    = {abs/1406.2282},
  year      = {2014},
  url       = {http://arxiv.org/abs/1406.2282},
  timestamp = {Tue, 31 May 2016 18:15:20 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/WangWLYG14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Aubry14,
  title={Seeing 3D chairs: exemplar part-based 2D-3D alignment using a large dataset of CAD models},
  author={Aubry, Mathieu and Maturana, Daniel and Efros, Alexei, and Russell, Bryan and Sivic, Josef},
  booktitle={CVPR},
  year={2014},
}

@inproceedings{SUN,
  added-at = {2014-07-31T00:00:00.000+0200},
  author = {Xiao, Jianxiong and Hays, James and Ehinger, Krista A. and Oliva, Aude and Torralba, Antonio},
  biburl = {http://www.bibsonomy.org/bibtex/232294b312a372e89fbb447d12d904dc7/dblp},
  booktitle = {CVPR},
  crossref = {conf/cvpr/2010},
  ee = {http://doi.ieeecomputersociety.org/10.1109/CVPR.2010.5539970},
  interhash = {496f3934a4f2a511117f43d385da847c},
  intrahash = {32294b312a372e89fbb447d12d904dc7},
  isbn = {978-1-4244-6984-0},
  keywords = {dblp},
  pages = {3485-3492},
  publisher = {IEEE Computer Society},
  timestamp = {2015-06-19T16:09:09.000+0200},
  title = {SUN database: Large-scale scene recognition from abbey to zoo.},
  url = {http://dblp.uni-trier.de/db/conf/cvpr/cvpr2010.html#XiaoHEOT10},
  year = 2010
}


@inproceedings{LSUN,
	author     = {Fisher Yu and Yinda Zhang and Shuran Song and Ari Seff and Jianxiong Xiao},
	title      = {{LSUN}: Construction of a Large-scale Image Dataset using Deep Learning with Humans in the Loop},
	booktitle  = arXiv,
	year       = {2015},
}

@inproceedings{PICTURE,
  added-at = {2015-10-16T00:00:00.000+0200},
  author = {Kulkarni, Tejas D. and Kohli, Pushmeet and Tenenbaum, Joshua B. and Mansinghka, Vikash K.},
  biburl = {http://www.bibsonomy.org/bibtex/28cb5b89a60ae4e2624c880bfb7c50638/dblp},
  booktitle = {CVPR},
  crossref = {conf/cvpr/2015},
  ee = {http://dx.doi.org/10.1109/CVPR.2015.7299068},
  interhash = {a234af7842af65c7bfe363459cfd6e3d},
  intrahash = {8cb5b89a60ae4e2624c880bfb7c50638},
  isbn = {978-1-4673-6964-0},
  keywords = {dblp},
  pages = {4390-4399},
  publisher = {IEEE Computer Society},
  timestamp = {2016-04-29T11:54:14.000+0200},
  title = {Picture: A probabilistic programming language for scene perception.},
  url = {http://dblp.uni-trier.de/db/conf/cvpr/cvpr2015.html#KulkarniKTM15},
  year = 2015
}

@TECHREPORT{Yu03computationalmodels,
    author = {Stella Yu},
    title = {Computational Models of Perceptual Organization},
    institution = {Robotics Institute, Carnegie Mellon University},
    year = {2003}
}
@book{Knill:1996:PBI:239481,
 editor = {Knill, David C. and Richards, Whitman},
 title = {Perception As Bayesian Inference},
 year = {1996},
 isbn = {0-521-46109-X},
 publisher = {Cambridge University Press},
 address = {New York, NY, USA},
} 
@inproceedings{bruno,
  author = {Olshausen, Bruno},
  booktitle = {The Cognitive Neurosciences},
  publisher = {MIT Press},
  timestamp = {2016-04-29T11:54:14.000+0200},
  title = {Perception as an Inference Problem},
  year = 2013
}


@incollection{NIPS2014_5423,
title = {Generative Adversarial Nets},
author = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {2672--2680},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5423-generative-adversarial-nets.pdf}
}

@inproceedings{Sheikh_2008_6196,
   author = "Ijaz Akhter and Yaser Ajmal Sheikh and Sohaib Khan and Takeo Kanade",
   title = "Nonrigid Structure from Motion in Trajectory Space",
   booktitle = "Neural Information Processing Systems",
   month = "December",
   year = "2008",
}


@inproceedings{DBLP:conf/cvpr/NarihiraMY15,
  author    = {Takuya Narihira and
               Michael Maire and
               Stella X. Yu},
  title     = {Learning lightness from human judgement on relative reflectance},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2015, Boston, MA, USA, June 7-12, 2015},
  pages     = {2965--2973},
  year      = {2015},
  crossref  = {DBLP:conf/cvpr/2015},
  url       = {http://dx.doi.org/10.1109/CVPR.2015.7298915},
  doi       = {10.1109/CVPR.2015.7298915},
  timestamp = {Thu, 28 Apr 2016 10:52:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/cvpr/NarihiraMY15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{h36m_pami,
author = {Ionescu, Catalin and Papava, Dragos and Olaru, Vlad and Sminchisescu,  Cristian},
title = {Human3.6M: Large Scale Datasets and Predictive Methods for 3D Human Sensing in Natural Environments},
journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
publisher = {IEEE Computer Society},
volume = {36},
number = {7},
pages = {1325-1339},
month = {jul},
year = {2014}
}

@article{DBLP:journals/corr/KulkarniWKT15,
  author    = {Tejas D. Kulkarni and
               Will Whitney and
               Pushmeet Kohli and
               Joshua B. Tenenbaum},
  title     = {Deep Convolutional Inverse Graphics Network},
  journal   = {CoRR},
  volume    = {abs/1503.03167},
  year      = {2015},
  url       = {http://arxiv.org/abs/1503.03167},
  timestamp = {Thu, 09 Apr 2015 11:33:20 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/KulkarniWKT15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/DongLHT15,
  author    = {Chao Dong and
               Chen Change Loy and
               Kaiming He and
               Xiaoou Tang},
  title     = {Image Super-Resolution Using Deep Convolutional Networks},
  journal   = {CoRR},
  volume    = {abs/1501.00092},
  year      = {2015},
  url       = {http://arxiv.org/abs/1501.00092},
  timestamp = {Mon, 02 Feb 2015 14:12:25 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/DongLHT15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{larochelle2011,
  title={The Neural Autoregressive Distribution Estimator},
  author={Hugo Larochelle and Iain Murray},
  journal={JMLR: W\&CP},
  volume={15},
  pages={29--37},
  year={2011}
}

@article{DBLP:journals/corr/NarihiraMY15,
  author    = {Takuya Narihira and
               Michael Maire and
               Stella X. Yu},
  title     = {Direct Intrinsics: Learning Albedo-Shading Decomposition by Convolutional
               Regression},
  journal   = {CoRR},
  volume    = {abs/1512.02311},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.02311},
  timestamp = {Sat, 02 Jan 2016 11:38:49 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/NarihiraMY15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/BrunaSL15,
  author    = {Joan Bruna and
               Pablo Sprechmann and
               Yann LeCun},
  title     = {Super-Resolution with Deep Convolutional Sufficient Statistics},
  journal   = {CoRR},
  volume    = {abs/1511.05666},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.05666},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/BrunaSL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@INPROCEEDINGS{FirmanCVPR2016,
 author    = {Firman, Michael and Mac Aodha, Oisin and Julier, Simon and Brostow, Gabriel J.},
 title     = {{Structured Prediction of Unobserved Voxels From a Single Depth Image}},
 booktitle = {CVPR},
 year      = {2016},
}

@inproceedings{Efros:1999:TSN:850924.851569,
 author = {Efros, Alexei A. and Leung, Thomas K.},
 title = {Texture Synthesis by Non-Parametric Sampling},
 booktitle = {Proceedings of the International Conference on Computer Vision-Volume 2 - Volume 2},
 series = {ICCV '99},
 year = {1999},
 isbn = {0-7695-0164-8},
 pages = {1033--},
 url = {http://dl.acm.org/citation.cfm?id=850924.851569},
 acmid = {851569},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
} 


@misc{jang2016categorical,
  abstract = {Categorical variables are a natural choice for representing discrete
structure in the world. However, stochastic neural networks rarely use
categorical latent variables due to the inability to backpropagate through
samples. In this work, we present an efficient gradient estimator that replaces
the non-differentiable sample from a categorical distribution with a
differentiable sample from a novel Gumbel-Softmax distribution. This
distribution has the essential property that it can be smoothly annealed into a
categorical distribution. We show that our Gumbel-Softmax estimator outperforms
state-of-the-art gradient estimators on structured output prediction and
unsupervised generative modeling tasks with categorical latent variables, and
enables large speedups on semi-supervised classification.},
  added-at = {2017-03-20T09:53:49.000+0100},
  author = {Jang, Eric and Gu, Shixiang and Poole, Ben},
  biburl = {https://www.bibsonomy.org/bibtex/21b45b213a40f3498cc2ababb0d0be83b/suqbar},
  description = {[1611.01144] Categorical Reparameterization with Gumbel-Softmax},
  interhash = {157733069613834cff7c133ed27aae43},
  intrahash = {1b45b213a40f3498cc2ababb0d0be83b},
  keywords = {categorical gumbel-sofmax},
  note = {cite arxiv:1611.01144},
  timestamp = {2017-04-04T08:40:54.000+0200},
  title = {Categorical Reparameterization with Gumbel-Softmax},
  url = {http://arxiv.org/abs/1611.01144},
  year = 2016
}




@article{DBLP:journals/corr/MakhzaniSJG15,
  author    = {Alireza Makhzani and
               Jonathon Shlens and
               Navdeep Jaitly and
               Ian J. Goodfellow},
  title     = {Adversarial Autoencoders},
  journal   = {CoRR},
  volume    = {abs/1511.05644},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.05644},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MakhzaniSJG15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/YehCLHD16,
  author    = {Raymond Yeh and
               Chen Chen and
               Teck{-}Yian Lim and
               Mark Hasegawa{-}Johnson and
               Minh N. Do},
  title     = {Semantic Image Inpainting with Perceptual and Contextual Losses},
  journal   = {CoRR},
  volume    = {abs/1607.07539},
  year      = {2016},
  url       = {http://arxiv.org/abs/1607.07539},
  timestamp = {Wed, 05 Oct 2016 14:51:31 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/YehCLHD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{Raiko:2014:INA:2968826.2968863,
 author = {Raiko, Tapani and Yao, Li and Cho, KyungHyun and Bengio, Yoshua},
 title = {Iterative Neural Autoregressive Distribution Estimator (NADE-k)},
 booktitle = {Proceedings of the 27th International Conference on Neural Information Processing Systems},
 series = {NIPS'14},
 year = {2014},
 location = {Montreal, Canada},
 pages = {325--333},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=2968826.2968863},
 acmid = {2968863},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 

@article{sonderby2014apparent,
  title={Amortised MAP Inference for Image Super-resolution},
  author={S{\o}nderby, Casper Kaae and Caballero, Jose and Theis ,Lucas and Shi, Wenzhe and Husz\'{a}r, Ferenc},
  journal={arXiv preprint arXiv:1610.04490},
  year={2016}
}

@inproceedings{3dgan,
    author = {Jiajun Wu, Chengkai Zhang, Tianfan Xue, William T. Freeman, and Joshua B. Tenenbaum},
    Title = {Learning a Probabilistic Latent Space of Object Shapes via 3D Generative-Adversarial Modeling},
    Booktitle = NIPS,
    Year = {2016}
}

@article{DBLP:journals/corr/YehCLHD16,
  author    = {Raymond Yeh and
               Chen Chen and
               Teck{-}Yian Lim and
               Mark Hasegawa{-}Johnson and
               Minh N. Do},
  title     = {Semantic Image Inpainting with Perceptual and Contextual Losses},
  journal   = {CoRR},
  volume    = {abs/1607.07539},
  year      = {2016},
  url       = {http://arxiv.org/abs/1607.07539},
  timestamp = {Wed, 05 Oct 2016 14:51:31 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/YehCLHD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{pathakCVPR16context,
    Author = {Pathak, Deepak and
    Kr\"ahenb\"uhl, Philipp and
    Donahue, Jeff and
    Darrell, Trevor and
    Efros, Alexei},
    Title = {Context Encoders:
    Feature Learning by Inpainting},
    Booktitle = CVPR,
    Year = {2016}
}


@article{DBLP:journals/corr/EigenPF14,
  author    = {David Eigen and
               Christian Puhrsch and
               Rob Fergus},
  title     = {Depth Map Prediction from a Single Image using a Multi-Scale Deep
               Network},
  journal   = {CoRR},
  volume    = {abs/1406.2283},
  year      = {2014},
  url       = {http://arxiv.org/abs/1406.2283},
  timestamp = {Tue, 01 Jul 2014 11:58:08 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/EigenPF14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/iccv/EfrosL99,
  author    = {Alexei A. Efros and
               Thomas K. Leung},
  title     = {Texture Synthesis by Non-parametric Sampling},
  booktitle = {{ICCV}},
  pages     = {1033--1038},
  year      = {1999},
  url       = {http://dx.doi.org/10.1109/ICCV.1999.790383},
  doi       = {10.1109/ICCV.1999.790383},
  timestamp = {Thu, 12 May 2016 10:37:23 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/iccv/EfrosL99},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Yang:2010:ISV:1892456.1892463,
 author = {Yang, Jianchao and Wright, John and Huang, Thomas S. and Ma, Yi},
 title = {Image Super-resolution via Sparse Representation},
 journal = {Trans. Img. Proc.},
 issue_date = {November 2010},
 volume = {19},
 number = {11},
 month = nov,
 year = {2010},
 issn = {1057-7149},
 pages = {2861--2873},
 numpages = {13},
 url = {http://dx.doi.org/10.1109/TIP.2010.2050625},
 doi = {10.1109/TIP.2010.2050625},
 acmid = {1892463},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
 keywords = {Face hallucination, face hallucination, image super-resolution (SR), nonnegative matrix factorization, sparse coding, sparse representation},
} 


@inproceedings{f-gan-training-generative-neural-samplers-using-variational-divergence-minimization,
author = {Sebastian Nowozin, Botond Cseke, Ryota Tomioka},
title = {f-GAN: Training Generative Neural Samplers using Variational Divergence Minimization},
booktitle = {Neural Information Processing Systems 2016},
year = {2016},
month = {October},
abstract = {Generative neural samplers are probabilistic models that implement sampling using feedforward neural networks: they take a random input vector and produce a sample from a probability distribution defined by the network weights. These models are expressive and allow efficient computation of samples and derivatives, but cannot be used for computing likelihoods or for marginalization. The generative-adversarial training method allows to train such models through the use of an auxiliary discriminative neural network. We show that the generative-adversarial approach is a special case of an existing more general variational divergence estimation approach. We show that any f-divergence can be used for training generative neural samplers. We discuss the benefits of various choices of divergence functions on training complexity and the quality of the obtained generative models.},
publisher = {Neural Information Processing Systems},
address = {},
pages = {},
journal = {},
volume = {},
chapter = {},
isbn = {},
}


@article{DBLP:journals/corr/RadfordMC15,
  author    = {Alec Radford and
               Luke Metz and
               Soumith Chintala},
  title     = {Unsupervised Representation Learning with Deep Convolutional Generative
               Adversarial Networks},
  journal   = {CoRR},
  volume    = {abs/1511.06434},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.06434},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RadfordMC15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}




@article{Gilbert2007677,
title = "Brain States: Top-Down Influences in Sensory Processing ",
journal = "Neuron ",
volume = "54",
number = "5",
pages = "677 - 696",
year = "2007",
note = "",
issn = "0896-6273",
doi = "http://dx.doi.org/10.1016/j.neuron.2007.05.019",
url = "http://www.sciencedirect.com/science/article/pii/S0896627307003765",
author = "Charles D. Gilbert and Mariano Sigman"
}

@ARTICLE{10.3389/fpsyg.2012.00620,
  
AUTHOR={Panichello, Matthew and Cheung, Olivia and Bar, Moshe},   
	 
TITLE={Predictive Feedback and Conscious Visual Experience},      
	
JOURNAL={Frontiers in Psychology},      
	
VOLUME={3},      

PAGES={620},     
	
YEAR={2013},      
	  
URL={http://journal.frontiersin.org/article/10.3389/fpsyg.2012.00620},       
	
DOI={10.3389/fpsyg.2012.00620},      
	
ISSN={1664-1078},   
   
ABSTRACT={The human brain continuously generates predictions about the environment based on learned regularities in the world. These predictions actively and efficiently facilitate the interpretation of incoming sensory information. We review evidence that, as a result of this facilitation, predictions directly influence conscious experience. Specifically, we propose that predictions enable rapid generation of conscious percepts and bias the contents of awareness in situations of uncertainty. The possible neural mechanisms underlying this facilitation are discussed. }
}

@inproceedings{Gal:2016:DBA:3045390.3045502,
 author = {Gal, Yarin and Ghahramani, Zoubin},
 title = {Dropout As a Bayesian Approximation: Representing Model Uncertainty in Deep Learning},
 booktitle = {Proceedings of the 33rd International Conference on International Conference on Machine Learning - Volume 48},
 series = {ICML'16},
 year = {2016},
 location = {New York, NY, USA},
 pages = {1050--1059},
 numpages = {10},
 url = {http://dl.acm.org/citation.cfm?id=3045390.3045502},
 acmid = {3045502},
 publisher = {JMLR.org},
} 



@inproceedings{andriluka14cvpr,
    author = {Mykhaylo Andriluka and Leonid Pishchulin and Peter Gehler and Schiele, Bernt},
    title = {2D Human Pose Estimation: {N}ew Benchmark and State of the Art Analysis},
    booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
    year = {2014},
    month = {June}
}


@Inbook{Wu2016,
author="Wu, Jiajun
and Xue, Tianfan
and Lim, Joseph J.
and Tian, Yuandong
and Tenenbaum, Joshua B.
and Torralba, Antonio
and Freeman, William T.",
editor="Leibe, Bastian
and Matas, Jiri
and Sebe, Nicu
and Welling, Max",
title="Single Image 3D Interpreter Network",
bookTitle="Computer Vision -- ECCV 2016: 14th European Conference, Amsterdam, The Netherlands, October 11-14, 2016, Proceedings, Part VI",
year="2016",
publisher="Springer International Publishing",
address="Cham",
pages="365--382",
isbn="978-3-319-46466-4",
doi="10.1007/978-3-319-46466-4_22",
url="http://dx.doi.org/10.1007/978-3-319-46466-4_22"
}

@techreport{amos2016openface,
  title={OpenFace: A general-purpose face recognition
    library with mobile applications},
  author={Amos, Brandon and Bartosz Ludwiczuk and Satyanarayanan, Mahadev},
  year={2016},
  institution={CMU-CS-16-118, CMU School of Computer Science},
}

@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}

@inproceedings{Theis2016a,
  author = "L. Theis and A. van den Oord and M. Bethge",
  title = "A note on the evaluation of generative models",
  year = 2016,
  booktitle = "International Conference on Learning Representations",
  month = "Apr",
  keywords = "generative modeling",
  url = "http://arxiv.org/abs/1511.01844"
}

@article{DBLP:journals/corr/MathieuCL15,
  author    = {Micha{\"{e}}l Mathieu and
               Camille Couprie and
               Yann LeCun},
  title     = {Deep multi-scale video prediction beyond mean square error},
  journal   = {CoRR},
  volume    = {abs/1511.05440},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.05440},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MathieuCL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{wei2016cpm,
    author = {Shih-En Wei and Varun Ramakrishna and Takeo Kanade and Yaser Sheikh},
    booktitle = {CVPR},
    title = {Convolutional pose machines},
    year = {2016}
}


@article{rezende2014stochastic,
  title={Stochastic backpropagation and approximate inference in deep generative models},
  author={Rezende, Danilo Jimenez and Mohamed, Shakir and Wierstra, Daan},
  journal={arXiv preprint arXiv:1401.4082},
  year={2014}
}

@inproceedings{handa2016gvnn,
  title={gvnn: Neural network library for geometric computer vision},
  author={Handa, Ankur and Bloesch, Michael and P{\u{a}}tr{\u{a}}ucean, Viorica and Stent, Simon and McCormac, John and Davison, Andrew},
  booktitle={Computer Vision--ECCV 2016 Workshops},
  pages={67--82},
  year={2016},
  organization={Springer International Publishing}
}

@article{flownet2,
  author    = {Eddy Ilg and
               Nikolaus Mayer and
               Tonmoy Saikia and
               Margret Keuper and
               Alexey Dosovitskiy and
               Thomas Brox},
  title     = {FlowNet 2.0: Evolution of Optical Flow Estimation with Deep Networks},
  journal   = {CoRR},
  volume    = {abs/1612.01925},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.01925},
  timestamp = {Mon, 02 Jan 2017 11:09:15 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/IlgMSKDB16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@misc{blender,
  author = {{Blender Online Coummunity}},
  organization = {Blender Foundation},
  title = {Blender},
  url = {https://www.blender.org/},
}



@article{DBLP:journals/corr/ChenWLSTLCC16,
  author    = {Wenzheng Chen and
               Huan Wang and
               Yangyan Li and
               Hao Su and
               Changhe Tu and
               Dani Lischinski and
               Daniel Cohen{-}Or and
               Baoquan Chen},
  title     = {Synthesizing Training Images for Boosting Human 3D Pose Estimation},
  journal   = {CoRR},
  volume    = {abs/1604.02703},
  year      = {2016},
  url       = {http://arxiv.org/abs/1604.02703},
  timestamp = {Mon, 02 May 2016 18:22:52 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/ChenWLSTLCC16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@misc{caesar,
  author = {Robinette, K., Daanen, H. and Paquet, E.},
  organization = {3DIM’99},
  title = {The CAESAR project: A 3-D surface anthropometry survey.},
}

@inproceedings{Wulff:ECCVws:2012,
 title = {Lessons and insights from creating a synthetic optical flow benchmark},
 author = {Wulff, J. and Butler, D. J. and Stanley, G. B. and Black, M. J.},
 booktitle = {ECCV Workshop on Unsolved Problems in Optical Flow and Stereo Estimation},
 editor = {{A. Fusiello et al. (Eds.)}},
 publisher = {Springer-Verlag},
 series = {Part II, LNCS 7584},
 month = oct,
 pages = {168--177},
 year = {2012}
}

@article{sun,
	author     = {Jianxiong Xiao and Krista A. Ehinger and James Hays and Antonio Torralba and Aude Oliva},
	title      = {{SUN} Database: Exploring a Large Collection of Scene Categories},
	journal    = {IJCV},
	year       = {2014},
}





@techreport{shapenet2015,
  title       = {{ShapeNet: An Information-Rich 3D Model Repository}},
  author      = {Chang, Angel X. and Funkhouser, Thomas and Guibas, Leonidas and Hanrahan, Pat and Huang, Qixing and Li, Zimo and Savarese, Silvio and Savva, Manolis and Song, Shuran and Su, Hao and Xiao, Jianxiong and Yi, Li and Yu, Fisher},
  number      = {arXiv:1512.03012 [cs.GR]},
  institution = {Stanford University --- Princeton University --- Toyota Technological Institute at Chicago},
  year        = {2015}
}

@inproceedings{epicflow,
TITLE = {{EpicFlow}: Edge-Preserving Interpolation of Correspondences for Optical Flow},
  AUTHOR = {Revaud, Jerome and Weinzaepfel, Philippe and Harchaoui, Zaid and Schmid, Cordelia},
  BOOKTITLE = {CVPR}, 
  YEAR = {2015},
}

@article{deepflow,
  TITLE = {{DeepMatching}: Hierarchical Deformable Dense Matching},
  AUTHOR = {Revaud, Jerome and Weinzaepfel, Philippe and Harchaoui, Zaid and Schmid, Cordelia},
  JOURNAL = {IJCV},
  YEAR = {2016},
}

@article{DBLP:journals/corr/MirzaO14,
  author    = {Mehdi Mirza and
               Simon Osindero},
  title     = {Conditional Generative Adversarial Nets},
  journal   = {CoRR},
  volume    = {abs/1411.1784},
  year      = {2014},
  url       = {http://arxiv.org/abs/1411.1784},
  timestamp = {Mon, 01 Dec 2014 14:32:13 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MirzaO14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{CycleGAN2017,
  title={Unpaired Image-to-Image Translation using Cycle-Consistent Adversarial Networks},
  author={Zhu, Jun-Yan and Park, Taesung and Isola, Phillip and Efros, Alexei A},
  journal={arXiv preprint arXiv:1703.10593},
  year={2017}
}

@article{DBLP:journals/corr/AlldieckKM17,
  author    = {Thiemo Alldieck and
               Marc Kassubeck and
               Marcus A. Magnor},
  title     = {Optical Flow-based 3D Human Motion Estimation from Monocular Video},
  journal   = {CoRR},
  volume    = {abs/1703.00177},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.00177},
  timestamp = {Mon, 03 Apr 2017 12:41:34 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/AlldieckKM17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{unpublished,
  title={Unpaired Image-to-Image Translation using Cycle-Consistent Adversarial Networks},
  author={Zhu, Jun-Yan and Park, Taesung and Isola, Phillip and Efros, Alexei A},
  journal={arXiv preprint arXiv:1703.10593},
  year={2017}
}

 @InProceedings{sfmnet,
  author = 	 {Vijayanarasimhan S. and  Ricco S. and  Schmid C. and  Sukthankar R. and Fragkiadaki K.},
  title = 	 {SfM-Net: Learning of Structure and Motion from Video},
  booktitle = {arxiv},
  year = 	 2017}
  
   @InProceedings{tinghuisfm,
  author = 	 {Tinghui Zhou and Matthew Brown and Noah Snavely and David G. Lowe},
  title = 	 {Unsupervised Learning of Depth and Ego-Motion from Video},
  booktitle = {arxiv},
  year = 	 2017}





@inproceedings{Thewlis2016,
title = {Fully-Trainable Deep Matching},
author = {James Thewlis and Shuai Zheng and Philip H.S. Torr and Andrea Vedaldi},
booktitle={BMVC},
year = {2016}
}

@inproceedings{Kong:ICCV:2015,
  title = {Intrinsic Depth: Improving Depth Transfer with Intrinsic Images},
  author = {Kong, Naejin and Black, Michael J.},
  booktitle = {IEEE International Conference on Computer Vision (ICCV)},
  pages = {3514--3522},
  month = dec,
  year = {2015}
}

@ARTICLE{Geiger2013IJRR,
  author = {Andreas Geiger and Philip Lenz and Christoph Stiller and Raquel Urtasun},
  title = {Vision meets Robotics: The KITTI Dataset},
  journal = {International Journal of Robotics Research (IJRR)},
  year = {2013}
} 

@InProceedings{sturm12iros,
	author = {J. Sturm and N. Engelhard and F. Endres and W. Burgard and D. Cremers},
	title = "A Benchmark for the Evaluation of {RGB-D SLAM} Systems",
	booktitle = "IROS",
	year = "2012",
}

@Inbook{Russell2014,
author="Russell, Chris
and Yu, Rui
and Agapito, Lourdes",
editor="Fleet, David
and Pajdla, Tomas
and Schiele, Bernt
and Tuytelaars, Tinne",
title="Video Pop-up: Monocular 3D Reconstruction of Dynamic Scenes",
bookTitle="Computer Vision -- ECCV 2014: 13th European Conference, Zurich, Switzerland, September 6-12, 2014, Proceedings, Part VII",
year="2014",
publisher="Springer International Publishing",
address="Cham",
pages="583--598",
isbn="978-3-319-10584-0",
doi="10.1007/978-3-319-10584-0_38",
url="http://dx.doi.org/10.1007/978-3-319-10584-0_38"
}

@InProceedings{sturm12iros,
	author = {J. Sturm and N. Engelhard and F. Endres and W. Burgard and D. Cremers},
	title = "A Benchmark for the Evaluation of {RGBD} {SLAM} Systems",
	booktitle = "IROS",
	year = "2012",
}

@inproceedings{conf/cvpr/PrestLCSF12,
  added-at = {2014-07-31T00:00:00.000+0200},
  author = {Prest, Alessandro and Leistner, Christian and Civera, Javier and Schmid, Cordelia and Ferrari, Vittorio},
  biburl = {http://www.bibsonomy.org/bibtex/2826cada174d8324d3429d3f27682708f/dblp},
  booktitle = {CVPR},
  crossref = {conf/cvpr/2012},
  ee = {http://doi.ieeecomputersociety.org/10.1109/CVPR.2012.6248065},
  interhash = {c77cf607bee39b622c42e08da6d1da68},
  intrahash = {826cada174d8324d3429d3f27682708f},
  isbn = {978-1-4673-1226-4},
  keywords = {dblp},
  timestamp = {2015-06-19T15:56:14.000+0200},
  title = {Learning object class detectors from weakly annotated video.},
  url = {http://dblp.uni-trier.de/db/conf/cvpr/cvpr2012.html#PrestLCSF12},
  year = 2012
}

@inproceedings{DBLP:journals/corr/WalkerDGH16,
  author    = {Jacob Walker and
               Carl Doersch and
               Abhinav Gupta and
               Martial Hebert},
  title     = {An Uncertain Future: Forecasting from Static Images using Variational
               Autoencoders},
  booktitle = {ECCV},
  year      = {2016},
}

@article{Horn:1981,
 author = {Horn, Berthold K.P. and Schunck, Brian G.},
 title = {Determining Optical Flow},
 year = {1981},
 journal = {Artificial Intelligence},
 volume = 17,
} 


@inproceedings{Silberman:ECCV12,
  author    = {Nathan Silberman and Derek Hoiem and Pushmeet Kohli and Rob Fergus},
  title     = {Indoor Segmentation and Support Inference from {RGBD} Images},
  booktitle = {ECCV},
  year      = {2012}
}


@INPROCEEDINGS{Geiger2012CVPR,
  author = {Andreas Geiger and Philip Lenz and Raquel Urtasun},
  title = {Are we ready for Autonomous Driving? {T}he {KITTI} Vision Benchmark Suite},
  booktitle = {CVPR},
  year = {2012}
} 

@inproceedings{Butler:ECCV:2012,
title = {A naturalistic open source movie for optical flow evaluation},
author = {Butler, D. J. and Wulff, J. and Stanley, G. B. and Black, M. J.},
booktitle = {ECCV},
year = 2012,
}


@InProceedings{Hornacek_2014_CVPR,
author = {Hornacek, Michael and Fitzgibbon, Andrew and Rother, Carsten},
title = {{SphereFlow}: 6 {DoF} Scene Flow from {RGB-D} Pairs},
booktitle = {CVPR},
year = {2014}
}




@article{Nir_IJCV2008,
    abstract = {{A novel optical flow estimation process based on a spatio-temporal model with varying coefficients multiplying a set of basis functions at each pixel is introduced. Previous optical flow estimation methodologies did not use such an over parameterized representation of the flow field as the problem is ill-posed even without introducing any additional parameters: Neighborhood based methods of the Lucas---Kanade type determine the flow at each pixel by constraining the flow to be described by a few parameters in small neighborhoods. Modern variational methods represent the optic flow directly via the flow field components at each pixel. The benefit of over-parametrization becomes evident in the smoothness term, which instead of directly penalizing for changes in the optic flow, accumulates a cost of deviating from the assumed optic flow model. Our proposed method is very general and the classical variational optical flow techniques are special cases of it, when used in conjunction with constant basis functions. Experimental results with the novel flow estimation process yield significant improvements with respect to the best results published so far.}},
    address = {Hingham, MA, USA},
    author = {Nir, Tal and Bruckstein, AlfredM and Kimmel, Ron},
    journal = {IJCV},
    citeulike-article-id = {6766220},
    citeulike-linkout-0 = {http://portal.acm.org/citation.cfm?id=1331491},
    citeulike-linkout-1 = {http://dx.doi.org/10.1007/s11263-007-0051-2},
    citeulike-linkout-2 = {http://link.springer.com/article/10.1007/s11263-007-0051-2},
    doi = {10.1007/s11263-007-0051-2},
    issn = {0920-5691},
    keywords = {computer\_vision, optic\_flow, variational\_method},
    number = {2},
    pages = {205--216},
    posted-at = {2016-05-24 16:29:23},
    priority = {2},
    publisher = {Springer US},
    title = {{Over-Parameterized Variational Optical Flow}},
    url = {http://dx.doi.org/10.1007/s11263-007-0051-2},
    volume = {76},
    year = {2008}
}

@article{KILNER2013R1057,
title = "What We Know Currently about Mirror Neurons",
journal = "Current Biology",
volume = "23",
number = "23",
pages = "R1057 - R1062",
year = "2013",
note = "",
issn = "0960-9822",
doi = "http://dx.doi.org/10.1016/j.cub.2013.10.051",
url = "http://www.sciencedirect.com/science/article/pii/S0960982213013262",
author = "J.M. Kilner and R.N. Lemon",

}


@article{Ramachandran00,
  abstract = {The discovery of mirror neurons in the frontal lobes of monkeys, and their potential relevance to human brain evolution — which I speculate on in this essay — is the single most important "unreported" (or at least, unpublicized) story of the decade. I predict that mirror neurons will do for psychology what DNA did for biology: they will provide a unifying framework and help explain a host of mental abilities that have hitherto remained mysterious and inaccessible to experiments.
},
  added-at = {2007-01-23T18:03:44.000+0100},
  author = {Ramachandran, V.S.},
  biburl = {https://www.bibsonomy.org/bibtex/21f56be84a986504a25a4b620e8c8b3d7/yish},
  date = {00]},
  description = {EDGE: MIRROR NEURONS},
  interhash = {a0170113f3387eb21d84c02f7e7f6f47},
  intrahash = {1f56be84a986504a25a4b620e8c8b3d7},
  journal = {Edge},
  keywords = {imported},
  timestamp = {2007-01-23T18:03:44.000+0100},
  title = {MIRROR NEURONS and imitation learning as the driving force behind "the great leap forward" in human evolution},
  url = {http://www.edge.org/3rd_culture/ramachandran/ramachandran_index.html},
  volume = 69,
  year = 2000
}





@InProceedings{Fragkiadaki_2015_CVPR,
author = {Fragkiadaki, Katerina and Arbelaez, Pablo and Felsen, Panna and Malik, Jitendra},
title = {Learning to Segment Moving Objects in Videos},
booktitle = {CVPR},
month = {June},
year = {2015}
}

@InProceedings{kerl13iros,
  author =    {C. Kerl and J. Sturm and D. Cremers},
  title =     {Dense Visual {SLAM} for {RGB-D} Cameras},
  booktitle = {IROS},
  year =      2013,
  keywords={dense visual odometry,dense visual slam,rgb-d,rgb-d benchmark}
}

@article{DBLP:journals/corr/GodardAB16,
  author    = {Cl{\'{e}}ment Godard and
               Oisin {Mac Aodha} and
               Gabriel J. Brostow},
  title     = {Unsupervised Monocular Depth Estimation with Left-Right Consistency},
  journal   = {CoRR},
  volume    = {abs/1609.03677},
  year      = {2016},
  url       = {http://arxiv.org/abs/1609.03677},
  timestamp = {Mon, 03 Oct 2016 17:51:10 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/GodardAB16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@INPROCEEDINGS{Geiger2012CVPR,
  author = {Andreas Geiger and Philip Lenz and Raquel Urtasun},
  title = {Are we ready for Autonomous Driving? The KITTI Vision Benchmark Suite},
  booktitle = {Conference on Computer Vision and Pattern	Recognition (CVPR)},
  year = {2012}
}
@INPROCEEDINGS{Menze2015CVPR,
  author = {Moritz Menze and Andreas Geiger},
  title = {Object Scene Flow for Autonomous Vehicles},
  booktitle = {Conference on Computer Vision and Pattern	Recognition (CVPR)},
  year = {2015}
} 
@inproceedings{mocapcmu,
author={http://mocap.cs.cmu.edu/},
title={CMU mocap database},
}


@inproceedings{schoeps14ismar,
author={T. Sch\"ops and J. Engel and D. Cremers},
title={Semi-Dense Visual Odometry for {AR} on a Smartphone},
year= {2014},
booktitle = "ISMAR",
}

@inproceedings{engel14eccv,
author={J. Engel and T. Sch\"ops and D. Cremers},
title={{LSD-SLAM}: Large-Scale Direct Monocular {SLAM}},
year= {2014},
booktitle = "ECCV",
keywords={rgb-d, monocular, slam, semidense, lsdslam},
award = {Oral Presentation}
}

@inproceedings{Izadi:2011:KRR:2047196.2047270,
 author = {Izadi, Shahram and Kim, David and Hilliges, Otmar and Molyneaux, David and Newcombe, Richard and Kohli, Pushmeet and Shotton, Jamie and Hodges, Steve and Freeman, Dustin and Davison, Andrew and Fitzgibbon, Andrew},
 title = {KinectFusion: Real-time 3D Reconstruction and Interaction Using a Moving Depth Camera},
 booktitle = {Proceedings of the 24th Annual ACM Symposium on User Interface Software and Technology},
 series = {UIST '11},
 year = {2011},
 isbn = {978-1-4503-0716-1},
 location = {Santa Barbara, California, USA},
 pages = {559--568},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/2047196.2047270},
 doi = {10.1145/2047196.2047270},
 acmid = {2047270},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {3D, AR, GPU, depth cameras, geometry-aware interactions, physics, surface reconstruction, tracking},
} 


@inproceedings{garg2016unsupervised,
  title={Unsupervised CNN for single view depth estimation: Geometry to the rescue},
  author={Garg, Ravi and Kumar, BG Vijay and Carneiro, Gustavo and Reid, Ian},
  booktitle={European Conference on Computer Vision},
  pages={740--756},
  year={2016},
  organization={Springer}
}

@article{DBLP:journals/corr/GargBR16,
  author    = {Ravi Garg and
               Vijay Kumar BG and
               Ian D. Reid},
  title     = {Unsupervised {CNN} for Single View Depth Estimation: Geometry to the
               Rescue},
  journal   = {CoRR},
  volume    = {abs/1603.04992},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.04992},
  timestamp = {Fri, 08 Apr 2016 07:34:30 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/GargBR16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Bergen:1992:HMM:645305.648720,
 author = {Bergen, James R. and Anandan, P. and Hanna, Keith J. and Hingorani, Rajesh},
 title = {Hierarchical Model-Based Motion Estimation},
 booktitle = {ECCV},
 year = {1992},
} 


@article{DBLP:journals/corr/FragkiadakiAFM14,
  author    = {Katerina Fragkiadaki and
               Pablo Andr{\'{e}}s Arbel{\'{a}}ez and
               Panna Felsen and
               Jitendra Malik},
  title     = {Spatio-Temporal Moving Object Proposals},
  journal   = {CoRR},
  volume    = {abs/1412.6504},
  year      = {2014},
  url       = {http://arxiv.org/abs/1412.6504},
  timestamp = {Thu, 01 Jan 2015 19:51:08 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/FragkiadakiAFM14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{citeulike:2638091,
    abstract = {{Traditional plane alignment techniques are typically performed between pairs of frames. In this paper, we present a method for extending existing two-frame planar motion estimation techniques into a simultaneous multi-frame estimation, by exploiting multiframe subspace constraints of planar surfaces. The paper has three main contributions: 1 ) we show that when the camera calibration does not change, the collection of all parametric image motions of a planar surface in the scene across...}},
    author = {Manor, L. Z. and Irani, M.},
    citeulike-article-id = {2638091},
    citeulike-linkout-0 = {http://citeseerx.ist.psu.edu/viewdoc/summary?doi=10.1.1.12.8166},
    journal = {PAMI},
    keywords = {optical-flow-multi-frame},
    number = {10},
    pages = {1105--1116},
    posted-at = {2008-04-07 16:42:55},
    priority = {2},
    title = {{Multi-Frame Estimation of Planar Motion}},
    url = {http://citeseerx.ist.psu.edu/viewdoc/summary?doi=10.1.1.12.8166},
    volume = {22},
    year = {2000}
}



@article{monodepthlr2016,
  author       = {Godard, Clément and Mac Aodha, Oisin and Brostow, Gabriel J.},
  title        = {Unsupervised Monocular Depth Estimation with Left-Right Consistency},
  journal      = "CoRR",
  volume       = {abs/1609.03677},
  year         = {2016},
}

@inproceedings{stn,
  author    = {Max Jaderberg and
               Karen Simonyan and
               Andrew Zisserman and
               Koray Kavukcuoglu},
  title     = {Spatial Transformer Networks},
  booktitle = {NIPS}, 
  year      = {2015}
}

Don't use this one -- use the ECCV one below
@article{DBLP:journals/corr/YuHD16,
  author    = {Jason J. Yu and
               Adam W. Harley and
               Konstantinos G. Derpanis},
  title     = {Back to Basics: Unsupervised Learning of Optical Flow via Brightness
               Constancy and Motion Smoothness},
  journal   = {CoRR},
  volume    = {abs/1608.05842},
  year      = {2016},
  url       = {http://arxiv.org/abs/1608.05842},
  timestamp = {Fri, 02 Sep 2016 17:46:24 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/YuHD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{back_to_basics:2016,
  author    = {Jason J. Yu and
               Adam W. Harley and
               Konstantinos G. Derpanis},
  title     = {Back to Basics: Unsupervised Learning of Optical Flow via Brightness
               Constancy and Motion Smoothness},
  booktitle = "ECCV",
  year = 2016,
}


@InProceedings{flownet,
  author       = "A. Dosovitskiy and P. Fischer and E. Ilg and P. H{\"a}usser and C. Hazirbas and V. Golkov and P. Smagt and D. Cremers and T. Brox",
  title        = "{FlowNet}: Learning Optical Flow with Convolutional Networks",
  booktitle    = "ICCV",
  year         = "2015",
}

@inproceedings{interpreter,
author="Wu, Jiajun
and Xue, Tianfan
and Lim, Joseph J.
and Tian, Yuandong
and Tenenbaum, Joshua B.
and Torralba, Antonio
and Freeman, William T.",
title="Single Image {3D} Interpreter Network",
bookTitle="ECCV",
year="2016",
}


@article{SE3-Nets,
 author = {A. Byravan and D. Fox},
 title = {{SE3-Nets}: Learning Rigid Body Motion using Deep Neural Networks},
 journal = "CoRR",
 volume = "abs/1606.02378",
 year = 2016,
}

@InProceedings{flyingthings16,
	author = {N. Mayer and E. Ilg and P. H\"ausser and P. Fischer and D. Cremers and A. Dosovitskiy and T. Brox},
title = {A large dataset to train convolutional networks for disparity, optical flow, and scene flow estimation},
booktitle = {CVPR},
year = {2016}
}



@INPROCEEDINGS{5459407, 
author={Brubaker, Marcus A. and Sigal, L. and Fleet, D.J.}, 
booktitle={Computer Vision, 2009 IEEE 12th International Conference on}, 
title={Estimating contact dynamics}, 
year={2009}, 
pages={2389-2396}, 
keywords={Biological system modeling;Geometry;Gravity;Humans;Inference algorithms;Joints;Motion estimation;Solid modeling;Testing;Tracking}, 
doi={10.1109/ICCV.2009.5459407}, 
ISSN={1550-5499}, 
month={Sept}
}

@inproceedings{conf/eccv/BhatSP02,
  added-at = {2011-06-30T00:00:00.000+0200},
  author = {Bhat, Kiran S. and Seitz, Steven M. and Popovic, Jovan},
  biburl = {http://www.bibsonomy.org/bibtex/20fafe53b2d695d4262da2e3aa2219521/dblp},
  booktitle = {ECCV},
  crossref = {conf/eccv/2002-1},
  editor = {Heyden, Anders and Sparr, Gunnar and Nielsen, Mads and Johansen, Peter},
  ee = {http://dx.doi.org/10.1007/3-540-47969-4_37},
  interhash = {3cc5e0f9b763368da2cb82bfddb514b9},
  intrahash = {0fafe53b2d695d4262da2e3aa2219521},
  isbn = {3-540-43745-2},
  keywords = {dblp},
  pages = {551-565},
  publisher = {Springer},
  series = {Lecture Notes in Computer Science},
  timestamp = {2011-07-01T11:39:44.000+0200},
  title = {Computing the Physical Parameters of Rigid-Body Motion from Video.},
  url = {http://dblp.uni-trier.de/db/conf/eccv/eccv2002-1.html#BhatSP02},
  volume = 2350,
  year = 2002
}


@incollection{NIPS2015_5780,
title = {Galileo: Perceiving Physical Object Properties by Integrating a Physics Engine with Deep Learning},
author = {Wu, Jiajun and Yildirim, Ilker and Lim, Joseph J and Freeman, Bill and Tenenbaum, Josh},
booktitle = {Advances in Neural Information Processing Systems 28},
editor = {C. Cortes and N.D. Lawrence and D.D. Lee and M. Sugiyama and R. Garnett and R. Garnett},
pages = {127--135},
year = {2015},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5780-galileo-perceiving-physical-object-properties-by-integrating-a-physics-engine-with-deep-learning.pdf}
}

@misc {Kristan2016a,
	title = {The Visual Object Tracking VOT2016 challenge results},
	url = {http://www.springer.com/gp/book/9783319488806},
	author = {Matej Kristan and Ale\v{s} Leonardis and Jiri Matas and Michael Felsberg and Roman Pflugfelder and Luka \v{C}ehovin and Tomas Vojir and Gustav H\"{a}ger and Alan Luke\v{z}i\v{c} and Gustavo Fernandez},
	month = {Oct},
	year = {2016},
	howpublished = {Springer}
}


@article{DBLP:journals/corr/Leal-TaixeMRRS15,
  author    = {Laura Leal{-}Taix{\'{e}} and
               Anton Milan and
               Ian D. Reid and
               Stefan Roth and
               Konrad Schindler},
  title     = {MOTChallenge 2015: Towards a Benchmark for Multi-Target Tracking},
  journal   = {CoRR},
  volume    = {abs/1504.01942},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.01942},
  archivePrefix = {arXiv},
  eprint    = {1504.01942},
  timestamp = {Wed, 07 Jun 2017 14:40:39 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/Leal-TaixeMRRS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/MottaghiBRF15,
  author    = {Roozbeh Mottaghi and
               Hessam Bagherinezhad and
               Mohammad Rastegari and
               Ali Farhadi},
  title     = {Newtonian Image Understanding: Unfolding the Dynamics of Objects in
               Static Images},
  journal   = {CoRR},
  volume    = {abs/1511.04048},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.04048},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MottaghiBRF15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{conf/iccv/SalzmannU11,
  added-at = {2012-01-19T00:00:00.000+0100},
  author = {Salzmann, Mathieu and Urtasun, Raquel},
  biburl = {http://www.bibsonomy.org/bibtex/24d6e35c0f411d7427b602d8e24304f0f/dblp},
  booktitle = {ICCV},
  crossref = {conf/iccv/2011},
  editor = {Metaxas, Dimitris N. and Quan, Long and Sanfeliu, Alberto and Gool, Luc J. Van},
  ee = {http://dx.doi.org/10.1109/ICCV.2011.6126480},
  interhash = {56d5fa22b622d3e98adf7879ee4573f7},
  intrahash = {4d6e35c0f411d7427b602d8e24304f0f},
  isbn = {978-1-4577-1101-5},
  keywords = {dblp},
  pages = {2064-2071},
  publisher = {IEEE},
  timestamp = {2012-01-20T11:33:25.000+0100},
  title = {Physically-based motion models for 3D tracking: A convex formulation.},
  url = {http://dblp.uni-trier.de/db/conf/iccv/iccv2011.html#SalzmannU11},
  year = 2011
}



@article{DBLP:journals/corr/AgrawalNAML16,
  author    = {Pulkit Agrawal and
               Ashvin Nair and
               Pieter Abbeel and
               Jitendra Malik and
               Sergey Levine},
  title     = {Learning to Poke by Poking: Experiential Learning of Intuitive Physics},
  journal   = {CoRR},
  volume    = {abs/1606.07419},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.07419},
  archivePrefix = {arXiv},
  eprint    = {1606.07419},
  timestamp = {Wed, 07 Jun 2017 14:42:59 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/AgrawalNAML16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/FragkiadakiALM15,
  author    = {Katerina Fragkiadaki and
               Pulkit Agrawal and
               Sergey Levine and
               Jitendra Malik},
  title     = {Learning Visual Predictive Models of Physics for Playing Billiards},
  journal   = {ICLR},
  year      = {2015}
}



@inproceedings{DBLP:conf/bmvc/KyriazisOA11,
  author    = {Nikolaos Kyriazis and
               Iason Oikonomidis and
               Antonis A. Argyros},
  title     = {Binding Computer Vision to Physics Based Simulation: The Case Study
               of a Bouncing Ball},
  booktitle = {British Machine Vision Conference, {BMVC} 2011, Dundee, UK, August
               29 - September 2, 2011. Proceedings},
  pages     = {1--11},
  year      = {2011},
  crossref  = {DBLP:conf/bmvc/2011},
  url       = {http://dx.doi.org/10.5244/C.25.43},
  doi       = {10.5244/C.25.43},
  timestamp = {Wed, 24 Apr 2013 17:19:07 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/bmvc/KyriazisOA11},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{conf/eccv/BhatSP02,
  added-at = {2011-06-30T00:00:00.000+0200},
  author = {Bhat, Kiran S. and Seitz, Steven M. and Popovic, Jovan},
  biburl = {http://www.bibsonomy.org/bibtex/20fafe53b2d695d4262da2e3aa2219521/dblp},
  booktitle = {ECCV (1)},
  crossref = {conf/eccv/2002-1},
  editor = {Heyden, Anders and Sparr, Gunnar and Nielsen, Mads and Johansen, Peter},
  ee = {http://dx.doi.org/10.1007/3-540-47969-4_37},
  interhash = {3cc5e0f9b763368da2cb82bfddb514b9},
  intrahash = {0fafe53b2d695d4262da2e3aa2219521},
  isbn = {3-540-43745-2},
  keywords = {dblp},
  pages = {551-565},
  publisher = {Springer},
  series = {Lecture Notes in Computer Science},
  timestamp = {2011-07-01T11:39:44.000+0200},
  title = {Computing the Physical Parameters of Rigid-Body Motion from Video.},
  url = {http://dblp.uni-trier.de/db/conf/eccv/eccv2002-1.html#BhatSP02},
  volume = 2350,
  year = 2002
}

@inproceedings{42854,
title = {Large-Scale Object Classification Using Label Relation Graphs},
author  = {Jia Deng and Nan Ding and Yangqing Jia and Andrea Frome and Kevin Murphy and Samy Bengio and Yuan Li and Hartmut Neven and Hartwig Adam},
year  = 2014,
booktitle = {European Conference on Computer Vision}
}



@article{smith2005development,
  title={The development of embodied cognition: Six lessons from babies},
  author={Smith, Linda and Gasser, Michael},
  journal={Artificial life},
  volume={11},
  number={1-2},
  pages={13--29},
  year={2005}
}

@article{hansen2001completely,
  title={Completely derandomized self-adaptation in evolution strategies},
  author={Hansen, Nikolaus and Ostermeier, Andreas},
  journal={Evolutionary computation},
  volume={9},
  number={2},
  pages={159--195},
  year={2001},
  publisher={MIT Press}
}

@article{actionconditioned,
  title={Action-Conditional Video Prediction using Deep Networks in Atari Games},
  author={Oh, Junhyuk and Guo, Xiaoxiao and Lee, Honglak and Lewis, Richard and Singh, Satinder},
  journal={arXiv preprint arXiv:1507.08750},
  year={2015}
}

@inproceedings{hamrick2011internal,
  title={Internal physics models guide probabilistic judgments about object dynamics},
  author={Hamrick, Jessica and Battaglia, Peter and Tenenbaum, Joshua B},
  booktitle={Proceedings of the 33rd annual conference of the cognitive science society},
  pages={1545--1550},
  year={2011},
  organization={Cognitive Science Society Austin, TX}
}

@article{jordan1992forward,
  title={Forward models: Supervised learning with a distal teacher},
  author={Jordan, Michael I and Rumelhart, David E},
  journal={Cognitive science},
  volume={16},
  number={3},
  pages={307--354},
  year={1992},
  publisher={Wiley Online Library}
}

@article{wolpert1995internal,
  title={An internal model for sensorimotor integration},
  author={Wolpert, Daniel M and Ghahramani, Zoubin and Jordan, Michael I},
  journal={Science-AAAS-Weekly Paper Edition},
  volume={269},
  number={5232},
  pages={1880--1882},
  year={1995},
  publisher={New York, NY:[sn] 1880-}
}



@article{thesisblocks,
  title={Machine perception of three-dimensional solids},
  author={Roberts, Lawrence},
  year={1963},
  publisher={MIT}
}

@article{haruno2001mosaic,
  title={Mosaic model for sensorimotor learning and control},
  author={Haruno, Masahiko and Wolpert, David H and Kawato, Mitsuo},
  journal={Neural computation},
  volume={13},
  number={10},
  pages={2201--2220},
  year={2001},
  publisher={MIT Press}
}

@inproceedings{todorov2003unsupervised,
  title={Unsupervised learning of sensory-motor primitives},
  author={Todorov, Emanuel and Ghahramani, Zoubin},
  booktitle={Engineering in Medicine and Biology Society, 2003. Proceedings of the 25th Annual International Conference of the IEEE},
  volume={2},
  pages={1750--1753},
  year={2003},
  organization={IEEE}
}

@article{DBLP:journals/corr/WahlstromSD15,
  author    = {Niklas Wahlstr{\"{o}}m and
               Thomas B. Sch{\"{o}}n and
               Marc Peter Deisenroth},
  title     = {From Pixels to Torques: Policy Learning with Deep Dynamical Models},
  journal   = {CoRR},
  volume    = {abs/1502.02251},
  year      = {2015},
  url       = {http://arxiv.org/abs/1502.02251},
  timestamp = {Mon, 02 Mar 2015 00:00:00 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/WahlstromSD15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/DonahueHGRVSD14,
  author    = {Jeff Donahue and
               Lisa Anne Hendricks and
               Sergio Guadarrama and
               Marcus Rohrbach and
               Subhashini Venugopalan and
               Kate Saenko and
               Trevor Darrell},
  title     = {Long-term Recurrent Convolutional Networks for Visual Recognition
               and Description},
  journal   = {CoRR},
  year      = {2014},
}

@article{DeepMindContinuous,
  author    = {Timothy P. Lillicrap and Jonathan J. Hunt and Alexander Pritzel and Nicolas Heess and Tom Erez and Yuval Tassa and David Silver and Daan Wierstra},
  title     = {Continuous control with deep reinforcement learning},
  journal   = {CoRR},
  volume    = {abs/1509.02971},
  year      = {2015}
}

@article{DBLP:journals/corr/WatterSBR15,
  author    = {Manuel Watter and
               Jost Tobias Springenberg and
               Joschka Boedecker and
               Martin A. Riedmiller},
  title     = {Embed to Control: {A} Locally Linear Latent Dynamics Model for Control
               from Raw Images},
  journal   = {CoRR},
  volume    = {abs/1506.07365},
  year      = {2015},
  url       = {http://arxiv.org/abs/1506.07365},
  timestamp = {Wed, 01 Jul 2015 15:10:24 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/WatterSBR15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/ijcnn/LangeRV12,
  author    = {Sascha Lange and
               Martin A. Riedmiller and
               Arne Voigtl{\"{a}}nder},
  title     = {Autonomous reinforcement learning on raw visual input data in a real
               world application},
  booktitle = {The 2012 International Joint Conference on Neural Networks (IJCNN),
               Brisbane, Australia, June 10-15, 2012},
  pages     = {1--8},
  year      = {2012},
  crossref  = {DBLP:conf/ijcnn/2012},
  url       = {http://dx.doi.org/10.1109/IJCNN.2012.6252823},
  doi       = {10.1109/IJCNN.2012.6252823},
  timestamp = {Wed, 01 Apr 2015 20:06:23 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/ijcnn/LangeRV12},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/icra/BootsBF14,
  author    = {Byron Boots and
               Arunkumar Byravan and
               Dieter Fox},
  title     = {Learning predictive models of a depth camera {\&} manipulator
               from raw execution traces},
  booktitle = {2014 {IEEE} International Conference on Robotics and Automation, {ICRA}
               2014, Hong Kong, China, May 31 - June 7, 2014},
  pages     = {4021--4028},
  year      = {2014},
  crossref  = {DBLP:conf/icra/2014},
  url       = {http://dx.doi.org/10.1109/ICRA.2014.6907443},
  doi       = {10.1109/ICRA.2014.6907443},
  timestamp = {Tue, 07 Oct 2014 13:28:58 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icra/BootsBF14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/LevineFDA15,
  author    = {Sergey Levine and
               Chelsea Finn and
               Trevor Darrell and
               Pieter Abbeel},
  title     = {End-to-End Training of Deep Visuomotor Policies},
  journal   = {CoRR},
  volume    = {abs/1504.00702},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.00702},
  timestamp = {Sat, 02 May 2015 17:50:32 +0200},
  biburl    = {http://dblp2.uni-trier.de/rec/bib/journals/corr/LevineFDA15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{GuptaEfrosHebert_ECCV10,
   author="Abhinav Gupta and Alexei A. Efros and Martial Hebert", 
   title="Blocks World Revisited: Image Understanding Using Qualitative Geometry and Mechanics", 
   booktitle="European Conference on Computer Vision(ECCV)", 
   year="2010", 
}


@inproceedings{Urtasun:2006:PTG:1153170.1153448,
 author = {Urtasun, Raquel and Fleet, David J. and Fua, Pascal},
 title = {3D People Tracking with Gaussian Process Dynamical Models},
 booktitle = {CVPR},
 year = {2006}
} 


@article{Weng:2006:VOT:1223195.1223208,
 author = {Weng, Shiuh-Ku and Kuo, Chung-Ming and Tu, Shu-Kang},
 title = {Video Object Tracking Using Adaptive Kalman Filter},
 journal = {J. Vis. Comun. Image Represent.},
 issue_date = {December, 2006},
 volume = {17},
 number = {6},
 year = {2006},
 issn = {1047-3203},
 pages = {1190--1208},
 numpages = {19},
 url = {http://dx.doi.org/10.1016/j.jvcir.2006.03.004},
 doi = {10.1016/j.jvcir.2006.03.004},
 acmid = {1223208},
 publisher = {Academic Press, Inc.},
 address = {Orlando, FL, USA},
 keywords = {Adaptive Kalman filter, HSI color space, Occlusion ratio},
} 

  @inproceedings{Brand:1997:CHM:794189.794420,
  author = {Brand, M. and Oliver, N. and Pentland, A.},
  title = {Coupled hidden Markov models for complex action recognition},
  booktitle = {CVPR},
  year = {1997}
  }

  @article{Ghahramani:1997:FHM:274158.274165,
  author = {Ghahramani, Zoubin and Jordan, Michael I.},
  title = {Factorial Hidden Markov Models},
  journal = {Mach. Learn.},
  volume = {29},
  year = {1997}
  }

@inproceedings{lenz_deepMPC_2015,
  title={DeepMPC: Learning Deep Latent Features for Model Predictive Control},
  author={Ian Lenz and Ross Knepper and Ashutosh Saxena},
  year={2015},
  booktitle={RSS}
}


@article{citeulike:13838961,
    author = {Abadi, Mart\'{\i}n and Agarwal, Ashish and Barham, Paul and Brevdo, Eugene and Chen, Zhifeng and Citro, Craig and Corrado, Greg S. and Davis, Andy and Dean, Jeffrey and Devin, Matthieu and Ghemawat, Sanjay and Goodfellow, Ian and Harp, Andrew and Irving, Geoffrey and Isard, Michael and Jia, Yangqing and Jozefowicz, Rafal and Kaiser, Lukasz and Kudlur, Manjunath and Levenberg, Josh and Man\'{e}, Dan and Monga, Rajat and Moore, Sherry and Murray, Derek and Olah, Chris and Schuster, Mike and Shlens, Jonathon and Steiner, Benoit and Sutskever, Ilya and Talwar, Kunal and Tucker, Paul and Vanhoucke, Vincent and Vasudevan, Vijay and Vi\'{e}gas, Fernanda and Vinyals, Oriol and Warden, Pete and Wattenberg, Martin and Wicke, Martin and Yu, Yuan and Zheng, Xiaoqiang},
    title = {{TensorFlow}: Large-Scale Machine Learning on Heterogeneous Distributed Systems},
    journal = {arXiv:1603.04467},
    year = 2016,
}


@INPROCEEDINGS{Viola01rapidobject,
    author = {Paul Viola and Michael Jones},
    title = {Rapid object detection using a boosted cascade of simple features},
    booktitle = {},
    year = {2001},
    pages = {511--518}
}

@article{Chetverikov2005299,
title = "Robust Euclidean alignment of 3D point sets: the trimmed iterative closest point algorithm ",
journal = "Image and Vision Computing ",
volume = "23",
number = "3",
pages = "299 - 309",
year = "2005",
note = "",
author = "Dmitry Chetverikov and Dmitry Stepanov and Pavel Krsek"
}



@INPROCEEDINGS{jooiccv2015,
author = {Hanbyul Joo, Hao Liu, Lei Tan, Lin Gui, Bart Nabbe, Iain Matthews, Takeo Kanade, Shohei Nobuhara, and Yaser Sheikh},
title = {Panoptic Studio: A Massively Multiview System for Social Motion Capture},
booktitle = {ICCV},
year = {2015}
}



@INPROCEEDINGS{4409106, 
author={Saragih, J. and Goecke, R.}, 
booktitle={Computer Vision, 2007. ICCV 2007. IEEE 11th International Conference on}, 
title={A Nonlinear Discriminative Approach to AAM Fitting}, 
year={2007}, 
month={Oct}, 
pages={1-8}, 
keywords={computer vision;convergence of numerical methods;image registration;iterative methods;learning (artificial intelligence);AAM fitting formulation;active appearance model;boosting procedure;convergence rates;deformable visual object modeling;deformable visual object registration;iterative framework;linear parameter update model;nonlinear discriminative approach;Active appearance model;Cost function;Deformable models;Error correction;Fitting;Parametric statistics;Power engineering and energy;Power generation;Principal component analysis;Shape}, 
doi={10.1109/ICCV.2007.4409106}, 
ISSN={1550-5499},}

@incollection{NIPS2014_5573,
title = {Joint Training of a Convolutional Network and a Graphical Model for Human Pose Estimation},
author = {Tompson, Jonathan J and Jain, Arjun and LeCun, Yann and Bregler, Christoph},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N.D. Lawrence and K.Q. Weinberger},
pages = {1799--1807},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5573-joint-training-of-a-convolutional-network-and-a-graphical-model-for-human-pose-estimation.pdf}
}


@article{Mellinger:2012:TGC:2190635.2190636,
 author = {Mellinger, Daniel and Michael, Nathan and Kumar, Vijay},
 title = {Trajectory Generation and Control for Precise Aggressive Maneuvers with Quadrotors},
 journal = {Int. J. Rob. Res.},
 issue_date = {April     2012},
 volume = {31},
 number = {5},
 month = apr,
 year = {2012},
 issn = {0278-3649},
 pages = {664--674},
 numpages = {11},
 url = {http://dx.doi.org/10.1177/0278364911434236},
 doi = {10.1177/0278364911434236},
 acmid = {2190636},
 publisher = {Sage Publications, Inc.},
 address = {Thousand Oaks, CA, USA},
 keywords = {Trajectory generation, control, quadrotors},
} 

@inproceedings{YangR_CVPR_2011,
    author = "Yang, Yi and Ramanan, Deva",
    booktitle = "CVPR",
    year = "2011",
    title = "Articulated pose estimation with flexible mixtures-of-parts"
}


@INPROCEEDINGS{1315258, 
author={Agarwal, A. and Triggs, B.}, 
booktitle={Computer Vision and Pattern Recognition, 2004. CVPR 2004. Proceedings of the 2004 IEEE Computer Society Conference on}, 
title={3D human pose from silhouettes by relevance vector regression}, 
year={2004}, 
month={June}, 
volume={2}, 
pages={II-882-II-888 Vol.2}, 
keywords={errors;image segmentation;image sequences;learning (artificial intelligence);least squares approximations;motion estimation;multidimensional signal processing;regression analysis;3D human pose;direct nonlinear regression;histogram-of-shape-contexts descriptors;human motion capture data;image silhouettes;learning based method;mean angular errors;monocular image sequences;regularized least squares;relevance vector machine;relevance vector regression;shape descriptor vectors;silhouette segmentation errors;Biological system modeling;Humans;Image sequences;Kernel;Labeling;Learning systems;Robustness;Shape;Testing;Vectors}, 
doi={10.1109/CVPR.2004.1315258}, 
ISSN={1063-6919},}


@Inproceedings {export:145347,
author       = {Jamie Shotton and Andrew Fitzgibbon and Mat Cook and Toby Sharp and Mark
                Finocchio and Richard Moore and Alex Kipman and Andrew Blake},
booktitle    = {CVPR},
month        = {June},
publisher    = {IEEE},
title        = {Real-Time Human Pose Recognition in Parts from a Single Depth Image},
url          = {http://research.microsoft.com/apps/pubs/default.aspx?id=145347},
year         = {2011},
}

@inproceedings{DollarCVPR10pose,
  author = "P. Doll\'ar and P. Welinder and P. Perona",
  title = "Cascaded Pose Regression",
  booktitle = "CVPR",
  year = "2010",
}

@inproceedings{ionescu2014iterated,
  title={Iterated second-order label sensitive pooling for 3d human pose estimation},
  author={Ionescu, Catalin and Carreira, Joao and Sminchisescu, Cristian},
  booktitle={Computer Vision and Pattern Recognition (CVPR), 2014 IEEE Conference on},
  pages={1661--1668},
  year={2014},
  organization={IEEE}
}

@inproceedings{li2013fixed,
  title={Fixed-point model for structured labeling},
  author={Li, Quannan and Wang, Jingdong and Tu, Zhuowen and Wipf, David P},
  booktitle={Proceedings of the 30th International Conference on Machine Learning (ICML-13)},
  pages={214--221},
  year={2013}
}

@inproceedings{tu2008auto,
  title={Auto-context and its application to high-level vision tasks},
  author={Tu, Zhuowen},
  booktitle={Computer Vision and Pattern Recognition, 2008. CVPR 2008. IEEE Conference on},
  pages={1--8},
  year={2008},
  organization={IEEE}
}

@article{lafferty2001conditional,
  title={Conditional random fields: Probabilistic models for segmenting and labeling sequence data},
  author={Lafferty, John and McCallum, Andrew and Pereira, Fernando CN},
  year={2001}
}

@article{krahenbuhl2012efficient,
  title={Efficient inference in fully connected crfs with gaussian edge potentials},
  author={Kr{\"a}henb{\"u}hl, Philipp and Koltun, Vladlen},
  journal={arXiv preprint arXiv:1210.5644},
  year={2012}
}





@article{zhu2015segdeepm,
  title={segDeepM: Exploiting segmentation and context in deep neural networks for object detection},
  author={Zhu, Yukun and Urtasun, Raquel and Salakhutdinov, Ruslan and Fidler, Sanja},
  journal={arXiv preprint arXiv:1502.04275},
  year={2015}
}

@article{gidaris2015object,
  title={Object detection via a multi-region \& semantic segmentation-aware CNN model},
  author={Gidaris, Spyros and Komodakis, Nikos},
  journal={arXiv preprint arXiv:1505.01749},
  year={2015}
}

@incollection{ramakrishna2014pose,
  title={Pose Machines: Articulated Pose Estimation via Inference Machines},
  author={Ramakrishna, Varun and Munoz, Daniel and Hebert, Martial and Bagnell, James Andrew and Sheikh, Yaser},
  booktitle={Computer Vision--ECCV 2014},
  pages={33--47},
  year={2014},
  publisher={Springer International Publishing}
}

@article{weiss2012structured,
  title={Structured prediction cascades},
  author={Weiss, David and Sapp, Benjamin and Taskar, Ben},
  journal={arXiv preprint arXiv:1208.3279},
  year={2012}
}

@inproceedings{heitz2009cascaded,
  title={Cascaded classification models: Combining models for holistic scene understanding},
  author={Heitz, Geremy and Gould, Stephen and Saxena, Ashutosh and Koller, Daphne},
  booktitle={Advances in Neural Information Processing Systems},
  pages={641--648},
  year={2009}
}

@article{DBLP:journals/corr/SadeghianAS17,
  author    = {Amir Sadeghian and
               Alexandre Alahi and
               Silvio Savarese},
  title     = {Tracking The Untrackable: Learning To Track Multiple Cues with Long-Term
               Dependencies},
  journal   = {CoRR},
  volume    = {abs/1701.01909},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.01909},
  timestamp = {Wed, 07 Jun 2017 14:40:23 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/SadeghianAS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article {depthadaptive,
author = {Ying, Chris and Fragkiadaki, Katerina},
title = {Depth-Adaptive  Computational Policies for Efficient
Visual Tracking},
journal = {EMMCVPR},
year = {2017}
}


@article {TOPS:TOPS12155,
author = {Lupyan, Gary and Bergen, Benjamin},
title = {How Language Programs the Mind},
journal = {Topics in Cognitive Science},
volume = {8},
number = {2},
issn = {1756-8765},
url = {http://dx.doi.org/10.1111/tops.12155},
doi = {10.1111/tops.12155},
pages = {408--424},
keywords = {Language, Language and thought, Embodiment, Categorization, Language evolution},
year = {2016},
}

@article{anonymous2018zero-shot,
  title={Zero-Shot Visual Imitation},
  author={Anonymous},
  journal={International Conference on Learning Representations},
  year={2018},
  url={https://openreview.net/forum?id=BkisuzWRW}
}

@article{DBLP:journals/corr/MnihBMGLHSK16,
  author    = {Volodymyr Mnih and
               Adri{\`{a}} Puigdom{\`{e}}nech Badia and
               Mehdi Mirza and
               Alex Graves and
               Timothy P. Lillicrap and
               Tim Harley and
               David Silver and
               Koray Kavukcuoglu},
  title     = {Asynchronous Methods for Deep Reinforcement Learning},
  journal   = {CoRR},
  volume    = {abs/1602.01783},
  year      = {2016},
  url       = {http://arxiv.org/abs/1602.01783},
  archivePrefix = {arXiv},
  eprint    = {1602.01783},
  timestamp = {Wed, 07 Jun 2017 14:43:09 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/MnihBMGLHSK16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{interactive,
  author    = {https://simons.berkeley.edu/workshops/machinelearning2017-1},
  year      = {2017}
}

@article{DBLP:journals/corr/RahmatizadehAB16,
  author    = {Rouhollah Rahmatizadeh and
               Pooya Abolghasemi and
               Ladislau B{\"{o}}l{\"{o}}ni},
  title     = {Learning Manipulation Trajectories Using Recurrent Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1603.03833},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.03833},
  archivePrefix = {arXiv},
  eprint    = {1603.03833},
  timestamp = {Wed, 07 Jun 2017 14:40:59 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/RahmatizadehAB16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/SermanetXL16,
  author    = {Pierre Sermanet and
               Kelvin Xu and
               Sergey Levine},
  title     = {Unsupervised Perceptual Rewards for Imitation Learning},
  journal   = {CoRR},
  volume    = {abs/1612.06699},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.06699},
  archivePrefix = {arXiv},
  eprint    = {1612.06699},
  timestamp = {Wed, 07 Jun 2017 14:42:07 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/SermanetXL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{MullingKKP2012_2,
  title = {Learning to Select and Generalize Striking Movements in Robot Table Tennis},
  author = {M{\"u}lling, K. and Kober, J. and Kroemer, O. and Peters, J.},
  journal = {International Journal of Robotics Research},
  volume = {32},
  number = {3},
  pages = {263-279},
  year = {2013}
}



@article {CDEP:CDEP12032,
author = {Waxman, Sandra and Fu, Xiaolan and Arunachalam, Sudha and Leddon, Erin and Geraghty, Kathleen and Song, Hyun-joo},
title = {Are Nouns Learned Before Verbs? Infants Provide Insight Into a Long-Standing Debate},
journal = {Child Development Perspectives},
volume = {7},
number = {3},
issn = {1750-8606},
url = {http://dx.doi.org/10.1111/cdep.12032},
doi = {10.1111/cdep.12032},
pages = {155--159},
keywords = {language development, cognitive development, cross-linguistic studies, infancy},
year = {2013},
}


@InProceedings{Su_2015_ICCV,
    Title={Render for CNN: Viewpoint Estimation in Images Using CNNs Trained with Rendered 3D Model Views},
    Author={Su, Hao and Qi, Charles R. and Li, Yangyan and Guibas, Leonidas J.},
    Booktitle={The IEEE International Conference on Computer Vision (ICCV)},
    month = {December},
    Year= {2015}
}

@article{nowozin2011structured,
  title={Structured learning and prediction in computer vision},
  author={Nowozin, Sebastian and Lampert, Christoph H},
  journal={Foundations and Trends{\textregistered} in Computer Graphics and Vision},
  volume={6},
  number={3--4},
  pages={185--365},
  year={2011},
  publisher={Now Publishers Inc.}
}

@inproceedings{stollenga2014deep,
  title={Deep networks with internal selective attention through feedback connections},
  author={Stollenga, Marijn F and Masci, Jonathan and Gomez, Faustino and Schmidhuber, J{\"u}rgen},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3545--3553},
  year={2014}
}

@article{pinheiro2013recurrent,
  title={Recurrent convolutional neural networks for scene parsing},
  author={Pinheiro, Pedro HO and Collobert, Ronan},
  journal={arXiv preprint arXiv:1306.2795},
  year={2013}
}

@article{kass1988snakes,
  title={Snakes: Active contour models},
  author={Kass, Michael and Witkin, Andrew and Terzopoulos, Demetri},
  journal={International journal of computer vision},
  volume={1},
  number={4},
  pages={321--331},
  year={1988},
  publisher={Springer}
}

@article{cootes1995active,
  title={Active shape models-their training and application},
  author={Cootes, Timothy F and Taylor, Christopher J and Cooper, David H and Graham, Jim},
  journal={Computer vision and image understanding},
  volume={61},
  number={1},
  pages={38--59},
  year={1995},
  publisher={Elsevier}
}

@article{felzenszwalb2010object,
  title={Object detection with discriminatively trained part-based models},
  author={Felzenszwalb, Pedro F and Girshick, Ross B and McAllester, David and Ramanan, Deva},
  journal={Pattern Analysis and Machine Intelligence, IEEE Transactions on},
  volume={32},
  number={9},
  pages={1627--1645},
  year={2010},
  publisher={IEEE}
}

@inproceedings{xiong2013supervised,
  title={Supervised descent method and its applications to face alignment},
  author={Xiong, Xuehan and De la Torre, Fernando},
  booktitle={Computer Vision and Pattern Recognition (CVPR), 2013 IEEE Conference on},
  pages={532--539},
  year={2013},
  organization={IEEE}
}


@article{Hochreiter:1997:LSM:1246443.1246450,
 author = {Hochreiter, Sepp and Schmidhuber, J\"{u}rgen},
 title = {Long Short-Term Memory},
 journal = {Neural Comput.},
 issue_date = {November 15, 1997},
 volume = {9},
 number = {8},
 year = {1997},
 issn = {0899-7667},
 pages = {1735--1780},
 numpages = {46},
 url = {http://dx.doi.org/10.1162/neco.1997.9.8.1735},
 doi = {10.1162/neco.1997.9.8.1735},
 acmid = {1246450},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 

@article{DBLP:journals/corr/Graves13,
  author    = {Alex Graves},
  title     = {Generating Sequences With Recurrent Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1308.0850},
  year      = {2013},
  url       = {http://arxiv.org/abs/1308.0850},
  timestamp = {Tue, 10 Dec 2013 12:03:02 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/Graves13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@techreport{Welch:1995:IKF:897831,
 author = {Welch, Greg and Bishop, Gary},
 title = {An Introduction to the Kalman Filter},
 year = {1995},
 publisher = {University of North Carolina at Chapel Hill},
 address = {Chapel Hill, NC, USA},
} 

@article{Vincent:2010:SDA:1756006.1953039,
 author = {Vincent, Pascal and Larochelle, Hugo and Lajoie, Isabelle and Bengio, Yoshua and Manzagol, Pierre-Antoine},
 title = {Stacked Denoising Autoencoders: Learning Useful Representations in a Deep Network with a Local Denoising Criterion},
 journal = {J. Mach. Learn. Res.},
 issue_date = {3/1/2010},
 volume = {11},
 year = {2010},
 issn = {1532-4435},
 pages = {3371--3408},
 numpages = {38},
 url = {http://dl.acm.org/citation.cfm?id=1756006.1953039},
 acmid = {1953039},
 publisher = {JMLR.org},
} 


@article{Mayne20142967,
title = "Model predictive control: Recent developments and future promise ",
journal = "Automatica ",
volume = "50",
number = "12",
pages = "2967 - 2986",
year = "2014",
note = "",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/j.automatica.2014.10.128",
url = "http://www.sciencedirect.com/science/article/pii/S0005109814005160",
author = "David Q. Mayne",
keywords = "Model predictive control ",
abstract = "Abstract This paper recalls a few past achievements in Model Predictive Control, gives an overview of some current developments and suggests a few avenues for future research. "
}

@inproceedings{DBLP:journals/corr/MisraZH16,
  author    = {Ishan Misra and
               C. Lawrence Zitnick and
               Martial Hebert},
  title     = {Unsupervised Learning using Sequential Verification for Action Recognition},
  booktitle={ECCV},
  year      = {2016},
}



@inproceedings{DBLP:journals/corr/WangG15a,
  author    = {Xiaolong Wang and
               Abhinav Gupta},
  title     = {Unsupervised Learning of Visual Representations using Videos},
  booktitle = {ICCV},
  year      = {2015}
}

@article{Wiskott:2002:SFA:638940.638941,
 author = {Wiskott, Laurenz and Sejnowski, Terrence J.},
 title = {Slow Feature Analysis: Unsupervised Learning of Invariances},
 journal = {Neural Comput.},
 issue_date = {April 2002},
 volume = {14},
 number = {4},
 year = {2002},
 issn = {0899-7667},
 pages = {715--770},
 numpages = {56},
 url = {http://dx.doi.org/10.1162/089976602317318938},
 doi = {10.1162/089976602317318938},
 acmid = {638941},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 


@inproceedings{DBLP:conf/icml/BellemareVT14,
  author    = {Marc G. Bellemare and
               Joel Veness and
               Erik Talvitie},
  title     = {Skip Context Tree Switching},
  booktitle = {Proceedings of the 31th International Conference on Machine Learning,
               {ICML} 2014, Beijing, China, 21-26 June 2014},
  pages     = {1458--1466},
  year      = {2014},
  crossref  = {DBLP:conf/icml/2014},
  url       = {http://jmlr.org/proceedings/papers/v32/bellemare14.html},
  timestamp = {Fri, 07 Nov 2014 20:42:30 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icml/BellemareVT14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{DBLP:conf/icmla/KietzmannR09,
  author    = {Tim C. Kietzmann and
               Martin A. Riedmiller},
  title     = {The Neuro Slot Car Racer: Reinforcement Learning in a Real World Setting},
  booktitle = {International Conference on Machine Learning and Applications, {ICMLA}
               2009, Miami Beach, Florida, USA, December 13-15, 2009},
  pages     = {311--316},
  year      = {2009},
  crossref  = {DBLP:conf/icmla/2009},
  url       = {http://dx.doi.org/10.1109/ICMLA.2009.15},
  doi       = {10.1109/ICMLA.2009.15},
  timestamp = {Wed, 06 May 2015 16:20:33 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icmla/KietzmannR09},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/MnihKSGAWR13,
  author    = {Volodymyr Mnih and
               Koray Kavukcuoglu and
               David Silver and
               Alex Graves and
               Ioannis Antonoglou and
               Daan Wierstra and
               Martin A. Riedmiller},
  title     = {Playing Atari with Deep Reinforcement Learning},
  journal   = {CoRR},
  volume    = {abs/1312.5602},
  year      = {2013},
  url       = {http://arxiv.org/abs/1312.5602},
  timestamp = {Wed, 01 Apr 2015 20:06:15 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MnihKSGAWR13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{DBLP:conf/icra/BootsBF14,
  author    = {Byron Boots and
               Arunkumar Byravan and
               Dieter Fox},
  title     = {Learning predictive models of a depth camera {\&} manipulator
               from raw execution traces},
  booktitle = {2014 {IEEE} International Conference on Robotics and Automation, {ICRA}
               2014, Hong Kong, China, May 31 - June 7, 2014},
  pages     = {4021--4028},
  year      = {2014},
  crossref  = {DBLP:conf/icra/2014},
  url       = {http://dx.doi.org/10.1109/ICRA.2014.6907443},
  doi       = {10.1109/ICRA.2014.6907443},
  timestamp = {Tue, 07 Oct 2014 13:28:58 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icra/BootsBF14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/LevineFDA15,
  author    = {Sergey Levine and
               Chelsea Finn and
               Trevor Darrell and
               Pieter Abbeel},
  title     = {End-to-End Training of Deep Visuomotor Policies},
  journal   = {CoRR},
  volume    = {abs/1504.00702},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.00702},
  timestamp = {Sat, 02 May 2015 17:50:32 +0200},
  biburl    = {http://dblp2.uni-trier.de/rec/bib/journals/corr/LevineFDA15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{lenz_deepMPC_2015,
  title={DeepMPC: Learning Deep Latent Features for Model Predictive Control},
  author={Ian Lenz and Ross Knepper and Ashutosh Saxena},
  year={2015},
  booktitle={RSS}
}



@article{DBLP:journals/corr/DonahueHGRVSD14,
  author    = {Jeff Donahue and
               Lisa Anne Hendricks and
               Sergio Guadarrama and
               Marcus Rohrbach and
               Subhashini Venugopalan and
               Kate Saenko and
               Trevor Darrell},
  title     = {Long-term Recurrent Convolutional Networks for Visual Recognition
               and Description},
  journal   = {CoRR},
  year      = {2014},
}



@INPROCEEDINGS{4408986, 
author={A. Rabinovich and A. Vedaldi and C. Galleguillos and E. Wiewiora and S. Belongie}, 
booktitle={2007 IEEE 11th International Conference on Computer Vision}, 
title={Objects in Context}, 
year={2007}, 
pages={1-8}, 
keywords={image representation;image segmentation;object recognition;optimisation;conditional random field;contextual relevance;image representation;image segmentation;object label agreement;object recognition;semantic object context;visual object categorization;Computer science;Computer vision;Context modeling;Electrical capacitance tomography;Image segmentation;Layout;Object recognition;Psychology;Statistics;Training data}, 
doi={10.1109/ICCV.2007.4408986}, 
ISSN={1550-5499}, 
month={Oct},}



@article{DBLP:journals/corr/VinyalsTBE14,
  author    = {Oriol Vinyals and
               Alexander Toshev and
               Samy Bengio and
               Dumitru Erhan},
  title     = {Show and Tell: {A} Neural Image Caption Generator},
  journal   = {CoRR},
  volume    = {abs/1411.4555},
  year      = {2014},
  url       = {http://arxiv.org/abs/1411.4555},
  timestamp = {Mon, 01 Dec 2014 14:32:13 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/VinyalsTBE14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{citeulike:11039228,
    abstract = {{Predictions of the near future can optimize the accuracy and speed of sensory processing as well as of behavioral responses. Previous experience and contextual cues are essential elements in the generation of a subjective prediction. Using a blocked fMRI paradigm, we investigated the pattern of neural activation in anticipation of a sensory stimulus and during the processing of the somatosensory stimulus itself. Tickling was chosen as the somatosensory stimulus rather than simple touch in order to increase the probability to get a high degree of anticipation. The location and nature of the stimulus were well defined to the subject. The state of anticipation was initiated by attributing an uncertainty regarding the time of stimulus onset. The network of activation and deactivation during anticipation of the expected stimulus was similar to that engaged during the actual sensory stimulation. The areas that were activated during both states included the contralateral primary sensory cortex, bilateral areas in the inferior parietal lobules, the putative area SII, the right anterior cingulate cortex and areas in the right prefrontal cortex. Similarly, common decreases were observed in areas of sensorimotor cortex located outside the area representing the target of stimulus, i.e., areas that process information which is irrelevant to the attended process. The overlapping pattern of change, during the somatosensory stimulation and the anticipation, furthers the idea that predictions are subserved by a neuronal network similar to that which subserves the processing of actual sensory input. Moreover, this study indicates that activation of primary somatosensory cortex can be obtained without intra-modal sensory input. These findings suggest that anticipation may invoke a tonic top-down regulation of neural activity}},
    author = {Carlsson, K. and Petrovic, P. and Skare, S. and Petersson, K. M. and Ingvar, M.},
    citeulike-article-id = {11039228},
    citeulike-linkout-0 = {\#},
    comment = {UI - 20396805 DA - 20000918},
    journal = {J.Cogn Neurosci.},
    keywords = {adult, anatomy, cinguli, cognition, comparative, conduction, cortex, cues, defense, female, gyrus, histology, human, imaging, lobe, magnetic, male, nerve, net, neural, parietal, perception, perceptual, physical, physiology, prefrontal, probability, resonance, rest, somatosensory, stimulation, study, supportnon-usgovt, touch},
    location = {Karolinska Institute/Karolinska Hospital, Sweden},
    month = jul,
    number = {0898-929X LA - eng PT - Clinical Trial PT - Journal Article},
    pages = {691--703},
    posted-at = {2012-08-10 15:13:09},
    priority = {2},
    title = {{Tickling expectations: neural processing in anticipation of a sensory stimulus}},
    url = {\#},
    volume = {12},
    year = {2000}
}


@article{citeulike:13324644,
    abstract = {{An essential aspect of episodic memory is the formation of associations between neutral sensory cues in the environment. In light of recent evidence that this critical aspect of learning does not require the hippocampus, we tested the involvement of the retrosplenial cortex (RSC) in this process using a chemogenetic approach that allowed us to temporarily silence neurons along the entire rostrocaudal extent of the RSC. A viral vector containing the gene for a synthetic inhibitory G-protein-coupled receptor (hM4Di) was infused into RSC. When the receptor was later activated by systemic injection of clozapine-N-oxide, neural activity in RSC was transiently silenced (confirmed using a patch-clamp procedure). Rats expressing hM4Di and control rats were trained in a sensory preconditioning procedure in which a tone and light were paired on some trials and a white noise stimulus was presented alone on the other trials during the Preconditioning phase. Thus, rats were given the opportunity to form an association between a tone and a light in the absence of reinforcement. Later, the light was paired with food. During the test phase when the auditory cues were presented alone, controls exhibited more conditioned responding during presentation of the tone compared with the white noise reflecting the prior formation of a tone-light association. Silencing RSC neurons during the Preconditioning phase prevented the formation of an association between the tone and light and eliminated the sensory preconditioning effect. These findings indicate that RSC may contribute to episodic memory formation by linking essential sensory stimuli during learning.}},
    author = {Robinson, Siobhan and Todd, Travis P. and Pasternak, Anna R. and Luikart, Bryan W. and Skelton, Patrick D. and Urban, Daniel J. and Bucci, David J.},
    citeulike-article-id = {13324644},
    citeulike-linkout-0 = {http://dx.doi.org/10.1523/jneurosci.1349-14.2014},
    citeulike-linkout-1 = {http://www.jneurosci.org/content/34/33/10982.abstract},
    citeulike-linkout-2 = {http://www.jneurosci.org/content/34/33/10982.full.pdf},
    day = {13},
    doi = {10.1523/jneurosci.1349-14.2014},
    issn = {1529-2401},
    journal = {The Journal of Neuroscience},
    keywords = {genetics},
    number = {33},
    pages = {10982--10988},
    posted-at = {2014-08-13 18:35:53},
    priority = {2},
    publisher = {Society for Neuroscience},
    title = {{Chemogenetic Silencing of Neurons in Retrosplenial Cortex Disrupts Sensory Preconditioning}},
    url = {http://dx.doi.org/10.1523/jneurosci.1349-14.2014},
    volume = {34},
    year = {2014}
}


@article{DBLP:journals/corr/abs-1301-3781,
  author    = {Tomas Mikolov and
               Kai Chen and
               Greg Corrado and
               Jeffrey Dean},
  title     = {Efficient Estimation of Word Representations in Vector Space},
  journal   = {CoRR},
  volume    = {abs/1301.3781},
  year      = {2013},
  url       = {http://arxiv.org/abs/1301.3781},
  timestamp = {Mon, 18 Feb 2013 20:50:59 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/abs-1301-3781},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{citeulike:778023,
       author = {Hinton, G. E. and Salakhutdinov, R. R.},
       journal = {Science},
    keywords = {algorithm, compexity, computation, data, neural\_networks},
    month = jul,
    number = {5786},
    pages = {504--507},
    pmid = {16873662},
    posted-at = {2008-02-27 22:55:12},
    priority = {2},
    publisher = {American Association for the Advancement of Science},
    title = {{Reducing the Dimensionality of Data with Neural Networks}},
    url = {http://dx.doi.org/10.1126/science.1127647},
    volume = {313},
    year = {2006}
}


@article{Vincent:2010:SDA:1756006.1953039,
 author = {Vincent, Pascal and Larochelle, Hugo and Lajoie, Isabelle and Bengio, Yoshua and Manzagol, Pierre-Antoine},
 title = {Stacked Denoising Autoencoders: Learning Useful Representations in a Deep Network with a Local Denoising Criterion},
 journal = {J. Mach. Learn. Res.},
 issue_date = {3/1/2010},
 volume = {11},
 year = {2010},
 issn = {1532-4435},
 pages = {3371--3408},
 numpages = {38},
 url = {http://dl.acm.org/citation.cfm?id=1756006.1953039},
 acmid = {1953039},
 publisher = {JMLR.org},
} 


@inproceedings{DBLP:journals/jmlr/Maaten09,
  author    = {Laurens van der Maaten},
  title     = {Learning a Parametric Embedding by Preserving Local Structure},
  booktitle = {AISTATS},
  year      = {2009}
}

@inproceedings{DBLP:conf/interspeech/MikolovKBCK10,
  author    = {Tomas Mikolov and
               Martin Karafi{\'{a}}t and
               Luk{\'{a}}s Burget and
               Jan Cernock{\'{y}} and
               Sanjeev Khudanpur},
  title     = {Recurrent neural network based language model},
  booktitle = {{INTERSPEECH} 2010, 11th Annual Conference of the International Speech
               Communication Association, Makuhari, Chiba, Japan, September 26-30,
               2010},
  pages     = {1045--1048},
  year      = {2010},
  crossref  = {DBLP:conf/interspeech/2010},
  url       = {http://www.isca-speech.org/archive/interspeech_2010/i10_1045.html},
  timestamp = {Thu, 09 Apr 2015 14:27:21 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/interspeech/MikolovKBCK10},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Brooks:1979:AMV:1624861.1624890,
 author = {Brooks, Rodney A. and Creiner, Russell and Binford, Thomas O.},
 title = {The ACRONYM Model-based Vision System},
 booktitle = {Proceedings of the 6th International Joint Conference on Artificial Intelligence - Volume 1},
 series = {IJCAI'79},
 year = {1979},
 isbn = {0-934613-47-8},
 location = {Tokyo, Japan},
 pages = {105--113},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=1624861.1624890},
 acmid = {1624890},
 publisher = {Morgan Kaufmann Publishers Inc.},
 address = {San Francisco, CA, USA},
} 




@inproceedings{DBLP:conf/slt/MikolovZ12,
  author    = {Tomas Mikolov and
               Geoffrey Zweig},
  title     = {Context dependent recurrent neural network language model},
  booktitle = {2012 {IEEE} Spoken Language Technology Workshop (SLT), Miami, FL,
               USA, December 2-5, 2012},
  pages     = {234--239},
  year      = {2012},
  crossref  = {DBLP:conf/slt/2012},
  url       = {http://dx.doi.org/10.1109/SLT.2012.6424228},
  doi       = {10.1109/SLT.2012.6424228},
  timestamp = {Tue, 12 Feb 2013 15:35:36 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/slt/MikolovZ12},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@MISC{Williams95gradient-basedlearning,
    author = {Ronald J. Williams and David Zipser},
    title = {Gradient-Based Learning Algorithms for Recurrent Networks and Their Computational Complexity},
    year = {1995}
}
@article{Bengio:2003:NPL:944919.944966,
 author = {Bengio, Yoshua and Ducharme, R{\'e}jean and Vincent, Pascal and Janvin, Christian},
 title = {A Neural Probabilistic Language Model},
 journal = {J. Mach. Learn. Res.},
 issue_date = {3/1/2003},
 volume = {3},
 year = {2003},
 issn = {1532-4435},
 pages = {1137--1155},
 numpages = {19},
 url = {http://dl.acm.org/citation.cfm?id=944919.944966},
 acmid = {944966},
 publisher = {JMLR.org},
} 

@inproceedings{Efros03, 
  title = {Recognizing Action at a Distance}, 
  author = {Alexei A. Efros and Alexander C. Berg and Greg Mori and
Jitendra Malik}, 
  booktitle = {ICCV}, 
  year = 2003 }
  
@inproceedings{DBLP:conf/interspeech/KombrinkMKB11,
  author    = {Stefan Kombrink and
               Tomas Mikolov and
               Martin Karafi{\'{a}}t and
               Luk{\'{a}}s Burget},
  title     = {Recurrent Neural Network Based Language Modeling in Meeting Recognition},
  booktitle = {INTERSPEECH},
  year      = {2011},
}

@ARTICLE{Brown92class-basedn-gram,
    author = {Peter F. Brown and Peter V. deSouza and Robert L. Mercer and Vincent J. Della Pietra and Jenifer C. Lai},
    title = {Class-Based n-gram Models of Natural Language},
    journal = {Computational Linguistics},
    year = {1992},
    volume = {18},
    pages = {467--479}
}

@InProceedings{ICML2011Sutskever_524,
  author =    {Ilya Sutskever and James Martens and Geoffrey Hinton},
  title =     {Generating Text with Recurrent Neural Networks },
  booktitle = {ICML},
  year =      {2011}
}
@article{Hochreiter:1997:LSM:1246443.1246450,
 author = {Hochreiter, Sepp and Schmidhuber, J\"{u}rgen},
 title = {Long Short-Term Memory},
 journal = {Neural Comput.},
 issue_date = {November 15, 1997},
 volume = {9},
 number = {8},
 year = {1997},
 issn = {0899-7667},
 pages = {1735--1780},
 numpages = {46},
 url = {http://dx.doi.org/10.1162/neco.1997.9.8.1735},
 doi = {10.1162/neco.1997.9.8.1735},
 acmid = {1246450},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 

@inproceedings{DBLP:conf/icml/GravesJ14,
  author    = {Alex Graves and
               Navdeep Jaitly},
  title     = {Towards End-To-End Speech Recognition with Recurrent Neural Networks},
  booktitle = {Proceedings of the 31th International Conference on Machine Learning,
               {ICML} 2014, Beijing, China, 21-26 June 2014},
  pages     = {1764--1772},
  year      = {2014},
  crossref  = {DBLP:conf/icml/2014},
  url       = {http://jmlr.org/proceedings/papers/v32/graves14.html},
  timestamp = {Fri, 07 Nov 2014 20:42:30 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icml/GravesJ14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/Graves13,
  author    = {Alex Graves},
  title     = {Generating Sequences With Recurrent Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1308.0850},
  year      = {2013},
  url       = {http://arxiv.org/abs/1308.0850},
  timestamp = {Tue, 10 Dec 2013 12:03:02 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/Graves13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@book{DBLP:series/sci/2012-385,
  author    = {Alex Graves},
  title     = {Supervised Sequence Labelling with Recurrent Neural Networks},
  series    = {Studies in Computational Intelligence},
  volume    = {385},
  publisher = {Springer},
  year      = {2012},
  url       = {http://dx.doi.org/10.1007/978-3-642-24797-2},
  doi       = {10.1007/978-3-642-24797-2},
  isbn      = {978-3-642-24796-5},
  timestamp = {Tue, 20 Mar 2012 09:00:13 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/series/sci/2012-385},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/CarreiraAFM15,
  author    = {Jo{\~{a}}o Carreira and
               Pulkit Agrawal and
               Katerina Fragkiadaki and
               Jitendra Malik},
  title     = {Human Pose Estimation with Iterative Error Feedback},
  journal   = {CoRR},
  volume    = {abs/1507.06550},
  year      = {2015},
  url       = {http://arxiv.org/abs/1507.06550},
  archivePrefix = {arXiv},
  eprint    = {1507.06550},
  timestamp = {Wed, 07 Jun 2017 14:42:58 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/CarreiraAFM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@misc{Authors14,
 author = {Authors},
 title = {The frobnicatable foo filter},
 note = {Face and Gesture  submission ID 324. Supplied as additional material {\tt fg324.pdf}},
 year = 2014
}


@inproceedings{bh-sm-00,
 author = {Brand, Matthew and Hertzmann, Aaron},
 title = {Style Machines},
 series = {SIGGRAPH},
 year = {2000}
}

@article{hpp-sthm-05,
 author = {Hsu, Eugene and Pulli, Kari and Popovi\'{c}, Jovan},
 title = {Style Translation for Human Motion},
 journal = {ACM Transactions on Graphics},
 issue_date = {July 2005},
 volume = {24},
 number = {3},
 month = jul,
 year = {2005},
 pages = {1082--1089},
 numpages = {8},
 publisher = {ACM Press},
 address = {New York, NY, USA},
}

@inproceedings{prm-lslmh-00,
author = "Pavlovic, Vladimir and James M. Rehg and John MacCormick",

booktitle = "Neural Information Processing Systems (NIPS)",

title = "Learning switching linear models of human motion",
year = "2000",
}


@inproceedings{Urtasun:2006:PTG:1153170.1153448,
 author = {Urtasun, Raquel and Fleet, David J. and Fua, Pascal},
 title = {3D People Tracking with Gaussian Process Dynamical Models},
 booktitle = {CVPR},
 year = {2006}
} 


@article{Fox:IEEESPM2010,
title={Bayesian Nonparametric Methods for Learning {M}arkov Switching Processes},
author={Fox, E.B. and Sudderth, E.B. and Jordan, M.I. and Willsky, A.S.},
journal={Signal Processing Magazine, IEEE},
volume={27},
number={6},
pages={43--54},
year={2010},
}


@article{wfh-gpdmh-08,
 author = {Wang, Jack M. and Fleet, David J. and Hertzmann, Aaron},
 title = {Gaussian Process Dynamical Models for Human Motion},
 journal = {TPAMI},
 volume = {30},
 year = {2008}
} 

@inproceedings{wfh-mgpms-07,
 author = {Wang, Jack M. and Fleet, David J. and Hertzmann, Aaron},
 title = {Multifactor Gaussian Process Models for Style-content Separation},
 booktitle = {ICML},
 year = {2007}
}

@inproceedings{ufgpd-tclvm-08,
  author    = {Raquel Urtasun and
               David J. Fleet and
               Andreas Geiger and
               Jovan Popovic and
               Trevor Darrell and
               Neil D. Lawrence},
  title     = {Topologically-constrained latent variable models},
  booktitle = {ICML},
  year      = {2008}
}

@inProceedings{vpsKpsTulsianiM14,
author    = {Shubham Tulsiani and Jitendra Malik},
title     = {Viewpoints and Keypoints},
year={2015},
booktitle={CVPR}
}

@inproceedings{thr-mhmub-06,
  author    = {Graham W. Taylor and
               Geoffrey E. Hinton and
               Sam T. Roweis},
  title     = {Modeling Human Motion Using Binary Latent Variables},
  booktitle = {NIPS},
  year      = {2006}
}

@inproceedings{th-fcrbm-09,
  author    = {Graham W. Taylor and
               Geoffrey E. Hinton},
  title     = {Factored conditional restricted Boltzmann Machines for modeling motion
               style},
  booktitle = {ICML},
  year      = {2009}
}


@article{h36m_pami,
author = {Ionescu, Catalin and Papava, Dragos and Olaru, Vlad and Sminchisescu,  Cristian},
title = {Human3.6M: Large Scale Datasets and Predictive Methods for 3D Human Sensing in Natural Environments},
journal = {TPAMI},
volume = {36},
number = {7},
year = {2014}
}


@inproceedings{sht-rtrbm-08,
  author    = {Ilya Sutskever and
               Geoffrey E. Hinton and
               Graham W. Taylor},
  title     = {The Recurrent Temporal Restricted Boltzmann Machine},
  booktitle = {NIPS},
  year      = {2008}
}


@misc{Authors14b,
 author = {Authors},
 title = {Frobnication tutorial},
 note = {Supplied as additional material {\tt tr.pdf}},
 year = 2014
}

@article{Alpher02,
author = {A. Alpher},
title = {Frobnication},
journal = {Journal of Foo},
volume = 12, 
number = 1, 
pages = {234--778}, 
year = 2002
}

@article{Alpher03,
author = {A. Alpher and  J.~P.~N. Fotheringham-Smythe},
title = {Frobnication revisited},
journal = {Journal of Foo},
volume = 13, 
number = 1, 
pages = {234--778}, 
year = 2003
}


@article{Sigal:2012:LPE:2205801.2205829,
 author = {Sigal, Leonid and Isard, Michael and Haussecker, Horst and Black, Michael J.},
 title = {Loose-limbed People: Estimating {3D} Human Pose and Motion Using Non-parametric Belief Propagation},
 journal = {IJCV},
 volume = {98},
 year = {2012}
}

@inproceedings{conf/cvpr/SappWT11,
  added-at = {2011-08-23T00:00:00.000+0200},
  author = {Sapp, Benjamin and Weiss, David and Taskar, Ben},
  booktitle = {CVPR},
  title = {Parsing human motion with stretchable models.},
  year = 2011
}

@inproceedings{Ramakrishna:2012:RHP:2404742.2404786,
 author = {Ramakrishna, Varun and Kanade, Takeo and Sheikh, Yaser},
 title = {Reconstructing 3D Human Pose from 2D Image Landmarks},
 booktitle = {ECCV},
 year = {2012}
} 


@inproceedings{MODEC,
  author    = {Ben Sapp and
               Ben Taskar},
  title     = {MODEC:Multimodal Decomposable Models for Human Pose Estimation},
  booktitle = {CVPR},
  year      = {2013}
}


@article{Alpher04,
author = {A. Alpher and J.~P.~N. Fotheringham-Smythe and G. Gamow},
title = {Can a machine frobnicate?},
journal = {Journal of Foo},
volume = 14, 
number = 1, 
pages = {234--778}, 
year = 2004
}


  @article{Wang94representingmoving,
      author = {Y. A. Wang and H. Adelson},
      title = {Representing Moving Images with Layers},
      journal = {TIP},
      year = {1994},
  }

@article{10.1109/CVPR.1997.609375,
  author = {Yair Weiss},
  title = {Smoothness in Layers: Motion segmentation using nonparametric mixture estimation.},
  journal ={CVPR},
  year={1997},

  }
  
  @article{DBLP:journals/corr/SimonyanVZ13,
  author    = {Karen Simonyan and
               Andrea Vedaldi and
               Andrew Zisserman},
  title     = {Deep Inside Convolutional Networks: Visualising Image Classification
               Models and Saliency Maps},
  journal   = {CoRR},
  volume    = {abs/1312.6034},
  year      = {2013},
  ee        = {http://arxiv.org/abs/1312.6034},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

  @article{DBLP:journals/corr/GirshickDDM13,
  author    = {Ross B. Girshick and
               Jeff Donahue and
               Trevor Darrell and
               Jitendra Malik},
  title     = {Rich feature hierarchies for accurate object detection and
               semantic segmentation},
  journal   = {CoRR},
  volume    = {abs/1311.2524},
  year      = {2013},
  ee        = {http://arxiv.org/abs/1311.2524},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}
  
    @incollection{NIPS2012_0534,
    Title = {ImageNet Classification with Deep Convolutional Neural Networks},
    Booktitle = {NIPS},
    Author = {Alex Krizhevsky and Ilya Sutskever and Geoffrey E. Hinton},
      Year = {2012},
   } 

   @inproceedings{Zuffi:ICCV:2013,
  title = {Estimating Human Pose with Flowing Puppets},
  author = {Zuffi, Silvia and Romero, Javier and Schmid, Cordelia and Black, Michael J},
  booktitle = {IEEE International Conference on Computer Vision (ICCV)},
  pages = {3312-3319},
  year = {2013}
}

  @inproceedings{DBLP:conf/eccv/VedaldiZ12,
  author    = {Andrea Vedaldi and
               Andrew Zisserman},
  title     = {Self-similar Sketch},
  booktitle = {ECCV (2)},
  year      = {2012},
  pages     = {87-100},
  ee        = {http://dx.doi.org/10.1007/978-3-642-33709-3_7},
  crossref  = {DBLP:conf/eccv/2012-2},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

  @inproceedings{RenMalik07,
	  author = "Xiaofeng Ren and Jitendra Malik",
	  title = "Tracking as Repeated Figure/Ground Segmentation",
	  booktitle = {CVPR},
	  year = "2007"
	  }

  @article{ncut,
  author = {Jianbo Shi and Jitendra Malik},
  title = {Normalized Cuts and Image Segmentation},
  journal = {TPAMI},
  year = {2000},
  }


  @article{10.1109/TPAMI.2005.202,
  author = {Jiangjian Xiao and Mubarak Shah},
  title = {Motion Layer Extraction in the Presence of Occlusion Using Graph Cuts},
  journal ={TPAMI},
  year = {2005},
  }

  @article{1340323,
  author = {Pawan Kumar, M. and Torr, P. H. and Zisserman, A.},
  title = {Learning Layered Motion Segmentations of Video},
  journal = {IJCV},
  volume = {76},
  year = {2008},
  }

  @article{10.1109/CVPR.1997.609375,
  author = {Yair Weiss},
  title = {Smoothness in Layers: Motion segmentation using nonparametric mixture estimation.},
  journal ={CVPR},
  year={1997},

  }
@inproceedings{DBLP:conf/eccv/FabletB02,
  author    = {Ronan Fablet and
               Michael J. Black},
  title     = {Automatic Detection and Tracking of Human Motion with a
               View-Based Representation},
  booktitle = {ECCV},
  year      = {2002}
}
@inproceedings{Shi_1994_3266,
   author = "Jianbo Shi and Carlo Tomasi",
   title = "Good Features to Track",
   booktitle = "CVPR",
   year = "1994",
}

@inproceedings{Rehg:1995:MTS:839277.840114,
 author = {Rehg, J. M. and Kanade, T.},
 title = {Model-based tracking of self-occluding articulated objects},
 booktitle = {ICCV},
 series = {ICCV},
 year = {1995},
}
@inproceedings{DBLP:conf/cvpr/FossatiDLF07,
  author    = {Andrea Fossati and
               Miodrag Dimitrijevic and
               Vincent Lepetit and
               Pascal Fua},
  title     = {Bridging the Gap between Detection and Tracking for 3D Monocular
               Video-Based Motion Capture},
  booktitle = {CVPR},
  year      = {2007},
  ee        = {http://dx.doi.org/10.1109/CVPR.2007.383297},
  crossref  = {DBLP:conf/cvpr/2007},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}
@inproceedings{DBLP:conf/eccv/SidenbladhBF00,
  author    = {Hedvig Sidenbladh and
               Michael J. Black and
               David J. Fleet},
  title     = {Stochastic Tracking of 3D Human Figures Using 2D Image Motion},
  booktitle = {ECCV},
  year      = {2000}
}



@inproceedings{HuayanWang:2011:MIR:2191740.2191905,
 author = {Huayan Wang and Koller, D.},
 title = {Multi-level inference by relaxed dual decomposition for human pose segmentation},
 booktitle = {CVPR},
 year = {2011}}



@INPROCEEDINGS{Johnson_combiningdiscriminative,
    author = {Sam Johnson and Mark Everingham},
    title = {Combining discriminative appearance and segmentation cues for articulated human pose estimation},
    booktitle = {MLVMA},
    year = {2009}
}


@INPROCEEDINGS{Sminchisescu05discriminativedensity,
    author = {Cristian Sminchisescu and Atul Kanaujia and Zhiguo Li and Dimitris Metaxas},
    title = {Discriminative Density Propagation for {3D} Human Motion Estimation},
    booktitle = {In CVPR},
    year = {2005}
}

@book{Gibson1979-GIBTEA,
	author = {James J. Gibson},
	publisher = {Houghton Mifflin},
	year = {1979},
	title = {The Ecological Approach to Visual Perception}
}

@INPROCEEDINGS{motionperception,
    author = {Gunnar Johansson},
    title = {Visual perception of biological motion and a model for its analysis},
    booktitle = {Percept. Psychophys.},
    year = {1973},
    volume={14},
    pages = {201--211}
}




@article{DBLP:journals/cacm/ShottonSKFFBCM13,
  author    = {Jamie Shotton and
               Toby Sharp and
               Alex Kipman and
               Andrew W. Fitzgibbon and
               Mark Finocchio and
               Andrew Blake and
               Mat Cook and
               Richard Moore},
  title     = {Real-time human pose recognition in parts from single depth
               images},
  journal   = {Commun. ACM},
  volume    = {56},
  number    = {1},
  year      = {2013},
  pages     = {116-124},
  ee        = {http://doi.acm.org/10.1145/2398356.2398381},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@article{10.1109/CVPR.2004.303,
author = {Jiang Gao and Robert T. Collins and Alexander G. Hauptmann and Howard D. Wactlar},
title = {Articulated Motion Modeling for Activity Analysis},
journal ={2012 IEEE Computer Society Conference on Computer Vision and Pattern Recognition Workshops},
volume = {1},
issn = {1063-6919},
year = {2004},
pages = {20},
doi = {http://doi.ieeecomputersociety.org/10.1109/CVPR.2004.303},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}


@INPROCEEDINGS{609381,
author={Black, M.J. and Yacoob, Y. and Jepson, A.D. and Fleet, D.J.},
booktitle={CVPR},
title={Learning parameterized models of image motion},
year={1997}}


@inproceedings{DBLP:conf/nips/WuBGBSSD02,
  author    = {Wei Wu and
               Michael J. Black and
               Yun Gao and
               Elie Bienenstock and
               Mijail Serruya and
               A. Shaikhouni and
               John P. Donoghue},
  title     = {Neural Decoding of Cursor Motion Using a Kalman Filter},
  booktitle = {NIPS},
  year      = {2002},
  pages     = {117-124},
  ee        = {http://books.nips.cc/papers/files/nips15/NS03.pdf},
  crossref  = {DBLP:conf/nips/2002},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


  @inproceedings{DBLP:conf/cvpr/AndrilukaRS08,
    author    = {Mykhaylo Andriluka and
		Stefan Roth and
		Bernt Schiele},
    title     = {People-tracking-by-detection and people-detection-by-tracking},
    booktitle = {CVPR},
    year      = {2008},
    ee        = {http://dx.doi.org/10.1109/CVPR.2008.4587583},
    crossref  = {DBLP:conf/cvpr/2008},
    bibsource = {DBLP, http://dblp.uni-trier.de}
  }
  @inproceedings{RenMalik07,
	  author = "Xiaofeng Ren and Jitendra Malik",
	  title = "Tracking as Repeated Figure/Ground Segmentation",
	  booktitle = {CVPR},
	  year = "2007"
	  }

  @article{ncut,
  author = {Jianbo Shi and Jitendra Malik},
  title = {Normalized Cuts and Image Segmentation},
  journal = {TPAMI},
  year = {2000},
  }
@inproceedings{DBLP:conf/cvpr/FragkiadakiZS12,
  author    = {Katerina Fragkiadaki and
               Geng Zhang and
               Jianbo Shi},
  title     = {Video segmentation by tracing discontinuities in a trajectory
               embedding},
  booktitle = {CVPR},
  year      = {2012}
}


  @article{10.1109/TPAMI.2005.202,
  author = {Jiangjian Xiao and Mubarak Shah},
  title = {Motion Layer Extraction in the Presence of Occlusion Using Graph Cuts},
  journal ={TPAMI},
  year = {2005},
  }

  @article{1340323,
  author = {Pawan Kumar, M. and Torr, P. H. and Zisserman, A.},
  title = {Learning Layered Motion Segmentations of Video},
  journal = {IJCV},
  volume = {76},
  year = {2008},
  }





  @InProceedings{Fradet09a,
    author = {Fradet, Matthieu and Robert, Philippe and P\'{e}rez, Patrick},
    Title = {Clustering point trajectories with various life-spans},
    BookTitle = {CVMP},
  year={2009}
  }





  @article{10.1109/ICCV.2001.10061,
  author = {Stella X. Yu and Jianbo Shi},
  title = {Segmentation with Pairwise Attraction and Repulsion},
  journal ={ICCV},
  Volume={75},
  year = {2001},
  }

  @article{1286005,
  author = {Wu, Bo and Nevatia, Ram},
  title = {Detection and Tracking of Multiple, Partially Occluded Humans by Bayesian Combination of Edgelet based Part Detectors},
  journal = {IJCV},
  year = {2007},
  }

  @inproceedings{bibbyeccv08,
    author = {C. Bibby and I. Reid},
    title = {Robust Real-Time Visual Tracking using Pixel-Wise Posteriors},
    booktitle={ECCV},
    year = "2008",
  }


  @InProceedings{BroxSegmentationCVPR11,
    author       = "Thomas Brox and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Object Segmentation by Alignment of Poselet Activations to Image Contours",
    booktitle    = "CVPR",
    year         = "2011"
  }

  @article{10.1109/ICCV.1995.466815,
  author = {J. Costeira and T. Kanade},
  title = {A multi-body factorization method for motion analysis},
  journal ={ICCV},
  year = {1995},
  }

  @inproceedings{Efros_2006_5395,
    author = "Bryan C. Russell and AlexeiA. Efros and Josef Sivic and William T. Freeman and Andrew Zisserman",
    title = "Using Multiple Segmentations to Discover Objects and their Extent in Image Collections",
    booktitle = "CVPR",
    year = "2006",
  }

  @inproceedings{malisiewicz-bmvc07,
    Author =	 {Tomasz Malisiewicz and Alexei A. Efros},
    Booktitle =	 {BMVC},
    Title =	 {Improving Spatial Support for Objects via Multiple Segmentations},
    Year =	 2007
  }

  @ARTICLE{1273918,
  author={Martin, D.R. and Fowlkes, C.C. and Malik, J.},
  journal={TPAMI},
  title={Learning to detect natural image boundaries using local brightness, color, and texture cues},
  year={2004},
  volume={26}
  }
@INPROCEEDINGS{Brox04highaccuracy,
    author = {Thomas Brox and Andrï¿œs Bruhn and Nils Papenberg and Joachim Weickert},
    title = {High Accuracy Optical Flow Estimation Based on a Theory for Warping},
    booktitle = {},
    year = {2004},
    pages = {25--36},
    publisher = {Springer}
}




  @INPROCEEDINGS{5539818,
  author={Bibby, C. and Reid, I.},
  booktitle={CVPR},
  title={Real-time tracking of multiple occluding objects using level sets},
  year={2010}}


  @inproceedings{Mitzel:2010:MTS:1886063.1886094,
  author = {Mitzel, Dennis and Horbert, Esther and Ess, Andreas and Leibe, Bastian},
  title = {Multi-person tracking with sparse detection and continuous segmentation},
  booktitle = {ECCV},
  year={2010}
  }

  @inproceedings{Mitzel:2011:MTS:1886063.1886094,
  author = {Mitzel, Dennis and Horbert, Esther and Ess, Andreas and Leibe, Bastian},
  title = {Level-Set Person Segmentation and Tracking with Multi-Region Appearemnce Models and Top-Down Shape Information},
  booktitle = {ICCV},
  series = {2011}
  }


  @InProceedings{lezama11,
    author = {Lezama, J. and Alahari, K. and Sivic, J. and Laptev, I.},
    title = {Track to the Future: Spatio-temporal Video Segmentation with Long-range Motion Cues},
    booktitle = {CVPR},
    year = {2011}
  }
  @InProceedings{shuwang2,
    author = {Shu Wang and Huchuan Lu and Fan Yang and Ming-Hsuan Yang},
    title = {Superpixel Tracking},
    booktitle = {ICCV},
    year = {2011}
  }
  @InProceedings{OB11,
    author       = "P. Ochs and T. Brox",
    title        = "Object segmentation in video: a hierarchical variational approach for turning point trajectories into dense regions",
    booktitle    = "ICCV",
    year         = "2011"}
  @incollection {springerlink:10.1007/978-3-642-15555-0_27,
    author = {Rahtu, Esa and Kannala, Juho and Salo, Mikko and Heikkilï¿œ, Janne},
    affiliation = {Machine Vision Group, University of Oulu, Finland},
    title = {Segmenting Salient Objects from Images and Videos},
    booktitle = {ECCV},
    year={2010},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }

  @Article{19146246,
  TITLE = {On the plausibility of the discriminant center-surround hypothesis for visual saliency.},
  AUTHOR = {Gao, Dashan and Mahadevan, Vijay and Vasconcelos, Nuno},
  journal = {Journal of vision},
  volume = {8},
  year = {2008}
  }


  @Article{Mahadevan10spatiotemporalsaliency,
      author = {Vijay Mahadevan and Nuno Vasconcelos},
      title = {Spatiotemporal Saliency in Dynamic Scenes},
      journal = {TPAMI},
      volume = {32},
      year = {2010},
  }


  @InProceedings{background_subtraction_free_camera,
    author = {Yaser Sheikh, Omar Javed, and Takeo Kanade},
    title = {Background Subtraction for Freely Moving Cameras},
    booktitle = {ICCV},
    year = {2009},
  }
  @conference{vondrick2010,
    title={Efficiently Scaling Up Video Annotation with Crowdsourced Marketplaces},
    author={Carl Vondrick and Deva Ramanan and Donald Patterson},
    booktitle={ECCV},
    year = {2010},
  }

  @conference{StellaRepulsion,
      author = {Stella X. Yu and Jianbo Shi},
      title = {Understanding Popout through Repulsion},
      booktitle= {CVPR},
      year={2001},
  }

  @article{10.1109/TPAMI.2009.167,
  author = {Pedro F. Felzenszwalb and Ross B. Girshick and David McAllester and Deva Ramanan},
  title = {Object Detection with Discriminatively Trained Part-Based Models},
  journal ={TPAMI},
    year = {2010},
  volume={32},
  }

  @INPROCEEDINGS{Avidan05ensembletracking,
      author = {Shai Avidan},
      title = {Ensemble Tracking},
      booktitle = {CVPR},
      year = {2005},
  }

  @INPROCEEDINGS{planningtracking,
      author = {Haifeng Gong and Jack Simy and Maxim Likhachev and Jianbo Shi},
      title = {Multi-hypothesis Motion Planning for Visual Object Tracking},
      booktitle = {ICCV},
      year = {2011},
  }

  @incollection {SLIC,
    title={SLIC Superpixels},
    author={Radhakrishna Achanta and Appu Shaji and Kevin Smith and Aurelien Lucchi and Pascal Fua and Sabine Susstrunk},
    booktitle={EPFL Technical Report no. 149300, June 2010},
  }


@inproceedings{DBLP:conf/cvpr/UrtasunD08,
  author    = {Raquel Urtasun and
               Trevor Darrell},
  title     = {Sparse probabilistic regression for activity-independent
               human pose inference},
  booktitle = {CVPR},
  year      = {2008},
  ee        = {http://dx.doi.org/10.1109/CVPR.2008.4587360},
  crossref  = {DBLP:conf/cvpr/2008},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{DBLP:journals/pami/XuJM12,
  author    = {Li Xu and
               Jiaya Jia and
               Yasuyuki Matsushita},
  title     = {Motion Detail Preserving Optical Flow Estimation},
  journal   = {TPAMI},
  volume    = {34},
  year      = {2012},
}

  @incollection {springerlink:10.1007/978-3-540-88688-4_58,
    author = {Huang, Chang and Wu, Bo and Nevatia, Ramakant},
    title = {Robust Object Tracking by Hierarchical Association of Detection Responses},
    booktitle = {ECCV},
    year={2008},
  }
  
  @article{DBLP:journals/corr/RenHG015,
  author    = {Shaoqing Ren and
               Kaiming He and
               Ross B. Girshick and
               Jian Sun},
  title     = {Faster {R-CNN:} Towards Real-Time Object Detection with Region Proposal
               Networks},
  journal   = {CoRR},
  volume    = {abs/1506.01497},
  year      = {2015},
  url       = {http://arxiv.org/abs/1506.01497},
  timestamp = {Wed, 07 Jun 2017 14:42:40 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RenHG015},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @inproceedings{DBLP:conf/cvpr/CechS07,
    author    = {Jan Cech and Radim S{\'a}ra},
    title     = {Efficient Sampling of Disparity Space for Fast And Accurate Matching},
    booktitle = {CVPR},
    year      = {2007}
  }
  @inproceedings{DBLP:conf/iccv/PellegriniESG09,
    author    = {Stefano Pellegrini and
		Andreas Ess and
		Konrad Schindler and
		Luc J. Van Gool},
    title     = {You'll never walk alone: Modeling social behavior for multi-target
		tracking},
    booktitle = {ICCV},
    year      = {2009}
  }


  @InProceedings{eth_biwi_00483,
    author = {B. Leibe and N. Cornelis and K. Cornelis and L. Van Gool},
    title = {Dynamic 3D Scene Analysis from a Moving Vehicle},
    booktitle = {CVPR},
    year = {2007},
  }

  @article{10.1109/TPAMI.2010.143,
  author = {Thomas Brox and Jitendra Malik},
  title = {Large Displacement Optical Flow: Descriptor Matching in Variational Motion Estimation},
  journal ={TPAMI},
  year = {2010},
  }
  
  
  @article{DBLP:journals/corr/HeZRS15,
  author    = {Kaiming He and
               Xiangyu Zhang and
               Shaoqing Ren and
               Jian Sun},
  title     = {Deep Residual Learning for Image Recognition},
  journal   = {CoRR},
  volume    = {abs/1512.03385},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.03385},
  timestamp = {Wed, 07 Jun 2017 14:41:17 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/HeZRS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/SrivastavaLM17,
  author    = {Shashank Srivastava and
               Igor Labutov and
               Tom M. Mitchell},
  title     = {Joint Concept Learning and Semantic Parsing from Natural Language
               Explanations},
  booktitle = {Proceedings of the 2017 Conference on Empirical Methods in Natural
               Language Processing, {EMNLP} 2017, Copenhagen, Denmark, September
               9-11, 2017},
  pages     = {1528--1537},
  year      = {2017},
  crossref  = {DBLP:conf/emnlp/2017},
  url       = {http://aclanthology.info/papers/D17-1161/d17-1161},
  timestamp = {Fri, 15 Sep 2017 17:29:54 +0200},
  biburl    = {http://dblp.org/rec/bib/conf/emnlp/SrivastavaLM17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@Article{dm-elav-86, 
author = "Gerald Dejong and Raymond Mooney", 
year = "1986", 
title = "Explanation-Based Learning: An Alternative View", 
journal = "Machine Learning", 
volume = "1", 
pages = "145--176", 
publisher = "Kluwer", 
} 
Hide BibTex Record


@inproceedings{Perazzi2016,
  author = {F. Perazzi and J. Pont-Tuset and B. McWilliams and L. {Van Gool} and M. Gross and A. Sorkine-Hornung},
  title = {A Benchmark Dataset and Evaluation Methodology for Video Object Segmentation},
  booktitle = {Computer Vision and Pattern Recognition},
  year = {2016}
}
  
  @article{DBLP:journals/corr/HeGDG17,
  author    = {Kaiming He and
               Georgia Gkioxari and
               Piotr Doll{\'{a}}r and
               Ross B. Girshick},
  title     = {Mask {R-CNN}},
  journal   = {CoRR},
  volume    = {abs/1703.06870},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.06870},
  timestamp = {Wed, 07 Jun 2017 14:42:32 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/HeGDG17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @inproceedings{citeulike:9244127,
      author = {Li, Yuan and Huang, Chang and Nevatia, R.},
    booktitle = {CVPR},
      title = {Learning to associate: HybridBoosted multi-target tracker for crowded scene},
      year = {2009}
  }


@article{Hofsten19971799,
title = "Development of smooth pursuit tracking in young infants ",
journal = "Vision Research ",
volume = "37",
number = "13",
pages = "1799 - 1810",
year = "1997",
note = "",
issn = "0042-6989",
doi = "http://dx.doi.org/10.1016/S0042-6989(96)00332-X",
url = "http://www.sciencedirect.com/science/article/pii/S004269899600332X",
author = "Claes Von Hofsten and Kerstin Rosander",
keywords = "Eye movements",
keywords = "Infants",
keywords = "Smooth pursuit",
keywords = "Saccades",
keywords = "Head movements "
}


  @article {springerlink:10.1007/s11263-008-0136-6,
  title = {Particle Video: Long-Range Motion Estimation Using Point Trajectories},
    author = {Sand, Peter and Teller, Seth},
    affiliation = {MIT Computer Science and Artificial Intelligence Laboratory Cambridge MA 02139 USA},
    journal = {IJCV},
    year = {2008}
  }
  @INPROCEEDINGS{Dalal05histogramsof,
      author = {Navneet Dalal and Bill Triggs},
      title = {Histograms of Oriented Gradients for Human Detection},
      booktitle = {CVPR},
      year = {2005}
  }

  @InProceedings{yma,
    author = { Rao, S. and Tron, R. and Vidal, R. and Ma, Y. },
    title = {Motion segmentation via robust subspace separation in the presence of outlying, incomplete, or corrupted trajectories.},
    booktitle = {CVPR},
    year={2008},
  }

  @inproceedings{Grabner:2008:SOB:1478392.1478414,
  author = {Grabner, Helmut and Leistner, Christian and Bischof, Horst},
  title = {Semi-supervised On-Line Boosting for Robust Tracking},
  booktitle = {ECCV},
  year = {2008},
  }


  @inproceedings{citeulike:2085974,
      author = {Grabner , H. and Bischof, H.},
    title = {Online Boosting and Vision},
      booktitle = {CVPR},
      year = {2006}
  }

  @INPROCEEDINGS{5573752,
  author={Zhang Tao and Fei Shumin and Hu Gang},
  booktitle={Control Conference (CCC)},
  title={Target tracking with particle filter based on multiple cues fusion},
  year={2010}}

  @INPROCEEDINGS{Okuma04aboosted,
      author = {Kenji Okuma and Ali Taleghani and Nando De Freitas and O De Freitas and James J. Little and David G. Lowe},
      title = {A Boosted Particle Filter: Multitarget Detection and Tracking},
      booktitle = {ECCV},
      year = {2004},
  }


  @InProceedings{sparsesubsp,
    author = {Elhamifar, E. and Vidal, R.},
    title = {Sparse subspace clustering},
    booktitle = {CVPR},
    year = {2009}
  }




  @INPROCEEDINGS{BrostowCipollaCVPR2006,
    AUTHOR       = {Gabriel J. Brostow and Roberto Cipolla},
    TITLE        = {Unsupervised Bayesian Detection of Independent Motion in Crowds},
    BOOKTITLE    = {CVPR},
    YEAR         = {2006},
  }
  @article{GrundmannKwatra2010,
    author = {Matthias Grundmann and Vivek Kwatra and Mei Han and Irfan Essa},
    title = {Efficient Hierarchical Graph Based Video Segmentation},
    journal = {CVPR},
    year = {2010},
  }



  @incollection {mhvs,
    author = {Amelio Vazquez-Reina and Shai Avidan and Hanspeter Pfister and Eric Miller},
    title = {Multiple Hypothesis Video Segmentation from Superpixel Flows},
    booktitle = {ECCV},
  year={2010},
  }



  @article{phycho,
    author = {H. C. Nothdurft},
    title = {Feature analysis and the role of similarity in preattentive vision},
    journal = {Perception and Psychophysics},
    volume={52},
    year = {1992},
  }




  @INPROCEEDINGS{5206727,
  author={Chunhui Gu and Lim, J.J. and Arbelaez, P. and Malik, J.},
  booktitle={CVPR},
  year={2009},
  title={Recognition using regions},
  }
  @InProceedings{citeulike:942103,
      title = {Bottom-up/top-down image parsing by attribute graph grammar},
      author = {Han, Feng and Zhu, Song-Chun},
      journal = {ICCV},
  year={ 2005},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {CVPR},
  year={2009},
  }
@InProceedings{eth_biwi_00555,
  author = {S. Gammeter and A. Ess and T. Jaeggli and K. Schindler and B. Leibe and and L. van Gool},
  title = {Articulated Multibody Tracking Under Egomotion},
  booktitle = {ECCV},
  year = {2008}
}


@INPROCEEDINGS{unified,
author={Xiangyang Lan and Huttenlocher, D.P.},
booktitle={CVPR},
title={A unified spatio-temporal articulated model for tracking},
year={2004},
volume={1}}


  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }

  @InProceedings{Yan06general,
    title     = {A General Framework for Motion Segmentation: Independent, Articulated, Rigid, Non-rigid, Degenerate and Non-degenerate.},
    author = {J. Yan and M. Pollefeys},
    booktitle = {ECCV},
  year={ 2006},
  }

  @InProceedings{Ayer,
    title     = {Layered representation of motion video using robust maximum-likelihood estimation of mixture models and MDL encoding},
    author = {S. Ayer and H. S. Sawhney},
    booktitle = {ICCV},
  year={ 1995},
  }

  @article{10.1109/CVPR.2005.335,
  author = {Deva Ramanan and D. A. Forsyth and Andrew Zisserman},
  title = {Strike a Pose: Tracking People by Finding Stylized Poses},
  journal ={CVPR},
  year = {2005},
  }
  
  @article{citeulike:13375196,
    author = {Tompson, Jonathan and Stein, Murphy and Lecun, Yann and Perlin, Ken},
    journal = {ACM Trans. Graph.},
    title = {{Real-Time Continuous Pose Recovery of Human Hands Using Convolutional Networks}},
    year = {2014}
}



  @inproceedings{DBLP:conf/nips/TompsonJLB14,
  author    = {Jonathan J. Tompson and
               Arjun Jain and
               Yann LeCun and
               Christoph Bregler},
  title     = {Joint Training of a Convolutional Network and a Graphical Model for
               Human Pose Estimation},
  booktitle = {NIPS},
  year      = {2014}
  }
  
  @inproceedings{Sapp:2010:CMA:1888028.1888060,
 author = {Sapp, Benjamin and Toshev, Alexander and Taskar, Ben},
 title = {Cascaded Models for Articulated Pose Estimation},
 booktitle = {Proceedings of the 11th European Conference on Computer Vision: Part II},
 series = {ECCV'10},
 year = {2010},
 isbn = {3-642-15551-0, 978-3-642-15551-2},
 location = {Heraklion, Crete, Greece},
 pages = {406--420},
 numpages = {15},
 url = {http://dl.acm.org/citation.cfm?id=1888028.1888060},
 acmid = {1888060},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 
  
  
  
@article{DBLP:journals/corr/ToshevS13,
  author    = {Alexander Toshev and
               Christian Szegedy},
  title     = {DeepPose: Human Pose Estimation via Deep Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1312.4659},
  year      = {2013},
  ee        = {http://arxiv.org/abs/1312.4659},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}



  @inproceedings{DBLP:conf/eccv/SappTT10,
  author    = {Benjamin Sapp and
               Alexander Toshev and
               Ben Taskar},
  title     = {Cascaded Models for Articulated Pose Estimation},
  booktitle = {ECCV (2)},
  year      = {2010},
  pages     = {406-420},
  ee        = {http://dx.doi.org/10.1007/978-3-642-15552-9_30},
  crossref  = {DBLP:conf/eccv/2010-2},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{10.1109/TPAMI.2008.35,
author = {Mun Wai Lee and Ramakant Nevatia},
title = {Human Pose Tracking in Monocular Sequence Using Multilevel Structured Models},
journal ={IEEE Transactions on Pattern Analysis and Machine Intelligence},
volume = {31},
number = {1},
issn = {0162-8828},
year = {2009},
pages = {27-38},
doi = {http://doi.ieeecomputersociety.org/10.1109/TPAMI.2008.35},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
}

  @inproceedings{DBLP:conf/iccv/CheriyadatR09,
    author    = {Anil Cheriyadat and
		Richard J. Radke},
    title     = {Non-negative matrix factorization of partial track data
		for motion segmentation},
    booktitle = {ICCV},
    year      = {2009}
  }

@inproceedings{Kuo:2015:DLO:2919332.2919793,
 author = {Kuo, Weicheng and Hariharan, Bharath and Malik, Jitendra},
 title = {DeepBox: Learning Objectness with Convolutional Networks},
 booktitle = {Proceedings of the 2015 IEEE International Conference on Computer Vision (ICCV)},
 series = {ICCV '15},
 year = {2015},
 isbn = {978-1-4673-8391-2},
 pages = {2479--2487},
 numpages = {9},
 url = {http://dx.doi.org/10.1109/ICCV.2015.285},
 doi = {10.1109/ICCV.2015.285},
 acmid = {2919793},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
} 



@Inbook{Xiang2016,
author="Xiang, Yu
and Kim, Wonhui
and Chen, Wei
and Ji, Jingwei
and Choy, Christopher
and Su, Hao
and Mottaghi, Roozbeh
and Guibas, Leonidas
and Savarese, Silvio",
editor="Leibe, Bastian
and Matas, Jiri
and Sebe, Nicu
and Welling, Max",
title="ObjectNet3D: A Large Scale Database for 3D Object Recognition",
bookTitle="Computer Vision -- ECCV 2016: 14th European Conference, Amsterdam, The Netherlands, October 11-14, 2016, Proceedings, Part VIII",
year="2016",
publisher="Springer International Publishing",
address="Cham",
pages="160--176",
abstract="We contribute a large scale database for 3D object recognition, named ObjectNet3D, that consists of 100 categories, 90,127 images, 201,888 objects in these images and 44,147 3D shapes. Objects in the 2D images in our database are aligned with the 3D shapes, and the alignment provides both accurate 3D pose annotation and the closest 3D shape annotation for each 2D object. Consequently, our database is useful for recognizing the 3D pose and 3D shape of objects from 2D images. We also provide baseline experiments on four tasks: region proposal generation, 2D object detection, joint 2D detection and 3D object pose estimation, and image-based 3D shape retrieval, which can serve as baselines for future research using our database. Our database is available online at                     http://cvgl.stanford.edu/projects/objectnet3d                                      .",
isbn="978-3-319-46484-8",
doi="10.1007/978-3-319-46484-8_10",
url="https://doi.org/10.1007/978-3-319-46484-8_10"
}

@Inbook{Kuettel2012,
author="Kuettel, Daniel
and Guillaumin, Matthieu
and Ferrari, Vittorio",
editor="Fitzgibbon, Andrew
and Lazebnik, Svetlana
and Perona, Pietro
and Sato, Yoichi
and Schmid, Cordelia",
title="Segmentation Propagation in ImageNet",
bookTitle="Computer Vision -- ECCV 2012: 12th European Conference on Computer Vision, Florence, Italy, October 7-13, 2012, Proceedings, Part VII",
year="2012",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="459--473",
abstract="ImageNet is a large-scale hierarchical database of object classes. We propose to automatically populate it with pixelwise segmentations, by leveraging existing manual annotations in the form of class labels and bounding-boxes. The key idea is to recursively exploit images segmented so far to guide the segmentation of new images. At each stage this propagation process expands into the images which are easiest to segment at that point in time, e.g. by moving to the semantically most related classes to those segmented so far. The propagation of segmentation occurs both (a) at the image level, by transferring existing segmentations to estimate the probability of a pixel to be foreground, and (b) at the class level, by jointly segmenting images of the same class and by importing the appearance models of classes that are already segmented. Through an experiment on 577 classes and 500k images we show that our technique (i) annotates a wide range of classes with accurate segmentations; (ii) effectively exploits the hierarchical structure of ImageNet; (iii) scales efficiently; (iv) outperforms a baseline GrabCut [1] initialized on the image center, as well as our recent segmentation transfer technique [2] on which this paper is based. Moreover, our method also delivers state-of-the-art results on the recent iCoseg dataset for co-segmentation.",
isbn="978-3-642-33786-4",
doi="10.1007/978-3-642-33786-4_34",
url="https://doi.org/10.1007/978-3-642-33786-4_34"
}


@article{DBLP:journals/corr/SukhbaatarSWF15,
  author    = {Sainbayar Sukhbaatar and
               Arthur Szlam and
               Jason Weston and
               Rob Fergus},
  title     = {Weakly Supervised Memory Networks},
  journal   = {CoRR},
  volume    = {abs/1503.08895},
  year      = {2015},
  url       = {http://arxiv.org/abs/1503.08895},
  archivePrefix = {arXiv},
  eprint    = {1503.08895},
  timestamp = {Wed, 07 Jun 2017 14:40:08 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/SukhbaatarSWF15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/AndorAWSPGPC16,
  author    = {Daniel Andor and
               Chris Alberti and
               David Weiss and
               Aliaksei Severyn and
               Alessandro Presta and
               Kuzman Ganchev and
               Slav Petrov and
               Michael Collins},
  title     = {Globally Normalized Transition-Based Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1603.06042},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.06042},
  archivePrefix = {arXiv},
  eprint    = {1603.06042},
  timestamp = {Wed, 07 Jun 2017 14:42:37 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/AndorAWSPGPC16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/SwayamdiptaBDS16,
  author    = {Swabha Swayamdipta and
               Miguel Ballesteros and
               Chris Dyer and
               Noah A. Smith},
  title     = {Greedy, Joint Syntactic-Semantic Parsing with Stack LSTMs},
  journal   = {CoRR},
  volume    = {abs/1606.08954},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.08954},
  archivePrefix = {arXiv},
  eprint    = {1606.08954},
  timestamp = {Wed, 07 Jun 2017 14:40:31 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/SwayamdiptaBDS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{DBLP:journals/corr/TaiSM15,
  author    = {Kai Sheng Tai and
               Richard Socher and
               Christopher D. Manning},
  title     = {Improved Semantic Representations From Tree-Structured Long Short-Term
               Memory Networks},
  journal   = {CoRR},
  volume    = {abs/1503.00075},
  year      = {2015},
  url       = {http://arxiv.org/abs/1503.00075},
  archivePrefix = {arXiv},
  eprint    = {1503.00075},
  timestamp = {Wed, 07 Jun 2017 14:43:13 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/TaiSM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Krishnamurthy2014JointSA,
  title={Joint Syntactic and Semantic Parsing with Combinatory Categorial Grammar},
  author={Jayant Krishnamurthy and Tom M. Mitchell},
  booktitle={ACL},
  year={2014}
}

@inproceedings{AAA,
author = {Socher, Richard and Bauer, John and Manning, Christoper and Andrew Y., Ng},
year = {2013},
month = {08},
pages = {455-465},
title = {Parsing with Compositional Vector Grammars},
volume = {1},
booktitle = {ACL 2013 - 51st Annual Meeting of the Association for Computational Linguistics, Proceedings of the Conference}
}



@article{Bahdanau2014NeuralMT,
  title={Neural Machine Translation by Jointly Learning to Align and Translate},
  author={Dzmitry Bahdanau and Kyunghyun Cho and Yoshua Bengio},
  journal={CoRR},
  year={2014},
  volume={abs/1409.0473}
}


@article{DBLP:journals/corr/DosovitskiyK16,
  author    = {Alexey Dosovitskiy and
               Vladlen Koltun},
  title     = {Learning to Act by Predicting the Future},
  journal   = {CoRR},
  volume    = {abs/1611.01779},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.01779},
  archivePrefix = {arXiv},
  eprint    = {1611.01779},
  timestamp = {Wed, 07 Jun 2017 14:43:00 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/DosovitskiyK16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/LevinePKQ16,
  author    = {Sergey Levine and
               Peter Pastor and
               Alex Krizhevsky and
               Deirdre Quillen},
  title     = {Learning Hand-Eye Coordination for Robotic Grasping with Deep Learning
               and Large-Scale Data Collection},
  journal   = {CoRR},
  volume    = {abs/1603.02199},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.02199},
  archivePrefix = {arXiv},
  eprint    = {1603.02199},
  timestamp = {Wed, 07 Jun 2017 14:41:34 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LevinePKQ16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@INPROCEEDINGS{1544874, 
author={E. B. Sudderth and A. Torralba and W. T. Freeman and A. S. Willsky}, 
booktitle={Tenth IEEE International Conference on Computer Vision (ICCV'05) Volume 1}, 
title={Learning hierarchical models of scenes, objects, and parts}, 
year={2005}, 
volume={2}, 
pages={1331-1338 Vol. 2}, 
keywords={feature extraction;natural scenes;object detection;object recognition;feature detection;hierarchical probabilistic model;image database;low-level interest operator;natural scenes;object centered coordinate frame;object detection;object recognition;Computer science;Computer vision;Dictionaries;Graphical models;Image databases;Layout;Object detection;Random variables;Spatial databases;Visual databases}, 
doi={10.1109/ICCV.2005.137}, 
ISSN={1550-5499}, 
month={Oct},}



@INPROCEEDINGS{Carlson10towardan,
    author = {Andrew Carlson and Justin Betteridge and Bryan Kisiel and Burr Settles and Estevam R. Hruschka and Tom M. Mitchell},
    title = {Toward an architecture for never-ending language learning},
    booktitle = {In AAAI},
    year = {2010}
}


@INPROCEEDINGS{6751285, 
author={X. Chen and A. Shrivastava and A. Gupta}, 
booktitle={2013 IEEE International Conference on Computer Vision}, 
title={NEIL: Extracting Visual Knowledge from Web Data}, 
year={2013}, 
pages={1409-1416}, 
keywords={Internet;knowledge acquisition;NEIL;Web data;common sense relationships;never ending image learner;semi-supervised learning algorithm;visual knowledge extraction;Computers;Data mining;Detectors;Knowledge based systems;Semantics;Semisupervised learning;Visualization;attributes;common sense relationships;macro vision;never ending learning;object detection;scene classification;semi-supervised learning;visual knowledge base}, 
doi={10.1109/ICCV.2013.178}, 
ISSN={1550-5499}, 
month={Dec},}



  @Article{ Perse2009612,
  title = "A trajectory-based analysis of coordinated team activity in a basketball game",
  journal = "Computer Vision and Image Understanding",
  volume = "113",
  year = "2009",
  }

  @inproceedings{morariu11eventstructure,
    author    = {Vlad I. Morariu and Larry S. Davis},
    title     = {Multi-agent event recognition in structured scenarios.},
    booktitle = {CVPR},
    year      = {2011}
  }

@article{DBLP:journals/corr/KingS16,
  author    = {Jennifer E. King and
               Siddhartha S. Srinivasa},
  title     = {Rearrangement Planning via Heuristic Search},
  journal   = {CoRR},
  volume    = {abs/1603.08642},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.08642},
  archivePrefix = {arXiv},
  eprint    = {1603.08642},
  timestamp = {Wed, 07 Jun 2017 14:40:58 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/KingS16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

  @inproceedings{storyline,
    author    = {Abhinav Gupta and Praveen Srinivasan and Jianbo Shi and Larry S. Davis},
    title     = {Understanding videos, constructing plots learning a visually grounded storyline model from annotated videos},
    booktitle = {CVPR},
    year      = {2009}
  }

  @inproceedings{benfold2011stable,
	  author = {Benfold, Ben and Reid, Ian},
	  title = {Stable Multi-Target Tracking in Real-Time Surveillance Video},
	  booktitle = {CVPR},
	  year = {2011}
  }


  @ARTICLE{790429,
  author={Wilson, A.D. and Bobick, A.F.},
  journal={TPAMI},
  title={Parametric hidden Markov models for gesture recognition},
  year={1999},
  volume={21}
  }



  @article{experts,
  author = {Terence D. Sanger and Robert A. Jacobs and Steven J. Nowlan and Geoffrey E. Hinton},
  title = {Adaptive Mixtures of Local Experts},
  journal = {Neural Computation},
  volume = {3},
  year = {1991}
  }


  @INPROCEEDINGS{lips,
  author={Bregler, C. and Omohundro, S.M.},
  booktitle={ICCV},
  title={Nonlinear manifold learning for visual speech recognition},
  year={1995}
  }



  @inproceedings{BN,
  author = {Shaogang Gong and Tao Xiang},
  title = {Recognition of Group Activities using Dynamic Probabilistic Networks},
  booktitle = {ICCV},
  year={2003}
  }


  @article{HMMMO,
  author = {Aaron F. Bobick and Andrew D. Wilson},
  title = {A State-Based Approach to the Representation and Recognition of Gesture},
  journal = {TPAMI},
  volume = {19}
  }

  @inproceedings{Brand:1997:CHM:794189.794420,
  author = {Brand, M. and Oliver, N. and Pentland, A.},
  title = {Coupled hidden Markov models for complex action recognition},
  booktitle = {CVPR},
  year = {1997}
  }

  @article{Ghahramani:1997:FHM:274158.274165,
  author = {Ghahramani, Zoubin and Jordan, Michael I.},
  title = {Factorial Hidden Markov Models},
  journal = {Mach. Learn.},
  volume = {29},
  year = {1997}
  }


  @INPROCEEDINGS{4270099,
  author={Laxton, B. and Jongwoo Lim and Kriegman, D.},
  booktitle={CVPR},
  title={Leveraging temporal, contextual and ordering constraints for recognizing complex activities in video},
  year={2007}
  }


  @article{DBLP:journals/jmlr/SiracusaF09,
    author    = {Michael Siracusa and John Fisher},
    title     = {Tractable Bayesian Inference of Time-Series Dependence Structure},
    journal   = {Journal of Machine Learning Research - Proceedings Track},
    volume    = {5},
    year      = {2009}
  }



  @article{parametrized,
  author = {Yaser Yacoob and Michael J. Black},
  title = {Parameterized Modeling and Recognition of Activities},
  journal = {Computer Vision and Image Understanding},
  volume = {73},
  year = {1999}
  }




  @inproceedings{Bobick:1995:STS:839277.840051,
  author = {Bobick, A. F. and Wilson, A. D.},
  title = {A state-based technique for the summarization and recognition of gesture},
  booktitle = {ICCV},
  year = {1995}
  }


  @inproceedings{Niebles:2010:MTS:1888028.1888059,
  author = {Niebles, Juan Carlos and Chen, Chih-Wei and Fei-Fei, Li},
  title = {Modeling temporal structure of decomposable motion segments for activity classification},
  booktitle = {ECCV},
  year = {2010}
  }



  @inproceedings{NCA,
  author = {Jacob Goldberger and Sam T. Roweis and Geoffrey E. Hinton and Ruslan Salakhutdinov},
  title = {Neighbourhood Components Analysis},
  booktitle = {Neural Information Processing Systems},
  year = {2004}
  }

  @article{Hakeem:2007:LDR:1265999.1266287,
  author = {Hakeem, Asaad and Shah, Mubarak},
  title = {Learning, detection and representation of multi-agent events in videos},
  journal = {Artif. Intell.},
  volume = {171},
  year = {2007}
  }



  @INPROCEEDINGS{Zelnik-manor01event-basedanalysis,
      author = {Lihi Zelnik-manor and Michal Irani},
      title = {Event-based analysis of video},
      booktitle = {CVPR},
      year = {2001}
  }

  @inproceedings{Jebara:2007:SCE:1421665.1421685,
  author = {Jebara, Tony and Song, Yingbo and Thadani, Kapil},
  title = {Spectral Clustering and Embedding with Hidden Markov Models},
  booktitle = {European conference on Machine Learning},
  year = {2007}
  }
  @article{10.1109/CVPR.1997.609375,
  author = {Yair Weiss},
  title = {Smoothness in Layers: Motion segmentation using nonparametric mixture estimation.},
  journal ={CVPR},
  year={1997},

  }

  @article{ncut,
  author = {Jianbo Shi and Jitendra Malik},
  title = {Normalized Cuts and Image Segmentation},
  journal = {TPAMI},
  year = {2000},
  }


  @article{10.1109/TPAMI.2005.202,
  author = {Jiangjian Xiao and Mubarak Shah},
  title = {Motion Layer Extraction in the Presence of Occlusion Using Graph Cuts},
  journal ={TPAMI},
  year = {2005},
  }

  @article{1340323,
  author = {Pawan Kumar, M. and Torr, P. H. and Zisserman, A.},
  title = {Learning Layered Motion Segmentations of Video},
  journal = {IJCV},
  volume = {76},
  year = {2008},
  }



  @ARTICLE{Wang94representingmoving,
      author = {Y. A. Wang and H. Adelson},
      title = {Representing Moving Images with Layers},
      journal = {TIP},
      year = {1994},
  }

  @InProceedings{Fradet09a,
    author = {Fradet, Matthieu and Robert, Philippe and P\'{e}rez, Patrick},
    Title = {Clustering point trajectories with various life-spans},
    BookTitle = {CVMP},
  year={2009}
  }





  @article{10.1109/ICCV.2001.10061,
  author = {Stella X. Yu and Jianbo Shi},
  title = {Segmentation with Pairwise Attraction and Repulsion},
  journal ={ICCV},
  Volume={75},
  year = {2001},
  }

  @article{1286005,
  author = {Wu, Bo and Nevatia, Ram},
  title = {Detection and Tracking of Multiple, Partially Occluded Humans by Bayesian Combination of Edgelet based Part Detectors},
  journal = {IJCV},
  year = {2007},
  }


  @inproceedings{DBLP:conf/iccv/CheriyadatR09,
    author    = {Anil Cheriyadat and
		Richard J. Radke},
    title     = {Non-negative matrix factorization of partial track data
		for motion segmentation},
    booktitle = {ICCV},
    year      = {2009},
    pages     = {865-872},
    ee        = {http://dx.doi.org/10.1109/ICCV.2009.5459311},
    crossref  = {DBLP:conf/iccv/2009},
    bibsource = {DBLP, http://dblp.uni-trier.de}
  }

  @article{Canny86,
      author = {Canny, J.},
      journal = {TPAMI},
      title = {{A Computational Approach to Edge Detection}},
      url = {http://dx.doi.org/10.1109/TPAMI.1986.4767851},
      volume = {PAMI-8},
      year = {1986}
  }

  @article{10.1109/ICCV.1995.466815,
  author = {J. Costeira and T. Kanade},
  title = {A multi-body factorization method for motion analysis},
  journal ={ICCV},
  year = {1995},
  }

  @ARTICLE{1273918,
  author={Martin, D.R. and Fowlkes, C.C. and Malik, J.},
  journal={TPAMI},
  title={Learning to detect natural image boundaries using local brightness, color, and texture cues},
  year={2004},
  volume={26}
  }

  @INPROCEEDINGS{139492,
  author={Perona, P. and Malik, J.},
  booktitle={ICCV},
  title={Detecting and localizing edges composed of steps, peaks and roofs },
  year={1990}
  }

  @incollection {springerlink:10.1007/978-3-642-15555-0_21,
    author = {Brox, Thomas and Malik, Jitendra},
    affiliation = {University of California at Berkeley},
    title = {Object Segmentation by Long Term Analysis of Point Trajectories},
    booktitle = {ECCV},
    year={2010}
  }

  @incollection {springerlink:10.1007/978-3-642-15555-0_27,
    author = {Rahtu, Esa and Kannala, Juho and Salo, Mikko and Heikkilï¿œ, Janne},
    affiliation = {Machine Vision Group, University of Oulu, Finland},
    title = {Segmenting Salient Objects from Images and Videos},
    booktitle = {ECCV},
    year={2010},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }

  @Article{19146246,
  TITLE = {On the plausibility of the discriminant center-surround hypothesis for visual saliency.},
  AUTHOR = {Gao, Dashan and Mahadevan, Vijay and Vasconcelos, Nuno},
  journal = {Journal of vision},
  volume = {8},
  year = {2008}
  }


  @Article{Mahadevan10spatiotemporalsaliency,
      author = {Vijay Mahadevan and Nuno Vasconcelos},
      title = {Spatiotemporal Saliency in Dynamic Scenes},
      journal = {TPAMI},
      volume = {32},
      year = {2010},
  }


  @InProceedings{background_subtraction_free_camera,
    author = {Yaser Sheikh, Omar Javed, and Takeo Kanade},
    title = {Background Subtraction for Freely Moving Cameras},
    booktitle = {ICCV},
    year = {2009},
  }
  @conference{vondrick2010,
    title={Efficiently Scaling Up Video Annotation with Crowdsourced Marketplaces},
    author={Carl Vondrick and Deva Ramanan and Donald Patterson},
    booktitle={ECCV},
    year = {2010},
  }

@article{DBLP:journals/corr/PatrauceanHC15,
  author    = {Viorica Patraucean and
               Ankur Handa and
               Roberto Cipolla},
  title     = {Spatio-temporal video autoencoder with differentiable memory},
  journal   = {CoRR},
  volume    = {abs/1511.06309},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.06309},
  timestamp = {Tue, 01 Dec 2015 19:22:34 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/PatrauceanHC15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @conference{StellaRepulsion,
      author = {Stella X. Yu and Jianbo Shi},
      title = {Understanding Popout through Repulsion},
      booktitle= {CVPR},
      year={2001},
  }

  @article{10.1109/TPAMI.2009.167,
  author = {Pedro F. Felzenszwalb and Ross B. Girshick and David McAllester and Deva Ramanan},
  title = {Object Detection with Discriminatively Trained Part-Based Models},
  journal ={TPAMI},
    year = {2010},
  volume={32},
  }

  @inproceedings{Datta_2008_6037,
   author = "Ankur Datta and Yaser Ajmal Sheikh and Takeo Kanade",
   title = "Linear Motion Estimation for Systems of Articulated Planes",
   booktitle = "CVPR",
   month = "June",
   year = "2008",
}

@inproceedings{DBLP:conf/cvpr/FragkiadakiHS13,
  author    = {Katerina Fragkiadaki and
               Han Hu and
               Jianbo Shi},
  title     = {Pose from Flow and Flow from Pose},
  booktitle = {CVPR},
  year      = {2013},
}

@inproceedings{DBLP:conf/cvpr/LadickyTZ13,
  author    = {Lubor Ladicky and
               Philip H. S. Torr and
               Andrew Zisserman},
  title     = {Human Pose Estimation Using a Joint Pixel-wise and Part-wise
               Formulation},
  booktitle = {CVPR},
  year      = {2013}
}

@inproceedings{Zuffi:ICCV:2013,
  title = {Estimating Human Pose with Flowing Puppets},
  author = {Zuffi, Silvia and Romero, Javier and Schmid, Cordelia and Black, Michael J},
  booktitle = {ICCV},
   year = {2013}
}

@ARTICLE{1542030,
author={Agarwal, A. and Triggs, B.},
journal={Pattern Analysis and Machine Intelligence, IEEE Transactions on}, title={Recovering 3D human pose from monocular images},
year={2006},
volume={28},
number={1},
pages={44-58},
keywords={computer vision;image motion analysis;image sequences;learning (artificial intelligence);regression analysis;support vector machines;3D human pose;histogram-of-shape-contexts descriptors;human motion estimation;image silhouettes;learning-based method;monocular image sequences;nonlinear regression;relevance vector machine regression;ridge regression;shape descriptor vectors;silhouette shape;support vector machine regression;Biological system modeling;Humans;Image segmentation;Image sequences;Kernel;Labeling;Learning systems;Robustness;Shape;Support vector machines;Index Terms- Computer vision;human motion estimation;machine learning;multivariate regression.;Algorithms;Artificial Intelligence;Humans;Image Interpretation, Computer-Assisted;Imaging, Three-Dimensional;Joints;Pattern Recognition, Automated;Photography;Posture;Reproducibility of Results;Sensitivity and Specificity;Subtraction Technique},
doi={10.1109/TPAMI.2006.21},
ISSN={0162-8828},}



@inproceedings {420,
	title = {Monocular 3D Pose Estimation and Tracking by Detection},
	booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	year = {2010},
	month = {06/2010},
	address = {San Francisco, USA},
	author = {Mykhaylo Andriluka and Stefan Roth and Schiele, Bernt}
}

@inproceedings{DBLP:conf/cvpr/PirsiavashR12,
  author    = {Hamed Pirsiavash and
               Deva Ramanan},
  title     = {Detecting activities of daily living in first-person camera
               views},
  booktitle = {CVPR},
  year      = {2012},
  pages     = {2847-2854},
  ee        = {http://doi.ieeecomputersociety.org/10.1109/CVPR.2012.6248010},
  crossref  = {DBLP:conf/cvpr/2012},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@inproceedings{Sun:CVPR:10,
  title = {Secrets of optical flow estimation and their principles},
  author = {Sun, D. and Roth, S. and Black, M. J.},
  booktitle = {CVPR},
  year = {2010}
}



@inproceedings{DBLP:conf/eccv/DesaiR12,
  author    = {Chaitanya Desai and
               Deva Ramanan},
  title     = {Detecting Actions, Poses, and Objects with Relational Phraselets},
  booktitle = {ECCV},
  year      = {2012}
}


@INPROCEEDINGS{Sigal06measurelocally,
    author = {Leonid Sigal and Michael J. Black},
    title = {Measure locally, reason globally: Occlusion-sensitive articulated pose estimation},
    booktitle = {CVPR},
    year = {2006}
}

@article{DBLP:journals/pami/Memisevic13,
  author    = {Roland Memisevic},
  title     = {Learning to Relate Images},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {35},
  number    = {8},
  pages     = {1829--1846},
  year      = {2013},
  url       = {http://doi.ieeecomputersociety.org/10.1109/TPAMI.2013.53},
  doi       = {10.1109/TPAMI.2013.53},
  timestamp = {Tue, 25 Jun 2013 20:04:57 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/pami/Memisevic13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@incollection{springerlink:10.1007/978-3-642-15549-9_17,
    author = {Eichner, Marcin and Ferrari, Vittorio},
    booktitle = {ECCV},
    title = {{We Are Family: Joint Pose Estimation of Multiple Persons}},
    year = {2010}
}


@inproceedings{DBLP:conf/nips/MichalskiMK14,
  author    = {Vincent Michalski and
               Roland Memisevic and
               Kishore Reddy Konda},
  title     = {Modeling Deep Temporal Dependencies with Recurrent Grammar Cells""},
  booktitle = {Advances in Neural Information Processing Systems 27: Annual Conference
               on Neural Information Processing Systems 2014, December 8-13 2014,
               Montreal, Quebec, Canada},
  pages     = {1925--1933},
  year      = {2014},
  crossref  = {DBLP:conf/nips/2014},
  url       = {http://papers.nips.cc/paper/5549-modeling-deep-temporal-dependencies-with-recurrent-grammar-cells},
  timestamp = {Wed, 10 Dec 2014 21:34:12 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/nips/MichalskiMK14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@INCOLLECTION{ferrariprogressive,
author = {V. Ferrari and M.J. MarÃ­n-JimÃ©nez and A. Zisserman},
title = {{2D} Human Pose Estimation in {TV} Shows},
booktitle = {Statistical and Geometrical Approaches to Visual Motion Analysis},
year = {2009}}
@inproceedings{pressigout:inria-00351874,
    hal_id = {inria-00351874},
    url = {http://hal.inria.fr/inria-00351874},
    title = {{Hybrid tracking approach using optical flow and pose estimation}},
    author = {Pressigout, Muriel and Marchand, Eric and Memin, Etienne},
    abstract = {{This paper proposes an hybrid approach to estimate the 3D pose of an object. The integration of texture information based on image intensities in a more classical non-linear edge-based pose estimation computation has proven to highly increase the reliability of the tracker. We propose in this work to exploit the data provided by an optical flow algorithm for a similar purpose. The advantage of using the optical flow is that it does not require any a priori knowledge on the object appearance. The registration of 2D and 3D cues for monocular tracking is performed by a non linear minimization. Results obtained show that using optical flow enables to perform robust 3D hybrid tracking even without any texture model}},
    language = {Anglais},
    affiliation = {Institut d'Electronique et de T{\'e}l{\'e}communications de Rennes - IETR , LAGADIC - INRIA - IRISA , VISTA - INRIA - IRISA},
    booktitle = {{IEEE Int. Conf. on Image Processing, ICIP'08}},
    address = {San Diego, California, France},
    audience = {internationale },
    year = {2008},
    pdf = {http://hal.inria.fr/inria-00351874/PDF/2008\_icip\_pressigout.pdf},
}







  @inproceedings{conf/cvpr/BreglerM98,
  author = {Bregler, Christoph and Malik, Jitendra},
  booktitle = {CVPR},
  title = {Tracking People with Twists and Exponential Maps.},
  year = 1998
}
@InProceedings{Bro06k,
  author       = "T. Brox and B. Rosenhahn and D. Cremers and H.-P. Seidel",
  title        = "High accuracy optical flow serves 3-D pose tracking: exploiting contour and flow based constraints",
  booktitle    = "ECCV",
  year         = "2006"
}

@article{DBLP:journals/corr/RusuRDSKKPH16,
  author    = {Andrei A. Rusu and
               Neil C. Rabinowitz and
               Guillaume Desjardins and
               Hubert Soyer and
               James Kirkpatrick and
               Koray Kavukcuoglu and
               Razvan Pascanu and
               Raia Hadsell},
  title     = {Progressive Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1606.04671},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.04671},
  timestamp = {Wed, 07 Jun 2017 14:40:25 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RusuRDSKKPH16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@InProceedings{Ferrari08,
  author       = "Ferrari, V. and Marin-Jimenez, M. and Zisserman, A.",
  title        = "Progressive Search Space Reduction for Human Pose Estimation",
  booktitle    = "IEEE Conference on Computer Vision and Pattern Recognition",
  year         = "2008",
}


  @incollection {SLIC,
    title={SLIC Superpixels},
    author={Radhakrishna Achanta and Appu Shaji and Kevin Smith and Aurelien Lucchi and Pascal Fua and Sabine Susstrunk},
    booktitle={EPFL Technical Report no. 149300, June 2010},
  }
  @incollection {springerlink:10.1007/978-3-642-15549-9_32,
    author = {Sundaram, Narayanan and Brox, Thomas and Keutzer, Kurt},
    title = {Dense Point Trajectories by {GPU}-Accelerated Large Displacement Optical Flow},
    booktitle = {ECCV},
    year={2010},

  }
  @incollection {springerlink:10.1007/978-3-540-88688-4_58,
    author = {Huang, Chang and Wu, Bo and Nevatia, Ramakant},
    title = {Robust Object Tracking by Hierarchical Association of Detection Responses},
    booktitle = {ECCV},
    year={2008},
  }

  @InProceedings{eth_biwi_00483,
    author = {B. Leibe and N. Cornelis and K. Cornelis and L. Van Gool},
    title = {Dynamic 3D Scene Analysis from a Moving Vehicle},
    booktitle = {CVPR},
    year = {2007},
  }

  @article{10.1109/TPAMI.2010.143,
  author = {Thomas Brox and Jitendra Malik},
  title = {Large Displacement Optical Flow: Descriptor Matching in Variational Motion Estimation},
  journal ={TPAMI},
  year = {2010},

  }


  @article {springerlink:10.1007/s11263-008-0136-6,
  title = {Particle Video: Long-Range Motion Estimation Using Point Trajectories},
    author = {Sand, Peter and Teller, Seth},
    affiliation = {MIT Computer Science and Artificial Intelligence Laboratory Cambridge MA 02139 USA},
    journal = {IJCV},
    year = {2008}
  }

  @InProceedings{yma,
    author = { Rao, S. and Tron, R. and Vidal, R. and Ma, Y. },
    title = {Motion segmentation via robust subspace separation in the presence of outlying, incomplete, or corrupted trajectories.},
    booktitle = {CVPR},
  year={2008},
  }



  @InProceedings{sparsesubsp,
    author = {Elhamifar, E. and Vidal, R.},
    title = {Sparse subspace clustering},
    booktitle = {CVPR},
    year = {2009}
  }




  @INPROCEEDINGS{BrostowCipollaCVPR2006,
    AUTHOR       = {Gabriel J. Brostow and Roberto Cipolla},
    TITLE        = {Unsupervised Bayesian Detection of Independent Motion in Crowds},
    BOOKTITLE    = {CVPR},
    YEAR         = {2006},
  }
  @article{GrundmannKwatra2010,
    author = {Matthias Grundmann and Vivek Kwatra and Mei Han and Irfan Essa},
    title = {Efficient Hierarchical Graph Based Video Segmentation},
    journal = {CVPR},
    year = {2010},
  }



  @incollection {mhvs,
    author = {Amelio Vazquez-Reina and Shai Avidan and Hanspeter Pfister and Eric Miller},
    title = {Multiple Hypothesis Video Segmentation from Superpixel Flows},
    booktitle = {ECCV},
  year={2010},
  }
  @INPROCEEDINGS{4761133,
  author={Izadi, M. and Saeedi, P.},
  booktitle={Pattern Recognition, 2008. ICPR 2008. 19th International Conference on},
  title={Robust region-based background subtraction and shadow removing using color and gradient information},
  year={2008}
  }

  @INPROCEEDINGS{784637,
  author={Stauffer, C. and Grimson, W.E.L.},
  booktitle={CVPR},
  title={Adaptive background mixture models for real-time tracking},
  year={1999}}


  @inproceedings{Zivkovic:2004:IAG:1018428.1020644,
  author = {Zivkovic, Zoran},
  title = {Improved Adaptive Gaussian Mixture Model for Background Subtraction},
  booktitle = {ICPR},
  year = {2004}
  }


  @article{Felzenszwalb:2004:EGI:981793.981796,
  author = {Felzenszwalb, Pedro F. and Huttenlocher, Daniel P.},
  title = {Efficient Graph-Based Image Segmentation},
  journal = {IJCV},
  volume = {59},
  year = {2004}
  }

  @article{phycho,
    author = {H. C. Nothdurft},
    title = {Feature analysis and the role of similarity in preattentive vision},
    journal = {Perception and Psychophysics},
    volume={52},
    year = {1992},
  }

  @inproceedings{DBLP:conf/eccv/Ren08,
    author    = {Xiaofeng Ren},
    title     = {Multi-scale Improves Boundary Detection in Natural Images},
    booktitle = {ECCV (3)},
    year      = {2008},
    pages     = {533-545},
    ee        = {http://dx.doi.org/10.1007/978-3-540-88690-7_40},
    crossref  = {DBLP:conf/eccv/2008-3},
    bibsource = {DBLP, http://dblp.uni-trier.de}
  }



  @INPROCEEDINGS{5206727,
  author={Chunhui Gu and Lim, J.J. and Arbelaez, P. and Malik, J.},
  booktitle={CVPR},
  year={2009},
  title={Recognition using regions}
  }
  @InProceedings{citeulike:942103,
      title = {Bottom-up/top-down image parsing by attribute graph grammar},
      author = {Han, Feng and Zhu, Song-Chun},
      journal = {ICCV},
  year={ 2005}
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {CVPR},
  year={2009},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }

  @InProceedings{Yan06general,
    title     = {A General Framework for Motion Segmentation: Independent, Articulated, Rigid, Non-rigid, Degenerate and Non-degenerate.},
    author = {J. Yan and M. Pollefeys},
    booktitle = {ECCV},
  year={ 2006},
  }

  @InProceedings{Ayer,
    title     = {Layered representation of motion video using robust maximum-likelihood estimation of mixture models and MDL encoding},
    author = {S. Ayer and H. S. Sawhney},
    booktitle = {ICCV},
  year={ 1995},
  }

  @article{10.1109/CVPR.2005.335,
  author = {Deva Ramanan and D. A. Forsyth and Andrew Zisserman},
  title = {Strike a Pose: Tracking People by Finding Stylized Poses},
  journal ={CVPR},
  year = {2005},
  }
  
    @incollection{NIPS2012_0534,
    Title = {ImageNet Classification with Deep Convolutional Neural Networks},
    Url = {http://books.nips.cc/papers/files/nips25/NIPS2012_0534.pdf},
    Booktitle = {Advances in Neural Information Processing Systems 25},
    Author = {Alex Krizhevsky and Ilya Sutskever and Geoffrey E. Hinton},
    Editor = {P. Bartlett and F.c.n. Pereira and C.j.c. Burges and L. Bottou and K.q. Weinberger},
    Year = {2012},
    Pages = {1106--1114}
   } 
   
@inproceedings{DBLP:conf/iccv/ParkR11,
  author    = {Dennis Park and Deva Ramanan},
  title     = {N-best maximal decoders for part models},
  booktitle = {ICCV},
  year      = {2011},
  pages     = {2627-2634},
  ee        = {http://dx.doi.org/10.1109/ICCV.2011.6126552},
  crossref  = {DBLP:conf/iccv/2011},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Batra:2012:DMS:2403138.2403140,
 author = {Batra, Dhruv and Yadollahpour, Payman and Guzman-Rivera, Abner and Shakhnarovich, Gregory},
 title = {Diverse "M"-best solutions in markov random fields},
 booktitle = {ECCV},
 year = {2012}
} 


@inproceedings{Batra:2012:DMS:2403138.2403140,
 author = {Batra, Dhruv and Yadollahpour, Payman and Guzman-Rivera, Abner and Shakhnarovich, Gregory},
 title = {Diverse M-best solutions in markov random fields},
 booktitle = {Proceedings of the 12th European conference on Computer Vision - Volume Part V},
 series = {ECCV'12},
 year = {2012},
 isbn = {978-3-642-33714-7},
 location = {Florence, Italy},
 pages = {1--16},
 numpages = {16},
 url = {http://dx.doi.org/10.1007/978-3-642-33715-4_1},
 doi = {10.1007/978-3-642-33715-4_1},
 acmid = {2403140},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
}


@InProceedings{Weiss_2013_ICCV,
author = {David Weiss and Benjamin Sapp and Ben Taskar},
title = {Dynamic Structured Model Selection},
booktitle = {ICCv},
month = {December},
year = {2013}
} 


@inproceedings{DBLP:conf/iros/KoppulaS13,
  author    = {Hema Swetha Koppula and
               Ashutosh Saxena},
  title     = {Anticipating human activities for reactive robotic response},
  booktitle = {2013 {IEEE/RSJ} International Conference on Intelligent Robots and
               Systems, Tokyo, Japan, November 3-7, 2013},
  pages     = {2071},
  year      = {2013},
  crossref  = {DBLP:conf/iros/2013},
  url       = {http://dx.doi.org/10.1109/IROS.2013.6696634},
  doi       = {10.1109/IROS.2013.6696634},
  timestamp = {Fri, 10 Jan 2014 20:22:57 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/iros/KoppulaS13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{YangR_CVPR_2011,
    author = "Yang, Yi and Ramanan, Deva",
    booktitle = "CVPR",
    year = "2011",
    title = "Articulated pose estimation with flexible mixtures-of-parts"
}

@INPROCEEDINGS{Felzenszwalb00efficientmatching,
    author = {Pedro F. Felzenszwalb and Daniel P. Huttenlocher},
    title = {Efficient Matching of Pictorial Structures},
    booktitle = {CVPR},
    year = {2000},
}

@inproceedings{YangWang:2011:LHP:2191740.2192189,
 author = {Yang Wang and Duan Tran and Zicheng Liao},
 title = {Learning hierarchical poselets for human parsing},
 booktitle = {Proceedings of the 2011 IEEE Conference on Computer Vision and Pattern Recognition},
 series = {CVPR '11},
 year = {2011},
 isbn = {978-1-4577-0394-2},
 pages = {1705--1712},
 numpages = {8},
 url = {http://dx.doi.org/10.1109/CVPR.2011.5995519},
 doi = {10.1109/CVPR.2011.5995519},
 acmid = {2192189},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
 keywords = {max-margin framework, hierarchical poselets, human parsing, part-based model, rigid parts, human anatomy, structured model},
}

@article{Grady:2006:RWI:1175896.1176220,
 author = {Grady, Leo},
 title = {Random Walks for Image Segmentation},
 journal = {IEEE Trans. Pattern Anal. Mach. Intell.},
 issue_date = {November 2006},
 volume = {28},
 number = {11},
 month = nov,
 year = {2006},
 issn = {0162-8828},
 pages = {1768--1783},
 numpages = {16},
 url = {http://dx.doi.org/10.1109/TPAMI.2006.233},
 doi = {10.1109/TPAMI.2006.233},
 acmid = {1176220},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
 keywords = {Image segmentation, Image segmentation, interactive segmentation, graph theory, random walks, combinatorial Dirichlet problem, harmonic functions, Laplace equation, graph cuts, boundary completion., Laplace equation, boundary completion., combinatorial Dirichlet problem, graph cuts, graph theory, harmonic functions, interactive segmentation, random walks},
} 



@inproceedings{DBLP:conf/cvpr/JohnsonE11,
  author    = {Sam Johnson and
               Mark Everingham},
  title     = {Learning effective human pose estimation from inaccurate
               annotation},
  booktitle = {CVPR},
  year      = {2011}
}

@misc{Jia13caffe,
   Author = {Yangqing Jia},
   Title = { {Caffe}: An Open Source Convolutional Architecture for Fast Feature Embedding},
   Year  = {2013}
}

@inproceedings{MODEC,
  author    = {Ben Sapp and
               Ben Taskar},
  title     = {MODEC:Multimodal Decomposable Models for Human Pose Estimation},
  booktitle = {CVPR},
  year      = {2013}
}


















  @Article{ Perse2009612,
  title = "A trajectory-based analysis of coordinated team activity in a basketball game",
  journal = "Computer Vision and Image Understanding",
  volume = "113",
  year = "2009",
  }

  @inproceedings{morariu11eventstructure,
    author    = {Vlad I. Morariu and Larry S. Davis},
    title     = {Multi-agent event recognition in structured scenarios.},
    booktitle = {CVPR},
    year      = {2011}
  }


  @inproceedings{storyline,
    author    = {Abhinav Gupta and Praveen Srinivasan and Jianbo Shi and Larry S. Davis},
    title     = {Understanding videos, constructing plots learning a visually grounded storyline model from annotated videos},
    booktitle = {CVPR},
    year      = {2009}
  }


  @ARTICLE{790429,
  author={Wilson, A.D. and Bobick, A.F.},
  journal={TPAMI},
  title={Parametric hidden Markov models for gesture recognition},
  year={1999},
  volume={21}
  }



  @article{experts,
  author = {Terence D. Sanger and Robert A. Jacobs and Steven J. Nowlan and Geoffrey E. Hinton},
  title = {Adaptive Mixtures of Local Experts},
  journal = {Neural Computation},
  volume = {3},
  year = {1991}
  }


  @INPROCEEDINGS{lips,
  author={Bregler, C. and Omohundro, S.M.},
  booktitle={ICCV},
  title={Nonlinear manifold learning for visual speech recognition},
  year={1995}
  }



  @inproceedings{BN,
  author = {Shaogang Gong and Tao Xiang},
  title = {Recognition of Group Activities using Dynamic Probabilistic Networks},
  booktitle = {ICCV},
  year={2003}
  }


  @article{HMMMO,
  author = {Aaron F. Bobick and Andrew D. Wilson},
  title = {A State-Based Approach to the Representation and Recognition of Gesture},
  journal = {TPAMI},
  volume = {19}
  }

  @inproceedings{Brand:1997:CHM:794189.794420,
  author = {Brand, M. and Oliver, N. and Pentland, A.},
  title = {Coupled hidden Markov models for complex action recognition},
  booktitle = {CVPR},
  year = {1997}
  }

  @article{Ghahramani:1997:FHM:274158.274165,
  author = {Ghahramani, Zoubin and Jordan, Michael I.},
  title = {Factorial Hidden Markov Models},
  journal = {Mach. Learn.},
  volume = {29},
  year = {1997}
  }


  @INPROCEEDINGS{4270099,
  author={Laxton, B. and Jongwoo Lim and Kriegman, D.},
  booktitle={CVPR},
  title={Leveraging temporal, contextual and ordering constraints for recognizing complex activities in video},
  year={2007}
  }


  @article{DBLP:journals/jmlr/SiracusaF09,
    author    = {Michael Siracusa and John Fisher},
    title     = {Tractable Bayesian Inference of Time-Series Dependence Structure},
    journal   = {Journal of Machine Learning Research - Proceedings Track},
    volume    = {5},
    year      = {2009}
  }



  @article{parametrized,
  author = {Yaser Yacoob and Michael J. Black},
  title = {Parameterized Modeling and Recognition of Activities},
  journal = {Computer Vision and Image Understanding},
  volume = {73},
  year = {1999}
  }




  @inproceedings{Bobick:1995:STS:839277.840051,
  author = {Bobick, A. F. and Wilson, A. D.},
  title = {A state-based technique for the summarization and recognition of gesture},
  booktitle = {ICCV},
  year = {1995}
  }

  @inproceedings{Xu:2008:SBV:1478392.1478446,
  author = {Xu, Li and Chen, Jianing and Jia, Jiaya},
  title = {A Segmentation Based Variational Model for Accurate Optical Flow Estimation},
  booktitle = {ECCV},
  year = {2008}
  }

  @inproceedings{Niebles:2010:MTS:1888028.1888059,
  author = {Niebles, Juan Carlos and Chen, Chih-Wei and Fei-Fei, Li},
  title = {Modeling temporal structure of decomposable motion segments for activity classification},
  booktitle = {ECCV},
  year = {2010}
  }

  @InProceedings{Bro11c,
    author       = "P. Sundberg and T. Brox and M. Maire and P. Arbelaez and J. Malik",
    title        = "Occlusion boundary detection and figure/ground assignment from optical flow",
    booktitle    = "CVPR",
    year         = "2011"
  }

  @inproceedings{Stein_2007_5836,
    author = "Andrew Stein and Derek Hoiem and Martial Hebert",
    title = "Learning to Find Object Boundaries Using Motion Cues",
    booktitle = "IEEE International Conference on Computer Vision (ICCV)",
    month = "October",
    year = "2007",
    Notes = "Dataset available from http://www.cs.cmu.edu/~stein/occlusion_data"
  }


  @article{Hakeem:2007:LDR:1265999.1266287,
  author = {Hakeem, Asaad and Shah, Mubarak},
  title = {Learning, detection and representation of multi-agent events in videos},
  journal = {Artif. Intell.},
  volume = {171},
  year = {2007}
  }


  @INPROCEEDINGS{Zelnik-manor01event-basedanalysis,
      author = {Lihi Zelnik-manor and Michal Irani},
      title = {Event-based analysis of video},
      booktitle = {CVPR},
      year = {2001}
  }

  @inproceedings{Jebara:2007:SCE:1421665.1421685,
  author = {Jebara, Tony and Song, Yingbo and Thadani, Kapil},
  title = {Spectral Clustering and Embedding with Hidden Markov Models},
  booktitle = {European conference on Machine Learning},
  year = {2007}
  }

  @article{Jebara:2004:PPK:1005332.1016786,
  author = {Jebara, Tony and Kondor, Risi and Howard, Andrew},
  title = {Probability Product Kernels},
  journal = {J. Mach. Learn. Res.},
  volume = {5},
  year = {2004}
  }

  @INPROCEEDINGS{Gong99recognitionof,
      author = {Shaogang Gong and Michael Walter},
      title = {Recognition of Temporal Structures: Learning Prior and Propagating Observation Augmented Densities via Hidden Markov States},
      booktitle = {ICCV},
      year = {1999},
  }

  @article{Brand:2000:DSA:351581.351608,
  author = {Brand, Matthew and Kettnaker, Vera},
  title = {Discovery and Segmentation of Activities in Video},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }


  @INPROCEEDINGS{Brown01productsof,
      author = {Andrew D. Brown and Andrew D. Brown and Geoffrey E. Hinton and Geoffrey E. Hinton},
      title = {Products of Hidden Markov Models},
      booktitle = {In Proceedings of Artificial Intelligence and Statistics},
      year = {2001},
  }


  @inproceedings{malisiewicz-nips09,
    Author =	 {Tomasz Malisiewicz and Alexei A. Efros},
    Booktitle =	 {NIPS},
    Title =	 {Beyond Categories: The Visual Memex Model for Reasoning About Object Relationships},
    Year =	 2009
  }


  @inproceedings{yamato,
  author = {J. Yamato and J. Ohya and K. Ishii},
  title = {Recognizing human action in time-sequential images using a hidden Markov model},
  booktitle = {CVPR},
  year = {1994},
  }



  @INPROCEEDINGS{Elgammal04separatingstyle,
      author = {Ahmed Elgammal and Chan-su Lee},
      title = {Separating style and content on a nonlinear manifold},
      booktitle = {CVPR},
      year = {2004}
  }

  @INPROCEEDINGS{Tenenbaum97separatingstyle,
      author = {Joshua B. Tenenbaum and William T. Freeman},
      title = {Separating style and content},
      booktitle = {In Advances in neural},
      year = {1997}
  }

@article{DBLP:journals/corr/LeeKP016,
  author    = {Kenton Lee and
               Tom Kwiatkowski and
               Ankur P. Parikh and
               Dipanjan Das},
  title     = {Learning Recurrent Span Representations for Extractive Question Answering},
  journal   = {CoRR},
  volume    = {abs/1611.01436},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.01436},
  archivePrefix = {arXiv},
  eprint    = {1611.01436},
  timestamp = {Wed, 07 Jun 2017 14:41:54 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LeeKP016},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/LiuAESR15,
  author    = {Wei Liu and
               Dragomir Anguelov and
               Dumitru Erhan and
               Christian Szegedy and
               Scott E. Reed and
               Cheng{-}Yang Fu and
               Alexander C. Berg},
  title     = {{SSD:} Single Shot MultiBox Detector},
  journal   = {CoRR},
  volume    = {abs/1512.02325},
  year      = {2015},
  url       = {http://arxiv.org/abs/1512.02325},
  timestamp = {Wed, 07 Jun 2017 14:42:54 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LiuAESR15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @inproceedings{DBLP:conf/cvpr/LvN07,
    author    = {Fengjun Lv and
		Ramakant Nevatia},
    title     = {Single View Human Action Recognition using Key Pose Matching and Viterbi Path Searching},
    booktitle = {CVPR},
    year      = {2007}
  }


  @inproceedings { 158,
	  title = {Linear Embeddings in Non-Rigid Structure From Motion},
	  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	  year = {2009},
	  address = {Miami, FL},
	  author = {Vincent Rabaud and Serge Belongie}
  }



  @INPROCEEDINGS{4270260,
  author={Goh, A. and Vidal, R.},
  booktitle={CVPR},
  title={Segmenting Motions of Different Types by Unsupervised Manifold Clustering},
  year={2007},
  }


  @incollection {springerlink:10.1007/11551188_37,
    author = {Wang, Fei and Zhang, Changshui},
    title = {Spectral Clustering for Time Series},
    booktitle = {Pattern Recognition and Data Mining},
    volume = {3686},
    year = {2005}
  }

  @INPROCEEDINGS{4587385,
  author={Xiaozhe Wang and Liang Wang and Wirth, A.},
  booktitle={CVPR},
  title={Pattern discovery in motion time series via structure-based spectral clustering},
  year={2008}
  }


  @article{Stauffer:2000:LPA:351581.351588,
  author = {Stauffer, Chris and Grimson, W. Eric L.},
  title = {Learning Patterns of Activity Using Real-Time Tracking},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }

  @incollection{Nanopoulos:2001:FCT:766914.766918,
  author = {Nanopoulos, Alex and Alcock, Rob and Manolopoulos, Yannis},
  title = {Information processing and technology},
  year = {2001},
  }

  BibTeX | EndNote | ACM Ref

  @inproceedings{Shi:2006:LTS:1153171.1153641,
  author = {Shi, Yifan and Bobick, Aaron and Essa, Irfan},
  title = {Learning Temporal Sequence Model from Partially Labeled Data},
  booktitle = {CVPR},
  year = {2006}
  }


  @article{Murase,
  author = {Murase, Hiroshi and Nayar, Shree K.},
  title = {Visual learning and recognition of 3-D objects from appearance},
  journal = {IJCV},
  volume = {14},
  year = {1995}
  }


  @INPROCEEDINGS{698609,
  author={Bobick, A.F. and Ivanov, Y.A.},
  booktitle={CVPR},
  title={Action recognition using probabilistic parsing},
  year={1998}
  }

  @inproceedings{Ryoo:2006:RCH:1153171.1153651,
  author = {Ryoo, M. S. and Aggarwal, J. K.},
  title = {Recognition of Composite Human Activities through Context-Free Grammar Based Representation},
  booktitle = {CVPR},
  year = {2006}
  }


  @INPROCEEDINGS{Hadsell06dimensionalityreduction,
      author = {Raia Hadsell and Sumit Chopra and Yann Lecun},
      title = {Dimensionality reduction by learning an invariant mapping},
      booktitle = {CVPR},
      year = {2006}
  }


  @incollection{NIPS2010_0893,
  title = {Pose-Sensitive Embedding by Nonlinear NCA Regression},
  author = {Graham Taylor and Rob Fergus and George Williams and Ian Spiro and Christoph Bregler},
  booktitle = {NIPS},
  year = {2010}
  }
  @InProceedings{lezama11,
    author = {Lezama, J. and Alahari, K. and Sivic, J. and Laptev, I.},
    title = {Track to the Future: Spatio-temporal Video Segmentation with Long-range Motion Cues},
    booktitle = {CVPR},
    year = {2011}
  }
  @InProceedings{shuwang2,
    author = {Shu Wang and Huchuan Lu and Fan Yang and Ming-Hsuan Yang},
    title = {Superpixel Tracking},
    booktitle = {ICCV},
    year = {2011}
  }
  @InProceedings{OB11,
    author       = "P. Ochs and T.Brox",
    title        = "Object segmentation in video: a hierarchical variational approach for turning point trajectories into dense regions",
    booktitle    = "ICCV",
    year         = "2011",
    url          = "http://lmb.informatik.uni-freiburg.de/Publications/2011/OB11"
  }

  @InProceedings{raptisS10,
    author = 	{Raptis, M. and Soatto, S.},
    title = 	{Tracklet Descriptors for Action Modeling and Video Analysis},
    booktitle = 	{ECCV},
    year = 	{2010}
  }


  @book{Fukunaga:1990:ISP:92131,
  author = {Fukunaga, Keinosuke},
  title = {Introduction to statistical pattern recognition (2nd ed.)},
  year = {1990}
  }


  @ARTICLE{Roweis00nonlineardimensionality,
      author = {Sam T. Roweis and Lawrence K. Saul},
      title = {Nonlinear dimensionality reduction by locally linear embedding},
      journal = {SCIENCE},
      year = {2000},
      volume = {290}
  }

  @article{Turk_Pentland_1991,
  title={Face recognition using eigenfaces},
  journal={CVPR},
  year={1991}
  }


  @INPROCEEDINGS{Laptev03space-timeinterest,
      author = {Ivan Laptev and Tony Lindeberg},
      title = {Space-time Interest Points},
      booktitle = {ICCV},
      year = {2003}
  }


  @INPROCEEDINGS{Kim07r.:tensor,
      author = {Tae-kyun Kim and Shu-fai Wong and Roberto Cipolla},
      title = {Tensor Canonical Correlation Analysis for Action Classification},
      booktitle = {CVPR},
      year = {2007}
  }


  @inproceedings{Fragkiadaki:topology,
  author = {Fragkiadaki, Katerina and Shi, Jianbo},
  title = {Exploiting Motion and Topology for Segmenting and tracking Under Entanglement.},
  booktitle = {CVPR},
  year = {2011},
  }

  @INPROCEEDINGS{Jianbo03multiclassspectral,
      author = {Yu,Stella and Shi, Jianbo},
      title = {Multiclass Spectral Clustering},
      booktitle = {ICCV},
      year = {2003}
  }



  @INPROCEEDINGS{lu_cvpr2011,
      author = {Wei-Lwun Lu and Jo-Anne Ting and Kevin P. Murphy and James J. Little},
      booktitle = {Identifying Players in Broadcast Sports Videos using Conditional Random Fields},
      journal = {Proceedings of the 2011 IEEE Conference on Computer Vision and Pattern Recognition},
      year = {2011}
  }

  @article{DBLP:journals/pami/BoykovVZ01,
    author    = {Yuri Boykov and Olga Veksler and Ramin Zabih},
    title     = {Fast Approximate Energy Minimization via Graph Cuts},
    journal   = {TPAMI},
    volume    = {23},
    year      = {2001}
  }

  @article{GEAN:GEAN31,
  author = {Matula, David W. and Sokal, Robert R.},
  title = {Properties of Gabriel Graphs Relevant to Geographic Variation Research and the Clustering of Points in the Plane},
  journal = {Geographical Analysis},
  volume = {12},
  year = {1980}
  }


  @INPROCEEDINGS{global_Pb,
  AUTHOR = {Michael Maire and Pablo Arbelaez and Charless Fowlkes and Jitendra Malik},
  TITLE = {Using contours to detect and localize junctions in natural images.},
  booktitle = {CVPR},
  YEAR = {2008}
  }


  @inproceedings{Yu:2010:AIO:1873951.1874105,
  author = {Yu, Haonan and Li, Jia and Tian, Yonghong and Huang, Tiejun},
  title = {Automatic interesting object extraction from images using complementary saliency maps},
  booktitle = {Proceedings of the international conference on Multimedia},
  year = {2010}
  }
  @inproceedings{DBLP:conf/accv/DonoserRB09,
    author    = {Michael Donoser and Hayko Riemenschneider and  Horst Bischof},
    title     = {Efficient Partial Shape Matching of Outer Contours},
    booktitle = {ACCV},
    year      = {2009}
  }

  @inproceedings{RenFM05a,
	  author = "Xiaofeng Ren and Charless C. Fowlkes and Jitendra Malik",
	  title = "Scale-invariant contour completion using conditional random fields",
	  booktitle = {ICCV},
	  year = "2005"
	  }
@INPROCEEDINGS{Xiao06bilateralfiltering-based,
    author = {Jiangjian Xiao and Hui Cheng and Harpreet Sawhney and Cen Rao and Michael Isnardi and Sarnoff Corporation},
    title = {Bilateral filtering-based optical flow estimation with occlusion detection},
    booktitle = {ECCV},
    year = {2006},
}

  @TechReport{RenFM05tech,
	  author = "Xiaofeng Ren and Charless C. Fowlkes and Jitendra Malik",
	  title = "Mid-level cues improve boundary detection",
	  institution =  {UC Berkeley},
	  number =       {UCB//CSD-05-1382},
	  year =         {2005}
	  }

  @InProceedings{BroxSegmentationCVPR11,
    author       = "Thomas Brox and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Object Segmentation by Alignment of Poselet Activations to Image Contours",
    booktitle    = "IEEE International Conference on Computer Vision and Pattern Recognition (CVPR)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }
  @InProceedings{HariharanSemanticContoursICCV11,
    author       = "Bharath Hariharan and Pablo Arbelaez and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Semantic Contours from Inverse Detectors",
    booktitle    = "International Conference on Computer Vision (ICCV)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }
  @inproceedings{DBLP:conf/eccv/RiemenschneiderDB10,
    author    = {Hayko Riemenschneider and Michael Donoser and Horst Bischof},
    title     = {Using Partial Edge Contour Matches for Efficient Object
		Category Localization},
    booktitle = {ECCV},
    year      = {2010}
  }

  


  @inproceedings{MoriREM04,
	  author = "Greg Mori and Xiaofeng Ren and Alexei A. Efros and Jitendra Malik",
	  title = "Recovering human body configurations: combining segmentation and recognition.",
	  booktitle = {Proc. IEEE Conf. Comput. Vision and Pattern Recogn.},
	  volume = 2,
	  pages = "326-333",
	  year = "2004",
	  }



  @inproceedings{Latecki2010,
    author    = {Tianyang Ma and Longin Jan Latecki},
    title     = { From Partial Shape Matching through Local Deformation to Robust Global Shape Similarity for Object Detection},
    booktitle = {CVPR},
    year      = {2011}
  }
  @article{Jebara:2004:PPK:1005332.1016786,
  author = {Jebara, Tony and Kondor, Risi and Howard, Andrew},
  title = {Probability Product Kernels},
  journal = {J. Mach. Learn. Res.},
  volume = {5},
  year = {2004}
  }

  @INPROCEEDINGS{Gong99recognitionof,
      author = {Shaogang Gong and Michael Walter},
      title = {Recognition of Temporal Structures: Learning Prior and Propagating Observation Augmented Densities via Hidden Markov States},
      booktitle = {ICCV},
      year = {1999},
  }

  @article{Brand:2000:DSA:351581.351608,
  author = {Brand, Matthew and Kettnaker, Vera},
  title = {Discovery and Segmentation of Activities in Video},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }


  @INPROCEEDINGS{Brown01productsof,
      author = {Andrew D. Brown and Andrew D. Brown and Geoffrey E. Hinton and Geoffrey E. Hinton},
      title = {Products of Hidden Markov Models},
      booktitle = {In Proceedings of Artificial Intelligence and Statistics},
      year = {2001},
  }


  @inproceedings{malisiewicz-nips09,
    Author =	 {Tomasz Malisiewicz and Alexei A. Efros},
    Booktitle =	 {NIPS},
    Title =	 {Beyond Categories: The Visual Memex Model for Reasoning About Object Relationships},
    Year =	 2009
  }


  @inproceedings{yamato,
  author = {J. Yamato and J. Ohya and K. Ishii},
  title = {Recognizing human action in time-sequential images using a hidden Markov model},
  booktitle = {CVPR},
  year = {1994},
  }



  @INPROCEEDINGS{Elgammal04separatingstyle,
      author = {Ahmed Elgammal and Chan-su Lee},
      title = {Separating style and content on a nonlinear manifold},
      booktitle = {CVPR},
      year = {2004}
  }

  @INPROCEEDINGS{Tenenbaum97separatingstyle,
      author = {Joshua B. Tenenbaum and William T. Freeman},
      title = {Separating style and content},
      booktitle = {In Advances in neural},
      year = {1997}
  }

  @inproceedings{DBLP:conf/cvpr/LvN07,
    author    = {Fengjun Lv and
		Ramakant Nevatia},
    title     = {Single View Human Action Recognition using Key Pose Matching and Viterbi Path Searching},
    booktitle = {CVPR},
    year      = {2007}
  }


  @inproceedings { 158,
	  title = {Linear Embeddings in Non-Rigid Structure From Motion},
	  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	  year = {2009},
	  address = {Miami, FL},
	  author = {Vincent Rabaud and Serge Belongie}
  }



  @INPROCEEDINGS{4270260,
  author={Goh, A. and Vidal, R.},
  booktitle={CVPR},
  title={Segmenting Motions of Different Types by Unsupervised Manifold Clustering},
  year={2007},
  }


  @incollection {springerlink:10.1007/11551188_37,
    author = {Wang, Fei and Zhang, Changshui},
    title = {Spectral Clustering for Time Series},
    booktitle = {Pattern Recognition and Data Mining},
    volume = {3686},
    year = {2005}
  }


@INPROCEEDINGS{Wang06gaussianprocess,
    author = {Jack M. Wang and David J. Fleet and Aaron Hertzmann},
    title = {Gaussian process dynamical models},
    booktitle = {In NIPS},
    year = {2006},
    pages = {1441--1448},
    publisher = {MIT Press}
}


  @INPROCEEDINGS{4587385,
  author={Xiaozhe Wang and Liang Wang and Wirth, A.},
  booktitle={CVPR},
  title={Pattern discovery in motion time series via structure-based spectral clustering},
  year={2008}
  }


  @article{Stauffer:2000:LPA:351581.351588,
  author = {Stauffer, Chris and Grimson, W. Eric L.},
  title = {Learning Patterns of Activity Using Real-Time Tracking},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }

  @incollection{Nanopoulos:2001:FCT:766914.766918,
  author = {Nanopoulos, Alex and Alcock, Rob and Manolopoulos, Yannis},
  title = {Information processing and technology},
  year = {2001},
  }

  BibTeX | EndNote | ACM Ref

  @inproceedings{Shi:2006:LTS:1153171.1153641,
  author = {Shi, Yifan and Bobick, Aaron and Essa, Irfan},
  title = {Learning Temporal Sequence Model from Partially Labeled Data},
  booktitle = {CVPR},
  year = {2006}
  }


  @article{Murase,
  author = {Murase, Hiroshi and Nayar, Shree K.},
  title = {Visual learning and recognition of 3-D objects from appearance},
  journal = {IJCV},
  volume = {14},
  year = {1995}
  }


  @INPROCEEDINGS{698609,
  author={Bobick, A.F. and Ivanov, Y.A.},
  booktitle={CVPR},
  title={Action recognition using probabilistic parsing},
  year={1998}
  }

  @inproceedings{Ryoo:2006:RCH:1153171.1153651,
  author = {Ryoo, M. S. and Aggarwal, J. K.},
  title = {Recognition of Composite Human Activities through Context-Free Grammar Based Representation},
  booktitle = {CVPR},
  year = {2006}
  }


  @INPROCEEDINGS{Hadsell06dimensionalityreduction,
      author = {Raia Hadsell and Sumit Chopra and Yann Lecun},
      title = {Dimensionality reduction by learning an invariant mapping},
      booktitle = {CVPR},
      year = {2006}
  }


  @incollection{NIPS2010_0893,
  title = {Pose-Sensitive Embedding by Nonlinear NCA Regression},
  author = {Graham Taylor and Rob Fergus and George Williams and Ian Spiro and Christoph Bregler},
  booktitle = {NIPS},
  year = {2010}
  }
  @InProceedings{BroxSegmentationCVPR11,
    author       = "Thomas Brox and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Object Segmentation by Alignment of Poselet Activations to Image Contours",
    booktitle    = "IEEE International Conference on Computer Vision and Pattern Recognition (CVPR)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }
  @InProceedings{HariharanSemanticContoursICCV11,
    author       = "Bharath Hariharan and Pablo Arbelaez and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Semantic Contours from Inverse Detectors",
    booktitle    = "International Conference on Computer Vision (ICCV)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }

  @InProceedings{raptisS10,
    author = 	{Raptis, M. and Soatto, S.},
    title = 	{Tracklet Descriptors for Action Modeling and Video Analysis},
    booktitle = 	{ECCV},
    year = 	{2010}
  }


  @book{Fukunaga:1990:ISP:92131,
  author = {Fukunaga, Keinosuke},
  title = {Introduction to statistical pattern recognition (2nd ed.)},
  year = {1990}
  }


  @ARTICLE{Roweis00nonlineardimensionality,
      author = {Sam T. Roweis and Lawrence K. Saul},
      title = {Nonlinear dimensionality reduction by locally linear embedding},
      journal = {SCIENCE},
      year = {2000},
      volume = {290}
  }

  @article{Turk_Pentland_1991,
  title={Face recognition using eigenfaces},
  journal={CVPR},
  year={1991}
  }


  @INPROCEEDINGS{Laptev03space-timeinterest,
      author = {Ivan Laptev and Tony Lindeberg},
      title = {Space-time Interest Points},
      booktitle = {ICCV},
      year = {2003}
  }


  @INPROCEEDINGS{Kim07r.:tensor,
      author = {Tae-kyun Kim and Shu-fai Wong and Roberto Cipolla},
      title = {Tensor Canonical Correlation Analysis for Action Classification},
      booktitle = {CVPR},
      year = {2007}
  }

  @ARTICLE{Shao_trackingalgorithm,
      author = {Jie Shao and Shaohua Kevin Zhou},
      title = {Tracking Algorithm Using Background-Foreground Motion Models and Multiple Cues},
      journal = {ICASSP}
  }
  @INPROCEEDINGS{Taylor03fusionof,
      author = {Geoffrey Taylor and Lindsay Kleeman},
      title = {Fusion of Multimodal Visual Cues for Model-Based Object Tracking},
      booktitle = {ACRA},
      year = {2003}
  }

  @inproceedings{DBLP:conf/accv/KumarBD07,
    author    = {Pankaj Kumar and
		Michael J. Brooks and
		Anthony R. Dick},
    title     = {Adaptive Multiple Object Tracking Using Colour and Segmentation
		Cues},
    booktitle = {ACCV},
    year      = {2007}
  }

  @InProceedings{rodriguez11b,
    author = "Rodriguez, M. and Sivic, J. and Laptev, I. and Audibert, J.-Y.",
    title = "Density-aware person detection and tracking in crowds",
    booktitle = "ICCV",
    year = "2011"
  }

  @inproceedings{Fragkiadaki:topology,
  author = {Fragkiadaki, Katerina and Shi, Jianbo},
  title = {Exploiting Motion and Topology for Segmenting and tracking Under Entanglement.},
  booktitle = {CVPR},
  year = {2011},
  }



@inproceedings{DBLP:conf/eccv/WangM08,
  author    = {Yang Wang and
               Greg Mori},
  title     = {Multiple Tree Models for Occlusion and Spatial Constraints
               in Human Pose Estimation},
  booktitle = {ECCV},
  year      = {2008}
}



  @InProceedings{BourdevPoseletsECCV10,
    author       = "Lubomir Bourdev and Subhransu Maji and Thomas Brox and Jitendra Malik",
    title        = "Detecting People Using Mutually Consistent Poselet Activations",
    booktitle    = "ECCV",
    year         = "2010",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }

  @inproceedings{partsagain,
  author = {Michael Maire and Stella Yu and Pietro Perona},
  title = {Object Detection and Segmentation from Joint Embedding of Parts and Pixels},
  booktitle = {ICCV},
  year = {2011},
  }

  @INPROCEEDINGS{Jianbo03multiclassspectral,
      author = {Yu,Stella and Shi, Jianbo},
      title = {Multiclass Spectral Clustering},
      booktitle = {ICCV},
      year = {2003}
  }



  @INPROCEEDINGS{lu_cvpr2011,
      author = {Wei-Lwun Lu and Jo-Anne Ting and Kevin P. Murphy and James J. Little},
      booktitle = {Identifying Players in Broadcast Sports Videos using Conditional Random Fields},
      journal = {Proceedings of the 2011 IEEE Conference on Computer Vision and Pattern Recognition},
      year = {2011}
  }

  @article{DBLP:journals/pami/BoykovVZ01,
    author    = {Yuri Boykov and Olga Veksler and Ramin Zabih},
    title     = {Fast Approximate Energy Minimization via Graph Cuts},
    journal   = {TPAMI},
    volume    = {23},
    year      = {2001}
  }

  @article{GEAN:GEAN31,
  author = {Matula, David W. and Sokal, Robert R.},
  title = {Properties of Gabriel Graphs Relevant to Geographic Variation Research and the Clustering of Points in the Plane},
  journal = {Geographical Analysis},
  volume = {12},
  year = {1980}
  }


  @INPROCEEDINGS{global_Pb,
  AUTHOR = {Michael Maire and Pablo Arbelaez and Charless Fowlkes and Jitendra Malik},
  TITLE = {Using contours to detect and localize junctions in natural images.},
  booktitle = {CVPR},
  YEAR = {2008}
  }


  @inproceedings{Yu:2010:AIO:1873951.1874105,
  author = {Yu, Haonan and Li, Jia and Tian, Yonghong and Huang, Tiejun},
  title = {Automatic interesting object extraction from images using complementary saliency maps},
  booktitle = {Proceedings of the international conference on Multimedia},
  year = {2010}
  }
  @inproceedings{DBLP:conf/accv/DonoserRB09,
    author    = {Michael Donoser and Hayko Riemenschneider and  Horst Bischof},
    title     = {Efficient Partial Shape Matching of Outer Contours},
    booktitle = {ACCV},
    year      = {2009}
  }

  @inproceedings{DBLP:conf/eccv/RiemenschneiderDB10,
    author    = {Hayko Riemenschneider and Michael Donoser and Horst Bischof},
    title     = {Using Partial Edge Contour Matches for Efficient Object
		Category Localization},
    booktitle = {ECCV},
    year      = {2010}
  }

  @inproceedings{Latecki2010,
    author    = {Tianyang Ma and Longin Jan Latecki},
    title     = { From Partial Shape Matching through Local Deformation to Robust Global Shape Similarity for Object Detection},
    booktitle = {CVPR},
    year      = {2011}
  }



  @ARTICLE{Wang94representingmoving,
      author = {Y. A. Wang and H. Adelson},
      title = {Representing Moving Images with Layers},
      journal = {TIP},
      year = {1994},
  }

  @InProceedings{Fradet09a,
    author = {Fradet, Matthieu and Robert, Philippe and P\'{e}rez, Patrick},
    Title = {Clustering point trajectories with various life-spans},
    BookTitle = {CVMP},
  year={2009}
  }





  @article{10.1109/ICCV.2001.10061,
  author = {Stella X. Yu and Jianbo Shi},
  title = {Segmentation with Pairwise Attraction and Repulsion},
  journal ={ICCV},
  Volume={75},
  year = {2001},
  }

  @article{1286005,
  author = {Wu, Bo and Nevatia, Ram},
  title = {Detection and Tracking of Multiple, Partially Occluded Humans by Bayesian Combination of Edgelet based Part Detectors},
  journal = {IJCV},
  year = {2007},
  }

  @inproceedings{bibbyeccv08,
    author = {C. Bibby and I. Reid},
    title = {Robust Real-Time Visual Tracking using Pixel-Wise Posteriors},
    booktitle={ECCV},
    year = "2008",
  }

  ]
  @InProceedings{BroxSegmentationCVPR11,
    author       = "Thomas Brox and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Object Segmentation by Alignment of Poselet Activations to Image Contours",
    booktitle    = "CVPR",
    year         = "2011"
  }

  @article{10.1109/ICCV.1995.466815,
  author = {J. Costeira and T. Kanade},
  title = {A multi-body factorization method for motion analysis},
  journal ={ICCV},
  year = {1995},
  }

  @inproceedings{Efros_2006_5395,
    author = "Bryan C. Russell and AlexeiA. Efros and Josef Sivic and William T. Freeman and Andrew Zisserman",
    title = "Using Multiple Segmentations to Discover Objects and their Extent in Image Collections",
    booktitle = "CVPR",
    year = "2006",
  }

  @inproceedings{malisiewicz-bmvc07,
    Author =	 {Tomasz Malisiewicz and Alexei A. Efros},
    Booktitle =	 {BMVC},
    Title =	 {Improving Spatial Support for Objects via Multiple Segmentations},
    Year =	 2007
  }

  @ARTICLE{1273918,
  author={Martin, D.R. and Fowlkes, C.C. and Malik, J.},
  journal={TPAMI},
  title={Learning to detect natural image boundaries using local brightness, color, and texture cues},
  year={2004},
  volume={26}
  }
@INPROCEEDINGS{Brox04highaccuracy,
    author = {Thomas Brox and Andrï¿œs Bruhn and Nils Papenberg and Joachim Weickert},
    title = {High Accuracy Optical Flow Estimation Based on a Theory for Warping},
    booktitle = {},
    year = {2004},
    pages = {25--36},
    publisher = {Springer}
}

 


  @INPROCEEDINGS{5539818,
  author={Bibby, C. and Reid, I.},
  booktitle={CVPR},
  title={Real-time tracking of multiple occluding objects using level sets},
  year={2010}}


  @inproceedings{Mitzel:2010:MTS:1886063.1886094,
  author = {Mitzel, Dennis and Horbert, Esther and Ess, Andreas and Leibe, Bastian},
  title = {Multi-person tracking with sparse detection and continuous segmentation},
  booktitle = {ECCV},
  year={2010}
  }

  @inproceedings{Mitzel:2011:MTS:1886063.1886094,
  author = {Mitzel, Dennis and Horbert, Esther and Ess, Andreas and Leibe, Bastian},
  title = {Level-Set Person Segmentation and Tracking with Multi-Region Appearemnce Models and Top-Down Shape Information},
  booktitle = {ICCV},
  series = {2011}
  }


  @InProceedings{lezama11,
    author = {Lezama, J. and Alahari, K. and Sivic, J. and Laptev, I.},
    title = {Track to the Future: Spatio-temporal Video Segmentation with Long-range Motion Cues},
    booktitle = {CVPR},
    year = {2011}
  }
  @InProceedings{shuwang2,
    author = {Shu Wang and Huchuan Lu and Fan Yang and Ming-Hsuan Yang},
    title = {Superpixel Tracking},
    booktitle = {ICCV},
    year = {2011}
  }
  @InProceedings{OB11,
    author       = "P.Ochs and T.Brox",
    title        = "Object segmentation in video: a hierarchical variational approach for turning point trajectories into dense regions",
    booktitle    = "ICCV",
    year         = "2011"}
  @incollection {springerlink:10.1007/978-3-642-15555-0_27,
    author = {Rahtu, Esa and Kannala, Juho and Salo, Mikko and Heikkilï¿œ, Janne},
    affiliation = {Machine Vision Group, University of Oulu, Finland},
    title = {Segmenting Salient Objects from Images and Videos},
    booktitle = {ECCV},
    year={2010},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }
@INPROCEEDINGS{Gall09motioncapture,
    author = {Juergen Gall and Carsten Stoll and Edilson De Aguiar and Christian Theobalt and Bodo Rosenhahn and Hans-peter Seidel and Mpi Informatik},
    title = {Motion capture using joint skeleton tracking and surface estimation},
    booktitle = {In IEEE Conf. on Computer Vision and Pattern Recognition},
    year = {2009}
}

  @Article{19146246,
  TITLE = {On the plausibility of the discriminant center-surround hypothesis for visual saliency.},
  AUTHOR = {Gao, Dashan and Mahadevan, Vijay and Vasconcelos, Nuno},
  journal = {Journal of vision},
  volume = {8},
  year = {2008}
  }


  @Article{Mahadevan10spatiotemporalsaliency,
      author = {Vijay Mahadevan and Nuno Vasconcelos},
      title = {Spatiotemporal Saliency in Dynamic Scenes},
      journal = {TPAMI},
      volume = {32},
      year = {2010},
  }


  @InProceedings{background_subtraction_free_camera,
    author = {Yaser Sheikh, Omar Javed, and Takeo Kanade},
    title = {Background Subtraction for Freely Moving Cameras},
    booktitle = {ICCV},
    year = {2009},
  }
  @conference{vondrick2010,
    title={Efficiently Scaling Up Video Annotation with Crowdsourced Marketplaces},
    author={Carl Vondrick and Deva Ramanan and Donald Patterson},
    booktitle={ECCV},
    year = {2010},
  }

  @conference{StellaRepulsion,
      author = {Stella X. Yu and Jianbo Shi},
      title = {Understanding Popout through Repulsion},
      booktitle= {CVPR},
      year={2001},
  }

  
  
  @article{DBLP:journals/corr/RanzatoSBMCC14,
  author    = {Marc'Aurelio Ranzato and
               Arthur Szlam and
               Joan Bruna and
               Micha{\"{e}}l Mathieu and
               Ronan Collobert and
               Sumit Chopra},
  title     = {Video (language) modeling: a baseline for generative models of natural
               videos},
  journal   = {CoRR},
  volume    = {abs/1412.6604},
  year      = {2014},
  url       = {http://arxiv.org/abs/1412.6604},
  timestamp = {Thu, 01 Jan 2015 19:51:08 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RanzatoSBMCC14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @article{10.1109/TPAMI.2009.167,
  author = {Pedro F. Felzenszwalb and Ross B. Girshick and David McAllester and Deva Ramanan},
  title = {Object Detection with Discriminatively Trained Part-Based Models},
  journal ={TPAMI},
    year = {2010},
  volume={32},
  }

@inproceedings{DBLP:conf/iccv/GirshickSKCF11,
  author    = {Ross B. Girshick and
               Jamie Shotton and
               Pushmeet Kohli and
               Antonio Criminisi and
               Andrew W. Fitzgibbon},
  title     = {Efficient regression of general-activity human poses from
               depth images},
  booktitle = {ICCV},
  year      = {2011},
  pages     = {415-422},
  ee        = {http://dx.doi.org/10.1109/ICCV.2011.6126270},
  crossref  = {DBLP:conf/iccv/2011},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


  @INPROCEEDINGS{Avidan05ensembletracking,
      author = {Shai Avidan},
      title = {Ensemble Tracking},
      booktitle = {CVPR},
      year = {2005},
  }

  @INPROCEEDINGS{planningtracking,
      author = {Haifeng Gong and Jack Simy and Maxim Likhachev and Jianbo Shi},
      title = {Multi-hypothesis Motion Planning for Visual Object Tracking},
      booktitle = {ICCV},
      year = {2011},
  }

  @incollection {SLIC,
    title={SLIC Superpixels},
    author={Radhakrishna Achanta and Appu Shaji and Kevin Smith and Aurelien Lucchi and Pascal Fua and Sabine Susstrunk},
    booktitle={EPFL Technical Report no. 149300, June 2010},
  }

  @incollection {springerlink:10.1007/978-3-540-88688-4_58,
    author = {Huang, Chang and Wu, Bo and Nevatia, Ramakant},
    title = {Robust Object Tracking by Hierarchical Association of Detection Responses},
    booktitle = {ECCV},
    year={2008},
  }

  @inproceedings{DBLP:conf/cvpr/CechS07,
    author    = {Jan Cech and Radim S{\'a}ra},
    title     = {Efficient Sampling of Disparity Space for Fast And Accurate Matching},
    booktitle = {CVPR},
    year      = {2007}
  }
  @inproceedings{DBLP:conf/iccv/PellegriniESG09,
    author    = {Stefano Pellegrini and
		Andreas Ess and
		Konrad Schindler and
		Luc J. Van Gool},
    title     = {You'll never walk alone: Modeling social behavior for multi-target
		tracking},
    booktitle = {ICCV},
    year      = {2009}
  }
  @INPROCEEDINGS{Yu02concurrentobject,
      author = {Stella X. Yu and Ralph Gross and Jianbo Shi},
      title = {Concurrent Object Recognition and Segmentation by Graph Partitioning},
      booktitle = {NIPS},
      year = {2002}
  }

  @InProceedings{eth_biwi_00483,
    author = {B. Leibe and N. Cornelis and K. Cornelis and L. Van Gool},
    title = {Dynamic 3D Scene Analysis from a Moving Vehicle},
    booktitle = {CVPR},
    year = {2007},
  }
@inproceedings{DBLP:conf/eccv/Black92,
  author    = {Michael J. Black},
  title     = {Combining Intensity and Motion for Incremental Segmentation
               and Tracking Over Long Image Sequences},
  booktitle = {ECCV},
  year      = {1992},
  pages     = {485-493},
  ee        = {http://dx.doi.org/10.1007/3-540-55426-2_54},
  crossref  = {DBLP:conf/eccv/1992},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}
  @article{10.1109/TPAMI.2010.143,
  author = {Thomas Brox and Jitendra Malik},
  title = {Large Displacement Optical Flow: Descriptor Matching in Variational Motion Estimation},
  journal ={TPAMI},
  year = {2010},

  }
  @inproceedings{citeulike:9244127,
      author = {Li, Yuan and Huang, Chang and Nevatia, R.},
    booktitle = {CVPR},
      title = {Learning to associate: HybridBoosted multi-target tracker for crowded scene},
      year = {2009}
  }


  @article {springerlink:10.1007/s11263-008-0136-6,
  title = {Particle Video: Long-Range Motion Estimation Using Point Trajectories},
    author = {Sand, Peter and Teller, Seth},
    affiliation = {MIT Computer Science and Artificial Intelligence Laboratory Cambridge MA 02139 USA},
    journal = {IJCV},
    year = {2008}
  }
  @INPROCEEDINGS{Dalal05histogramsof,
      author = {Navneet Dalal and Bill Triggs},
      title = {Histograms of Oriented Gradients for Human Detection},
      booktitle = {CVPR},
      year = {2005}
  }

  @InProceedings{yma,
    author = { Rao, S. and Tron, R. and Vidal, R. and Ma, Y. },
    title = {Motion segmentation via robust subspace separation in the presence of outlying, incomplete, or corrupted trajectories.},
    booktitle = {CVPR},
  year={2008},
  }

  @inproceedings{Grabner:2008:SOB:1478392.1478414,
  author = {Grabner, Helmut and Leistner, Christian and Bischof, Horst},
  title = {Semi-supervised On-Line Boosting for Robust Tracking},
  booktitle = {ECCV},
  year = {2008},
  }


  @inproceedings{citeulike:2085974,
      author = {Grabner , H. and Bischof, H.},
    title = {Online Boosting and Vision},
      booktitle = {CVPR},
      year = {2006}
  }

  @INPROCEEDINGS{5573752,
  author={Zhang Tao and Fei Shumin and Hu Gang},
  booktitle={Control Conference (CCC)},
  title={Target tracking with particle filter based on multiple cues fusion},
  year={2010}}

  @INPROCEEDINGS{Okuma04aboosted,
      author = {Kenji Okuma and Ali Taleghani and Nando De Freitas and O De Freitas and James J. Little and David G. Lowe},
      title = {A Boosted Particle Filter: Multitarget Detection and Tracking},
      booktitle = {ECCV},
      year = {2004},
  }


  @InProceedings{sparsesubsp,
    author = {Elhamifar, E. and Vidal, R.},
    title = {Sparse subspace clustering},
    booktitle = {CVPR},
    year = {2009}
  }




  @INPROCEEDINGS{BrostowCipollaCVPR2006,
    AUTHOR       = {Gabriel J. Brostow and Roberto Cipolla},
    TITLE        = {Unsupervised Bayesian Detection of Independent Motion in Crowds},
    BOOKTITLE    = {CVPR},
    YEAR         = {2006},
  }
  @article{GrundmannKwatra2010,
    author = {Matthias Grundmann and Vivek Kwatra and Mei Han and Irfan Essa},
    title = {Efficient Hierarchical Graph Based Video Segmentation},
    journal = {CVPR},
    year = {2010},
  }



  @incollection {mhvs,
    author = {Amelio Vazquez-Reina and Shai Avidan and Hanspeter Pfister and Eric Miller},
    title = {Multiple Hypothesis Video Segmentation from Superpixel Flows},
    booktitle = {ECCV},
  year={2010},
  }



  @article{phycho,
    author = {H. C. Nothdurft},
    title = {Feature analysis and the role of similarity in preattentive vision},
    journal = {Perception and Psychophysics},
    volume={52},
    year = {1992},
  }




  @article{commonfate,
    author = {M. Wertheimer},
    title = {Laws of organization in perceptual forms},
    journal = {A Sourcebook of Gestalt Psycycholgy (Partial translation)},
    year = {1938},
  }

  @INPROCEEDINGS{5206727,
  author={Chunhui Gu and Lim, J.J. and Arbelaez, P. and Malik, J.},
  booktitle={CVPR},
  year={2009},
  title={Recognition using regions},
  }
  @InProceedings{citeulike:942103,
      title = {Bottom-up/top-down image parsing by attribute graph grammar},
      author = {Han, Feng and Zhu, Song-Chun},
      journal = {ICCV},
  year={ 2005},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {CVPR},
    year={2009}
  }



  @InProceedings{Yan06general,
    title     = {A General Framework for Motion Segmentation: Independent, Articulated, Rigid, Non-rigid, Degenerate and Non-degenerate.},
    author = {J. Yan and M. Pollefeys},
    booktitle = {ECCV},
  year={2006},
  }

  @InProceedings{Ayer,
    title     = {Layered representation of motion video using robust maximum-likelihood estimation of mixture models and MDL encoding},
    author = {S. Ayer and H. S. Sawhney},
    booktitle = {ICCV},
  year={1995},
  }

  @article{101109CVPR2005335,
  author = {Deva Ramanan and D. A. Forsyth and Andrew Zisserman},
  title = {Strike a Pose: Tracking People by Finding Stylized Poses},
  journal ={CVPR},
  year = {2005},
  }

  @inproceedings{DBLP:conf/iccv/CheriyadatR09,
    author    = {Anil Cheriyadat and
		Richard J. Radke},
    title     = {Non-negative matrix factorization of partial track data
		for motion segmentation},
    booktitle = {ICCV},
    year      = {2009}
  }




  @inproceedings{Hoiem_2006_5467,
    author = "Derek Hoiem and Alexei Efros and Martial Hebert",
    title = "Putting Objects in Perspective",
    booktitle = "CVPR",
    year = "2006",
  }


  @Article{ Perse2009612,
  title = "A trajectory-based analysis of coordinated team activity in a basketball game",
  journal = "Computer Vision and Image Understanding",
  volume = "113",
  year = "2009",
  }

  @inproceedings{morariu11eventstructure,
    author    = {Vlad I. Morariu and Larry S. Davis},
    title     = {Multi-agent event recognition in structured scenarios.},
    booktitle = {CVPR},
    year      = {2011}
  }


  @inproceedings{storyline,
    author    = {Abhinav Gupta and Praveen Srinivasan and Jianbo Shi and Larry S. Davis},
    title     = {Understanding videos, constructing plots learning a visually grounded storyline model from annotated videos},
    booktitle = {CVPR},
    year      = {2009}
  }

  @inproceedings{benfold2011stable,
	  author = {Benfold, Ben and Reid, Ian},
	  title = {Stable Multi-Target Tracking in Real-Time Surveillance Video},
	  booktitle = {CVPR},
	  year = {2011}
  }


  @ARTICLE{790429,
  author={Wilson, A.D. and Bobick, A.F.},
  journal={TPAMI},
  title={Parametric hidden Markov models for gesture recognition},
  year={1999},
  volume={21}
  }



  @article{experts,
  author = {Terence D. Sanger and Robert A. Jacobs and Steven J. Nowlan and Geoffrey E. Hinton},
  title = {Adaptive Mixtures of Local Experts},
  journal = {Neural Computation},
  volume = {3},
  year = {1991}
  }


  @INPROCEEDINGS{lips,
  author={Bregler, C. and Omohundro, S.M.},
  booktitle={ICCV},
  title={Nonlinear manifold learning for visual speech recognition},
  year={1995}
  }



  @inproceedings{BN,
  author = {Shaogang Gong and Tao Xiang},
  title = {Recognition of Group Activities using Dynamic Probabilistic Networks},
  booktitle = {ICCV},
  year={2003}
  }


  @article{HMMMO,
  author = {Aaron F. Bobick and Andrew D. Wilson},
  title = {A State-Based Approach to the Representation and Recognition of Gesture},
  journal = {TPAMI},
  volume = {19}
  }

  @inproceedings{Brand:1997:CHM:794189.794420,
  author = {Brand, M. and Oliver, N. and Pentland, A.},
  title = {Coupled hidden Markov models for complex action recognition},
  booktitle = {CVPR},
  year = {1997}
  }

  @article{Ghahramani:1997:FHM:274158.274165,
  author = {Ghahramani, Zoubin and Jordan, Michael I.},
  title = {Factorial Hidden Markov Models},
  journal = {Mach. Learn.},
  volume = {29},
  year = {1997}
  }


  @INPROCEEDINGS{4270099,
  author={Laxton, B. and Jongwoo Lim and Kriegman, D.},
  booktitle={CVPR},
  title={Leveraging temporal, contextual and ordering constraints for recognizing complex activities in video},
  year={2007}
  }


  @article{DBLP:journals/jmlr/SiracusaF09,
    author    = {Michael Siracusa and John Fisher},
    title     = {Tractable Bayesian Inference of Time-Series Dependence Structure},
    journal   = {Journal of Machine Learning Research - Proceedings Track},
    volume    = {5},
    year      = {2009}
  }



  @article{parametrized,
  author = {Yaser Yacoob and Michael J. Black},
  title = {Parameterized Modeling and Recognition of Activities},
  journal = {Computer Vision and Image Understanding},
  volume = {73},
  year = {1999}
  }




  @inproceedings{Bobick:1995:STS:839277.840051,
  author = {Bobick, A. F. and Wilson, A. D.},
  title = {A state-based technique for the summarization and recognition of gesture},
  booktitle = {ICCV},
  year = {1995}
  }


  @inproceedings{Niebles:2010:MTS:1888028.1888059,
  author = {Niebles, Juan Carlos and Chen, Chih-Wei and Fei-Fei, Li},
  title = {Modeling temporal structure of decomposable motion segments for activity classification},
  booktitle = {ECCV},
  year = {2010}
  }


  @article{Hakeem:2007:LDR:1265999.1266287,
  author = {Hakeem, Asaad and Shah, Mubarak},
  title = {Learning, detection and representation of multi-agent events in videos},
  journal = {Artif. Intell.},
  volume = {171},
  year = {2007}
  }



  @INPROCEEDINGS{Zelnik-manor01event-basedanalysis,
      author = {Lihi Zelnik-manor and Michal Irani},
      title = {Event-based analysis of video},
      booktitle = {CVPR},
      year = {2001}
  }

  @inproceedings{Jebara:2007:SCE:1421665.1421685,
  author = {Jebara, Tony and Song, Yingbo and Thadani, Kapil},
  title = {Spectral Clustering and Embedding with Hidden Markov Models},
  booktitle = {European conference on Machine Learning},
  year = {2007}
  }
  @article{10.1109/CVPR.1997.609375,
  author = {Yair Weiss},
  title = {Smoothness in Layers: Motion segmentation using nonparametric mixture estimation.},
  journal ={CVPR},
  year={1997},

  }

  @article{ncut,
  author = {Jianbo Shi and Jitendra Malik},
  title = {Normalized Cuts and Image Segmentation},
  journal = {TPAMI},
  year = {2000},
  }


  @article{10.1109/TPAMI.2005.202,
  author = {Jiangjian Xiao and Mubarak Shah},
  title = {Motion Layer Extraction in the Presence of Occlusion Using Graph Cuts},
  journal ={TPAMI},
  year = {2005},
  }

  @article{1340323,
  author = {Pawan Kumar, M. and Torr, P. H. and Zisserman, A.},
  title = {Learning Layered Motion Segmentations of Video},
  journal = {IJCV},
  volume = {76},
  year = {2008},
  }



  @ARTICLE{Wang94representingmoving,
      author = {Y. A. Wang and H. Adelson},
      title = {Representing Moving Images with Layers},
      journal = {TIP},
      year = {1994},
  }

  @InProceedings{Fradet09a,
    author = {Fradet, Matthieu and Robert, Philippe and P\'{e}rez, Patrick},
    Title = {Clustering point trajectories with various life-spans},
    BookTitle = {CVMP},
  year={2009}
  }

@incollection{has,
year={2012},
booktitle={ECCV},
title={Has My Algorithm Succeeded? An Evaluator for Human Pose Estimators},
author={Jammalamadaka, Nataraj and Zisserman, Andrew and Eichner, Marcin and Ferrari, Vittorio and Jawahar, C.V.},

}




  @article{10.1109/ICCV.2001.10061,
  author = {Stella X. Yu and Jianbo Shi},
  title = {Segmentation with Pairwise Attraction and Repulsion},
  journal ={ICCV},
  Volume={75},
  year = {2001},
  }

  @article{1286005,
  author = {Wu, Bo and Nevatia, Ram},
  title = {Detection and Tracking of Multiple, Partially Occluded Humans by Bayesian Combination of Edgelet based Part Detectors},
  journal = {IJCV},
  year = {2007},
  }


  @inproceedings{DBLP:conf/iccv/CheriyadatR09,
    author    = {Anil Cheriyadat and
		Richard J. Radke},
    title     = {Non-negative matrix factorization of partial track data
		for motion segmentation},
    booktitle = {ICCV},
    year      = {2009},
    pages     = {865-872},
    ee        = {http://dx.doi.org/10.1109/ICCV.2009.5459311},
    crossref  = {DBLP:conf/iccv/2009},
    bibsource = {DBLP, http://dblp.uni-trier.de}
  }

  @article{Canny86,
      author = {Canny, J.},
      journal = {TPAMI},
      title = {{A Computational Approach to Edge Detection}},
      url = {http://dx.doi.org/10.1109/TPAMI.1986.4767851},
      volume = {PAMI-8},
      year = {1986}
  }

  @article{10.1109/ICCV.1995.466815,
  author = {J. Costeira and T. Kanade},
  title = {A multi-body factorization method for motion analysis},
  journal ={ICCV},
  year = {1995},
  }

  @ARTICLE{1273918,
  author={Martin, D.R. and Fowlkes, C.C. and Malik, J.},
  journal={TPAMI},
  title={Learning to detect natural image boundaries using local brightness, color, and texture cues},
  year={2004},
  volume={26}
  }

  @INPROCEEDINGS{139492,
  author={Perona, P. and Malik, J.},
  booktitle={ICCV},
  title={Detecting and localizing edges composed of steps, peaks and roofs },
  year={1990}
  }

 

  @incollection {springerlink:10.1007/978-3-642-15555-0_27,
    author = {Rahtu, Esa and Kannala, Juho and Salo, Mikko and Heikkilï¿œ, Janne},
    affiliation = {Machine Vision Group, University of Oulu, Finland},
    title = {Segmenting Salient Objects from Images and Videos},
    booktitle = {ECCV},
    year={2010},
  }
  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }
  
  @inproceedings{chaplot2020semantic,
  title={Semantic curiosity for active visual learning},
  author={Chaplot, Devendra Singh and Jiang, Helen and Gupta, Saurabh and Gupta, Abhinav},
  booktitle={European Conference on Computer Vision},
  pages={309--326},
  year={2020},
  organization={Springer}
}

  @Article{19146246,
  TITLE = {On the plausibility of the discriminant center-surround hypothesis for visual saliency.},
  AUTHOR = {Gao, Dashan and Mahadevan, Vijay and Vasconcelos, Nuno},
  journal = {Journal of vision},
  volume = {8},
  year = {2008}
  }


  @Article{Mahadevan10spatiotemporalsaliency,
      author = {Vijay Mahadevan and Nuno Vasconcelos},
      title = {Spatiotemporal Saliency in Dynamic Scenes},
      journal = {TPAMI},
      volume = {32},
      year = {2010},
  }


  @InProceedings{background_subtraction_free_camera,
    author = {Yaser Sheikh, Omar Javed, and Takeo Kanade},
    title = {Background Subtraction for Freely Moving Cameras},
    booktitle = {ICCV},
    year = {2009},
  }
  @conference{vondrick2010,
    title={Efficiently Scaling Up Video Annotation with Crowdsourced Marketplaces},
    author={Carl Vondrick and Deva Ramanan and Donald Patterson},
    booktitle={ECCV},
    year = {2010},
  }

  @conference{StellaRepulsion,
      author = {Stella X. Yu and Jianbo Shi},
      title = {Understanding Popout through Repulsion},
      booktitle= {CVPR},
      year={2001},
  }

  @article{10.1109/TPAMI.2009.167,
  author = {Pedro F. Felzenszwalb and Ross B. Girshick and David McAllester and Deva Ramanan},
  title = {Object Detection with Discriminatively Trained Part-Based Models},
  journal ={TPAMI},
    year = {2010},
  volume={32},
  }

  @inproceedings{Datta_2008_6037,
   author = "Ankur Datta and Yaser Ajmal Sheikh and Takeo Kanade",
   title = "Linear Motion Estimation for Systems of Articulated Planes",
   booktitle = "IEEE Conference on Computer Vision and Pattern Recognition",
   month = "June",
   year = "2008",
}

@INPROCEEDINGS{motionperception,
    author = {Gunnar Johansson},
    title = {Visual perception of biological motion and a model for its analysis},
    booktitle = {Percept. Psychophys.},
    year = {1973},
    volume={14},
    pages = {201--211}
}

@article{Sigal:2012:LPE:2205801.2205829,
 author = {Sigal, Leonid and Isard, Michael and Haussecker, Horst and Black, Michael J.},
 title = {Loose-limbed People: Estimating {3D} Human Pose and Motion Using Non-parametric Belief Propagation},
 journal = {IJCV},
 volume = {98},
 year = {2012}
}
@inproceedings{conf/cvpr/SappWT11,
  added-at = {2011-08-23T00:00:00.000+0200},
  author = {Sapp, Benjamin and Weiss, David and Taskar, Ben},
  booktitle = {CVPR},
  title = {Parsing human motion with stretchable models.},
  year = 2011
}





@inproceedings{DBLP:conf/fgr/JuBY96,
  author    = {Shanon X. Ju and
               Michael J. Black and
               Yaser Yacoob},
  title     = {Cardboard People: A Parameterized Model of Articulated Image
               Motion},
  booktitle = {FG},
  year      = {1996},
}

@InProceedings{Bro06k,
  author       = "T. Brox and B. Rosenhahn and D. Cremers and H.-P. Seidel",
  title        = "High accuracy optical flow serves 3-D pose tracking: exploiting contour and flow based constraints",
  booktitle    = "ECCV",
  year         = "2006"
}

  @incollection {SLIC,
    title={SLIC Superpixels},
    author={Radhakrishna Achanta and Appu Shaji and Kevin Smith and Aurelien Lucchi and Pascal Fua and Sabine Susstrunk},
    booktitle={EPFL Technical Report no. 149300, June 2010},
  }

  @incollection {springerlink:10.1007/978-3-540-88688-4_58,
    author = {Huang, Chang and Wu, Bo and Nevatia, Ramakant},
    title = {Robust Object Tracking by Hierarchical Association of Detection Responses},
    booktitle = {ECCV},
    year={2008},
  }

  @InProceedings{eth_biwi_00483,
    author = {B. Leibe and N. Cornelis and K. Cornelis and L. Van Gool},
    title = {Dynamic 3D Scene Analysis from a Moving Vehicle},
    booktitle = {CVPR},
    year = {2007},
  }

  @article{10.1109/TPAMI.2010.143,
  author = {Thomas Brox and Jitendra Malik},
  title = {Large Displacement Optical Flow: Descriptor Matching in Variational Motion Estimation},
  journal ={TPAMI},
  year = {2010},

  }


  @article {springerlink:10.1007/s11263-008-0136-6,
  title = {Particle Video: Long-Range Motion Estimation Using Point Trajectories},
    author = {Sand, Peter and Teller, Seth},
    affiliation = {MIT Computer Science and Artificial Intelligence Laboratory Cambridge MA 02139 USA},
    journal = {IJCV},
    year = {2008}
  }

  @InProceedings{yma,
    author = { Rao, S. and Tron, R. and Vidal, R. and Ma, Y. },
    title = {Motion segmentation via robust subspace separation in the presence of outlying, incomplete, or corrupted trajectories.},
    booktitle = {CVPR},
  year={2008},
  }



  @InProceedings{sparsesubsp,
    author = {Elhamifar, E. and Vidal, R.},
    title = {Sparse subspace clustering},
    booktitle = {CVPR},
    year = {2009}
  }




  @INPROCEEDINGS{BrostowCipollaCVPR2006,
    AUTHOR       = {Gabriel J. Brostow and Roberto Cipolla},
    TITLE        = {Unsupervised Bayesian Detection of Independent Motion in Crowds},
    BOOKTITLE    = {CVPR},
    YEAR         = {2006},
  }
  @article{GrundmannKwatra2010,
    author = {Matthias Grundmann and Vivek Kwatra and Mei Han and Irfan Essa},
    title = {Efficient Hierarchical Graph Based Video Segmentation},
    journal = {CVPR},
    year = {2010},
  }



  @incollection {mhvs,
    author = {Amelio Vazquez-Reina and Shai Avidan and Hanspeter Pfister and Eric Miller},
    title = {Multiple Hypothesis Video Segmentation from Superpixel Flows},
    booktitle = {ECCV},
  year={2010},
  }
  @INPROCEEDINGS{4761133,
  author={Izadi, M. and Saeedi, P.},
  booktitle={Pattern Recognition, 2008. ICPR 2008. 19th International Conference on},
  title={Robust region-based background subtraction and shadow removing using color and gradient information},
  year={2008}
  }

  @INPROCEEDINGS{784637,
  author={Stauffer, C. and Grimson, W.E.L.},
  booktitle={CVPR},
  title={Adaptive background mixture models for real-time tracking},
  year={1999}}


  @inproceedings{Zivkovic:2004:IAG:1018428.1020644,
  author = {Zivkovic, Zoran},
  title = {Improved Adaptive Gaussian Mixture Model for Background Subtraction},
  booktitle = {ICPR},
  year = {2004}
  }


  @article{Felzenszwalb:2004:EGI:981793.981796,
  author = {Felzenszwalb, Pedro F. and Huttenlocher, Daniel P.},
  title = {Efficient Graph-Based Image Segmentation},
  journal = {IJCV},
  volume = {59},
  year = {2004}
  }

  @article{phycho,
    author = {H. C. Nothdurft},
    title = {Feature analysis and the role of similarity in preattentive vision},
    journal = {Perception and Psychophysics},
    volume={52},
    year = {1992},
  }

  @inproceedings{DBLP:conf/eccv/Ren08,
    author    = {Xiaofeng Ren},
    title     = {Multi-scale Improves Boundary Detection in Natural Images},
    booktitle = {ECCV (3)},
    year      = {2008},
    pages     = {533-545},
    ee        = {http://dx.doi.org/10.1007/978-3-540-88690-7_40},
    crossref  = {DBLP:conf/eccv/2008-3},
    bibsource = {DBLP, http://dblp.uni-trier.de}
  }


@article{DBLP:journals/corr/BalogGBNT16,
  author    = {Matej Balog and
               Alexander L. Gaunt and
               Marc Brockschmidt and
               Sebastian Nowozin and
               Daniel Tarlow},
  title     = {DeepCoder: Learning to Write Programs},
  journal   = {CoRR},
  volume    = {abs/1611.01989},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.01989},
  archivePrefix = {arXiv},
  eprint    = {1611.01989},
  timestamp = {Wed, 07 Jun 2017 14:43:01 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/BalogGBNT16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @INPROCEEDINGS{5206727,
  author={Chunhui Gu and Lim, J.J. and Arbelaez, P. and Malik, J.},
  booktitle={CVPR},
  year={2009},
  title={Recognition using regions},
  }
  @InProceedings{citeulike:942103,
      title = {Bottom-up/top-down image parsing by attribute graph grammar},
      author = {Han, Feng and Zhu, Song-Chun},
      journal = {ICCV},
  year={ 2005},
  }

  @InProceedings{eth_biwi_00633,
    author = {Michael D. Breitenstein and Fabian Reichlin and Bastian Leibe and Esther Koller-Meier and Luc Van Gool},
    title = {Robust Tracking-by-Detection using a Detector Confidence Particle Filter},
    booktitle = {ICCV},
    year = {2009},
  }

  @InProceedings{Yan06general,
    title     = {A General Framework for Motion Segmentation: Independent, Articulated, Rigid, Non-rigid, Degenerate and Non-degenerate.},
    author = {J. Yan and M. Pollefeys},
    booktitle = {ECCV},
  year={ 2006},
  }
@inproceedings{Datta_2008_6037,
   author = "Ankur Datta and Yaser Ajmal Sheikh and Takeo Kanade",
   title = "Linear Motion Estimation for Systems of Articulated Planes",
   booktitle = "IEEE Conference on Computer Vision and Pattern Recognition",
   month = "June",
   year = "2008",
}

  @InProceedings{Ayer,
    title     = {Layered representation of motion video using robust maximum-likelihood estimation of mixture models and MDL encoding},
    author = {S. Ayer and H. S. Sawhney},
    booktitle = {ICCV},
  year={ 1995}
  }

  @article{10.1109/CVPR.2005.335,
  author = {Deva Ramanan and D. A. Forsyth and Andrew Zisserman},
  title = {Strike a Pose: Tracking People by Finding Stylized Poses},
  journal ={CVPR},
  year = {2005}
  }









@inproceedings{SheikhNIPS2008,
   author = "Ijaz Akhter and Yaser Ajmal Sheikh and Sohaib Khan and Takeo Kanade",
   title = "Nonrigid Structure from Motion in Trajectory Space",
   booktitle = "NIPS",
   year = "2008"
} 


  @Article{ Perse2009612,
  title = "A trajectory-based analysis of coordinated team activity in a basketball game",
  journal = "Computer Vision and Image Understanding",
  volume = "113",
  year = "2009"
  }

  @inproceedings{morariu11eventstructure,
    author    = {Vlad I. Morariu and Larry S. Davis},
    title     = {Multi-agent event recognition in structured scenarios.},
    booktitle = {CVPR},
    year      = {2011}
  }


  @inproceedings{storyline,
    author    = {Abhinav Gupta and Praveen Srinivasan and Jianbo Shi and Larry S. Davis},
    title     = {Understanding videos, constructing plots learning a visually grounded storyline model from annotated videos},
    booktitle = {CVPR},
    year      = {2009}
  }


  @ARTICLE{790429,
  author={Wilson, A.D. and Bobick, A.F.},
  journal={TPAMI},
  title={Parametric hidden Markov models for gesture recognition},
  year={1999},
  volume={21}
  }



  @article{experts,
  author = {Terence D. Sanger and Robert A. Jacobs and Steven J. Nowlan and Geoffrey E. Hinton},
  title = {Adaptive Mixtures of Local Experts},
  journal = {Neural Computation},
  volume = {3},
  year = {1991}
  }

@article{anonymous2018zero-shot,
  title={Zero-Shot Visual Imitation},
  author={Anonymous},
  journal={International Conference on Learning Representations},
  year={2018},
  url={https://openreview.net/forum?id=BkisuzWRW}
}


  @INPROCEEDINGS{lips,
  author={Bregler, C. and Omohundro, S.M.},
  booktitle={ICCV},
  title={Nonlinear manifold learning for visual speech recognition},
  year={1995}
  }



  @inproceedings{BN,
  author = {Shaogang Gong and Tao Xiang},
  title = {Recognition of Group Activities using Dynamic Probabilistic Networks},
  booktitle = {ICCV},
  year={2003}
  }


  @article{HMMMO,
  author = {Aaron F. Bobick and Andrew D. Wilson},
  title = {A State-Based Approach to the Representation and Recognition of Gesture},
  journal = {TPAMI},
  volume = {19}
  }

  @inproceedings{Brand:1997:CHM:794189.794420,
  author = {Brand, M. and Oliver, N. and Pentland, A.},
  title = {Coupled hidden Markov models for complex action recognition},
  booktitle = {CVPR},
  year = {1997}
  }

  @article{Ghahramani:1997:FHM:274158.274165,
  author = {Ghahramani, Zoubin and Jordan, Michael I.},
  title = {Factorial Hidden Markov Models},
  journal = {Mach. Learn.},
  volume = {29},
  year = {1997}
  }


  @INPROCEEDINGS{4270099,
  author={Laxton, B. and Jongwoo Lim and Kriegman, D.},
  booktitle={CVPR},
  title={Leveraging temporal, contextual and ordering constraints for recognizing complex activities in video},
  year={2007}
  }


  @article{DBLP:journals/jmlr/SiracusaF09,
    author    = {Michael Siracusa and John Fisher},
    title     = {Tractable Bayesian Inference of Time-Series Dependence Structure},
    journal   = {Journal of Machine Learning Research - Proceedings Track},
    volume    = {5},
    year      = {2009}
  }



  @article{parametrized,
  author = {Yaser Yacoob and Michael J. Black},
  title = {Parameterized Modeling and Recognition of Activities},
  journal = {Computer Vision and Image Understanding},
  volume = {73},
  year = {1999}
  }




  @inproceedings{Bobick:1995:STS:839277.840051,
  author = {Bobick, A. F. and Wilson, A. D.},
  title = {A state-based technique for the summarization and recognition of gesture},
  booktitle = {ICCV},
  year = {1995}
  }

  @inproceedings{Xu:2008:SBV:1478392.1478446,
  author = {Xu, Li and Chen, Jianing and Jia, Jiaya},
  title = {A Segmentation Based Variational Model for Accurate Optical Flow Estimation},
  booktitle = {ECCV},
  year = {2008}
  }

  @inproceedings{Niebles:2010:MTS:1888028.1888059,
  author = {Niebles, Juan Carlos and Chen, Chih-Wei and Fei-Fei, Li},
  title = {Modeling temporal structure of decomposable motion segments for activity classification},
  booktitle = {ECCV},
  year = {2010}
  }

  @InProceedings{Bro11c,
    author       = "P. Sundberg and T. Brox and M. Maire and P. Arbelaez and J. Malik",
    title        = "Occlusion boundary detection and figure/ground assignment from optical flow",
    booktitle    = "CVPR",
    year         = "2011"
  }

  @inproceedings{Stein_2007_5836,
    author = "Andrew Stein and Derek Hoiem and Martial Hebert",
    title = "Learning to Find Object Boundaries Using Motion Cues",
    booktitle = "IEEE International Conference on Computer Vision (ICCV)",
    month = "October",
    year = "2007",
    Notes = "Dataset available from http://www.cs.cmu.edu/~stein/occlusion_data"
  }
  
  @inproceedings{Zhou2015EndtoendLO,
  title={End-to-end learning of semantic role labeling using recurrent neural networks},
  author={Jie Zhou and Wei Xu},
  booktitle={ACL},
  year={2015}
}


  @article{Hakeem:2007:LDR:1265999.1266287,
  author = {Hakeem, Asaad and Shah, Mubarak},
  title = {Learning, detection and representation of multi-agent events in videos},
  journal = {Artif. Intell.},
  volume = {171},
  year = {2007}
  }


  
  @INPROCEEDINGS{Zelnik-manor01event-basedanalysis,
      author = {Lihi Zelnik-manor and Michal Irani},
      title = {Event-based analysis of video},
      booktitle = {CVPR},
      year = {2001}
  }

  @inproceedings{Jebara:2007:SCE:1421665.1421685,
  author = {Jebara, Tony and Song, Yingbo and Thadani, Kapil},
  title = {Spectral Clustering and Embedding with Hidden Markov Models},
  booktitle = {European conference on Machine Learning},
  year = {2007}
  }

  @article{Jebara:2004:PPK:1005332.1016786,
  author = {Jebara, Tony and Kondor, Risi and Howard, Andrew},
  title = {Probability Product Kernels},
  journal = {J. Mach. Learn. Res.},
  volume = {5},
  year = {2004}
  }

  @INPROCEEDINGS{Gong99recognitionof,
      author = {Shaogang Gong and Michael Walter},
      title = {Recognition of Temporal Structures: Learning Prior and Propagating Observation Augmented Densities via Hidden Markov States},
      booktitle = {ICCV},
      year = {1999},
  }

  @article{Brand:2000:DSA:351581.351608,
  author = {Brand, Matthew and Kettnaker, Vera},
  title = {Discovery and Segmentation of Activities in Video},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }


  @INPROCEEDINGS{Brown01productsof,
      author = {Andrew D. Brown and Andrew D. Brown and Geoffrey E. Hinton and Geoffrey E. Hinton},
      title = {Products of Hidden Markov Models},
      booktitle = {In Proceedings of Artificial Intelligence and Statistics},
      year = {2001},
  }


  @inproceedings{malisiewicz-nips09,
    Author =	 {Tomasz Malisiewicz and Alexei A. Efros},
    Booktitle =	 {NIPS},
    Title =	 {Beyond Categories: The Visual Memex Model for Reasoning About Object Relationships},
    Year =	 2009
  }


  @inproceedings{yamato,
  author = {J. Yamato and J. Ohya and K. Ishii},
  title = {Recognizing human action in time-sequential images using a hidden Markov model},
  booktitle = {CVPR},
  year = {1994},
  }



  @INPROCEEDINGS{Elgammal04separatingstyle,
      author = {Ahmed Elgammal and Chan-su Lee},
      title = {Separating style and content on a nonlinear manifold},
      booktitle = {CVPR},
      year = {2004}
  }

  @INPROCEEDINGS{Tenenbaum97separatingstyle,
      author = {Joshua B. Tenenbaum and William T. Freeman},
      title = {Separating style and content},
      booktitle = {In Advances in neural},
      year = {1997}
  }

  @inproceedings{DBLP:conf/cvpr/LvN07,
    author    = {Fengjun Lv and
		Ramakant Nevatia},
    title     = {Single View Human Action Recognition using Key Pose Matching and Viterbi Path Searching},
    booktitle = {CVPR},
    year      = {2007}
  }


  @inproceedings { 158,
	  title = {Linear Embeddings in Non-Rigid Structure From Motion},
	  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	  year = {2009},
	  address = {Miami, FL},
	  author = {Vincent Rabaud and Serge Belongie}
  }



  @INPROCEEDINGS{4270260,
  author={Goh, A. and Vidal, R.},
  booktitle={CVPR},
  title={Segmenting Motions of Different Types by Unsupervised Manifold Clustering},
  year={2007},
  }


  @incollection {springerlink:10.1007/11551188_37,
    author = {Wang, Fei and Zhang, Changshui},
    title = {Spectral Clustering for Time Series},
    booktitle = {Pattern Recognition and Data Mining},
    volume = {3686},
    year = {2005}
  }

  @INPROCEEDINGS{4587385,
  author={Xiaozhe Wang and Liang Wang and Wirth, A.},
  booktitle={CVPR},
  title={Pattern discovery in motion time series via structure-based spectral clustering},
  year={2008}
  }


  @article{Stauffer:2000:LPA:351581.351588,
  author = {Stauffer, Chris and Grimson, W. Eric L.},
  title = {Learning Patterns of Activity Using Real-Time Tracking},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }

  @incollection{Nanopoulos:2001:FCT:766914.766918,
  author = {Nanopoulos, Alex and Alcock, Rob and Manolopoulos, Yannis},
  title = {Information processing and technology},
  year = {2001},
  }

  BibTeX | EndNote | ACM Ref

  @inproceedings{Shi:2006:LTS:1153171.1153641,
  author = {Shi, Yifan and Bobick, Aaron and Essa, Irfan},
  title = {Learning Temporal Sequence Model from Partially Labeled Data},
  booktitle = {CVPR},
  year = {2006}
  }


  @article{Murase,
  author = {Murase, Hiroshi and Nayar, Shree K.},
  title = {Visual learning and recognition of 3-D objects from appearance},
  journal = {IJCV},
  volume = {14},
  year = {1995}
  }


  @INPROCEEDINGS{698609,
  author={Bobick, A.F. and Ivanov, Y.A.},
  booktitle={CVPR},
  title={Action recognition using probabilistic parsing},
  year={1998}
  }

  @inproceedings{Ryoo:2006:RCH:1153171.1153651,
  author = {Ryoo, M. S. and Aggarwal, J. K.},
  title = {Recognition of Composite Human Activities through Context-Free Grammar Based Representation},
  booktitle = {CVPR},
  year = {2006}
  }


  @INPROCEEDINGS{Hadsell06dimensionalityreduction,
      author = {Raia Hadsell and Sumit Chopra and Yann Lecun},
      title = {Dimensionality reduction by learning an invariant mapping},
      booktitle = {CVPR},
      year = {2006}
  }


  @incollection{NIPS2010_0893,
  title = {Pose-Sensitive Embedding by Nonlinear NCA Regression},
  author = {Graham Taylor and Rob Fergus and George Williams and Ian Spiro and Christoph Bregler},
  booktitle = {NIPS},
  year = {2010}
  }
  @InProceedings{lezama11,
    author = {Lezama, J. and Alahari, K. and Sivic, J. and Laptev, I.},
    title = {Track to the Future: Spatio-temporal Video Segmentation with Long-range Motion Cues},
    booktitle = {CVPR},
    year = {2011}
  }
  @InProceedings{shuwang2,
    author = {Shu Wang and Huchuan Lu and Fan Yang and Ming-Hsuan Yang},
    title = {Superpixel Tracking},
    booktitle = {ICCV},
    year = {2011}
  }
  @InProceedings{OB11,
    author       = "P.Ochs and T.Brox",
    title        = "Object segmentation in video: a hierarchical variational approach for turning point trajectories into dense regions",
    booktitle    = "IEEE International Conference on Computer Vision (ICCV)",
    year         = "2011",
    url          = "http://lmb.informatik.uni-freiburg.de/Publications/2011/OB11"
  }

  @InProceedings{raptisS10,
    author = 	{Raptis, M. and Soatto, S.},
    title = 	{Tracklet Descriptors for Action Modeling and Video Analysis},
    booktitle = 	{ECCV},
    year = 	{2010}
  }


  @book{Fukunaga:1990:ISP:92131,
  author = {Fukunaga, Keinosuke},
  title = {Introduction to statistical pattern recognition (2nd ed.)},
  year = {1990}
  }


  @ARTICLE{Roweis00nonlineardimensionality,
      author = {Sam T. Roweis and Lawrence K. Saul},
      title = {Nonlinear dimensionality reduction by locally linear embedding},
      journal = {SCIENCE},
      year = {2000},
      volume = {290}
  }

  @article{Turk_Pentland_1991,
  title={Face recognition using eigenfaces},
  journal={CVPR},
  year={1991}
  }


  @INPROCEEDINGS{Laptev03space-timeinterest,
      author = {Ivan Laptev and Tony Lindeberg},
      title = {Space-time Interest Points},
      booktitle = {ICCV},
      year = {2003}
  }


  @INPROCEEDINGS{Kim07r.:tensor,
      author = {Tae-kyun Kim and Shu-fai Wong and Roberto Cipolla},
      title = {Tensor Canonical Correlation Analysis for Action Classification},
      booktitle = {CVPR},
      year = {2007}
  }


  @inproceedings{Fragkiadaki:topology,
  author = {Fragkiadaki, Katerina and Shi, Jianbo},
  title = {Exploiting Motion and Topology for Segmenting and tracking Under Entanglement.},
  booktitle = {CVPR},
  year = {2011},
  }

  @INPROCEEDINGS{Jianbo03multiclassspectral,
      author = {Yu,Stella and Shi, Jianbo},
      title = {Multiclass Spectral Clustering},
      booktitle = {ICCV},
      year = {2003}
  }



  @INPROCEEDINGS{lu_cvpr2011,
      author = {Wei-Lwun Lu and Jo-Anne Ting and Kevin P. Murphy and James J. Little},
      booktitle = {Identifying Players in Broadcast Sports Videos using Conditional Random Fields},
      journal = {Proceedings of the 2011 IEEE Conference on Computer Vision and Pattern Recognition},
      year = {2011}
  }

  @article{DBLP:journals/pami/BoykovVZ01,
    author    = {Yuri Boykov and Olga Veksler and Ramin Zabih},
    title     = {Fast Approximate Energy Minimization via Graph Cuts},
    journal   = {TPAMI},
    volume    = {23},
    year      = {2001}
  }

  @article{GEAN:GEAN31,
  author = {Matula, David W. and Sokal, Robert R.},
  title = {Properties of Gabriel Graphs Relevant to Geographic Variation Research and the Clustering of Points in the Plane},
  journal = {Geographical Analysis},
  volume = {12},
  year = {1980}
  }


  @INPROCEEDINGS{global_Pb,
  AUTHOR = {Michael Maire and Pablo Arbelaez and Charless Fowlkes and Jitendra Malik},
  TITLE = {Using contours to detect and localize junctions in natural images.},
  booktitle = {CVPR},
  YEAR = {2008}
  }


  @inproceedings{Yu:2010:AIO:1873951.1874105,
  author = {Yu, Haonan and Li, Jia and Tian, Yonghong and Huang, Tiejun},
  title = {Automatic interesting object extraction from images using complementary saliency maps},
  booktitle = {Proceedings of the international conference on Multimedia},
  year = {2010}
  }
  @inproceedings{DBLP:conf/accv/DonoserRB09,
    author    = {Michael Donoser and Hayko Riemenschneider and  Horst Bischof},
    title     = {Efficient Partial Shape Matching of Outer Contours},
    booktitle = {ACCV},
    year      = {2009}
  }

  @inproceedings{RenFM05a,
	  author = "Xiaofeng Ren and Charless C. Fowlkes and Jitendra Malik",
	  title = "Scale-invariant contour completion using conditional random fields",
	  booktitle = {ICCV},
	  year = "2005"
	  }
@inproceedings{RenMalik07,
        author = "Xiaofeng Ren and Jitendra Malik",
        title = "Tracking as Repeated Figure/Ground Segmentation",
        booktitle = {Proc. IEEE Conf. Comput. Vision and Pattern Recogn.},
        year = "2007"
        }

@InProceedings{Buehler08,
   author = "Buehler, P. and Everingham, M. and Huttenlocher, D.~P. and Zisserman, A.",
   title = "Long Term Arm and Hand Tracking for Continuous Sign Language {TV} Broadcasts",
   booktitle = "Proceedings of the British Machine Vision Conference",
   year = "2008",
}


@inproceedings{DBLP:conf/iccv/IonescuLS11,
  author    = {Catalin Ionescu and
               Fuxin Li and
               Cristian Sminchisescu},
  title     = {Latent structured models for human pose estimation},
  booktitle = {ICCV},
  year      = {2011}
}

@inproceedings{Bray:2006:PSS:2168483.2168541,
 author = {Bray, Matthieu and Kohli, Pushmeet and Torr, Philip H. S.},
 title = {POSECUT: simultaneous segmentation and 3D pose estimation of humans using dynamic graph-cuts},
 booktitle = {ECCV},
 year = {2006}
}
@inproceedings{Dalal:2006:HDU:2168483.2168522,
 author = {Dalal, Navneet and Triggs, Bill and Schmid, Cordelia},
 title = {Human detection using oriented histograms of flow and appearance},
 series = {ECCV},
 year = {2006}
} 


@inproceedings{DBLP:conf/cvpr/GkioxariABM13,
  author    = {Georgia Gkioxari and
               Pablo Arbelaez and
               Lubomir D. Bourdev and
               Jitendra Malik},
  title     = {Articulated Pose Estimation Using Discriminative Armlet
               Classifiers},
  booktitle = {CVPR},
  year      = {2013}
}
@inproceedings {Pishchulin2013cvpr,
	title = {Poselet Conditioned Pictorial Structures},
	booktitle = {CVPR},
	year = {2013},
	author = {Leonid Pishchulin and Mykhaylo Andriluka and Peter Gehler and Schiele, Bernt}
}


@INPROCEEDINGS{5540232,
author={Karlinsky, L. and Dinerstein, M. and Harari, D. and Ullman, S.},
booktitle={CVPR},
title={The chains model for detecting parts by their context},
year={2010}}
@article{DBLP:journals/pami/FelzenszwalbGMR10,
  author    = {Pedro F. Felzenszwalb and
               Ross B. Girshick and
               David A. McAllester and
               Deva Ramanan},
  title     = {Object Detection with Discriminatively Trained Part-Based
               Models},
  journal   = {IEEE Trans. Pattern Anal. Mach. Intell.},
  volume    = {32},
  number    = {9},
  year      = {2010},
  pages     = {1627-1645},
  ee        = {http://doi.ieeecomputersociety.org/10.1109/TPAMI.2009.167},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{Gaidon:Virtual:CVPR2016,
    author = {Gaidon, A and Wang, Q and Cabon, Y and Vig, E},
    title = {Virtual Worlds as Proxy for Multi-Object Tracking Analysis},
    booktitle = {CVPR},
    year = {2016}
}


@inproceedings{parkhi11truth,
  Author    = {O. M. Parkhi and A. Vedaldi and C. V. Jawahar and A. Zisserman},
  Title     = {The Truth About Cats and Dogs},
  Booktitle = {Proceedings of the International
               Conference on Computer Vision ({ICCV})},
  Year      = {2011}}

@INPROCEEDINGS{6248070,
author={Qieyun Dai and Hoiem, D.},
booktitle={Computer Vision and Pattern Recognition (CVPR), 2012 IEEE Conference on}, title={Learning to localize detected objects},
year={2012},
pages={3322-3329},
keywords={image segmentation;learning (artificial intelligence);object detection;bounding box overlap;color models;edge cues;initial detector;learned graph cut segmentation;learning;object detection localization;pixel assignment;structural bounding box prediction;Color;Computational modeling;Detectors;Image color analysis;Image edge detection;Shape;Training},
doi={10.1109/CVPR.2012.6248070},
ISSN={1063-6919},}

@inproceedings{Karlinsky:2012:ULF:24030722403098,
 author = {Karlinsky, Leonid and Ullman, Shimon},
 title = {Using linking features in learning non-parametric part models},
 booktitle = {Proceedings of the 12th European conference on Computer Vision - Volume Part III},
 series = {ECCV'12},
 year = {2012},
 isbn = {978-3-642-33711-6},
 location = {Florence, Italy},
 pages = {326--339},
 numpages = {14},
 url = {http://dx.doi.org/10.1007/978-3-642-33712-3_24},
 doi = {10.1007/978-3-642-33712-3_24},
 acmid = {2403098},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
 keywords = {FLPM model, linking features, parts detection},
}




  @TechReport{RenFM05tech,
	  author = "Xiaofeng Ren and Charless C. Fowlkes and Jitendra Malik",
	  title = "Mid-level cues improve boundary detection",
	  institution =  {UC Berkeley},
	  number =       {UCB//CSD-05-1382},
	  year =         {2005}
	  }

  @InProceedings{BroxSegmentationCVPR11,
    author       = "Thomas Brox and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Object Segmentation by Alignment of Poselet Activations to Image Contours",
    booktitle    = "IEEE International Conference on Computer Vision and Pattern Recognition (CVPR)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }
  @InProceedings{HariharanSemanticContoursICCV11,
    author       = "Bharath Hariharan and Pablo Arbelaez and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Semantic Contours from Inverse Detectors",
    booktitle    = "International Conference on Computer Vision (ICCV)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }
  @inproceedings{DBLP:conf/eccv/RiemenschneiderDB10,
    author    = {Hayko Riemenschneider and Michael Donoser and Horst Bischof},
    title     = {Using Partial Edge Contour Matches for Efficient Object
		Category Localization},
    booktitle = {ECCV},
    year      = {2010}
  }

  @inproceedings{ArbelaezMFM_CVPR_2009,
      author = "Arbelaez, Pablo and Maire, Michael and Fowlkes, Charless C. and Malik, Jitendra",
      booktitle = "CVPR",
      year = "2009",
      title = "From Contours to Regions: An Empirical Evaluation"
  }

@incollection{NIPS2014_5349,
title = {Learning Deep Features for Scene Recognition using Places Database},
author = {Zhou, Bolei and Lapedriza, Agata and Xiao, Jianxiong and Torralba, Antonio and Oliva, Aude},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {487--495},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5349-learning-deep-features-for-scene-recognition-using-places-database.pdf}
}

  @inproceedings{MoriREM04,
	  author = "Greg Mori and Xiaofeng Ren and Alexei A. Efros and Jitendra Malik",
	  title = "Recovering human body configurations: combining segmentation and recognition.",
	  booktitle = {Proc. IEEE Conf. Comput. Vision and Pattern Recogn.},
	  volume = 2,
	  pages = "326-333",
	  year = "2004",
	  }



  @inproceedings{Latecki2010,
    author    = {Tianyang Ma and Longin Jan Latecki},
    title     = { From Partial Shape Matching through Local Deformation to Robust Global Shape Similarity for Object Detection},
    booktitle = {CVPR},
    year      = {2011}
  }
  @article{Jebara:2004:PPK:1005332.1016786,
  author = {Jebara, Tony and Kondor, Risi and Howard, Andrew},
  title = {Probability Product Kernels},
  journal = {J. Mach. Learn. Res.},
  volume = {5},
  year = {2004}
  }

  @INPROCEEDINGS{Gong99recognitionof,
      author = {Shaogang Gong and Michael Walter},
      title = {Recognition of Temporal Structures: Learning Prior and Propagating Observation Augmented Densities via Hidden Markov States},
      booktitle = {ICCV},
      year = {1999},
  }

  @article{Brand:2000:DSA:351581.351608,
  author = {Brand, Matthew and Kettnaker, Vera},
  title = {Discovery and Segmentation of Activities in Video},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }


  @INPROCEEDINGS{Brown01productsof,
      author = {Andrew D. Brown and Andrew D. Brown and Geoffrey E. Hinton and Geoffrey E. Hinton},
      title = {Products of Hidden Markov Models},
      booktitle = {In Proceedings of Artificial Intelligence and Statistics},
      year = {2001},
  }


  @inproceedings{malisiewicz-nips09,
    Author =	 {Tomasz Malisiewicz and Alexei A. Efros},
    Booktitle =	 {NIPS},
    Title =	 {Beyond Categories: The Visual Memex Model for Reasoning About Object Relationships},
    Year =	 2009
  }


  @inproceedings{yamato,
  author = {J. Yamato and J. Ohya and K. Ishii},
  title = {Recognizing human action in time-sequential images using a hidden Markov model},
  booktitle = {CVPR},
  year = {1994},
  }

 @inproceedings{Kuniyoshi,
  author = {Kuniyoshi Y.},
  title = {Learning from Examples: Imitation Learning and Emerging Cognition},
  booktitle = {Humanoid Robotics and Neuroscience: Science, Engineering and Society. },
  year = {2015},
  }
  
  
  @inproceedings{icml2015_schulman15, 
   Publisher = {JMLR Workshop and Conference Proceedings}, 
   title="Trust Region Policy Optimization", 
   Author={Schulman, John and Levine, Sergey and Abbeel, Pieter and Jordan, Michael and Moritz, Philipp}, 
   year="2015", 
   Booktitle="Proceedings of the 32nd International Conference on Machine Learning (ICML-15)", 
   Editor={David Blei and Francis Bach}, 
   pages="1889-1897", 
   url="http://jmlr.org/proceedings/papers/v37/schulman15.pdf" 
   }
  
  
  @article{DBLP:journals/corr/HasseltGS15,
  author    = {Hado van Hasselt and
               Arthur Guez and
               David Silver},
  title     = {Deep Reinforcement Learning with Double Q-learning},
  journal   = {CoRR},
  volume    = {abs/1509.06461},
  year      = {2015},
  url       = {http://arxiv.org/abs/1509.06461},
  archivePrefix = {arXiv},
  eprint    = {1509.06461},
  timestamp = {Wed, 07 Jun 2017 14:40:43 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/HasseltGS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


  @INPROCEEDINGS{Elgammal04separatingstyle,
      author = {Ahmed Elgammal and Chan-su Lee},
      title = {Separating style and content on a nonlinear manifold},
      booktitle = {CVPR},
      year = {2004}
  }

  @INPROCEEDINGS{Tenenbaum97separatingstyle,
      author = {Joshua B. Tenenbaum and William T. Freeman},
      title = {Separating style and content},
      booktitle = {In Advances in neural},
      year = {1997}
  }

  @inproceedings{DBLP:conf/cvpr/LvN07,
    author    = {Fengjun Lv and
		Ramakant Nevatia},
    title     = {Single View Human Action Recognition using Key Pose Matching and Viterbi Path Searching},
    booktitle = {CVPR},
    year      = {2007}
  }


  @inproceedings { 158,
	  title = {Linear Embeddings in Non-Rigid Structure From Motion},
	  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	  year = {2009},
	  address = {Miami, FL},
	  author = {Vincent Rabaud and Serge Belongie}
  }



  @INPROCEEDINGS{4270260,
  author={Goh, A. and Vidal, R.},
  booktitle={CVPR},
  title={Segmenting Motions of Different Types by Unsupervised Manifold Clustering},
  year={2007},
  }

@incollection{cycle,
year={2008},
isbn={978-3-540-88689-1},
booktitle={ECCV},
volume={5304},
series={Lecture Notes in Computer Science},
editor={Forsyth, David and Torr, Philip and Zisserman, Andrew},
doi={10.1007/978-3-540-88690-7_60},
title={Beyond Loose LP-Relaxations: Optimizing MRFs by Repairing Cycles},
url={http://dx.doi.org/10.1007/978-3-540-88690-7_60},
publisher={Springer Berlin Heidelberg},
author={Komodakis, Nikos and Paragios, Nikos},
pages={806-820}
}


  @incollection {springerlink:10.1007/11551188_37,
    author = {Wang, Fei and Zhang, Changshui},
    title = {Spectral Clustering for Time Series},
    booktitle = {Pattern Recognition and Data Mining},
    volume = {3686},
    year = {2005}
  }

  @INPROCEEDINGS{4587385,
  author={Xiaozhe Wang and Liang Wang and Wirth, A.},
  booktitle={CVPR},
  title={Pattern discovery in motion time series via structure-based spectral clustering},
  year={2008}
  }


  @article{Stauffer:2000:LPA:351581.351588,
  author = {Stauffer, Chris and Grimson, W. Eric L.},
  title = {Learning Patterns of Activity Using Real-Time Tracking},
  journal = {TPAMI},
  volume = {22},
  year = {2000}
  }

  @incollection{Nanopoulos:2001:FCT:766914.766918,
  author = {Nanopoulos, Alex and Alcock, Rob and Manolopoulos, Yannis},
  title = {Information processing and technology},
  year = {2001},
  }

  BibTeX | EndNote | ACM Ref

  @inproceedings{Shi:2006:LTS:1153171.1153641,
  author = {Shi, Yifan and Bobick, Aaron and Essa, Irfan},
  title = {Learning Temporal Sequence Model from Partially Labeled Data},
  booktitle = {CVPR},
  year = {2006}
  }


  @article{Murase,
  author = {Murase, Hiroshi and Nayar, Shree K.},
  title = {Visual learning and recognition of 3-D objects from appearance},
  journal = {IJCV},
  volume = {14},
  year = {1995}
  }


  @INPROCEEDINGS{698609,
  author={Bobick, A.F. and Ivanov, Y.A.},
  booktitle={CVPR},
  title={Action recognition using probabilistic parsing},
  year={1998}
  }

  @inproceedings{Ryoo:2006:RCH:1153171.1153651,
  author = {Ryoo, M. S. and Aggarwal, J. K.},
  title = {Recognition of Composite Human Activities through Context-Free Grammar Based Representation},
  booktitle = {CVPR},
  year = {2006}
  }
  
  @article{Williams:1989:LAC:1351124.1351135,
 author = {Williams, Ronald J. and Zipser, David},
 title = {A Learning Algorithm for Continually Running Fully Recurrent Neural Networks},
 journal = {Neural Comput.},
 volume = {1},
 number = {2},
 year = {1989}
} 

  @article{Elman,
 author = {Rodriguez, P. and Wiles, J and Elman, J.},
 title = {A recurrent neural network that learns to count},
 journal = {. Connection Science},
 volume = {1},
 year = {1999}
} 


  
  @INPROCEEDINGS{Cun90handwrittendigit,
    author = {Le Cun and B. Boser and J. S. Denker and D. Henderson and R. E. Howard and W. Hubbard and L. D. Jackel},
    title = {Handwritten Digit Recognition with a Back-Propagation Network},
    booktitle = {NIPS},
    year = {1990}
}



  @INPROCEEDINGS{Hadsell06dimensionalityreduction,
      author = {Raia Hadsell and Sumit Chopra and Yann Lecun},
      title = {Dimensionality reduction by learning an invariant mapping},
      booktitle = {CVPR},
      year = {2006}
  }


  @incollection{NIPS2010_0893,
  title = {Pose-Sensitive Embedding by Nonlinear NCA Regression},
  author = {Graham Taylor and Rob Fergus and George Williams and Ian Spiro and Christoph Bregler},
  booktitle = {NIPS},
  year = {2010}
  }
  
  @InProceedings{BroxSegmentationCVPR11,
    author       = "Thomas Brox and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Object Segmentation by Alignment of Poselet Activations to Image Contours",
    booktitle    = "IEEE International Conference on Computer Vision and Pattern Recognition (CVPR)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }
  @InProceedings{HariharanSemanticContoursICCV11,
    author       = "Bharath Hariharan and Pablo Arbelaez and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
    title        = "Semantic Contours from Inverse Detectors",
    booktitle    = "International Conference on Computer Vision (ICCV)",
    year         = "2011",
    url          = "http://www.eecs.berkeley.edu/~lbourdev/poselets"
  }

  @InProceedings{raptisS10,
    author = 	{Raptis, M. and Soatto, S.},
    title = 	{Tracklet Descriptors for Action Modeling and Video Analysis},
    booktitle = 	{ECCV},
    year = 	{2010}
  }


  @book{Fukunaga:1990:ISP:92131,
  author = {Fukunaga, Keinosuke},
  title = {Introduction to statistical pattern recognition (2nd ed.)},
  year = {1990}
  }


  @ARTICLE{Roweis00nonlineardimensionality,
      author = {Sam T. Roweis and Lawrence K. Saul},
      title = {Nonlinear dimensionality reduction by locally linear embedding},
      journal = {SCIENCE},
      year = {2000},
      volume = {290}
  }

  @article{Turk_Pentland_1991,
  title={Face recognition using eigenfaces},
  journal={CVPR},
  year={1991}
  }


  @INPROCEEDINGS{Laptev03space-timeinterest,
      author = {Ivan Laptev and Tony Lindeberg},
      title = {Space-time Interest Points},
      booktitle = {ICCV},
      year = {2003}
  }


  @INPROCEEDINGS{Kim07r.:tensor,
      author = {Tae-kyun Kim and Shu-fai Wong and Roberto Cipolla},
      title = {Tensor Canonical Correlation Analysis for Action Classification},
      booktitle = {CVPR},
      year = {2007}
  }

  
  @article{Taylor:2000:RAO:364058.364079,
 author = {Taylor, Camillo J.},
 title = {Reconstruction of Articulated Objects from Point Correspondences in a Single Uncalibrated Image},
 journal = {CVIU},
 volume = {80},
 year = {2000}
} 


  @ARTICLE{Shao_trackingalgorithm,
      author = {Jie Shao and Shaohua Kevin Zhou},
      title = {Tracking Algorithm Using Background-Foreground Motion Models and Multiple Cues},
      journal = {ICASSP}
  }
  @INPROCEEDINGS{Taylor03fusionof,
      author = {Geoffrey Taylor and Lindsay Kleeman},
      title = {Fusion of Multimodal Visual Cues for Model-Based Object Tracking},
      booktitle = {ACRA},
      year = {2003}
  }

  @inproceedings{DBLP:conf/accv/KumarBD07,
    author    = {Pankaj Kumar and
		Michael J. Brooks and
		Anthony R. Dick},
    title     = {Adaptive Multiple Object Tracking Using Colour and Segmentation
		Cues},
    booktitle = {ACCV},
    year      = {2007}
  }

@InProceedings{Kumar05,
   author = "Kumar, M.~P. and Torr, P.~H.~S. and Zisserman, A.",
   title = "{OBJ} {CUT}",
   booktitle = "CVPR",
   year = "2005"
}
@inproceedings{DBLP:conf/eccv/FragkiadakiZZS12,
  author    = {Katerina Fragkiadaki and
               Weiyu Zhang and
               Geng Zhang and
               Jianbo Shi},
  title     = {Two-Granularity Tracking: Mediating Trajectory and Detection
               Graphs for Tracking under Occlusions},
  booktitle = {ECCV},
  year      = {2012}
}


  @InProceedings{rodriguez11b,
    author = "Rodriguez, M. and Sivic, J. and Laptev, I. and Audibert, J.-Y.",
    title = "Density-aware person detection and tracking in crowds",
    booktitle = "ICCV",
    year = "2011"
  }
@inproceedings{DBLP:conf/iccv/Jiang09,
 author    = {Hao Jiang},
 title     = {Human pose estimation using consistent max-covering},
 booktitle = {ICCV},
 year      = {2009}
}

  @inproceedings{Fragkiadaki:topology,
  author = {Fragkiadaki, Katerina and Shi, Jianbo},
  title = {Exploiting Motion and Topology for Segmenting and tracking Under Entanglement.},
  booktitle = {CVPR},
  year = {2011},
  }
@INPROCEEDINGS{Ferrari092dhuman,
    author = {Vittorio Ferrari and Manuel Marín-jiménez and Andrew Zisserman},
    title = {{2D} human pose estimation in {TV} shows},
    booktitle = {In Dagstuhl post-proceedings},
    year = {2009}
}


  @inproceedings{partsagain,
  author = {Michael Maire and Stella Yu and Pietro Perona},
  title = {Object Detection and Segmentation from Joint Embedding of Parts and Pixels},
  booktitle = {ICCV},
  year = {2011},
  }

  @INPROCEEDINGS{Jianbo03multiclassspectral,
      author = {Yu,Stella and Shi, Jianbo},
      title = {Multiclass Spectral Clustering},
      booktitle = {ICCV},
      year = {2003}
  }



  @INPROCEEDINGS{lu_cvpr2011,
      author = {Wei-Lwun Lu and Jo-Anne Ting and Kevin P. Murphy and James J. Little},
      booktitle = {Identifying Players in Broadcast Sports Videos using Conditional Random Fields},
      journal = {Proceedings of the 2011 IEEE Conference on Computer Vision and Pattern Recognition},
      year = {2011}
  }

  @article{DBLP:journals/pami/BoykovVZ01,
    author    = {Yuri Boykov and Olga Veksler and Ramin Zabih},
    title     = {Fast Approximate Energy Minimization via Graph Cuts},
    journal   = {TPAMI},
    volume    = {23},
    year      = {2001}
  }

  @article{GEAN:GEAN31,
  author = {Matula, David W. and Sokal, Robert R.},
  title = {Properties of Gabriel Graphs Relevant to Geographic Variation Research and the Clustering of Points in the Plane},
  journal = {Geographical Analysis},
  volume = {12},
  year = {1980}
  }

@proceedings{citeulike:3504535,
    abstract = {{This paper addresses human pose recognition from video sequences by formulating it as a classification problem. Unlike much previous work we do not make any assumptions on the availability of clean segmentation. The first step of this work consists in a novel method of aligning the training images using 3D Mocap data. Next we define classes by discretizing a 2D manifold whose two dimensions are camera viewpoint and actions. Our main contribution is a pose detection algorithm based on random forests. A bottom-up approach is followed to build a decision tree by recursively clustering and merging the classes at each level. For each node of the decision tree we build a list of potentially discriminative features using the alignment of training images; in this paper we consider Histograms of Orientated Gradient (HOG). We finally grow an ensemble of trees by randomly sampling one of the selected HOG blocks at each node. Our proposed approach gives promising results with both fixed and moving cameras.}},
    author = {Rogez, G. and Rihan, J. and Ramalingam, S. and Orrite, C. and Torr, P. H. S.},
    booktitle = {Computer Vision and Pattern Recognition, 2008. CVPR 2008. IEEE Conference on},
    citeulike-article-id = {3504535},
    citeulike-linkout-0 = {http://dx.doi.org/10.1109/cvpr.2008.4587617},
    citeulike-linkout-1 = {http://ieeexplore.ieee.org/xpls/abs\_all.jsp?arnumber=4587617},
    doi = {10.1109/cvpr.2008.4587617},
    journal = {Computer Vision and Pattern Recognition, 2008. CVPR 2008. IEEE Conference on},
    keywords = {detection, exemplar-based, pose, random, trees},
    pages = {1--8},
    posted-at = {2008-11-11 22:03:40},
    priority = {2},
    title = {{Randomized trees for human pose detection}},
    url = {http://dx.doi.org/10.1109/cvpr.2008.4587617},
    year = {2008}
}




  @INPROCEEDINGS{global_Pb,
  AUTHOR = {Michael Maire and Pablo Arbelaez and Charless Fowlkes and Jitendra Malik},
  TITLE = {Using contours to detect and localize junctions in natural images.},
  booktitle = {CVPR},
  YEAR = {2008}
  }


  @inproceedings{Yu:2010:AIO:1873951.1874105,
  author = {Yu, Haonan and Li, Jia and Tian, Yonghong and Huang, Tiejun},
  title = {Automatic interesting object extraction from images using complementary saliency maps},
  booktitle = {Proceedings of the international conference on Multimedia},
  year = {2010}
  }
  @inproceedings{DBLP:conf/accv/DonoserRB09,
    author    = {Michael Donoser and Hayko Riemenschneider and  Horst Bischof},
    title     = {Efficient Partial Shape Matching of Outer Contours},
    booktitle = {ACCV},
    year      = {2009}
  }

  @inproceedings{DBLP:conf/eccv/RiemenschneiderDB10,
    author    = {Hayko Riemenschneider and Michael Donoser and Horst Bischof},
    title     = {Using Partial Edge Contour Matches for Efficient Object
		Category Localization},
    booktitle = {ECCV},
    year      = {2010}
  }
@article{DBLP:journals/cacm/ShottonSKFFBCM13,
  author    = {Jamie Shotton and
               Toby Sharp and
               Alex Kipman and
               Andrew W. Fitzgibbon and
               Mark Finocchio and
               Andrew Blake and
               Mat Cook and
               Richard Moore},
  title     = {Real-time human pose recognition in parts from single depth
               images},
  journal   = {Commun. ACM},
  volume    = {56},
  number    = {1},
  year      = {2013},
  pages     = {116-124},
  ee        = {http://doi.acm.org/10.1145/2398356.2398381},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@inproceedings{DBLP:conf/cvpr/SunKS12,
  author    = {Min Sun and
               Pushmeet Kohli and
               Jamie Shotton},
  title     = {Conditional regression forests for human pose estimation},
  booktitle = {CVPR},
  year      = {2012},
  pages     = {3394-3401},
  ee        = {http://doi.ieeecomputersociety.org/10.1109/CVPR.2012.6248079},
  crossref  = {DBLP:conf/cvpr/2012},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@article{Rogez:2012:FHP:2317226.2317274,
 author = {Rogez, Gr{\'e}gory and Rihan, Jonathan and Orrite-Uru\~{n}uela, Carlos and Torr, Philip H.},
 title = {Fast Human Pose Detection Using Randomized Hierarchical Cascades of Rejectors},
 journal = {Int. J. Comput. Vision},
 issue_date = {August    2012},
 volume = {99},
 number = {1},
 month = aug,
 year = {2012},
 issn = {0920-5691},
 pages = {25--52},
 numpages = {28},
 url = {http://dx.doi.org/10.1007/s11263-012-0516-9},
 doi = {10.1007/s11263-012-0516-9},
 acmid = {2317274},
 publisher = {Kluwer Academic Publishers},
 address = {Hingham, MA, USA},
 keywords = {Cascade classifiers, Human detection, Pose estimation},
}


  @inproceedings{Latecki2010,
    author    = {Tianyang Ma and Longin Jan Latecki},
    title     = { From Partial Shape Matching through Local Deformation to Robust Global Shape Similarity for Object Detection},
    booktitle = {CVPR},
    year      = {2011}
  }

@INPROCEEDINGS{Sigal03attractivepeople:,
    author = {Leonid Sigal and Michael Isard and Benjamin H. Sigelman and Michael J. Black},
    title = {Attractive People: Assembling Loose-Limbed Models Using Non-parametric Belief Propagation},
    booktitle = {in NIPS},
    year = {2003},
    pages = {1539--1546},
    publisher = {MIT Press}
}

@InProceedings{Richter_2016_ECCV,
author = {Stephan R. Richter and Vibhav Vineet and Stefan Roth and Vladlen Koltun},
title = {Playing for Data: Ground Truth from Computer Games},
booktitle = {European Conference on Computer Vision (ECCV)},
year = {2016},
editor = {Bastian Leibe and Jiri Matas and Nicu Sebe and Max Welling},
series = {LNCS}, 
volume = {9906}, 
publisher = {Springer International Publishing},
pages = {102--118}
}

@inproceedings{DBLP:conf/nips/SutskeverVL14,
  author    = {Ilya Sutskever and
               Oriol Vinyals and
               Quoc V. Le},
  title     = {Sequence to Sequence Learning with Neural Networks},
  booktitle = {NIPS},
  year      = {2014}
}



@article{Weng:2006:VOT:1223195.1223208,
 author = {Weng, Shiuh-Ku and Kuo, Chung-Ming and Tu, Shu-Kang},
 title = {Video Object Tracking Using Adaptive Kalman Filter},
 journal = {J. Vis. Comun. Image Represent.},
 issue_date = {December, 2006},
 volume = {17},
 number = {6},
 year = {2006},
 issn = {1047-3203},
 pages = {1190--1208},
 numpages = {19},
 url = {http://dx.doi.org/10.1016/j.jvcir.2006.03.004},
 doi = {10.1016/j.jvcir.2006.03.004},
 acmid = {1223208},
 publisher = {Academic Press, Inc.},
 address = {Orlando, FL, USA},
 keywords = {Adaptive Kalman filter, HSI color space, Occlusion ratio},
} 



@incollection{Smith88a,
    abstract = {{The Austrian philosopher Christian von Ehrenfels published his essay "On 'Gestalt Qualities'" in 1890. The essay initiated a current of thought which enjoyed a powerful position in the philosophy and psychology of the first half of this century and has more recently enjoyed a minor resurgence of interest in the area of cognitive science, above all in criticisms of the so-called 'strong programme' in artificial intelligence. The theory of Gestalt is of course associated most specifically with psychologists of the Berlin school such as Max Wertheimer, Wolfgang Kohler and Kurt Koffka. We shall see in what follows, however, that an adequate philosophical understanding of the Gestalt idea and of Ehrenfels' achievement will require a close examination not merely of the work of the Berlin school but also of a much wider tradition in Austrian and German philosophy in general.}},
    author = {Smith, Barry},
    booktitle = {Foundations of Gestalt Theory},
    citeulike-article-id = {13114130},
    day = {31},
    editor = {Smith, Barry},
    keywords = {gestalt\_theory},
    month = dec,
    pages = {11--81},
    posted-at = {2014-03-22 09:53:37},
    priority = {2},
    publisher = {Philosophia Verlag},
    title = {{Gestalt Theory: An Essay in Philosophy}},
    year = {1988}
}

@article{DBLP:journals/corr/IsolaZZE16,
  author    = {Phillip Isola and
               Jun{-}Yan Zhu and
               Tinghui Zhou and
               Alexei A. Efros},
  title     = {Image-to-Image Translation with Conditional Adversarial Networks},
  journal   = {CoRR},
  volume    = {abs/1611.07004},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.07004},
  timestamp = {Thu, 01 Dec 2016 19:32:08 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/IsolaZZE16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/HandaBPSMD16,
  author    = {Ankur Handa and
               Michael Bl{\"{o}}sch and
               Viorica Patraucean and
               Simon Stent and
               John McCormac and
               Andrew J. Davison},
  title     = {gvnn: Neural Network Library for Geometric Computer Vision},
  journal   = {CoRR},
  volume    = {abs/1607.07405},
  year      = {2016},
  url       = {http://arxiv.org/abs/1607.07405},
  timestamp = {Tue, 02 Aug 2016 12:59:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/HandaBPSMD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{IEF2015human,
 author = {Carreira, Joao and Agrawal, Pulkit and Fragkiadaki, Katerina and Malik, Jitendra},
 title = {Human Pose Estimation with Iterative Error Feedback},
 journal={arXiv preprint arXiv:1507.06550},
 Year = {2015}}
 
@article{tijmen,
  title={Optimizing neural networks that generate images},
  author={Tijmen Tieleman},
  journal={Ph.D. Thesis},
  year={2014}
}



@Article{Regolin1995,
author="Regolin, Lucia
and Vallortigara, Giorgio",
title="Perception of partly occluded objects by young chicks",
journal="Perception {\&} Psychophysics",
year="1995",
volume="57",
number="7",
pages="971--976",
abstract="Completion of partly occluded objects is a ubiquitous phenomenon in human visual perception. It is unclear, however, whether it occurs at all in other species: Studies on visual discrimination learning have revealed that animals usually attend to parts and features of the discriminative stimuli rather than to global object properties. We provide here the first demonstration of recognition of partly occluded objects in a bird species, the domestic chickGallus gallus, using the naturalistic setting made available by filial imprinting, a process whereby young birds form attachments to their mothers or some artificial substitute. In Experiment 1, newborn chicks were reared singly with a red cardboard triangle, to which they rapidly imprinted and therefore treated as a social partner. On Day 3 of life, the chicks were presented with pairs of objects composed of either isolated fragments or occluded parts of the imprinting stimulus. Chicks consistently chose to associate with complete or with partly occluded versions of the imprinting object rather than with separate fragments of it. Similarly, in Experiment 2, chicks reared with a partly occluded triangle chose to associate with a complete triangle rather than with a fragmented one, whereas chicks reared with a fragmented triangle chose to associate with a fragmented triangle and not with a complete one. Newborn chicks thus appear to behave as if they could experience amodal completion.",
issn="1532-5962",
doi="10.3758/BF03205456",
url="http://dx.doi.org/10.3758/BF03205456"
}
@inproceedings{Kong:ECCV:2014,
  title = {Intrinsic Video},
  author = {Kong, Naejin and Gehler, Peter V. and Black, Michael J.},
  booktitle = {Computer Vision -- ECCV 2014},
  volume = {8690},
  pages = {360--375},
  series = {Lecture Notes in Computer Science},
  editors = {D. Fleet  and T. Pajdla and B. Schiele  and T. Tuytelaars },
  publisher = {Springer International Publishing},
  month = sep,
  year = {2014}
}

@article{DBLP:journals/pami/YangHRF12,
  author    = {Yi Yang and
               Sam Hallman and
               Deva Ramanan and
               Charless C. Fowlkes},
  title     = {Layered Object Models for Image Segmentation},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {34},
  number    = {9},
  pages     = {1731--1743},
  year      = {2012},
  url       = {http://dx.doi.org/10.1109/TPAMI.2011.208},
  doi       = {10.1109/TPAMI.2011.208},
  timestamp = {Sat, 12 Mar 2016 09:04:20 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/pami/YangHRF12},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Tomasi:1992:SMI:144398.144403,
 author = {Tomasi, Carlo and Kanade, Takeo},
 title = {Shape and Motion from Image Streams Under Orthography: A Factorization Method},
 journal = {Int. J. Comput. Vision},
 issue_date = {Nov. 1992},
 volume = {9},
 number = {2},
 month = nov,
 year = {1992},
 issn = {0920-5691},
 pages = {137--154},
 numpages = {18},
 url = {http://dx.doi.org/10.1007/BF00129684},
 doi = {10.1007/BF00129684},
 acmid = {144403},
 publisher = {Kluwer Academic Publishers},
 address = {Hingham, MA, USA},
} 


@techreport{Barron:EECS-2013-117,
    Author = {Barron, Jonathan and Malik, Jitendra},
    Title = {Shape, Illumination, and Reflectance from Shading},
    Institution = {EECS Department, University of California, Berkeley},
    Year = {2013},
    Month = {May},
    URL = {http://www2.eecs.berkeley.edu/Pubs/TechRpts/2013/EECS-2013-117.html},
    Number = {UCB/EECS-2013-117},
    Abstract = {A fundamental problem in computer vision is that of inferring the intrinsic, 3D structure of the world from flat, 2D images of that world. Traditional methods for recovering scene properties such as shape, reflectance, or illumination rely on multiple observations of the same scene to overconstrain the problem. Recovering these same properties from a single image seems almost impossible in comparison --- there are an infinite number of shapes, paint, and lights that exactly reproduce a single image. However, certain explanations are more likely than others: surfaces tend to be smooth, paint tends to be uniform, and illumination tends to be natural. We therefore pose this problem as one of statistical inference, and define an optimization problem that searches for the most likely explanation of a single image. Our technique can be viewed as a superset of several classic computer vision problems (shape-from-shading, intrinsic images, color constancy, illumination estimation, etc) and outperforms all previous solutions to those constituent problems.}
}
@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={770--778},
  year={2016}
}



@article{DBLP:journals/corr/PintoG15,
  author    = {Lerrel Pinto and
               Abhinav Gupta},
  title     = {Supersizing Self-supervision: Learning to Grasp from 50K Tries and
               700 Robot Hours},
  journal   = {CoRR},
  volume    = {abs/1509.06825},
  year      = {2015},
  url       = {http://arxiv.org/abs/1509.06825},
  timestamp = {Wed, 07 Jun 2017 14:41:22 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/PintoG15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@inproceedings{rohrbach2012database,
  title={A Database for Fine Grained Activity Detection of Cooking Activities},
  author={Rohrbach, Marcus and Amin, Sikandar and Andriluka, Mykhaylo and Schiele, Bernt},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2012},
  organization={IEEE}
}

@inproceedings{rohrbach2013translating,
  title={Translating Video Content to Natural Language Descriptions},
  author={Rohrbach, Marcus and Wei, Qiu and Titov, Ivan and Thater, Stefan and Pinkal, Manfred and Schiele, Bernt},
  booktitle={IEEE International Conference on Computer Vision (ICCV)},
  year={2013}
}


@article{DBLP:journals/corr/HuARDS17,
  author    = {Ronghang Hu and
               Jacob Andreas and
               Marcus Rohrbach and
               Trevor Darrell and
               Kate Saenko},
  title     = {Learning to Reason: End-to-End Module Networks for Visual Question
               Answering},
  journal   = {CoRR},
  volume    = {abs/1704.05526},
  year      = {2017},
  url       = {http://arxiv.org/abs/1704.05526},
  archivePrefix = {arXiv},
  eprint    = {1704.05526},
  timestamp = {Wed, 07 Jun 2017 14:40:24 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/HuARDS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{malinowski2015ask,
  title={Ask Your Neurons: A Neural-based Approach to Answering Questions about Images},
  author={Malinowski, Mateusz and Rohrbach, Marcus and Fritz, Mario},
  booktitle={IEEE International Conference on Computer Vision (ICCV)},
  year={2015}
}

@InProceedings{VQA, 
author = {Stanislaw Antol and Aishwarya Agrawal and Jiasen Lu and Margaret Mitchell and Dhruv Batra and C. Lawrence Zitnick and Devi Parikh}, 
title = {{VQA}: {V}isual {Q}uestion {A}nswering}, 
booktitle = {International Conference on Computer Vision (ICCV)}, 
year = {2015}, 
}

@inproceedings{andreas2016learning,
  title={Learning to Compose Neural Networks for Question Answering},
  author={Andreas, Jacob and Rohrbach, Marcus and Darrell, Trevor and Klein, Dan},
  booktitle={North American Chapter of the Association for Computational Linguistics: Human Language Technologies (NAACL)},
  year={2016}
}

@inproceedings{fukui2016multimodal,
  title={Multimodal Compact Bilinear Pooling for Visual Question Answering and Visual Grounding},
  author={Fukui, Akira and Park, Dong Huk and Yang, Daylen and Rohrbach, Anna and Darrell, Trevor and Rohrbach, Marcus},
  booktitle={Conference on Empirical Methods in Natural Language Processing (EMNLP)},
  year={2016}
}
@InProceedings{Das_2013_CVPR,
author = {Das, Pradipto and Xu, Chenliang and Doell, Richard F. and Corso, Jason J.},
title = {A Thousand Frames in Just a Few Words: Lingual Description of Videos through Latent Topics and Sparse Object Stitching},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2013}
}

@article{DBLP:journals/corr/abs-1710-04615,
  author    = {Tianhao Zhang and
               Zoe McCarthy and
               Owen Jow and
               Dennis Lee and
               Ken Goldberg and
               Pieter Abbeel},
  title     = {Deep Imitation Learning for Complex Manipulation Tasks from Virtual
               Reality Teleoperation},
  journal   = {CoRR},
  volume    = {abs/1710.04615},
  year      = {2017},
  url       = {http://arxiv.org/abs/1710.04615},
  archivePrefix = {arXiv},
  eprint    = {1710.04615},
  timestamp = {Wed, 01 Nov 2017 19:05:43 +0100},
  biburl    = {http://dblp.org/rec/bib/journals/corr/abs-1710-04615},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{DBLP:journals/corr/NeelakantanLAMA16,
  author    = {Arvind Neelakantan and
               Quoc V. Le and
               Mart{\'{\i}}n Abadi and
               Andrew McCallum and
               Dario Amodei},
  title     = {Learning a Natural Language Interface with Neural Programmer},
  journal   = {CoRR},
  volume    = {abs/1611.08945},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.08945},
  archivePrefix = {arXiv},
  eprint    = {1611.08945},
  timestamp = {Wed, 07 Jun 2017 14:42:36 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/NeelakantanLAMA16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@INPROCEEDINGS{6619231, 
author={C. L. Zitnick and D. Parikh}, 
booktitle={2013 IEEE Conference on Computer Vision and Pattern Recognition}, 
title={Bringing Semantics into Focus Using Visual Abstraction}, 
year={2013}, 
pages={3009-3016}, 
keywords={image processing;abstract images;abstract scenes;complex visual information;high level semantic information;image hand labeling;linguistic semantic similarity;visual abstraction;Abstracts;Art;Feature extraction;Mutual information;Semantics;Speech;Visualization;abstract scenes;semantic understanding}, 
doi={10.1109/CVPR.2013.387}, 
ISSN={1063-6919}, 
month={June},}


@inproceedings{rohrbach2015dataset,
  title={A Dataset for Movie Description},
  author={Rohrbach, Anna and Rohrbach, Marcus and Tandon, Niket and Schiele, Bernt},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2015}
}

@inproceedings{rohrbach2012script,
  title={Script Data for Attribute-based Recognition of Composite Activities},
  author={Rohrbach, Marcus and Regneri, Michaela and Andriluka, Micha and Amin, Sikandar and Pinkal, Manfred and Schiele, Bernt},
  booktitle={ECCV 2012 : 12th European Conference on Computer Vision},
  year={2012},
  organization={Springer}
}

@inproceedings{rohrbach2016grounding,
  title={Grounding of Textual Phrases in Images by Reconstruction},
  author={Rohrbach, Anna and Rohrbach, Marcus and Hu, Ronghang and Darrell, Trevor and Schiele, Bernt},
  booktitle={European Conference on Computer Vision (ECCV)},
  year={2016}
}

@inproceedings{rohrbach2014coherent,
  title={Coherent Multi-Sentence Video Description with Variable Level of Detail},
  author={Rohrbach, Anna and Rohrbach, Marcus and Qiu, Wei and Friedrich, Annemarie and Pinkal, Manfred and Schiele, Bernt},
  booktitle={German Conference on Pattern Recognition (GCPR)},
  year={2014}
}

@inproceedings{hendricks2016generating,
  title={Generating Visual Explanations},
  author={Hendricks, Lisa Anne and Akata, Zeynep and Rohrbach, Marcus and Donahue, Jeff and Schiele, Bernt and Darrell, Trevor},
  booktitle={European Conference on Computer Vision (ECCV)},
  year={2016}
}

@inproceedings{venugopalan2017captioning,
  title={Captioning Images with Diverse Objects},
  author={Venugopalan, Subhashini and Hendricks, Lisa Anne and Rohrbach, Marcus and Mooney, Raymond and Darrell, Trevor and Saenko, Kate},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017}
}

@inproceedings{hu2017learning,
  title={Learning to Reason: End-to-End Module Networks for Visual Question Answering},
  author={Hu, Ronghang and Andreas, Jacob and Rohrbach, Marcus and Darrell, Trevor and Saenko, Kate},
  booktitle={IEEE International Conference on Computer Vision (ICCV)},
  year={2017}
}

@article{DBLP:journals/corr/AlemiCISU16,
  author    = {Alexander A. Alemi and
               Fran{\c{c}}ois Chollet and
               Geoffrey Irving and
               Christian Szegedy and
               Josef Urban},
  title     = {DeepMath - Deep Sequence Models for Premise Selection},
  journal   = {CoRR},
  volume    = {abs/1606.04442},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.04442},
  timestamp = {Wed, 07 Jun 2017 14:40:07 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/AlemiCISU16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Xiao:2017:LAA:3131944.3133941,
 author = {Xiao, Jianxiong},
 title = {Learning Affordance for Autonomous Driving},
 booktitle = {Proceedings of the 2Nd ACM International Workshop on Smart, Autonomous, and Connected Vehicular Systems and Services},
 series = {CarSys '17},
 year = {2017},
 isbn = {978-1-4503-5146-1},
 location = {Snowbird, Utah, USA},
 pages = {1--1},
 numpages = {1},
 url = {http://doi.acm.org/10.1145/3131944.3133941},
 doi = {10.1145/3131944.3133941},
 acmid = {3133941},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {autonomous driving, self-driving car},
} 


@article{DBLP:journals/corr/PintoG15,
  author    = {Lerrel Pinto and
               Abhinav Gupta},
  title     = {Supersizing Self-supervision: Learning to Grasp from 50K Tries and
               700 Robot Hours},
  journal   = {CoRR},
  volume    = {abs/1509.06825},
  year      = {2015},
  url       = {http://arxiv.org/abs/1509.06825},
  archivePrefix = {arXiv},
  eprint    = {1509.06825},
  timestamp = {Wed, 07 Jun 2017 14:41:22 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/PintoG15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@INPROCEEDINGS{Andrews03supportvector,
    author = {Stuart Andrews and Ioannis Tsochantaridis and Thomas Hofmann},
    title = {Support vector machines for multiple-instance learning},
    booktitle = {Advances in Neural Information Processing Systems 15},
    year = {2003},
    pages = {561--568},
    publisher = {MIT Press}
}

@article{DBLP:journals/corr/MaLH16,
  author    = {Xuezhe Ma and
               Zhengzhong Liu and
               Eduard H. Hovy},
  title     = {Unsupervised Ranking Model for Entity Coreference Resolution},
  journal   = {CoRR},
  volume    = {abs/1603.04553},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.04553},
  timestamp = {Wed, 07 Jun 2017 14:42:20 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/MaLH16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{shetty2017speaking,
  title={Speaking the Same Language: Matching Machine to Human Captions by Adversarial Training},
  author={Shetty, Rakshith and Rohrbach, Marcus and Hendricks, Lisa Anne and Fritz, Mario and Schiele, Bernt},
  booktitle={IEEE International Conference on Computer Vision (ICCV)},
  year={2017}
}

@inproceedings{rohrbach2017generating,
  title={Generating descriptions with grounded and co-referenced people},
  author={Rohrbach, Anna and Rohrbach, Marcus and Tang, Siyu and Oh, Seong Joon and Schiele, Bernt},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017}
}



@article{DBLP:journals/corr/YangHGDS15,
  author    = {Zichao Yang and
               Xiaodong He and
               Jianfeng Gao and
               Li Deng and
               Alexander J. Smola},
  title     = {Stacked Attention Networks for Image Question Answering},
  journal   = {CoRR},
  volume    = {abs/1511.02274},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.02274},
  timestamp = {Wed, 07 Jun 2017 14:41:59 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/YangHGDS15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{karpathy2015deep,
  title={Deep visual-semantic alignments for generating image descriptions},
  author={Karpathy, Andrej and Fei-Fei, Li},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3128--3137},
  year={2015}
}

@article{DBLP:journals/corr/LinMBHPRDZ14,
  author    = {Tsung{-}Yi Lin and
               Michael Maire and
               Serge J. Belongie and
               Lubomir D. Bourdev and
               Ross B. Girshick and
               James Hays and
               Pietro Perona and
               Deva Ramanan and
               Piotr Doll{\'{a}}r and
               C. Lawrence Zitnick},
  title     = {Microsoft {COCO:} Common Objects in Context},
  journal   = {CoRR},
  volume    = {abs/1405.0312},
  year      = {2014},
  url       = {http://arxiv.org/abs/1405.0312},
  timestamp = {Wed, 07 Jun 2017 14:41:35 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LinMBHPRDZ14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/SermanetXL16,
  author    = {Pierre Sermanet and
               Kelvin Xu and
               Sergey Levine},
  title     = {Unsupervised Perceptual Rewards for Imitation Learning},
  journal   = {CoRR},
  volume    = {abs/1612.06699},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.06699},
  archivePrefix = {arXiv},
  eprint    = {1612.06699},
  timestamp = {Wed, 07 Jun 2017 14:42:07 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/SermanetXL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{Liang:2016:LES:2991470.2866568,
 author = {Liang, Percy},
 title = {Learning Executable Semantic Parsers for Natural Language Understanding},
 journal = {Commun. ACM},
 issue_date = {September 2016},
 volume = {59},
 number = {9},
 month = aug,
 year = {2016},
 issn = {0001-0782},
 pages = {68--76},
 numpages = {9},
 url = {http://doi.acm.org/10.1145/2866568},
 doi = {10.1145/2866568},
 acmid = {2866568},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@article{DBLP:journals/corr/LocascioNDKB16,
  author    = {Nicholas Locascio and
               Karthik Narasimhan and
               Eduardo DeLeon and
               Nate Kushman and
               Regina Barzilay},
  title     = {Neural Generation of Regular Expressions from Natural Language with
               Minimal Domain Knowledge},
  journal   = {CoRR},
  volume    = {abs/1608.03000},
  year      = {2016},
  url       = {http://arxiv.org/abs/1608.03000},
  archivePrefix = {arXiv},
  eprint    = {1608.03000},
  timestamp = {Wed, 07 Jun 2017 14:40:18 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LocascioNDKB16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{DBLP:conf/acl/WangBL15,
  author    = {Yushi Wang and
               Jonathan Berant and
               Percy Liang},
  title     = {Building a Semantic Parser Overnight},
  booktitle = {Proceedings of the 53rd Annual Meeting of the Association for Computational
               Linguistics and the 7th International Joint Conference on Natural
               Language Processing of the Asian Federation of Natural Language Processing,
               {ACL} 2015, July 26-31, 2015, Beijing, China, Volume 1: Long Papers},
  pages     = {1332--1342},
  year      = {2015},
  crossref  = {DBLP:conf/acl/2015-1},
  url       = {http://aclweb.org/anthology/P/P15/P15-1129.pdf},
  timestamp = {Sun, 02 Aug 2015 19:26:07 +0200},
  biburl    = {http://dblp.org/rec/bib/conf/acl/WangBL15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/acl/IyerKCKZ17,
  author    = {Srinivasan Iyer and
               Ioannis Konstas and
               Alvin Cheung and
               Jayant Krishnamurthy and
               Luke Zettlemoyer},
  title     = {Learning a Neural Semantic Parser from User Feedback},
  booktitle = {Proceedings of the 55th Annual Meeting of the Association for Computational
               Linguistics, {ACL} 2017, Vancouver, Canada, July 30 - August 4, Volume
               1: Long Papers},
  pages     = {963--973},
  year      = {2017},
  crossref  = {DBLP:conf/acl/2017-1},
  url       = {https://doi.org/10.18653/v1/P17-1089},
  doi       = {10.18653/v1/P17-1089},
  timestamp = {Fri, 04 Aug 2017 16:38:24 +0200},
  biburl    = {http://dblp.org/rec/bib/conf/acl/IyerKCKZ17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/MisraLA17,
  author    = {Dipendra Kumar Misra and
               John Langford and
               Yoav Artzi},
  title     = {Mapping Instructions and Visual Observations to Actions with Reinforcement
               Learning},
  journal   = {CoRR},
  volume    = {abs/1704.08795},
  year      = {2017},
  url       = {http://arxiv.org/abs/1704.08795},
  archivePrefix = {arXiv},
  eprint    = {1704.08795},
  timestamp = {Wed, 07 Jun 2017 14:42:37 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/MisraLA17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}




@Inbook{Matuszek2013,
author="Matuszek, Cynthia
and Herbst, Evan
and Zettlemoyer, Luke
and Fox, Dieter",
editor="Desai, Jaydev P.
and Dudek, Gregory
and Khatib, Oussama
and Kumar, Vijay",
title="Learning to Parse Natural Language Commands to a Robot Control System",
bookTitle="Experimental Robotics: The 13th International Symposium on Experimental Robotics",
year="2013",
publisher="Springer International Publishing",
address="Heidelberg",
pages="403--415",
abstract="As robots become more ubiquitous and capable of performing complex tasks, the importance of enabling untrained users to interact with them has increased. In response, unconstrained natural-language interaction with robots has emerged as a significant research area. We discuss the problem of parsing natural language commands to actions and control structures that can be readily implemented in a robot execution system. Our approach learns a parser based on example pairs of English commands and corresponding control language expressions. We evaluate this approach in the context of following route instructions through an indoor environment, and demonstrate that our system can learn to translate English commands into sequences of desired actions, while correctly capturing the semantic intent of statements involving complex control structures. The procedural nature of our formal representation allows a robot to interpret route instructions online while moving through a previously unknown environment.",
isbn="978-3-319-00065-7",
doi="10.1007/978-3-319-00065-7_28",
url="https://doi.org/10.1007/978-3-319-00065-7_28"
}

@article{DBLP:journals/corr/LeeHLZ17,
  author    = {Kenton Lee and
               Luheng He and
               Mike Lewis and
               Luke Zettlemoyer},
  title     = {End-to-end Neural Coreference Resolution},
  journal   = {CoRR},
  volume    = {abs/1707.07045},
  year      = {2017},
  url       = {http://arxiv.org/abs/1707.07045},
  archivePrefix = {arXiv},
  eprint    = {1707.07045},
  timestamp = {Sat, 05 Aug 2017 14:56:20 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LeeHLZ17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/BahdanauCB14,
  author    = {Dzmitry Bahdanau and
               Kyunghyun Cho and
               Yoshua Bengio},
  title     = {Neural Machine Translation by Jointly Learning to Align and Translate},
  journal   = {CoRR},
  volume    = {abs/1409.0473},
  year      = {2014},
  url       = {http://arxiv.org/abs/1409.0473},
  archivePrefix = {arXiv},
  eprint    = {1409.0473},
  timestamp = {Wed, 07 Jun 2017 14:40:19 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/BahdanauCB14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{doi:10.1177/0278364915602060,
author = {Dipendra K. Misra and Jaeyong Sung and Kevin Lee and Ashutosh Saxena},
title ={Tell me Dave: Context-sensitive grounding of natural language to manipulation           instructions},
journal = {The International Journal of Robotics Research},
volume = {35},
number = {1-3},
pages = {281-300},
year = {2016},
doi = {10.1177/0278364915602060},

URL = { 
        https://doi.org/10.1177/0278364915602060
    
},
eprint = { 
        https://doi.org/10.1177/0278364915602060
    
}
,
    abstract = { It is important for a robot to be able to interpret natural language commands given by a human. In this paper, we consider performing a sequence of mobile manipulation tasks with instructions described in natural language. Given a new environment, even a simple task such as boiling water would be performed quite differently depending on the presence, location and state of the objects. We start by collecting a dataset of task descriptions in free-form natural language and the corresponding grounded task-logs of the tasks performed in an online robot simulator. We then build a library of verb–environment instructions that represents the possible instructions for each verb in that environment, these may or may not be valid for a different environment and task context. We present a model that takes into account the variations in natural language and ambiguities in grounding them to robotic instructions with appropriate environment context and task constraints. Our model also handles incomplete or noisy natural language instructions. It is based on an energy function that encodes such properties in a form isomorphic to a conditional random field. We evaluate our model on tasks given in a robotic simulator and show that it successfully outperforms the state of the art with 61.8\% accuracy. We also demonstrate a grounded robotic instruction sequence on a PR2 robot using the Learning from Demonstration approach. }
}

@inproceedings{Branavan:2009:RLM:1687878.1687892,
 author = {Branavan, S. R. K. and Chen, Harr and Zettlemoyer, Luke S. and Barzilay, Regina},
 title = {Reinforcement Learning for Mapping Instructions to Actions},
 booktitle = {Proceedings of the Joint Conference of the 47th Annual Meeting of the ACL and the 4th International Joint Conference on Natural Language Processing of the AFNLP: Volume 1 - Volume 1},
 series = {ACL '09},
 year = {2009},
 isbn = {978-1-932432-45-9},
 location = {Suntec, Singapore},
 pages = {82--90},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=1687878.1687892},
 acmid = {1687892},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
}




@inproceedings{mei16,
  address = {Phoenix, AZ},
  author = {Hongyuan Mei and Mohit Bansal and Matthew R. Walter},
  booktitle = {Proceedings of the National Conference on Artificial Intelligence (AAAI)},
  month = {February},
  pages = {2772--2778},
  title = {Listen, Attend, and Walk: Neural Mapping of Navigational Instructions to Action Sequences},
  year = {2016},
}



@InProceedings{zelle:aaai96,
title={Learning to Parse Database Queries using Inductive Logic Programming},
author={John M. Zelle and Raymond J. Mooney},
booktitle={AAAI/IAAI},
month={August},
address={Portland, OR},
publisher={AAAI Press/MIT Press},
pages={1050-1055},
url="http://www.cs.utexas.edu/users/ai-lab/?zelle:aaai96",
year={1996}
}

@article{DBLP:journals/corr/abs-1207-1420,
  author    = {Luke S. Zettlemoyer and
               Michael Collins},
  title     = {Learning to Map Sentences to Logical Form: Structured Classification
               with Probabilistic Categorial Grammars},
  journal   = {CoRR},
  volume    = {abs/1207.1420},
  year      = {2012},
  url       = {http://arxiv.org/abs/1207.1420},
  archivePrefix = {arXiv},
  eprint    = {1207.1420},
  timestamp = {Wed, 07 Jun 2017 14:41:47 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/abs-1207-1420},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{Clarke:2010:DSP:1870568.1870571,
 author = {Clarke, James and Goldwasser, Dan and Chang, Ming-Wei and Roth, Dan},
 title = {Driving Semantic Parsing from the World's Response},
 booktitle = {Proceedings of the Fourteenth Conference on Computational Natural Language Learning},
 series = {CoNLL '10},
 year = {2010},
 isbn = {978-1-932432-83-1},
 location = {Uppsala, Sweden},
 pages = {18--27},
 numpages = {10},
 url = {http://dl.acm.org/citation.cfm?id=1870568.1870571},
 acmid = {1870571},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
} 


@article{DBLP:journals/corr/HuMLHX16,
  author    = {Zhiting Hu and
               Xuezhe Ma and
               Zhengzhong Liu and
               Eduard H. Hovy and
               Eric P. Xing},
  title     = {Harnessing Deep Neural Networks with Logic Rules},
  journal   = {CoRR},
  volume    = {abs/1603.06318},
  year      = {2016},
  url       = {http://arxiv.org/abs/1603.06318},
  timestamp = {Wed, 07 Jun 2017 14:42:52 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/HuMLHX16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/ChenFLVGDZ15,
  author    = {Xinlei Chen and
               Hao Fang and
               Tsung{-}Yi Lin and
               Ramakrishna Vedantam and
               Saurabh Gupta and
               Piotr Doll{\'{a}}r and
               C. Lawrence Zitnick},
  title     = {Microsoft {COCO} Captions: Data Collection and Evaluation Server},
  journal   = {CoRR},
  volume    = {abs/1504.00325},
  year      = {2015},
  url       = {http://arxiv.org/abs/1504.00325},
  timestamp = {Wed, 07 Jun 2017 14:41:06 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/ChenFLVGDZ15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{antol2015vqa,
  title={Vqa: Visual question answering},
  author={Antol, Stanislaw and Agrawal, Aishwarya and Lu, Jiasen and Mitchell, Margaret and Batra, Dhruv and Lawrence Zitnick, C and Parikh, Devi},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={2425--2433},
  year={2015}
}

@inproceedings{fang2015captions,
  title={From captions to visual concepts and back},
  author={Fang, Hao and Gupta, Saurabh and Iandola, Forrest and Srivastava, Rupesh K and Deng, Li and Doll{\'a}r, Piotr and Gao, Jianfeng and He, Xiaodong and Mitchell, Margaret and Platt, John C and others},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1473--1482},
  year={2015}
}

@article{tenenbaumetal2006,
    abstract = {{Inductive inference allows humans to make powerful generalizations from sparse data when learning about word meanings, unobserved properties, causal relationships, and many other aspects of the world. Traditional accounts of induction emphasize either the power of statistical learning, or the importance of strong constraints from structured domain knowledge, intuitive theories or schemas. We argue that both components are necessary to explain the nature, use and acquisition of human knowledge, and we introduce a theory-based Bayesian framework for modeling inductive learning and reasoning as statistical inferences over structured knowledge representations.}},
    author = {Tenenbaum, Joshua B. and Griffiths, Thomas L. and Kemp, Charles},
    citeulike-article-id = {715656},
    citeulike-linkout-0 = {http://dx.doi.org/10.1016/j.tics.2006.05.009},
    citeulike-linkout-1 = {http://view.ncbi.nlm.nih.gov/pubmed/16797219},
    citeulike-linkout-2 = {http://www.hubmed.org/display.cgi?uids=16797219},
    citeulike-linkout-3 = {http://www.sciencedirect.com/science/article/B6VH9-4K7NHVY-1/2/04b4431587598b181b73ee9b39bdcb72},
    doi = {10.1016/j.tics.2006.05.009},
    issn = {1364-6613},
    journal = {Trends in cognitive sciences},
    keywords = {bayesian, human\_reasoning, probabilistic-inference, probabilistic-reasoning},
    month = jul,
    number = {7},
    pages = {309--318},
    pmid = {16797219},
    posted-at = {2010-07-26 00:18:39},
    priority = {2},
    title = {{Theory-based Bayesian models of inductive learning and reasoning.}},
    url = {http://dx.doi.org/10.1016/j.tics.2006.05.009},
    volume = {10},
    year = {2006}
}



@inproceedings{mitchell2012midge,
  title={Midge: Generating image descriptions from computer vision detections},
  author={Mitchell, Margaret and Han, Xufeng and Dodge, Jesse and Mensch, Alyssa and Goyal, Amit and Berg, Alex and Yamaguchi, Kota and Berg, Tamara and Stratos, Karl and Daum{\'e} III, Hal},
  booktitle={Proceedings of the 13th Conference of the European Chapter of the Association for Computational Linguistics},
  pages={747--756},
  year={2012},
  organization={Association for Computational Linguistics}
}

@article{sordoni2015neural,
  title={A neural network approach to context-sensitive generation of conversational responses},
  author={Sordoni, Alessandro and Galley, Michel and Auli, Michael and Brockett, Chris and Ji, Yangfeng and Mitchell, Margaret and Nie, Jian-Yun and Gao, Jianfeng and Dolan, Bill},
  journal={arXiv preprint arXiv:1506.06714},
  year={2015}
}

@article{devlin2015language,
  title={Language models for image captioning: The quirks and what works},
  author={Devlin, Jacob and Cheng, Hao and Fang, Hao and Gupta, Saurabh and Deng, Li and He, Xiaodong and Zweig, Geoffrey and Mitchell, Margaret},
  journal={arXiv preprint arXiv:1505.01809},
  year={2015}
}




@article{DBLP:journals/corr/FinnGL16,
  author    = {Chelsea Finn and
               Ian J. Goodfellow and
               Sergey Levine},
  title     = {Unsupervised Learning for Physical Interaction through Video Prediction},
  journal   = {CoRR},
  volume    = {abs/1605.07157},
  year      = {2016},
  url       = {http://arxiv.org/abs/1605.07157},
  timestamp = {Wed, 07 Jun 2017 14:42:02 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/FinnGL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@InProceedings{Yatskar_2016_CVPR,
author = {Yatskar, Mark and Zettlemoyer, Luke and Farhadi, Ali},
title = {Situation Recognition: Visual Semantic Role Labeling for Image Understanding },
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2016}
}

@article{DBLP:journals/corr/GuptaM15,
  author    = {Saurabh Gupta and
               Jitendra Malik},
  title     = {Visual Semantic Role Labeling},
  journal   = {CoRR},
  volume    = {abs/1505.04474},
  year      = {2015},
  url       = {http://arxiv.org/abs/1505.04474},
  timestamp = {Wed, 07 Jun 2017 14:42:30 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/GuptaM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/HuangLLN17,
  author    = {De{-}An Huang and
               Joseph J. Lim and
               Fei{-}Fei Li and
               Juan Carlos Niebles},
  title     = {Unsupervised Visual-Linguistic Reference Resolution in Instructional
               Videos},
  journal   = {CoRR},
  volume    = {abs/1703.02521},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.02521},
  timestamp = {Wed, 07 Jun 2017 14:40:45 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/HuangLLN17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{Schaal_TCS_1999,
  title = {Is imitation learning the route to humanoid robots?},
  author = {Schaal, S.},
  booktitle = {Trends in Cognitive Sciences},
  volume = {3},
  number = {6},
  pages = {233-242},
  year = {1999},
  note = {},
  crossref = {p1246},
  url = {http://www-clmc.usc.edu/publications/S/schaal-TICS1999.pdf; http://www-clmc.usc.edu/publications/S/schaal-TICS1999-rep.pdf}
}


@inproceedings{densecap,
  title={DenseCap: Fully Convolutional Localization Networks for Dense Captioning},
  author={Johnson, Justin and Karpathy, Andrej and Fei-Fei, Li},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and 
             Pattern Recognition},
  year={2016}
}


@inproceedings{krishnavisualgenome,
  title={Visual Genome: Connecting Language and Vision Using Crowdsourced Dense Image Annotations},
  author={Krishna, Ranjay and Zhu, Yuke and Groth, Oliver and Johnson, Justin and Hata, Kenji and Kravitz, Joshua and Chen, Stephanie and Kalanditis, Yannis and Li, Li-Jia and Shamma, David A and Bernstein, Michael and Fei-Fei, Li},
  year = {2016},
}

@inproceedings{Patterson2012SunAttributes,    
Author    = {Genevieve Patterson and James Hays},    
Title     = {SUN Attribute Database:
Discovering, Annotating, and Recognizing Scene Attributes},    
Booktitle = {Proceeding of the 25th Conference on Computer Vision and Pattern Recognition (CVPR)},    
Year      = {2012},  
}

@article{DBLP:journals/corr/JiaL16,
  author    = {Robin Jia and
               Percy Liang},
  title     = {Data Recombination for Neural Semantic Parsing},
  journal   = {CoRR},
  volume    = {abs/1606.03622},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.03622},
  timestamp = {Wed, 07 Jun 2017 14:40:39 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/JiaL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{DBLP:journals/corr/StadieAS17,
  author    = {Bradly C. Stadie and
               Pieter Abbeel and
               Ilya Sutskever},
  title     = {Third-Person Imitation Learning},
  journal   = {CoRR},
  volume    = {abs/1703.01703},
  year      = {2017},
  url       = {http://arxiv.org/abs/1703.01703},
  timestamp = {Wed, 07 Jun 2017 14:40:15 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/StadieAS17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@incollection{Nehaniv:2002:CP:762896.762899,
 author = {Nehaniv, Chrystopher L. and Dautenhahn, Kerstin},
 chapter = {The Correspondence Problem},
 title = {Imitation in Animals and Artifacts},
 editor = {Dautenhahn, Kerstin and Nehaniv, Chrystopher L.},
 year = {2002},
 isbn = {0-262-04203-7},
 pages = {41--61},
 numpages = {21},
 url = {http://dl.acm.org/citation.cfm?id=762896.762899},
 acmid = {762899},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
} 



@article{DBLP:journals/corr/FragkiadakiHAVR17,
  author    = {Katerina Fragkiadaki and
               Jonathan Huang and
               Alex Alemi and
               Sudheendra Vijayanarasimhan and
               Susanna Ricco and
               Rahul Sukthankar},
  title     = {Motion Prediction Under Multimodality with Conditional Stochastic
               Networks},
  journal   = {CoRR},
  volume    = {abs/1705.02082},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.02082},
  timestamp = {Wed, 07 Jun 2017 14:41:48 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/FragkiadakiHAVR17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{Argall:2009:SRL:1523530.1524008,
 author = {Argall, Brenna D. and Chernova, Sonia and Veloso, Manuela and Browning, Brett},
 title = {A Survey of Robot Learning from Demonstration},
 journal = {Robot. Auton. Syst.},
 issue_date = {May, 2009},
 volume = {57},
 number = {5},
 month = may,
 year = {2009},
 issn = {0921-8890},
 pages = {469--483},
 numpages = {15},
 url = {http://dx.doi.org/10.1016/j.robot.2008.10.024},
 doi = {10.1016/j.robot.2008.10.024},
 acmid = {1524008},
 publisher = {North-Holland Publishing Co.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 keywords = {Autonomous systems, Learning from demonstration, Machine learning, Robotics},
} 



@article{Hussein:2017:ILS:3071073.3054912,
 author = {Hussein, Ahmed and Gaber, Mohamed Medhat and Elyan, Eyad and Jayne, Chrisina},
 title = {Imitation Learning: A Survey of Learning Methods},
 journal = {ACM Comput. Surv.},
 issue_date = {June 2017},
 volume = {50},
 number = {2},
 month = apr,
 year = {2017},
 issn = {0360-0300},
 pages = {21:1--21:35},
 articleno = {21},
 numpages = {35},
 url = {http://doi.acm.org/10.1145/3054912},
 doi = {10.1145/3054912},
 acmid = {3054912},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Imitation learning, deep learning, feature representations, intelligent agents, learning from demonstrations, learning from experience, reinforcement learning, robotics, self-improvement},
} 


@article{DBLP:journals/corr/JiaL16,
  author    = {Robin Jia and
               Percy Liang},
  title     = {Data Recombination for Neural Semantic Parsing},
  journal   = {CoRR},
  volume    = {abs/1606.03622},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.03622},
  timestamp = {Wed, 07 Jun 2017 14:40:39 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/JiaL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Zhou2015EndtoendLO,
  title={End-to-end learning of semantic role labeling using recurrent neural networks},
  author={Jie Zhou and Wei Xu},
  booktitle={ACL},
  year={2015}
}


@InProceedings{vedantamLinICCV15,
author = {Ramakrishna Vedantam and Xiao Lin and Tanmay Batra and C. Lawrence Zitnick and Devi Parikh},
title = {Learning Common Sense Through Visual Abstraction},
booktitle = {International Conference on Computer Vision (ICCV)},
year = {2015}
}

@InProceedings{P15-1096,
  author = 	"Misra, Kumar Dipendra
		and Tao, Kejia
		and Liang, Percy
		and Saxena, Ashutosh",
  title = 	"Environment-Driven Lexicon Induction for High-Level Instructions",
  booktitle = 	"Proceedings of the 53rd Annual Meeting of the Association for Computational Linguistics and the 7th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)",
  year = 	"2015",
  publisher = 	"Association for Computational Linguistics",
  pages = 	"992--1002",
  location = 	"Beijing, China",
  doi = 	"10.3115/v1/P15-1096",
  url = 	"http://aclweb.org/anthology/P15-1096"
}



@article{DBLP:journals/corr/AgrawalNAML16,
  author    = {Pulkit Agrawal and
               Ashvin Nair and
               Pieter Abbeel and
               Jitendra Malik and
               Sergey Levine},
  title     = {Learning to Poke by Poking: Experiential Learning of Intuitive Physics},
  journal   = {CoRR},
  volume    = {abs/1606.07419},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.07419},
  timestamp = {Wed, 07 Jun 2017 14:42:59 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/AgrawalNAML16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/McCormacHLD16,
  author    = {John McCormac and
               Ankur Handa and
               Stefan Leutenegger and
               Andrew J. Davison},
  title     = {SceneNet {RGB-D:} 5M Photorealistic Images of Synthetic Indoor Trajectories
               with Ground Truth},
  journal   = {CoRR},
  volume    = {abs/1612.05079},
  year      = {2016},
  url       = {http://arxiv.org/abs/1612.05079},
  timestamp = {Wed, 07 Jun 2017 01:00:00 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/McCormacHLD16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{sigurdsson2016hollywood,
  author = {Gunnar A. Sigurdsson and G{\"u}l Varol and Xiaolong Wang and Ali Farhadi and Ivan Laptev and Abhinav Gupta},
  title={Hollywood in Homes: Crowdsourcing Data Collection for Activity Understanding},
  booktitle={European Conference on Computer Vision},
  year={2016},
  pdf = {http://arxiv.org/pdf/1604.01753.pdf},
  web = {http://allenai.org/plato/charades/}
}
  
  
@article{Ji:2013:CNN:2412386.2412939,
 author = {Ji, Shuiwang and Xu, Wei and Yang, Ming and Yu, Kai},
 title = {3D Convolutional Neural Networks for Human Action Recognition},
 journal = {IEEE Trans. Pattern Anal. Mach. Intell.},
 issue_date = {January 2013},
 volume = {35},
 number = {1},
 month = jan,
 year = {2013},
 issn = {0162-8828},
 pages = {221--231},
 numpages = {11},
 url = {http://dx.doi.org/10.1109/TPAMI.2012.59},
 doi = {10.1109/TPAMI.2012.59},
 acmid = {2412939},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
 keywords = {Deep learning, convolutional neural networks, 3D convolution, model combination, action recognition},
} 


@inproceedings{Branavan:2012:LHP:2390524.2390543,
 author = {Branavan, S. R. K. and Kushman, Nate and Lei, Tao and Barzilay, Regina},
 title = {Learning High-level Planning from Text},
 booktitle = {Proceedings of the 50th Annual Meeting of the Association for Computational Linguistics: Long Papers - Volume 1},
 series = {ACL '12},
 year = {2012},
 location = {Jeju Island, Korea},
 pages = {126--135},
 numpages = {10},
 url = {http://dl.acm.org/citation.cfm?id=2390524.2390543},
 acmid = {2390543},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
} 


@article{Chu:2015:RLH:2947721.2947949,
 author = {Chu, Vivian and McMahon, Ian and Riano, Lorenzo and McDonald, Craig G. and He, Qin and Martinez Perez-Tejada, Jorge and Arrigo, Michael and Darrell, Trevor and Kuchenbecker, Katherine J.},
 title = {Robotic Learning of Haptic Adjectives Through Physical Interaction},
 journal = {Robot. Auton. Syst.},
 issue_date = {January 2015},
 volume = {63},
 number = {P3},
 month = jan,
 year = {2015},
 issn = {0921-8890},
 pages = {279--292},
 numpages = {14},
 url = {http://dx.doi.org/10.1016/j.robot.2014.09.021},
 doi = {10.1016/j.robot.2014.09.021},
 acmid = {2947949},
 publisher = {North-Holland Publishing Co.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 keywords = {Haptics, Machine learning, Robotic perception, Tactile sensing, Time-series classification},
} 

@inproceedings{conf/emnlp/BerantCFL13,
  added-at = {2013-11-10T00:00:00.000+0100},
  author = {Berant, Jonathan and Chou, Andrew and Frostig, Roy and Liang, Percy},
  biburl = {https://www.bibsonomy.org/bibtex/2b7403aae1579048cfe77e88fb67a4704/dblp},
  booktitle = {EMNLP},
  ee = {http://aclweb.org/anthology//D/D13/D13-1160.pdf},
  interhash = {6f5f5cf4aab75502a5e67454eb6679b4},
  intrahash = {b7403aae1579048cfe77e88fb67a4704},
  isbn = {978-1-937284-97-8},
  keywords = {dblp},
  pages = {1533-1544},
  publisher = {ACL},
  timestamp = {2013-11-12T11:34:07.000+0100},
  title = {Semantic Parsing on Freebase from Question-Answer Pairs.},
  url = {http://dblp.uni-trier.de/db/conf/emnlp/emnlp2013.html#BerantCFL13},
  year = 2013
}

@inproceedings{Branavan:2009:RLM:1687878.1687892,
 author = {Branavan, S. R. K. and Chen, Harr and Zettlemoyer, Luke S. and Barzilay, Regina},
 title = {Reinforcement Learning for Mapping Instructions to Actions},
 booktitle = {Proceedings of the Joint Conference of the 47th Annual Meeting of the ACL and the 4th International Joint Conference on Natural Language Processing of the AFNLP: Volume 1 - Volume 1},
 series = {ACL '09},
 year = {2009},
 isbn = {978-1-932432-45-9},
 location = {Suntec, Singapore},
 pages = {82--90},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=1687878.1687892},
 acmid = {1687892},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
} 


@article{young-etal-2014,
    author = {Young, Peter and Lai, Alice and Hodosh, Micah and Hockenmaier, Julia},
    citeulike-article-id = {13652898},
    journal = {Transactions of the Association for Computational Linguistics},
    keywords = {semantics, vision},
    pages = {67--78},
    posted-at = {2015-06-22 00:30:56},
    priority = {2},
    title = {{From image descriptions to visual denotations: New similarity metrics for semantic inference over event descriptions}},
    volume = {2},
    year = {2014}
}

@inproceedings{Clarke:2010:DSP:1870568.1870571,
 author = {Clarke, James and Goldwasser, Dan and Chang, Ming-Wei and Roth, Dan},
 title = {Driving Semantic Parsing from the World's Response},
 booktitle = {Proceedings of the Fourteenth Conference on Computational Natural Language Learning},
 series = {CoNLL '10},
 year = {2010},
 isbn = {978-1-932432-83-1},
 location = {Uppsala, Sweden},
 pages = {18--27},
 numpages = {10},
 url = {http://dl.acm.org/citation.cfm?id=1870568.1870571},
 acmid = {1870571},
 publisher = {Association for Computational Linguistics},
 address = {Stroudsburg, PA, USA},
} 


@inproceedings{conf/emnlp/BerantCFL13,
  added-at = {2013-11-10T00:00:00.000+0100},
  author = {Berant, Jonathan and Chou, Andrew and Frostig, Roy and Liang, Percy},
  biburl = {https://www.bibsonomy.org/bibtex/2b7403aae1579048cfe77e88fb67a4704/dblp},
  booktitle = {EMNLP},
  crossref = {conf/emnlp/2013},
  ee = {http://aclweb.org/anthology//D/D13/D13-1160.pdf},
  interhash = {6f5f5cf4aab75502a5e67454eb6679b4},
  intrahash = {b7403aae1579048cfe77e88fb67a4704},
  isbn = {978-1-937284-97-8},
  keywords = {dblp},
  pages = {1533-1544},
  publisher = {ACL},
  timestamp = {2013-11-12T11:34:07.000+0100},
  title = {Semantic Parsing on Freebase from Question-Answer Pairs.},
  url = {http://dblp.uni-trier.de/db/conf/emnlp/emnlp2013.html#BerantCFL13},
  year = 2013
}




@paper{AAAI1612383,
	author = {Amos Azaria and Jayant Krishnamurthy and Tom Mitchell},
	title = {Instructable Intelligent Personal Agent},
	conference = {AAAI Conference on Artificial Intelligence},
	year = {2016},
	keywords = {Learning by Instructions; Instructable Agent; Learning in Natural Language},
	url = {https://www.aaai.org/ocs/index.php/AAAI/AAAI16/paper/view/12383}
}

@inproceedings{huang2016visual,
  title={Visual Storytelling},
  author={Huang, Ting-Hao K. and Ferraro, Francis and Mostafazadeh, Nasrin and Misra, Ishan and Devlin, Jacob and Agrawal, Aishwarya and Girshick, Ross and He, Xiaodong and Kohli, Pushmeet and Batra, Dhruv and others},
  booktitle={15th Annual Conference of the North American Chapter of the Association for Computational Linguistics (NAACL 2016)},
  year={2016}
}


@inproceedings{DBLP:conf/emnlp/HeLZ15,
  author    = {Luheng He and
               Mike Lewis and
               Luke Zettlemoyer},
  title     = {Question-Answer Driven Semantic Role Labeling: Using Natural Language
               to Annotate Natural Language},
  booktitle = {Proceedings of the 2015 Conference on Empirical Methods in Natural
               Language Processing, {EMNLP} 2015, Lisbon, Portugal, September 17-21,
               2015},
  pages     = {643--653},
  year      = {2015},
  crossref  = {DBLP:conf/emnlp/2015},
  url       = {http://aclweb.org/anthology/D/D15/D15-1076.pdf},
  timestamp = {Wed, 14 Oct 2015 09:56:24 +0200},
  biburl    = {http://dblp.org/rec/bib/conf/emnlp/HeLZ15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/LiangBLFL16,
  author    = {Chen Liang and
               Jonathan Berant and
               Quoc Le and
               Kenneth D. Forbus and
               Ni Lao},
  title     = {Neural Symbolic Machines: Learning Semantic Parsers on Freebase with
               Weak Supervision},
  journal   = {CoRR},
  volume    = {abs/1611.00020},
  year      = {2016},
  url       = {http://arxiv.org/abs/1611.00020},
  archivePrefix = {arXiv},
  eprint    = {1611.00020},
  timestamp = {Wed, 07 Jun 2017 14:42:59 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/LiangBLFL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{semantic-parsing-via-staged-query-graph-generation-question-answering-with-knowledge-base,
author = {Yih, Scott Wen-tau and Chang, Ming-Wei and He, Xiaodong and Gao, Jianfeng},
title = {Semantic Parsing via Staged Query Graph Generation: Question Answering with Knowledge Base},
booktitle = {},
year = {2015},
month = {July},
publisher = {ACL – Association for Computational Linguistics}
}

@INPROCEEDINGS{Mitchell93explanationbased,
    author = {Tom M. Mitchell},
    title = {Explanation based learning: A comparison of symbolic and neural network approaches},
    booktitle = {Proceedings of the Tenth International Conference on Machine Learning},
    year = {1993},
    pages = {197--204},
    publisher = {Morgan Kaufmann}
}

@inproceedings{zhou2015end,
  title={End-to-end learning of semantic role labeling using recurrent neural networks.},
  author={Zhou, Jie and Xu, Wei},
  booktitle={ACL (1)},
  pages={1127--1137},
  year={2015}
}
@article{DBLP:journals/corr/JohnsonHMHLZG17,
  author    = {Justin Johnson and
               Bharath Hariharan and
               Laurens van der Maaten and
               Judy Hoffman and
               Fei{-}Fei Li and
               C. Lawrence Zitnick and
               Ross B. Girshick},
  title     = {Inferring and Executing Programs for Visual Reasoning},
  journal   = {CoRR},
  volume    = {abs/1705.03633},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.03633},
  timestamp = {Wed, 07 Jun 2017 14:42:58 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/JohnsonHMHLZG17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{DBLP:conf/emnlp/HeLZ15,
  author    = {Luheng He and
               Mike Lewis and
               Luke Zettlemoyer},
  title     = {Question-Answer Driven Semantic Role Labeling: Using Natural Language
               to Annotate Natural Language},
  booktitle = {Proceedings of the 2015 Conference on Empirical Methods in Natural
               Language Processing, {EMNLP} 2015, Lisbon, Portugal, September 17-21,
               2015},
  pages     = {643--653},
  year      = {2015},
}

@article{DBLP:journals/corr/RajpurkarZLL16,
  author    = {Pranav Rajpurkar and
               Jian Zhang and
               Konstantin Lopyrev and
               Percy Liang},
  title     = {SQuAD: 100, 000+ Questions for Machine Comprehension of Text},
  journal   = {CoRR},
  volume    = {abs/1606.05250},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.05250},
  timestamp = {Wed, 07 Jun 2017 14:41:34 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/RajpurkarZLL16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/WestonBCM15,
  author    = {Jason Weston and
               Antoine Bordes and
               Sumit Chopra and
               Tomas Mikolov},
  title     = {Towards AI-Complete Question Answering: {A} Set of Prerequisite Toy
               Tasks},
  journal   = {CoRR},
  volume    = {abs/1502.05698},
  year      = {2015},
  url       = {http://arxiv.org/abs/1502.05698},
  timestamp = {Wed, 07 Jun 2017 14:42:32 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/WestonBCM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{DBLP:journals/corr/HewlettLJPFHKB16,
  author    = {Daniel Hewlett and
               Alexandre Lacoste and
               Llion Jones and
               Illia Polosukhin and
               Andrew Fandrianto and
               Jay Han and
               Matthew Kelcey and
               David Berthelot},
  title     = {WikiReading: {A} Novel Large-scale Language Understanding Task over
               Wikipedia},
  journal   = {CoRR},
  volume    = {abs/1608.03542},
  year      = {2016},
  url       = {http://arxiv.org/abs/1608.03542},
  timestamp = {Wed, 07 Jun 2017 14:41:20 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/HewlettLJPFHKB16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



